Cyclic Stochastic Optimization: Generalizations, Convergence, and Applications in Multi-Agent Systems

Stochastic approximation (SA) is a powerful class of iterative algorithms for nonlinear root-finding that can be used for minimizing a loss function, $L(\boldsymbol{\theta})$, with respect to a parameter vector $\boldsymbol{\theta}$, when only noisy observations of $L(\boldsymbol{\theta})$ or its gradient are available (through the natural connection between root-finding and minimization); SA algorithms can be thought of as stochastic line search methods where the entire parameter vector is updated at each iteration. The cyclic approach to SA is a variant of SA procedures where $\boldsymbol{\theta}$ is divided into multiple subvectors that are updated one at a time in a cyclic manner. This dissertation focuses on studying the asymptotic properties of cyclic SA and of the generalized cyclic SA (GCSA) algorithm, a variant of cyclic SA where the subvector to update may be selected according to a random variable or according to a predetermined pattern, and where the noisy update direction can be based on the updates of any SA algorithm (e.g., stochastic gradient, Kiefer--Wolfowitz, or simultaneous perturbation SA). The convergence of GCSA, asymptotic normality of GCSA (related to rate of convergence), and efficiency of GCSA relative to its non-cyclic counterpart are investigated both analytically and numerically. Specifically, conditions are obtained for the convergence with probability one of the GCSA iterates and for the asymptotic normality of the normalized iterates of a special case of GCSA. Further, an analytic expression is given for the asymptotic relative efficiency (when efficiency is defined in terms of mean squared error) between a special case of GCSA and its non-cyclic counterpart. Finally, an application of the cyclic SA scheme to a multi-agent stochastic optimization problem is investigated. This dissertation also contains two appendices.

==> CV.tex <==
%!TEX root = root.tex

\fancyhead{} % clear all header and footer fields
\fancyhead[L]{CURRICULUM VITAE} % except the center
\begin{vita}

%\begin{wrapfigure}{R}{0.3\textwidth}
%  \begin{center}
%    \includegraphics[width=0.2\textwidth]{rjvheadshot}
%  \end{center}
%  \caption{Karla Hern\'andez-Cuevas was born on November 1986 in Mexico City, Mexico.}
%\end{wrapfigure}


Karla Hern\'andez-Cuevas was born on November 1986 in Mexico City. Her interest in mathematics began in high-school after the local university, the University of Colima (Universidad de Colima), offered high-school seniors the opportunity to take mathematics and physics courses taught at an undergraduate-level. Her interest in applied mathematics deepened after interning at the Mathematical and Theoretical Biology Institute at Arizona State University where  she worked on determining optimal treatment strategies for patients with mental disorders. After graduating form high-school she went on to obtain her Bachelor's degree in mathematics in 2009 from the University of Colima. Her undergraduate dissertation involved predicting the outcomes of UEFA (Union of European Football Associations) Champions League matches. After obtaining her Bachelor's degree Karla went on to intern at the Institute for Innovation and Technological Development (Instituto de Innovaci\'on y Desarrollo Tecnol\'ogico) at the University of Colima. There, she participated in a state-wide campaign to control the spread of mosquito-borne diseases.

  In 2010 Karla was awarded a prestigious scholarship from the Mexican government's National Council of Science and Technology (CONACYT) to pursue her graduate studies at Johns Hopkins University (JHU).  During her second year at JHU Karla was part of a research team providing consultation on statistics for the Howard Hughes Medical Institute's Janelia research center.  In 2012 she obtained her Master's degree in Applied Mathematics \& Statistics from JHU and began her doctoral research with Dr. James C. Spall also at JHU.  Karla has given many talks and presentations at different conferences and universities
% The American Control Conference (2014, 2015, 2016), the Conference on In- formation Sciences and Systems (2013, 2015, 2016), the Conference on Applied Statistics in Defense (2014, 2016), University of Maryland's 8th Annual  Prob- ability and Statistics Day (2014), and the Joint SIAM--SMB Conference on the Life Sciences (2006). She has also given several talks
%and at JHU 
on topics which include stochastic optimization, computer vision, optimal control, optimal design of experiments, and multi-sensor data fusion. She is the author of several peer-reviewed publications and has been a reviewer for several journals and conferences and for John Wiley \& Sons. 


 During her graduate studies Karla took several courses on topics including statistics, probability, optimization, machine learning, computer vision, neural networks, applied optimal control, Monte Carlo methods, graph theory, bioinformatics, computational genomics, system identification, and stochastic optimization. She was also a teaching assistant for over a dozen courses,
% on a broad range of topics 
% (statistics, probability, mathematical finance, matrix analysis, dynamical systems, stochastic optimization, system identification, and Monte Carlo methods, to name a few). She 
 was the course instructor for two undergraduate courses in statistics, and served as the graduate representative of the Applied Mathematics \& Statistics department before JHU's Graduate Representatives Organization.
  
  

 



%\noindent{\bm{Languages:}}
%
% and is fluent in english and spanish and in the matlab, python, and R programming languages.

%\noindent{\bf{Education}}
%
%%Interest in math/physics during high-school college course at local university (Universidad de Colima) in Colima Mexico.
%
%%Obtained a bachelor's degree in mathematics from Universidad de Colima (University of Colima). Her capstone project was predicting the outcome of soccer matches.
%
%Summer program in MTBI at Arizona state u fueled her interest in applied mathematics where she worked on determining the optimal treatment strategies for patients with mental disorders using mathematical models.
%
%After graduating worked at the IIDET of the university on mosquito thing.
%
%In 2010 obtained prestigious CONACYT scholarship to pursue graduate studies at JHU. There she obtain masters in applied mathematics at JHU.
%
%Worked as a statistics consultant for Janelia.
%
%In 2012 began working on her doctoral research project with Dr. James C. Spall at JHU.
%
%
%\noindent{\bf{Courses}}
%
%During her graduate studies at Johns Hopkins Karla took several courses in statistics, probability, optimization, machine learning, computer vision, neural networks, applied optimal control, monte carlo methods, graph theory, bioinformatics, computational genomics, system identification, stochastic optimization, pattern recognition . She also took a language course in the German department.
%
%\noindent{\bf{Teaching}} 
%
%Karla has TA-ed for several courses on a broad range of topics (a few courses, statistics, probability, mathematical finance, matrix analysis, dynamical systems, stochsatic optimization, system identification, monte carlo methods). She was also the course instructor for two (different) undergraduate level courses in statistics. She also taught a review course in MATLAB and matrix analysis for incoming students to the masters in finance program.
%
%
%\noindent{\bf{Peer-Reviewed publications}}
%
%Author of several peer-reviewed publications.
%
%
%
%\noindent{\bf{Talks/Presentations}}
%
%Several talks and presentations at different conferences and universities. 
%
%The American Control Conference
%(2014, 2015, 2016), the Conference on Information Sciences and Systems (2013, 2015,
%2016), the Conference on Applied Statistics in Defense (2014, 2016), University of Maryland?s
%8th Annual Probability and Statistics Day (2014), and the Joint SIAM?SMB Conference
%on the Life Sciences (2006).
%
%
%
%She has also given several talks at JHU on topics which included research in
%stochastic optimization, computer vision, optimal control, optimal design of experiments, and multi-sensor data fusion.
%
%
%\noindent{\bf{Other}} 
%
%Graduate representative of the AMS department at the GRO.
%
%Co-supervised master student's research project.
%
%Reviewed a book proposal.
%
%Reviewer for several journals and conferences
%
%Fluent in spanish and english and has some knowledge of German and French. She is also fluent in the matlab, python, and R programming languages
%

\end{vita}

==> chapter4.tex <==
%!TEX root = root.tex

\chapter[Generalizations: Non-Cyclic Behavior]{Generalizations:\\ Non-Cyclic Behavior}
\label{sec:gen1}
\chaptermark{First Generalizations}

In this section, we provide conditions for the convergence of a non-seesaw generalization of CSG and CSPSA to a minimizer $\bm\uptheta^\ast$ of $L(\bm\uptheta)$. In these generalizations it is assumed that each subvector will be updated infinitely often (i.o.) w.p.1. While a strictly alternating (strictly seesaw) algorithm satisfies the assumption of updating each subvector i.o., the assumption allows for more general behavior. For example, if at each step a choice of whether to update the first subvector or the second is made according to a $\text{Bernoulli}(p)$ distribution with $0<p<1$ then the i.o. assumption will also be satisfied.

First we clarify that  our generalization to non-seesaw behavior {\it{includes}}, as a particular case, the cyclic seesaw case as discussed in the opening paragraph of this section. We will be assuming each subvector is updated i.o. w.p.1. For example, the sequence of updates could look something like:
\begin{align}
\label{eq:newnot}
\bm\uptheta(0){\overset{j_0}{\longrightarrow}}\bm\uptheta(1)\overset{j_1}{\longrightarrow} \bm\uptheta(2)\overset{j_2}{\longrightarrow} \bm\uptheta(3)\overset{j_3}{\longrightarrow} \cdots
\end{align}
%For simplicity we deviate from our usual notation involving ``intermediate'' updates and use the following instead:
%\begin{align}
%\bm{{\hat{\uptheta}}}_{0}{\overset{j_0}{\longrightarrow}} \bm{{\hat{\uptheta}}}_{1}\overset{j_1}{\longrightarrow} \bm{{\hat{\uptheta}}}_{2}\overset{j_2}{\longrightarrow} \bm{{\hat{\uptheta}}}_{3}\overset{j_3}{\longrightarrow} \cdots
%\end{align}
where $j_k\in\{0,1\}$. Eqn. (\ref{eq:newnot}) will be taken to mean that $\bm\uptheta(k+1)$ was obtained from $\bm\uptheta(k)$ by updating its $j_k$th subvector (recall $j_k$ will either be 1 or 2 to indicate whether the first or second subvector is updated). At each subiterateion, a decision is made to update the first or the second subvectors of the current estimate. As an example, consider the following sequence:
%To further clarify the change of notation, consider the following sequence generated with our usual (cyclic) notation: 
%Such a situation still assumes the existence of a global clock which keeps track of iteration number, namely $k$. 
%\begin{align*}
%\bm{{\hat{\uptheta}}}_{0}\rightarrow \bm{{\hat{\uptheta}}}_{0}^{(I)}\rightarrow \bm{{\hat{\uptheta}}}_{1}\rightarrow \bm{{\hat{\uptheta}}}_{1}^{(I)}\rightarrow\cdots
%\end{align*}
%In the new notation we would simply have:
\begin{align}
\label{eq:sampseq}
\bm\uptheta(0){\overset{1}{\longrightarrow}} \bm\uptheta(1)\overset{2}{\longrightarrow}\bm\uptheta(2)\overset{1}{\longrightarrow} \bm\uptheta(3)\overset{2}{\longrightarrow} \cdots,
\end{align}
the alternating behavior of the $j_k$'s indicates a cyclic seesaw algorithm was used so that:
\begin{align*}
\bm\uptheta(0)=\bm{{\hat{\uptheta}}}_{0},\ \ \bm\uptheta(1)=\bm{{\hat{\uptheta}}}_{0}^{(I)},\ \ \bm\uptheta(2)=\bm{{\hat{\uptheta}}}_{1},\ \ \bm\uptheta(3)=\bm{{\hat{\uptheta}}}_{1}^{(I)}, \cdots
\end{align*}
so that (\ref{eq:sampseq}) is equivalent to:
\begin{align}
\label{eq:simto}
\bm{{\hat{\uptheta}}}_{0}{{\longrightarrow}} \bm{{\hat{\uptheta}}}_{0}^{(I)}{\longrightarrow}\bm{{\hat{\uptheta}}}_{1}{\longrightarrow}\bm{{\hat{\uptheta}}}_{1}^{(I)}{\longrightarrow} \cdots,
\end{align}
Because the generalization discussed in this section does not imply a strictly alternating sequence of updates, another realization could look something like:
\begin{align}
\label{eq:posca}
\bm\uptheta(0){\overset{1}{\longrightarrow}} \bm\uptheta(1)\overset{1}{\longrightarrow} \bm\uptheta(2)\overset{2}{\longrightarrow} \bm\uptheta(3)\overset{2}{\longrightarrow} \cdots,
\end{align}
such a sequence will be represented in the equivalent notation:
\begin{align*}
\bm\uptheta(0)=\bm{{\hat{\uptheta}}}_{0},\ \bm\uptheta(1)=\bm{{\hat{\uptheta}}}_{0}^{(I)_1},\ \bm\uptheta(2)=\bm{{\hat{\uptheta}}}_{0}^{(I)_2}, \bm\uptheta(3)=\bm{{\hat{\uptheta}}}_{1}
\end{align*}
so that similar to the equivalence between (\ref{eq:sampseq}) and (\ref{eq:simto}), we can rewrite (\ref{eq:posca}) as:
\begin{align}
\label{eq:pazaak}
\bm{{\hat{\uptheta}}}_{0}{{\longrightarrow}} \bm{{\hat{\uptheta}}}_{0}^{(I)_1}{\longrightarrow}\bm{{\hat{\uptheta}}}_{0}^{(I)_2}{\longrightarrow}\bm{{\hat{\uptheta}}}_{1}{\longrightarrow} \cdots,
\end{align}
Note that the assumption of updating each subvector i.o. does not imply there is a particular cyclic seesaw pattern and the original notion of intermediate steps is lost.  In general, we will say an iteration is complete as soon as all subvectors have been updated at least once; during the $k$th iteration $\bm{{\hat{\uptheta}}}_{k}$ is obtained via a sequence of updates beginning at $\bm{{\hat{\uptheta}}}_{k-1}$. In the previous sequence we see that during the first iteration, the first subvector was updated twice while the second subvector was only updated once. However, by assumption both subvectors will (eventually) be updated infinitely often w.p.1. 


The proof of convergence  of this method in the setting where each coordinate is updated i.o. w.p.1 is identical to that of Theorem 1. The following sections discuss the generalization in more detail.
\section{Generalization of CSG  to Non-Seesaw Behavior}
\label{subsec:alternatingSG1}

The values $\bm{{\hat{\uptheta}}}_{k}$ in this generalized algorithm obey the following recursion:
\begin{align}
\label{eq:gencsg}
&\bm\uptheta({k+1})=\bm\uptheta(k)-a_{n_k}^{(j_k)}{\bm{Y}}^{(j_k)}(\bm\uptheta(k)),\\
&\bm\uptheta(0)=\bm{{\hat{\uptheta}}}_{0},\\
& \bm{{\hat{\uptheta}}}_{k} {\textnormal{ is defined recursively (see below),}}
\end{align}
where $n_k$ denotes the number of times subvector $j_k$ has been updated by time $k$ (recall that $j_k\in\{0,1\}$ when there are only two subvectors). While $j_k$ allows us to keep track of what gain sequence to use, $n_k$ tells us which element of that gain sequence is required (recall there are two gain sequences corresponding to the two subvectors). Furthermore, $\bm{{\hat{\uptheta}}}_{k}$ is defined recursively: given that $\bm{{\hat{\uptheta}}}_{k}=\bm\uptheta(m_1)$ for some nonnegative integer $m_1$, we have $\bm{{\hat{\uptheta}}}_{k+1}=\bm\uptheta(m_2)$ if $m_2$ is an integer strictly greater than $m_1$  and the sequence:
\begin{align*}
j_{m_1},\ j_{m_1+1},\ j_{m_1+2}, \cdots, j_{m_2}
\end{align*}
is the shortest sequence for $j_k$ beginning at $k=m_1$ that contains at least one $0$ and one $1$. In other words, given that $\bm{{\hat{\uptheta}}}_{k}=\bm\uptheta(m_1)$, the next iterate $\bm{{\hat{\uptheta}}}_{k+1}$ will be determined as soon as each subvector has been updated at least once. Because of this definition, it is possible for the number of subiterations to vary between iterations.

The following theorem states that under the same conditions of theorem 1 we can prove convergence of this generalization of CSG.

\noindent{\bf{Theorem 4}}: Let conditions A0--A4 hold. Furthermore, assume $E[{\bm{Y}}(\bm\uptheta)|\bm\uptheta]={\bm{g}}(\bm\uptheta)$ for all $\bm\uptheta$. Then, the generalization of the CSG algorithm given by eqn.(\ref{eq:gencsg}) to the case where each subvector is updated i.o. w.p.1 (i.e., $j_k=0$ i.o. and $j_k=2$ i.o. w.p.1) converges to $\bm\uptheta^{\ast}$ w.p.1.

\noindent{\it{Proof:}} As usual, all probabilistic arguments will be assumed to hold w.p.1. Given that each coordinate will be updated infinitely often, we know that (w.p.1) a realization:
\begin{align*}
\bm{{\hat{\uptheta}}}_{0}{\overset{j_0}{\longrightarrow}} \bm{{\hat{\uptheta}}}_{1}\overset{j_1}{\longrightarrow} \bm{{\hat{\uptheta}}}_{2}\overset{j_2}{\longrightarrow} \bm{{\hat{\uptheta}}}_{3}\overset{j_3}{\longrightarrow} \cdots
\end{align*}
will have $j_k=1$ infinitely often and $j_k=2$ infinitely often.  Adapting the proof of theorem 1 to the notation in eqn. (\ref{eq:gencsg}) we have:
\begin{align*}
E\left[f(\bm\uptheta(k+1))-f(\bm\uptheta(k))|\bm\uptheta(k)\right]\leq &-{\bm{f'}}(\bm\uptheta(k))^\top\bm{g}^{(j_k)}(\bm\uptheta(k))\left(a_{n_k}^{(j_k)}-b_3\cdot (a_{n_k}^{(j_k)})^2\right)\\
&+b_4\cdot(a_{n_k}^{j_k})^2(1+f(\bm\uptheta(k)).
\end{align*}
Now, we also make another natural adaptation of the notation from the proof of Theorem 1:
\begin{align*}
a_0\equiv a_{n_0}^{(j_0)}, \ a_1\equiv a_{n_1}^{(j_1)}, \ a_2\equiv a_{n_2}^{(j_2)}, \ a_3\equiv a_{n_3}^{(j_3)}, \ \cdots
\end{align*}
and:
\begin{align*}
\upvarphi_k\equiv \upvarphi(\bm\uptheta(k))\equiv\bm{f'}(\bm\uptheta(k))^\top\bm{g}^{(j_k)}(\bm\uptheta(k))
\end{align*}
Using our previous notation for $W_{k}$ and $\upalpha_k$ we derive (in the same manner as in the proof of theorem 1) the inequality:
\begin{align*}
E[W_{k+1}-W_k|\bm\uptheta(k)]\leq -\upalpha_k\upvarphi_k
\end{align*}
 so that $W_k$ is eventually (for $k$ large enough) a nonnegative supermartingale. As before, this implies $f(\bm\uptheta(k))$ has a finite limit. The rest of the proof is identical to that of Theorem 1. \hfill $\Box$
% similarly to ACC-2014, we have:
% \begin{align*}
% &\sum_{j_k=1}\upalpha_{k}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
% +&\sum_{j_k=0}\upalpha_{k}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(2)}(\bm{{\hat{\uptheta}}}_{k})<\infty.
% \end{align*}
%From this we obtain that $\bm{{\hat{\uptheta}}}_{k}\rightarrow \bm\uptheta^\ast$. 

While this proof also applies to the CSG algorithm we present it as a generalization in the hope that the underlying ideas will be made clearer by addressing the cyclic case first. Since we have proven convergence under the same conditions as those required in Theorem 1, the corollary to said theorem still applies.

\section{Generalization of CSPSA  to Non-Seesaw Behavior}
\label{subsec:alternatingSPSA}

Similarly to section \ref{subsec:alternatingSG1}, here we consider a generalized version of CSPSA where the assumption is that each subvector will be updated i.o. w.p.1. Similar to eq. (\ref{eq:gencsg}) this generalization of CSPSA is given by:
\begin{align}
\label{eq:gencspsa}
&\bm\uptheta(k+1)=\bm\uptheta(k)-a_{n_k}^{(j_k)}\left[{\bm{g}}^{(j_k)}(\bm\uptheta(k))+{\bm{\upbeta}_k^{(j_k)}}+{\bm{\upxi}_k^{(j_k)}}\right],\\
&\bm\uptheta(0)= \bm{{\hat{\uptheta}}}_{0},\\
& \bm{{\hat{\uptheta}}}_{k} {\textnormal{ is defined recursively (see below).}}
\end{align}
As in section \ref{subsec:alternatingSG1}, $n_k$ represents the number of times subvector $j_k$ has been updated by time $k$ and $\bm{{\hat{\uptheta}}}_{k}$ is obtained from $\bm{{\hat{\uptheta}}}_{k-1}$ as soon as each subvector has been updated at least once.
%a_{k}^{(2)}\left({\bm{g}}^{(2)}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upbeta}_{k}^{(2)}}+{\bm{\upxi}_{k}^{(2)}}\right)


To prove the convergence of this generalized version of SPSA we introduce a set of conditions that is very similar to the $A$ conditions (see for section \ref{sec:ay} for notation definition):
\begin{description} 
\item[C0] ${\bm{H}}(\bm\uptheta)$ has bounded entries for all $\bm\uptheta$,
\item[C1] $ \sum_{k=0}^{\infty}\left(a_{k}^{(j)}\right)^{2}<\infty$, $\sum_{k=0}^{\infty}a_{k}^{(j)}=\infty$,
\item[C2] $f(\bm\uptheta)\geq0$, $f(\bm\uptheta^{\ast})=0$, $f(\bm\uptheta)\rightarrow \infty$ as $\|\bm\uptheta\|\rightarrow \infty$,
\item[C3] ${\displaystyle{\inf_{\upvarepsilon<\|\bm\uptheta-\bm\uptheta^{\ast}\|<1/\upvarepsilon}}}{\bm{f'}}(\bm\uptheta)^\top\overline{{\bm{g}}}^{(j)}(\bm\uptheta)>0$, ${\bm{f'}}(\bm\uptheta)^\top\overline{{\bm{g}}}^{(j)}(\bm\uptheta)\geq0$ where $\overline{\bm{g}}^{(j)}(\bm\uptheta)$ is defined as:
\begin{align*}
\overline{\bm{g}}^{(j)}(\bm\uptheta)\equiv E[\hat{\bm{g}}^{(j)}|\bm\uptheta]=\bm{g}^{(j)}(\bm\uptheta)+E[\bm\upbeta^{(j)}|\bm\uptheta],
\end{align*}
\item[C4] $\|{\bar{\bm{g}}}^{(j)}(\bm\uptheta)\|^{2}+E[\|{\bm{\upxi}}^{(j)}(\bm\uptheta)\|^{2}|\bm\uptheta]\leq b_{1}(1+f(\bm\uptheta))+b_{2}{\bm{f'}}(\bm\uptheta)^\top\bar{{\bm{g}}}^{(j)}(\bm\uptheta)$ for constants $b_{1}$ and $b_{2}$; without loss of generality, these constants are assumed to be strictly positive,
%\item[C5] Assume $\{\bm\upbeta_{k}^{(j)}\}$ is bounded w.p.1 and $\bm\upbeta_{k}^{(j)}\rightarrow {\bm{0}}$ w.p.1 for $j=1,2$.
\end{description}
Sigma al
Conditions C0--C2 are identical to A0--A2 while C3 and C4 are modified versions of A3 and A4. 

\noindent{\bf{Theorem 5}}: Let conditions C0--C5 hold. Then, the generalization of the CSPSA algorithm given by eqn.(\ref{eq:gencsg}) to the case where each subvector is updated i.o. w.p.1 (i.e., $j_k=0$ i.o. and $j_k=2$ i.o. w.p.1) converges to $\bm\uptheta^{\ast}$ w.p.1.\\

\noindent {\it{Proof:}} First we have:
\begin{align*}
&E[f(\bm\uptheta(k+1))-f(\bm\uptheta(k))|\bm\uptheta(k)]=-a_{n_k}^{(j_k)}\bm{f'}(\bm\uptheta(k))^\top\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\\
%&-a_{n_k}^{(j_k)}\bm{f'}(\bm\uptheta(k))^\top E\big[\bm{\upbeta}^{(j_k)}_k\big|\bm\uptheta(k)\big]\\
%E[f(\bm\uptheta(k+1))|\bm\uptheta(k)]-f(\bm\uptheta(k))\\
%&=-a_{n_k}^{(j_k)}E\Big[{\bm{f'}}(\bm\uptheta(k))^\top\left({\bm{g}}^{(j_k)}(\bm\uptheta(k))+{\bm{\upbeta}_{k}^{(j_k)}}+{\bm{\upxi}_{k}^{(j_k)}}\right)\Big|\bm\uptheta(k)\Big]\\
%&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2E\left[\bm{Y}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k){\bm{Y}}^{(j_k)}(\bm\uptheta(k))\Big|\bm\uptheta(k)\right]\\
&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\\
%&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2E\left[\bm{\upbeta}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)\bm{\upbeta}^{(j_k)}(\bm\uptheta(k))\big|\bm\uptheta(k)\right]\\
&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2E\left[\bm{\upxi}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)\bm{\upxi}^{(j_k)}(\bm\uptheta(k))\big|\bm\uptheta(k)\right]
%&+\left(a_{n_k}^{(j_k)}\right)^2\bm{g}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)E\left[\bm{\upbeta}^{(j_k)}_k\big|\bm\uptheta(k)\right] 
\end{align*}
where $\bar{\bm\uptheta}_k=\uplambda\bm\uptheta(k)+(1-\uplambda)\bm\uptheta(k+1)$ for some $\uplambda\in[0,1]$. By C0 and C4 we have the following inequality:
\begin{align*}
&E[f(\bm\uptheta(k+1))-f(\bm\uptheta(k))|\bm\uptheta(k)]\leq-a_{n_k}^{(j_k)}\bm{f'}(\bm\uptheta(k))^\top\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\\
&+\frac{c}{2}\cdot\left(a_{n_k}^{(j_k)}\right)^2\left[b_1(1+f(\bm\uptheta(k)))+b_2\bm{f'}(\bm\uptheta(k))^\top\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\right]
\end{align*}
%\begin{align*}
%E[f(\bm{{\hat{\uptheta}}}_{k}^{(I)})-f(\bm{{\hat{\uptheta}}}_{k})|\bm{{\hat{\uptheta}}}_{k}]\leq&-a_k^{(1)}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
%&+\frac{c}{2}\cdot\left(a_{k}^{(1)}\right)^2\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
%&+\frac{c}{2} E\left[\bm\upxi^{(1)}(\bm{{\hat{\uptheta}}}_{k})^\top\bm\upxi^{(1)}(\bm{{\hat{\uptheta}}}_{k})\Big|\bm{{\hat{\uptheta}}}_{k}\right]\\
%=&-a_k^{(1)}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
%&+\frac{c}{2}\cdot\left(a_{k}^{(1)}\right)^2\left(\|\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\|^2+E[\|\bm{\upxi}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\|^2\big|\bm{{\hat{\uptheta}}}_{k}]\right)
%\end{align*}
%for a constant $c>0$. By condition A4:
Using our previous notation for $W_{k}$ and $\upalpha_k$ while replacing $\bm{g}$ with $\bar{\bm{g}}$ we derive (in the same manner as in the proof of theorem 1) the inequality:
\begin{align*}
E[W_{k+1}-W_k|\bm\uptheta(k)]\leq -\upalpha_k\upvarphi_k
\end{align*}
 so that $W_k$ is eventually (for $k$ large enough) a nonnegative supermartingale. As before, this implies $f(\bm\uptheta(k))$ has a finite limit. The rest of the proof is identical to that of Theorem 1. \hfill $\Box$

%\section{Deterministic Patterns}
%\section{Randomized Coordinate Selection}
%\section{Randomized Patterns}


==> thesis arXiv 2/CV.tex <==
%!TEX root = root.tex

\fancyhead{} % clear all header and footer fields
\fancyhead[L]{CURRICULUM VITAE} % except the center
\begin{vita}

%\begin{wrapfigure}{R}{0.3\textwidth}
%  \begin{center}
%    \includegraphics[width=0.2\textwidth]{rjvheadshot}
%  \end{center}
%  \caption{Karla Hern\'andez-Cuevas was born on November 1986 in Mexico City, Mexico.}
%\end{wrapfigure}


Karla Hern\'andez-Cuevas was born on November 1986 in Mexico City. Her interest in mathematics began in high-school after the local university, the University of Colima (Universidad de Colima), offered high-school seniors the opportunity to take mathematics and physics courses taught at an undergraduate-level. Her interest in applied mathematics deepened after interning at the Mathematical and Theoretical Biology Institute at Arizona State University where  she worked on determining optimal treatment strategies for patients with mental disorders. After graduating form high-school she went on to obtain her Bachelor's degree in mathematics in 2009 from the University of Colima. Her undergraduate dissertation involved predicting the outcomes of UEFA (Union of European Football Associations) Champions League matches. After obtaining her Bachelor's degree Karla went on to intern at the Institute for Innovation and Technological Development (Instituto de Innovaci\'on y Desarrollo Tecnol\'ogico) at the University of Colima. There, she participated in a state-wide campaign to control the spread of mosquito-borne diseases.

  In 2010 Karla was awarded a prestigious scholarship from the Mexican government's National Council of Science and Technology (CONACYT) to pursue her graduate studies at Johns Hopkins University (JHU).  During her second year at JHU Karla was part of a research team providing consultation on statistics for the Howard Hughes Medical Institute's Janelia research center.  In 2012 she obtained her Master's degree in Applied Mathematics \& Statistics from JHU and began her doctoral research with Dr. James C. Spall also at JHU.  Karla has given many talks and presentations at different conferences and universities
% The American Control Conference (2014, 2015, 2016), the Conference on In- formation Sciences and Systems (2013, 2015, 2016), the Conference on Applied Statistics in Defense (2014, 2016), University of Maryland's 8th Annual  Prob- ability and Statistics Day (2014), and the Joint SIAM--SMB Conference on the Life Sciences (2006). She has also given several talks
%and at JHU 
on topics which include stochastic optimization, computer vision, optimal control, optimal design of experiments, and multi-sensor data fusion. She is the author of several peer-reviewed publications and has been a reviewer for several journals and conferences and for John Wiley \& Sons. 


 During her graduate studies Karla took several courses on topics including statistics, probability, optimization, machine learning, computer vision, neural networks, applied optimal control, Monte Carlo methods, graph theory, bioinformatics, computational genomics, system identification, and stochastic optimization. She was also a teaching assistant for over a dozen courses,
% on a broad range of topics 
% (statistics, probability, mathematical finance, matrix analysis, dynamical systems, stochastic optimization, system identification, and Monte Carlo methods, to name a few). She 
 was the course instructor for two undergraduate courses in statistics, and served as the graduate representative of the Applied Mathematics \& Statistics department before JHU's Graduate Representatives Organization.
  
  

 



%\noindent{\bm{Languages:}}
%
% and is fluent in english and spanish and in the matlab, python, and R programming languages.

%\noindent{\bf{Education}}
%
%%Interest in math/physics during high-school college course at local university (Universidad de Colima) in Colima Mexico.
%
%%Obtained a bachelor's degree in mathematics from Universidad de Colima (University of Colima). Her capstone project was predicting the outcome of soccer matches.
%
%Summer program in MTBI at Arizona state u fueled her interest in applied mathematics where she worked on determining the optimal treatment strategies for patients with mental disorders using mathematical models.
%
%After graduating worked at the IIDET of the university on mosquito thing.
%
%In 2010 obtained prestigious CONACYT scholarship to pursue graduate studies at JHU. There she obtain masters in applied mathematics at JHU.
%
%Worked as a statistics consultant for Janelia.
%
%In 2012 began working on her doctoral research project with Dr. James C. Spall at JHU.
%
%
%\noindent{\bf{Courses}}
%
%During her graduate studies at Johns Hopkins Karla took several courses in statistics, probability, optimization, machine learning, computer vision, neural networks, applied optimal control, monte carlo methods, graph theory, bioinformatics, computational genomics, system identification, stochastic optimization, pattern recognition . She also took a language course in the German department.
%
%\noindent{\bf{Teaching}} 
%
%Karla has TA-ed for several courses on a broad range of topics (a few courses, statistics, probability, mathematical finance, matrix analysis, dynamical systems, stochsatic optimization, system identification, monte carlo methods). She was also the course instructor for two (different) undergraduate level courses in statistics. She also taught a review course in MATLAB and matrix analysis for incoming students to the masters in finance program.
%
%
%\noindent{\bf{Peer-Reviewed publications}}
%
%Author of several peer-reviewed publications.
%
%
%
%\noindent{\bf{Talks/Presentations}}
%
%Several talks and presentations at different conferences and universities. 
%
%The American Control Conference
%(2014, 2015, 2016), the Conference on Information Sciences and Systems (2013, 2015,
%2016), the Conference on Applied Statistics in Defense (2014, 2016), University of Maryland?s
%8th Annual Probability and Statistics Day (2014), and the Joint SIAM?SMB Conference
%on the Life Sciences (2006).
%
%
%
%She has also given several talks at JHU on topics which included research in
%stochastic optimization, computer vision, optimal control, optimal design of experiments, and multi-sensor data fusion.
%
%
%\noindent{\bf{Other}} 
%
%Graduate representative of the AMS department at the GRO.
%
%Co-supervised master student's research project.
%
%Reviewed a book proposal.
%
%Reviewer for several journals and conferences
%
%Fluent in spanish and english and has some knowledge of German and French. She is also fluent in the matlab, python, and R programming languages
%

\end{vita}

==> thesis arXiv 2/chapter0.tex <==
%!TEX root = root.tex

%% FRONTMATTER
\begin{frontmatter}

% generate title
\maketitle



\begin{abstract}


Stochastic approximation (SA) is a powerful class of iterative algorithms for nonlinear root-finding that can be used for minimizing a  loss function, $L(\bm\uptheta)$, with respect to a parameter vector $\bm\uptheta$, when only noisy observations of $L(\bm\uptheta)$ or its gradient are available (through the natural connection between root-finding and minimization); SA algorithms can be thought of as stochastic line search methods where the entire parameter vector is updated at each iteration. 
%
The cyclic approach to SA is a variant of SA procedures where $\bm\uptheta$ is divided into multiple subvectors that are updated one at a time in a cyclic manner. 

This dissertation focuses on studying the asymptotic properties of cyclic SA and of the generalized cyclic SA (GCSA) algorithm, a variant of cyclic SA where the subvector to update may be selected according to a random variable or according to a predetermined pattern, and where the noisy update direction can be based on the updates of any SA algorithm (e.g., stochastic gradient, Kiefer--Wolfowitz, or simultaneous perturbation SA). The convergence of GCSA, asymptotic normality of GCSA (related to rate of convergence), and efficiency of GCSA relative to its non-cyclic counterpart are investigated both analytically and numerically. Specifically, conditions are obtained for the convergence with probability one of the GCSA iterates and for the asymptotic normality of the normalized iterates of a special case of GCSA. Further, an analytic expression is given for the asymptotic relative efficiency (when efficiency is defined in terms of mean squared error) between a special case of GCSA and its non-cyclic counterpart. Finally, an application of the cyclic SA scheme to a multi-agent stochastic optimization problem is investigated.


This dissertation also contains two appendices. The first appendix generalizes Theorem 2.2 in Fabian (1968) (a seminal paper in the SA literature that derives general conditions for the asymptotic normality of SA procedures) to make the result more applicable to some modern applications of SA including (but not limited to) the GCSA algorithm, certain root-finding SA algorithms, and certain second-order SA algorithms. The second appendix considers the problem of determining the presence and location of a static object within an area of interest by combining information from multiple sensors using a maximum-likelihood-based approach.


\vfill
\noindent {\bf{Primary Reader and Advisor:}} James C. Spall\\
{\bf{Second Reader:}} Raman Arora
\end{abstract}

\begin{dedication}
 \begin{center}
{\it{To my parents.}}
\end{center}

\end{dedication}

\begin{acknowledgment}


 I would first like to thank my advisor, James Spall, for his invaluable guidance throughout my graduate studies. His dedication to his students, patience, admirable work ethic, and vast knowledge were instrumental in making my experience as a graduate student fruitful, enjoyable, and enriching. 


I would also like to give special thanks to Stephen Lee, my husband and best friend, for his friendship, support, and for the {\it{many}} interesting discussions we've shared (of a mathematical and non-mathematical nature) throughout our time together. I would also like to mention that the proof of Lemma \ref{lem:devil} was the result of a discussion with Stephen. 

I would also like to thank fellow graduate student Jingyi Zhu (currently a Ph.D. student at the department of Applied Mathematics \& Statistics at Johns Hopkins) for reading Chapter \ref{sec:cyclicseesaw} of my dissertation and for her detailed feedback which helped me improve the presentation of the chapter.

I would also like to express my gratitude to Raman Arora, Danial Naiman, Daniel Robinson, Maxim Bichuch, and John Wierman, the members of my dissertation defense committee, for their time with special thanks to Raman Arora, my second reader; reviewing such a lengthy dissertation is no small task and I sincerely appreciate his help.

I also want to thank all the professors whose courses I've had the pleasure of taking. Although I have taken several courses during my studies at Hopkins, the courses taught by professors James Fill, James Spall, and John Wierman stand out as having been instrumental to my research.

Last but not least, I would like to thank my family with special thanks to my parents. Without their support I would not be where I am today.

This work was financially supported by the National Council of Science and Technology (CONACYT) of Mexico, the Office of Naval Research via Navy contract N00024-13-D6400, the Acheson J. Duncan Fund for the Advancement of Research in Statistics, and Dr. James Spall's JHU/APL sabbatical professorship
at Johns Hopkins' Whiting School of Engineering.
\end{acknowledgment}



% generate table of contents
\tableofcontents

% generate list of tables
\listoftables

% generate list of figures
\listoffigures

\end{frontmatter}


==> thesis arXiv 2/chapter1.tex <==
%!TEX root = root.tex

\chapter{Introduction}
\label{chap:intro}
%\chaptermark{Introduction}

\section{Motivation}


The objective of unconstrained optimization problems is to minimize a real-valued loss function $L(\bm\uptheta)$ with respect to a parameter vector $\bm\uptheta\in \mathbb{R}^p$. 
%
An important limitation in many practical problems is the fact that the loss function itself is unknown in the sense that $L(\bm\uptheta)$ may only be observable in the presence of noise. For example, suppose that the loss function represents the expected output of a complex stochastic system that depends on $\bm\uptheta$. In this case, obtaining a closed form expression for $L(\bm\uptheta)$ (or even evaluating $L(\bm\uptheta)$ at a given $\bm\uptheta$) may be impossible since computing the expected output would require detailed knowledge of the stochastic process governing the output of the system. In this light, this dissertation makes a distinction between deterministic optimization, where the loss function is known and the optimization process is entirely deterministic, and stochastic optimization, where the optimization process involves some type of randomness (e.g., the optimization algorithm uses measurements of $L(\bm\uptheta)$ that are corrupted by random noise or there is a random choice made in the search direction as the algorithm iterates towards a solution). Stochastic approximation (SA) is a powerful class of iterative algorithms for nonlinear root-finding. These algorithms can also be used for stochastic optimization (through the natural connection between root-finding and minimization). The cyclic approach to SA is a particular variant of these iterative procedures in which only a subset of the parameter vector (referred to as a {\it{subvector}}) is updated at any given time. This dissertation focuses on studying the asymptotic properties (e.g., convergence and rate of convergence) of cyclic SA (and generalizations) for stochastic optimization.

  In the cyclic approach, the full parameter vector is divided into two or more subvectors and the process proceeds by sequentially updating each of the subvectors, while holding the remaining parameters at their most recent values. Thus, the cyclic approach is iterative in nature and at each iteration an estimate for the minimizer of $L(\bm\uptheta)$ is obtained. To illustrate the idea behind the cyclic approach, let $\hat{\bm{\uptheta}}_k$ denote the estimate obtained during the $k$th iteration. Furthermore, consider the special case of the cyclic approach where there are only two subvectors, $\hat{\bm{\uptheta}}_k^{[1]}$ and $\hat{\bm{\uptheta}}_k^{[2]}$, so that $\hat{\bm{\uptheta}}_k=[(\hat{\bm{\uptheta}}_k^{[1]})^\top,(\hat{\bm{\uptheta}}_k^{[2]})^\top]^\top$. Additionally, for simplicity assume the two subvectors are updated in a strictly-alternating manner.
%  
Here, the first step of an iteration of the cyclic approach would consist of updating $\hat{\bm{\uptheta}}_k^{[1]}$ while keeping $\hat{\bm{\uptheta}}_k^{[2]}$ fixed. This would give rise to the vector $[(\hat{\bm{\uptheta}}_{k+1}^{[1]})^\top,(\hat{\bm{\uptheta}}_k^{[2]})^\top]^\top$. In the second step $\hat{\bm{\uptheta}}_k^{[2]}$ would be updated while holding $\hat{\bm{\uptheta}}_{k+1}^{[1]}$ fixed, this would give rise to the vector $\hat{\bm{\uptheta}}_{k+1}=[(\hat{\bm{\uptheta}}_{k+1}^{[1]})^\top,(\hat{\bm{\uptheta}}_{k+1}^{[2]})^\top]^\top$.

  Independent of whether an optimization algorithm is stochastic or deterministic, cyclic schemes can help reduce the problem's complexity by focusing only on a subset of the parameter vector at any given time. For example, conditional optimization with respect to subsets of $\bm\uptheta$ may prove more tractable than
simultaneous (unconditional) optimization. Lee and Park (2008)\nocite{leenpark2008}, for example, use cyclic optimization to approach a structure-from-motion problem (presented as a deterministic optimization problem), where minimizing $L(\bm\uptheta)$ is difficult but where it is possible to obtain closed form expressions for the minimizers $L(\bm\uptheta)$ with respect to different subsets of $\bm\uptheta$. Lee and Park (2008)\nocite{leenpark2008} propose an algorithm that consists of sequentially minimizing the loss function with respect to the different subsets of $\bm\uptheta$. Although the authors do not provide any theoretical guarantees, the algorithm appears to exhibit good numerical performance. Another example lies in the area of communication networks. Here, one may be interested in jointly optimizing congestion control and scheduling (see, for example, Andrews 2006)\nocite{andrews2006congestion} and it may be the case that conditional solutions are more readily available.


 In the cyclic approach, the full parameter vector is divided into two or more subvectors and the process proceeds by sequentially optimizing each of the subvectors, while holding the remaining parameters at their most recent values. The cyclic approach is of special interest where there is need to extend a model to include new parameters since it allows for the preservation of resources dedicated to optimizing the original problem (e.g., the preservation of expensive software). In theory, one could alternate between updating the new parameters and the parameters from the original problem (existing resources could be reused with this approach).

A convenient feature of cyclic line search methods like block coordinate descent is that computing partial update directions (e.g., computing only a part of the gradient when the update directions are gradient-based) is often significantly less expensive than computing the full update direction. In this vein, Wright (2015)\nocite{wright2015} discusses how coordinate descent algorithms have grown in popularity because of their usefulness in data analysis, and machine learning. Wright (2015)\nocite{wright2015} gives a useful literature review of coordinate descent methods that are mostly limited to deterministic optimization algorithms, with the exception of randomized coordinate descent methods which can be seen as a special case of the stochastic gradient algorithm (a type of SA algorithm).

In the area of multi-agent optimization, the vector $\bm\uptheta$ can be divided into different subsets each of which is updated by a different agent (see, for example, Peterson et al. 2014\nocite{spie2014} and Botts et al. 2016, where $\bm\uptheta$ is a vector related to the positions of the agents)\nocite{bottsetal2016}. In general, agents may operate in a synchronous manner (i.e., agents synchronize the timing of their respective updates in some way, such as by taking turns performing updates) or in an asynchronous manner (i.e., agents do not synchronize the timing of their respective updates in any way). Cyclic optimization algorithms apply given
% provide a convenient model for 
 the manner in which agents operate and, under appropriate conditions, allow for rigorous theoretical analysis of multi-agent optimization algorithms. 

Despite the aforementioned desirable properties of cyclic optimization, convergence to a minimizer of $L(\bm\uptheta)$ (either global or local) is not generally guaranteed for cyclic algorithms. To illustrate this fact, consider an example where $L(\bm\uptheta)=-(\uptau_1+\uptau_2)$ and $\bm\uptheta\in \mathcal{S}\equiv \{[\uptau_1,\uptau_2]^\top{\text{such that $\uptau_1\in [0,1]$ and $\uptau_2\in[0,2(1-\uptau_1)]$}}\}$ (this set defines a region bounded by a right triangle with base corresponding to the interval $[0,1]$ on the $\uptau_1$-axis, right angle at $[0,0]^\top$, and height 2). This constrained optimization problem has a unique global minimum at $\bm\uptheta^\ast=[0,2]^\top$. Suppose now that a cyclic algorithm is implemented given that one alternates between minimizing $L(\bm\uptheta)$ with respect to $\uptau_1$ and $\uptau_2$, beginning with $\uptau_1$. Furthermore, suppose the algorithm is initialized at $\hat{\bm{\uptheta}}_0=[0,0]^\top$. In its first step, the algorithm will arrive at the point $\hat{\bm{\uptheta}}_1=[1,0]^\top$. Afterwards, the algorithm becomes ``stuck'' at this point since no update in the value of $\uptau_2$ can further educe the loss function value. Thus, this cyclic algorithm would never reach the global minimum at $\bm\uptheta^\ast$. Moreover, the point $\hat{\bm{\uptheta}}_1=[1,0]^\top$ is not even a {\it{local}} minimum. This can be seen by noting that the point $\bm\uptheta_\upepsilon= [1-\upepsilon, 2\upepsilon]^\top$ with $\upepsilon\in [0,1]$ is in the set $\mathcal{S}$
% that $\bm\uptheta_\upepsilon$ can be taken as close to $\hat{\bm{\uptheta}}_1$ as desired by making $\upepsilon$ small, 
 and that $L(\bm\uptheta_\upepsilon)=-(1+\upepsilon)< -1=L(\hat{\bm{\uptheta}}_1)$. For both deterministic- and stochastic optimization algorithms, knowing that a non-cyclic algorithm converges to a minimizer (either local or global) of $L(\bm\uptheta)$ does not automatically imply that their cyclic counterparts also converge to a minimizer or $L(\bm\uptheta)$.

This dissertation introduces the generalized cyclic SA (GCSA) algorithm, a cyclic algorithm where the subvectors are updated using SA. Loosely speaking, at each time increment a subvector of the parameter vector is selected and updated 
%in an update direction which 
according to a direction that
%
is obtained using SA (this includes many popular stochastic update directions including the those used in the Robbins--Monro, Kiefer--Wolfowitz, and simultaneous perturbation SA algorithms). In the GCSA algorithm the subvector to update is not necessarily selected following a deterministic pattern (the term ``generalized'' in ``generalized cyclic SA'' is used precisely to emphasize this fact). A special case of the GCSA algorithm, for example, allows the subvector that is to be updated
%to update 
to be selected according to a random variable that may depend on the iteration number. The following section reviews the literature for existing results on cyclic optimization. We cover both deterministic and stochastic implementations.

Before surveying the literature we first review the basic form of SA algorithms for nonlinear root-finding. This allows us to be more specific when comparing existing results to the results developed in this dissertation.
%
Given a vector $\bm\uptheta$ and a vector-valued function $\bm{f}(\bm\uptheta)$, the  basic SA algorithm for nonlinear root-finding attempts to find a solution to $\bm{f}(\bm\uptheta)=\bm{0}$ in an iterative manner using the recursion $\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k{\bm{Y}}_k(\hat{\bm{\uptheta}}_k)$, where $a_k>0$ is the gain sequence and $-{\bm{Y}}_k(\hat{\bm{\uptheta}}_k)$ is a vector-valued random variable representing a noisy observation of $-\bm{f}(\hat{\bm{\uptheta}}_k)$, the desired update direction. In the analysis of SA algorithms it is often useful to express the vector ${\bm{Y}}_k(\hat{\bm{\uptheta}}_k)$ as follows:
\begin{align}
\label{eq:imastandardupdaedirection}
{\bm{Y}}_k(\hat{\bm{\uptheta}}_k)= {\bm{f}}(\hat{\bm{\uptheta}}_k)+{\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k).
\end{align}
Typically, $\bm\upbeta_k(\hat{\bm{\uptheta}}_k)\equiv E\big[{\bm{Y}}_k(\hat{\bm{\uptheta}}_k)-\bm{f}(\hat{\bm{\uptheta}}_k)\big|\mathcal{F}_k\big]$, ${\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)\equiv {\bm{Y}}_k(\hat{\bm{\uptheta}}_k)-E\big[{\bm{Y}}_k(\hat{\bm{\uptheta}}_k)\big|\mathcal{F}_k\big]$, $\mathcal{F}_k$ is some representation of the history of the process, and $E[\mathcal{X}]$ represents the expected value of the random variable $\mathcal{X}$.
%
In the special case where $\bm{f}(\bm\uptheta)=\bm{g}(\bm\uptheta)$ is the gradient of $L(\bm\uptheta)$, that is when SA is used for stochastic optimization via nonlinear root-finding, $\bm{Y}_k(\hat{\bm{\uptheta}}_k)$ denotes a noisy estimate of the gradient. Here, it is common to replace the notation $\bm{Y}_k(\hat{\bm{\uptheta}}_k)$ with $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$. Therefore, we write $\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$,
%
(Section \ref{sec:dummieyouask} discusses SA in greater detail).


\section{Literature Review}
\label{sec:literaturesurveyrev}


In the 1980s, 1990s, and early 2000s,  Bertsekas and Tsitsiklis (1989)\nocite{bertsekasandtsitsiklis1989}, Luo and Tseng (1992)\nocite{luptseng1992}, Luo and Tseng (1993)\nocite{luptseng1993}, and Tseng (2001)\nocite{tseng2001} made important contributions to understanding the convergence properties of cyclic optimization procedures. However, their analysis focused on deterministic optimization problems, not on the stochastic optimization setting considered in this dissertation. A few more recent references investigating cyclic implementations in the area of deterministic optimization are Tseng and Yung (2009)\nocite{tsengandyun2009}, who investigate the convergence of block-coordinate gradient descent methods for linearly constrained non-smooth separable loss functions, and Spall (2012)\nocite{spallcyclicseesaw2012}, who investigates the convergence properties of general cyclic algorithms. The interested reader can also find a useful literature review of coordinate descent methods (largely for deterministic optimization) in Wright (2015)\nocite{wright2015}. 
%
 A few applications of cyclic procedures for deterministic optimization can be found in the papers by Canutescu and Dunbrack (2003)\nocite{canutescu2003}, who use cyclic procedures for a control problem in robotics, Lee and Park (2008)\nocite{leenpark2008}, who use cyclic optimization for a problem in computer vision, Li and Osher (2009)\nocite{liandosher2009}, who consider a compressed sensing problem, and Li and Petropulu (2014)\nocite{liandpetriouli2014}, who use the alternating directions method of multipliers (a cyclic procedure) for target location estimation. 

The previous references are concerned with cyclic schemes for solving deterministic optimization problems. In the area of stochastic optimization, one class of SA algorithms which at first appears to be related to GCSA is the class of two time-scales SA algorithm studied in Borkar (1997)\nocite{borkar1997} (see also Konda and Tsitsiklis 2004\nocite{kondaandtsitsiklis2004} for a similar setting). Here, a parameter vector, $\bm{X}(k)$, is updated using SA. In Borkar's (1997)\nocite{borkar1997} formulation, obtaining the SA update direction requires a second SA step. Specifically, using Borkar's (1997)\nocite{borkar1997} notation, there exists a vector $\bm{U}(k)$ such that:
\begin{subequations}
\begin{align}
\bm{X}(k+1)&=\bm{X}(k)+ a(k)\left[\bm{R}(\bm{X}(k),\bm{U}(k))+\bm{M}(k+1)\right],\label{eq:sandhoneygrow0}\\
\bm{U}(k+1)&=\bm{U}(k)+b(k)\left[\bm{G}(\bm{X}(k),\bm{U}(k))+\bm{N}(k+1)\right],
\label{eq:sandhoneygrow}
\end{align}
\end{subequations}
where $a(k)$ and $b(k)$ are real sequences, $\bm{R}(\cdot,\cdot)$ and $\bm{G}(\cdot,\cdot)$ are deterministic vector valued functions, and $\bm{M}(k+1)$ and $\bm{N}(k+1)$ are random noise terms. Thus, the terms in square brackets in (\ref{eq:sandhoneygrow0},b) are SA update directions for $\bm{X}(k)$ and $\bm{U}(k)$. 
%Implementing (\ref{eq:sandhoneygrow}) would require alternating between updating $\bm{X}(k)$ and $\bm{Y}(k)$. 
By letting $\bm\uptheta=[\bm{X}^\top,\bm{U}^\top]^\top$ and setting $\bm{R}(\cdot,\cdot)=\bm{G}(\cdot,\cdot)$ it may appear that any strictly alternating cyclic SA algorithm with disjoint subvectors is a special case of (\ref{eq:sandhoneygrow0},b), but this is not true.
To see that (\ref{eq:sandhoneygrow0},b) is not a cyclic recursion, note that the recursion in (\ref{eq:sandhoneygrow0},b) implies that the values of $\bm{X}(k+1)$ and $\bm{U}(k+1)$ are both obtained based on the vector $[\bm{X}(k)^\top,\bm{U}(k)^\top]^\top$. In a cyclic algorithm, however, the values of $\bm{X}(k+1)$ and $\bm{U}(k+1)$ would be obtained based on the vectors $[\bm{X}(k)^\top,\bm{U}(k)^\top]^\top$ and $[\bm{X}(k)^\top,\bm{U}(k+1)^\top]^\top$, respectively (assuming $\bm{X}(k)$ is updated first). Therefore, the pair in (\ref{eq:sandhoneygrow0},b) is not cyclic.  The remainder of this section discusses the results that most closely resemble GCSA.

Tsitsiklis (1994)\nocite{tsitsiklis1994} considers an asynchronous SA algorithm for finding a solution to $\bm{D}(\bm{x})=\bm{x}$, where $\bm{x}\in \mathbb{R}^p$ is a vector and $\bm{D}(\cdot)$ is a vector valued function, using possibly outdated information. Specifically, using Tsitsiklis' notation, the $i$th entry of $\bm{x}$, denoted by $x_i$, is updated according to the following recursion:
\begin{align}
x_i(t+1)&=x_i(t)-\upalpha_i(t)[D_i(\bm{x}^{i}(t))-x_i(t)+w_i(t)] \text{\ \ \ for $t\in T^i$},\notag\\
x_i(t+1)&=x_i(t)\text{\ \ \ for $t\notin T^i$},
\label{eq:singoayatailinchin}
\end{align}
where $T^{i}$ is a random set of (nonnegative integer) times at which $x_i$ is updated, $\upalpha_i(t)\in [0,1]$, $w_i(t)$ is a mean-zero noise term, $D_i$ denotes the $i$th entry of $\bm{D}$, and $\bm{x}^{i}(t)$ is a vector of (possibly) outdated components of $\bm{x}$, that is $\bm{x}^i=[x_1(\uptau_1^i(t)),\dots,x_p(\uptau_p^i(t))]^\top$, where $\uptau_j^i(t)\leq t$ is a nonnegative integer. If no information is outdated then $\bm{x}^i(t)=\bm{x}(t)$. It is in the case of delayed information that the resemblance to cyclic optimization becomes apparent. To see this, consider the special case of (\ref{eq:singoayatailinchin}) where $p$ is even, 
%
$T^{i}$ is the set of nonnegative odd numbers for $i\leq p/2$, $T^{i}$ is the set of even numbers for $i>p/2$, $\bm{x}^i(t)=\bm{x}(t)$ for $i\leq p/2$, and $\bm{x}^i(t)=[x_1(t+1), \dots, x_{p/2}(t+1), x_{p/2+1}(t),\dots, x_p(t)]^\top$ for $i>p/2$. The resulting algorithm is a special case of cyclic SA in which two subvectors of $\bm{x}(t)$ are updated in a strictly alternating manner.


One convenient property of (\ref{eq:singoayatailinchin}) is that it may be implemented in an asynchronous manner, that is the entries of $\bm{x}(t)$ that are updated at time $t$ can each be updating using outdated parameter vectors collected at possibly different times. The GCSA algorithm, in contrast, is synchronous in nature since the entries of the parameter vector that are updated at any given time must all be updated using the latest value of the parameter vector. Despite the advantage that an asynchronous algorithm presents over a synchronous algorithm, there are a few reasons why the theory regarding the convergence of (\ref{eq:singoayatailinchin}) does not apply to GCSA as is discussed next.

One of the conditions that Tsitsiklis (1994)\nocite{tsitsiklis1994} imposes for the convergence of (\ref{eq:singoayatailinchin}) requires the second moment of $w_i(t)$ to be bounded above by a function that depends on the magnitude of $\bm{x}(t)$ (see Assumption 2.e in Tsitsiklis 1992)\nocite{tsitsiklis1994}. When $\bm{x}(t)$ converges to some finite vector w.p.1 (e.g., to the solution of $\bm{F}(\bm{x})=\bm{x}$), Tsitsiklis' (1994)\nocite{tsitsiklis1994} assumption requires $w_i(t)$ to have bounded variance w.p.1. However, because 
%
(\ref{eq:singoayatailinchin}) can be thought of as a special case of (\ref{eq:imastandardupdaedirection}):
 \begin{align}
 \label{eq:latesincity}
%
&{\text{Update direction in first line of (\ref{eq:singoayatailinchin})}}= D_i(\bm{x}^{i}(t))-x_i(t)+w_i(t)\notag\\
&= {\underbrace{D_i(\bm{x}(t))-x_i(t)}_{\text{$i$th entry of $\bm{f}$ term in (\ref{eq:imastandardupdaedirection})}}}+{\underbrace{D_i(\bm{x}^{i}(t))-D_i(\bm{x}(t))+w_i(t)}_{{\text{$i$th entry of $\bm\upbeta+\bm\upxi$ term in (\ref{eq:imastandardupdaedirection})}}}},
%
 \end{align}
requiring $w_i(t)$ to have bounded second moment is equivalent to requiring the diagonal entries of the second moment matrix of ${\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)$ in (\ref{eq:imastandardupdaedirection}) to have bounded magnitude, an  assumption that is incompatible with many SA algorithms (such as the simultaneous perturbation SA algorithm) for which the variance of the noise can increase with time.
%
 In this dissertation we allow the variance of the noise to increase as the iteration number increases in order to accommodate a more general class of SA update directions. 
% 
 Another observation we make is that the vector ${\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)$ from (\ref{eq:imastandardupdaedirection}) has a very specific form in (\ref{eq:latesincity}).  In the GCSA algorithm, ${\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)$ term is allowed to have a form that is more appropriate for general SA procedures. 
%
 In conclusion, the assumptions imposed by Tsitsiklis (1994)\nocite{tsitsiklis1994} imply that the class of algorithms studied in Tsitsiklis (1994)\nocite{tsitsiklis1994} intersects the class of algorithms that fit into the GCSA framework although neither class of algorithms contains the other. Moreover, Tsitsiklis (1994)\nocite{tsitsiklis1994} does not discuss rate of convergence or provide results on asymptotic normality, both contributions of this dissertation.
 

Another algorithm closely related to GCSA appears in Borkar (1998)\nocite{borkar1998}. Here, the author investigates the asymptotic behavior of a distributed, asynchronous SA scheme in terms of a limiting
%
 differential equation. 
%
One important assumption made by Borkar (1998)\nocite{borkar1998} is that the update direction for the $i$th entry of the parameter vector is an unbiased estimate of the $i$th entry of $\bm{f}(\bm\uptheta)$, the function whose root is to be found (see equation 2.9 in Borkar 1998)\nocite{borkar1998}. This assumption is usually only valid for certain SA algorithms (e.g., the stochastic gradient algorithm) or deterministic optimization problems. The theory in this dissertation does not require the availability of unbiased estimates of the entries of $\bm{f}(\bm\uptheta)$. Another assumption made by Borkar (1998)\nocite{borkar1998} requires $\bm{f}(\bm\uptheta)$ to be Lipschitz continuous. In our setting (which focuses on stochastic optimization via root-finding so that $\bm{f}(\bm\uptheta)=\bm{g}(\bm\uptheta)$) this would be equivalent to requiring the gradient of $L(\bm\uptheta)$ to be Lipschitz continuous. We do not make such an assumption in the theory for convergence w.p.1 of the GCSA iterates. Additionally, Borkar (1998)\nocite{borkar1998} does not discuss rate of convergence or provide results on asymptotic normality, both contributions of this dissertation.

In this dissertation, the theory behind the GCSA algorithms allows the noisy update directions to be biased estimates of $\bm{f}(\bm\uptheta)$ and allows the noise term in (\ref{eq:imastandardupdaedirection}) (i.e., ${\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)$) to have a second moment matrix whose entries can increase in magnitude as a function of the iteration number. Algorithms that are related to GCSA but require the availability of unbiased estimates of $\bm{f}(\bm\uptheta)$ can be found in the papers by Borkar and Meyn (2000)\nocite{borkarmeyn2000}, Aboundai et al. (2002)\nocite{aboundaietal2002}, Bhatnagar (2011)\nocite{bhatnagar2011}, Bianchi and Jakubowicz (2013)\nocite{bianchiandjiakubowicz2013}, and Singh et al. (2014)\nocite{singhetal2014} (technically, the estimate for $\bm{f}(\bm\uptheta)$ in this last reference is and unbiased estimate of a vector that has the same roots as $\bm{f}(\bm\uptheta)$). Algorithms that are related to GCSA but require the term ${\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)$ in (\ref{eq:imastandardupdaedirection}) to have bounded variance can be found in the papers by Tsitsiklis (1984)\nocite{tsitsiklis1984}, Tsitsiklis et al. (1986)\nocite{tsitsiklisetal1986}, Solodov and Zavriev (1998)\nocite{solodovzavriev1998}, Ram et al. (2009b)\nocite{rametal2009b}, Nedi\'c and Bertsekas (2010)\nocite{nedicandbertsekas2010}, Ram et al. (2010)\nocite{rametal2010}, Xu and Yin (2015)\nocite{xyandyin2015}, and in Exercise 1.7.1 on p. 34 in Benveniste et al. (1990)\nocite{benveniste1990}. The distributed algorithms in Chapter 12 of Kushner and Yin (1997)\nocite{kushnyin1997} are also closely related to GCSA. However, the results in said chapter require the sequence of noisy update directions (i.e., the sequence ${\bm{Y}}_k(\hat{\bm{\uptheta}}_k)$) to be uniformly integrable (see Kushner and Yin 1997, Chapter 12, Assumptions A3.1 and A3.1$'$), an assumption that is too strong for some SA algorithms such as finite difference SA where the noise in the update direction generally makes the ${\bm{Y}}_k(\hat{\bm{\uptheta}}_k)$ vectors not uniformly integrable. This dissertation does not make the assumption of uniform integrability of the noisy update directions. 
%
 Lastly, a few results related to GCSA concerned with optimizing convex functions can be found in the papers by Ram et al. (2009a)\nocite{rametal2009a}, Necoara (2013)\nocite{necoara2013}, and Necoara and Petrascu (2014)\nocite{recoaraandpetrascu2014} (the theory in this dissertation does not assume convexity).

\section{This Work's Contribution}
This work's main contribution can be summarized by the following points:
\begin{enumerate}
\item	We derive conditions for the convergence with probability one of the GCSA algorithm to a root of the gradient of $L(\bm\uptheta)$.  The main convergence result is stated in Theorem \ref{thm:hoeshoo} of Section \ref{sec:convo}. A few corollaries based on special cases of GCSA are derived in the same section. Numerical results supporting the theory on convergence are provided in Section \ref{sec:convergencenumericos}.
\item We provide a generalization to Theorem 2.2 in Fabian (1968) (see Theorem \ref{thm:generalizefabian}) that allows us to show asymptotic normality for a special case of GCSA. Appendix \ref{sec:fabiansecgeneralize} explains how the generalization to Fabian's theorem also extends the theorem's result to include a broader range of SA algorithms of practical interest including certain second order SA and root-finding SA algorithms. 
\item We show the asymptotic normality of the normalized iterates of a special case of GCSA in which the subvector to update is selected according to a deterministic pattern (see Theorem \ref{thm:fnogg}). The result on asymptotic normality helps us define the asymptotic rate of convergence for the iterates of this special case of GCSA. Numerical results supporting the theory on asymptotic normality are provided in Section \ref{sec:normalitycenumericos}.
\item We discuss the importance of defining the cost of implementation when comparing the performances of two optimization algorithms. When cost is a measure of the number of basic arithmetic computations required, we discuss the type of arithmetic operations that can result in a significant difference between the per-iteration cost of implementing an algorithm
%
 and the per-iteration cost of implementing its cyclic counterpart. 
\item We provide an analytical estimate for the asymptotic efficiency of a special case of GCSA relative to the efficiency of its non-cyclic counterpart after taking into consideration the per-iteration costs of implementation. Here, efficiency is defined in terms of the mean-squared estimation errors. We show how the expression for asymptotic relative efficiency implies that either algorithm (cyclic or non-cyclic) can be more efficient. Numerical experiments computing the relative efficiency between cyclic and non-cyclic algorithms under different definitions of cost are provided in Section \ref{sec:Numericssimples}. 
\item In Chapter \ref{chap:multiagent} we apply the cyclic SA approach to a multi-agent optimization problem for tracking and surveillance. 
%
\item This dissertation also contains two appendices. Appendix \ref{sec:fabiansecgeneralize} contains a more detailed proof of Theorem \ref{thm:generalizefabian}, the theorem in Chapter \ref{sec:ROC} that generalizes Theorem 2.2 in Fabian (1968), and discusses a few applications of the generalized theorem. Appendix \ref{sec:ROC} considers the problem of determining the presence and location of a static object within an area of interest by combining information from multiple sensors using a maximum-likelihood-based approach.

\end{enumerate}
%
Two noteworthy assumptions made throughout this dissertation are that the loss function is differentiable and that the optimization problem is unconstrained. Future work could focus on investigating the constrained- and non-differentiable settings.


\section{Overview of Contents}
The main part of this work (Chapters \ref{chap:prems8}--\ref{chap:multiagent}) is organized as follows. First, Chapter \ref{chap:prems8} reviews the general stochastic optimization setting as well as the idea behind SA algorithms for stochastic optimization. 
%
Chapter \ref{chap:descriptionofGCSA} introduces the cyclic seesaw SA algorithm and the generalized cyclic SA algorithm (GCSA) that is the focus of this work.
% 
 Chapter \ref{sec:cyclicseesaw} focuses on deriving conditions for the convergence with probability one of the GCSA algorithm's iterates to a root of the gradient of the function to minimize. 
% 
  Chapter \ref{sec:ROC} generalizes a well-known result in the SA literature (Fabian 1968, Theorem 2.2) and uses the resulting generalization to prove asymptotic normality of the scaled iterates for a special case of GCSA. 
% 
  Chapter \ref{chap:imefficient} is concerned with computing the asymptotic efficiency (defined as the asymptotic mean-squared-error) of a special case of GCSA relative to that of its non-cyclic counterpart. The chapter begins by discussing the importance of defining the cost of implementation before attempting to compare any two algorithms. The chapter goes on to provide a comparison of the cost of implementing an SA algorithm in a cyclic manner versus the cost if implemented in a non-cyclic manner; a few definitions of cost are considered. Using the asymptotic normality result from Chapter \ref{sec:ROC}, Chapter \ref{chap:imefficient} computes the asymptotic relative efficiency between a special case of GCSA and its non-cyclic counterpart. Chapter \ref{chap:numericschap} contains numerical results that illustrate the theory of Chapters \ref{sec:cyclicseesaw}--\ref{chap:imefficient}. Chapter \ref{chap:multiagent} applies the cyclic approach to a multi-agent optimization problem where the loss function is time-varying and corrupted by noise. While the theory from Chapters \ref{sec:cyclicseesaw} and \ref{sec:ROC} (which is concerned with the optimization of a loss function that is not time-varying) is not fully applicable to this multi-agent problem (the main condition in Chapters \ref{sec:cyclicseesaw}--\ref{sec:ROC} not satisfied is the decaying gain sequence of SA; as a tracking problem the gains are not allowed to decay to zero), the purpose of the numerical example in this chapter is threefold. First, it addresses an important area surveillance and tracking problem. Second, it studies the performance of a cyclic implementation when the conditions from Chapters \ref{sec:cyclicseesaw} and \ref{sec:ROC} do not fully hold. Third, it serves to motivate directions for future work.
  
  
  Following Chapter \ref{chap:multiagent} this work is organized as follows. Appendix \ref{sec:fabiansecgeneralize} contains a more detailed proof of Theorem \ref{thm:generalizefabian}, a theorem in Chapter \ref{sec:ROC} that generalizes Theorem 2.2 in Fabian (1968). Appendix \ref{sec:fabiansecgeneralize} also discusses how the generalization makes Theorem 2.2 in Fabian (1968) applicable to a broader range of SA algorithms that extend beyond cyclic SA. In contrast to the content of Chapters \ref{chap:intro}--\ref{chap:multiagent} and Appendix \ref{sec:fabiansecgeneralize}, Appendix \ref{appen:systemid} is concerned with a topic that is unrelated to SA: it considers the problem of determining the presence and location of a static object within an area of interest by combining information from multiple sensors. A simple maximum-likelihood-based approach is investigated. Lastly, a list of frequently used notation is included at the end of this dissertation.

  





==> thesis arXiv 2/chapter1p.tex <==
%!TEX root = root.tex

\chapter{Preliminaries}
\label{chap:prems8}
%\chaptermark{Preliminaries}

This chapter lays the groundwork for our study of stochastic optimization based on nonlinear root-finding stochastic approximation (SA) algorithms. Section \ref{sec:stafff} formally introduces the general stochastic optimization setting and briefly reviews the relationship between root-finding and optimization. Section \ref{sec:dummieyouask} describes the basic form of SA algorithms for nonlinear root-finding. Lastly, Sections \ref{sec:sgfosa} and \ref{sec:coffee100} give three examples of well-known SA algorithms: stochastic gradient, finite difference SA, and simultaneous perturbation SA.
% stochastic gradient, finite difference stochastic approximation, and simultaneous perturbation stochastic approximation.
\section{Stochastic Optimization}
\label{sec:stafff}

The idea behind {\it{unconstrained optimization}} problems is the minimization of a real-valued loss function $L(\bm\uptheta)$ with respect to a parameter vector $\bm\uptheta$. When $L(\bm\uptheta)$ is a smooth function, its gradient is denoted by $\bm{g}(\bm\uptheta)\equiv \partial L(\bm\uptheta)/\partial \bm\uptheta$ and, in this case, the optimization problem can be reformulated as a root-finding problem where one attempts to solve $\bm{g}(\bm\uptheta)=\bm{0}$ (this equation is referred to as the {\it{gradient equation}}  and any solution is referred to as a {\it{root of the gradient}}). Here, the usual caveat applies: the set of all roots of the gradient may contain vectors other than global minimizers of $L(\bm\uptheta)$. Still, regardless of this caveat, the close relationship between minimization and root-finding implies many optimization algorithms rely on being able to evaluate either $L(\bm\uptheta)$ or $\bm{g}(\bm\uptheta)$. Take the steepest descent algorithm (e.g., Nocedal and Wright 2006, Chapter 2)\nocite{nocedalnwright2006}, for example. This algorithm is an iterative line-search algorithm in which an estimate, $\hat{\bm{\uptheta}}_k$, for a solution to the gradient equation is obtained during the $k$th iteration
%. Specifically, the steepest decent algorithm updates $\hat{\bm{\uptheta}}_k$ 
according to the recursion:
% the following recursion:
\begin{align}
\label{eq:exescriss}
\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k{\bm{g}}(\hat{\bm{\uptheta}}_k),
\end{align}
where $a_k$ is a strictly-positive scalar often referred to as the {\it{gain sequence}} (one valid choice for the gain sequence in the steepest descent algorithm is setting $a_k$ equal to a constant that does not depend on $k$). Under certain assumptions, $\hat{\bm{\uptheta}}_k$ converges to $\bm\uptheta^\ast$, a root of the gradient. It is apparent from (\ref{eq:exescriss}) that being able to evaluate $\bm{g}(\bm\uptheta)$ at $\{\hat{\bm{\uptheta}}_k\}_{k\geq0}$ is essential to the implementation of the steepest-descent algorithm. Similarly, many optimization algorithms rely on being able to evaluate $L(\bm\uptheta)$. Simple examples of this type of algorithm are the random search algorithms in Section 2.2 of Spall (2003). 
%Another class of algorithms that require being able to evaluate $L(\bm\uptheta)$ are trust-region algorithms (e.g., Nocedal and Wright 2006, Chapter 4)\nocite{nocedalnwright2006}.


In practice, it is often the case that evaluating the loss function or its gradient is difficult. As a simple example, consider a setting where there exists a complex stochastic model whose output depends on a set of parameters denoted by $\bm\uptheta$. Furthermore, suppose one wishes to find the value of $\bm\uptheta$ that minimizes the expected output of the model. Here, finding a closed form expression for $L(\bm\uptheta)$ would require computing the expected output for each $\bm\uptheta$, which might be {{infeasible}} due to the complexity of the model. When dealing with physical processes in the optimization process, rather than mathematical models, computing the expected value of the measurement/output for any given $\bm\uptheta$ could easily be {{impossible}} (rather than simply infeasible) since physical processes are often governed by rules unknown to the observer. While traditional optimization techniques cannot be implemented when neither $L(\bm\uptheta)$ nor $\bm{g}(\bm\uptheta)$ are known, stochastic optimization algorithms can use noisy measurements of either the loss function or its gradient in the minimization process. Hereafter, the term ``{\it{stochastic optimization}}'' will be used to refer to optimization problems where there is random noise in the measurements of $L(\bm\uptheta)$ or $\bm{g}(\bm\uptheta)$, or where there is a random choice made in the search direction as the algorithm iterates towards a solution. The term ``{\it{deterministic optimization}}'' will be used to refer to classical optimization problems, like steepest descent or Newton's method, where the minimization process is entirely deterministic.

%which attempt to minimize the loss function by using expressions for $L(\bm\uptheta)$ or $\bm{g}(\bm\uptheta)$ in a deterministic manner (e.g., steepest descent or Newton's method).
%
%to all other types of optimization problems.
%Stochastic optimization is more formally discussed next. 
  
  As mentioned in the previous paragraph, one type of stochastic optimization problem pertains to the case where one wishes to minimize a function $L(\bm\uptheta)$ when only noisy measurements of this function are available. In other words, it is assumed that the loss function is unknown but that it is possible to obtain measurements of a random variable $Q(\bm\uptheta,\bm{V})$ such that:
\begin{align}
\label{eq:chanchan}
Q(\bm\uptheta,{\bm{V}})=L(\bm\uptheta)+\upvarepsilon(\bm\uptheta,{\bm{V}}),
\end{align}
where $\bm{V}$ denotes a multivariate random variable and $\upvarepsilon(\bm\uptheta,{\bm{V}})$ is a noise term. The term $\upvarepsilon(\bm\uptheta,{\bm{V}})$ can then be interpreted as the error in measuring the function to minimize. In the special case where the expected value of $\upvarepsilon(\bm\uptheta,\bm{V})$ at $\bm\uptheta$ is equal to zero, a consequence of the law of large numbers is that it is possible to approximate $L(\bm\uptheta)$ at any given $\bm\uptheta$ by averaging several independent and identically distributed (i.i.d.) measurements of $Q(\bm\uptheta,\bm{V)}$. In theory, one could average several i.i.d. noisy loss function measurements to obtain $\bar{L}(\bm\uptheta_1),\dots, \bar{L}(\bm\uptheta_N)$, a set of estimates for $L(\bm\uptheta)$ at the points $\bm\uptheta=\bm\uptheta_1,\dots,\bm\uptheta_N$ (selected from the domain of $L(\bm\uptheta)$ via some deterministic or random scheme).
%to obtain an approximation to $L(\bm\uptheta)$ for $\bm\uptheta\in \{\bm\uptheta_1,\dots,\bm\uptheta_N\}$. 
Then, an approximation to $L(\bm\uptheta)$ for all $\bm\uptheta$, denoted by $\bar{L}(\bm\uptheta)$, could be obtained by interpolating the values of $\bar{L}(\bm\uptheta_i)$ (obtaining this interpolation may be a nontrivial task). Afterwards, one could attempt to minimize $\bar{L}(\bm\uptheta)$ using deterministic optimization algorithms with the hope that the minimizer of $\bar{L}(\bm\uptheta)$ is close to the minimizer or $L(\bm\uptheta)$ (the response surface methodology strategy, introduced by Box and Wilson in 1951\nocite{boxwilson1951}, is a more sophisticated variant of this approach). Such an approach, however, is not always practical since obtaining a good approximation to the loss function (an approximation to the loss function would be considered ``good'' if its minimizer is close to the minimizer of $L(\bm\uptheta)$) could require a prohibitive number of noisy function measurements. The following section describes the stochastic approximation setting, a general framework for stochastic nonlinear root-finding that is more appropriate for minimizing (\ref{eq:chanchan}) than the deterministic optimization approach discussed above. 

\section[Stochastic Approximation (SA)]{Stochastic Approximation}
\label{sec:dummieyouask}

There exist many stochastic optimization algorithms. Random search, genetic algorithms, simulated annealing, stochastic gradient, and simultaneous perturbation SA, are a few examples.
% Direct methods for deterministic optimization like random search and the Nelder--Mead algorithm have also been adapted (though small but crucial modifications) for use with noisy loss function measurements. 
This work will focus on {\it{stochastic approximation}} (SA) algorithms for stochastic optimization via nonlinear root-finding. SA algorithms are closely related to line-search methods and  can be used for stochastic optimization. This section formally defines SA and presents three important examples of SA algorithms: the {\it{stochastic gradient}} (SG) form of SA, {\it{finite difference}} SA (FDSA), and {\it{simultaneous perturbation}} SA (SPSA). Throughout the remainder of this work it is assumed that $\bm\uptheta=[\uptau_1,\dots,\uptau_p]^\top\in \mathbb{R}^p$ and $\bm\uptheta^\ast$ will denote a solution to $\bm{g}(\bm\uptheta)=\bm{0}$.

The basic SA algorithm for nonlinear root-finding is known as the Robbins--Monro algorithm (Robbins and Monro 1951)\nocite{robbinsmonro1951}.  Given a vector-valued function $\bm{f}(\bm\uptheta)$, the Robbins--Monro algorithm attempts to find a solution to $\bm{f}(\bm\uptheta)=\bm{0}$ in an iterative manner using the following recursion:
\begin{align}
\label{eq:formof}
\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k{\bm{Y}}_k(\hat{\bm{\uptheta}}_k),
\end{align}
where ${\bm{Y}}_k(\hat{\bm{\uptheta}}_k)$ is a vector-valued random variable representing a noisy observation of $\bm{f}(\hat{\bm{\uptheta}}_k)$, and $a_k>0$ is the gain sequence (step size). Unlike most deterministic optimization algorithms, the gain sequence in (\ref{eq:formof}) typically satisfies $a_k\rightarrow 0$. This dissertation is concerned with the special case where $\bm{f}(\bm\uptheta)=\bm{g}(\bm\uptheta)$. In this context, $\bm{Y}_k(\hat{\bm{\uptheta}}_k)$ denotes a noisy estimate of the gradient and it is common to replace the notation $\bm{Y}_k(\hat{\bm{\uptheta}}_k)$ in (\ref{eq:formof}) with $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$. Therefore, we write:
\begin{align}
\label{eq:youknownothing}
\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k),
\end{align}
where $\hat{\bm{g}}(\hat{\bm{\uptheta}}_k)$ is a noisy gradient measurement. 

Because $\hat{\bm{g}}(\hat{\bm{\uptheta}}_k)$ can be thought of as an estimate of $\bm{g}(\hat{\bm{\uptheta}}_k)$, the theory of SA for stochastic optimization often relies on rewriting the vector $\hat{\bm{g}}(\hat{\bm{\uptheta}}_k)$ as:
\begin{align}
\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)&= {\bm{g}}(\hat{\bm{\uptheta}}_k)+{\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k),
\label{eq:tennisey}
\end{align}
a special case of (\ref{eq:imastandardupdaedirection}), where $\bm\upbeta_k(\hat{\bm{\uptheta}}_k)= E\big[\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)-\bm{g}(\hat{\bm{\uptheta}}_k)\big|\mathcal{F}_k\big]$, ${\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)= \hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)-E\big[\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)\big|\mathcal{F}_k\big]$, $\mathcal{F}_k$ is some representation of the history of the process (the precise definition of $\mathcal{F}_k$ may vary from algorithm to algorithm), and $E[\mathcal{X}]$ represents the expected value of the random variable $\mathcal{X}$. One common choice of $\mathcal{F}_k$ is $\mathcal{F}_k=\hat{\bm{\uptheta}}_0,\dots,\hat{\bm{\uptheta}}_k$. In this case, $\bm\upbeta_k(\hat{\bm{\uptheta}}_k)$ represents the {\it{bias}} of $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$ (e.g., Bickel and Doksum 2007)\nocite{bickelndoksum2007} as an estimator of $\bm{g}(\hat{\bm{\uptheta}}_k)$ and the vector ${\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)$ is often referred to as the {\it{noise}} term. In the special case where $E\big[\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)\big|\hat{\bm{\uptheta}}_k\big]= \bm{g}(\hat{\bm{\uptheta}}_k)$, $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$ is said to be an unbiased estimate of the gradient at $\hat{\bm{\uptheta}}_k$. It is important to mention that the decomposition in (\ref{eq:tennisey}) is used only for theoretical purposes and, in practice, the bias and noise terms are never computed. Sections \ref{sec:sgfosa} and \ref{sec:coffee100} discuss special cases of (\ref{eq:youknownothing}) that differ in the way $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$ is computed.

\section[Stochastic Gradient (SG) Form of SA]{Stochastic Gradient Form of SA}
\label{sec:sgfosa}

The {\it{stochastic gradient}} (SG) algorithm for stochastic approximation (e.g., Spall 2003, Chapter 5) is a special case of the Robbins-Monro algorithm that requires the availability of a vector $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ such that $E\big[\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)\big|\hat{\bm{\uptheta}}_k\big]=\bm{g}(\hat{\bm{\uptheta}}_k)$ (i.e., the noisy gradient measurement must be an unbiased measurement of the gradient at $\hat{\bm{\uptheta}}_k$). The recursion defining $\hat{\bm{\uptheta}}_k$ in the SG algorithm is as follows:
\begin{align*}
%\label{eq:showdelairesd}
\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k),
\end{align*}
a special case of (\ref{eq:youknownothing}). Because $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ is an unbiased estimate of $\bm{g}(\hat{\bm{\uptheta}}_k)$ we write $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)=\bm{g}(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$, where $E[{\bm{\upxi}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)|\mathcal{F}_k]=\bm{0}$. In the area of simulation-based optimization, two popular algorithms that are special cases of the SG algorithm are the pure infinitesimal perturbation analysis (IPA) algorithm and the pure likelihood ratio function algorithm (Spall 2003, p. 418)\nocite{ISSO}. For both these algorithms, the random vector $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ can sometimes be obtained by assuming that is is possible to
%The vector $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ 
%may be obtained, for example, via deliberate injection of mean-zero noise to the vector $\bm{g}(\bm\uptheta)$ (this is sometimes done with the intention of avoiding becoming ``stuck'' at a local solution). 
%can sometimes be obtained by 
differentiate $Q(\bm\uptheta,\bm{V})$ with respect to $\bm\uptheta$ (e.g., Spall 2003, p. 134\nocite{ISSO}).
% .
% prompting the question: could the gradient of  $Q(\bm\uptheta,\bm{V})$ be used to obtain $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$, an unbiased estimate of $\bm{g}(\hat{\bm{\uptheta}}_k)$? 
 This approach is formally discussed next.


First note that (\ref{eq:chanchan}) implies $E[Q(\bm\uptheta,\bm{V})|\bm\uptheta]=L(\bm\uptheta)+E[\upvarepsilon(\bm\uptheta,{\bm{V}})|\bm\uptheta]$ so that:
\begin{align}
\label{eq:goodworkteak}
\frac{\partial}{\partial \bm\uptheta}E[Q(\bm\uptheta,\bm{V})|\bm\uptheta]={\bm{g}}(\bm\uptheta)+\frac{\partial E[\upvarepsilon(\bm\uptheta,{\bm{V}})|\bm\uptheta]}{\partial \bm\uptheta}.
\end{align}
 If $E[\bm\upvarepsilon(\bm\uptheta,\bm{V})|\bm\uptheta]$ does not depend on $\bm\uptheta$ (e.g., if $\bm\upvarepsilon$ is i.i.d. noise) then (\ref{eq:goodworkteak}) implies:
\begin{align}
\label{eq:chungie}
{\bm{g}}(\bm\uptheta)=\frac{\partial}{\partial \bm\uptheta}E[Q(\bm\uptheta,\bm{V})|\bm\uptheta]=\frac{\partial}{\partial \bm\uptheta}\int_{\Omega_{\bm{V}}}Q(\bm\uptheta,\bm{v})\ dP,
\end{align}
where $P$ denotes a probability measure and $\Omega_{\bm{V}}$ is the domain of $\bm{V}$. Consider the case where $\bm{V}$ is a continuous random variable with probability density function (pdf) $p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)$ that may depend on $\bm\uptheta$. 
%Let $p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)$ represent the density of ${\bm{V}}$ given $\bm\uptheta$ evaluated at $\bm{v}$. 
Then, (\ref{eq:chungie}) becomes:
\begin{align*}
%\label{eq:theintegralin}
{\bm{g}}(\bm\uptheta)=\frac{\partial}{\partial \bm\uptheta}\int_{\Omega_{\bm{V}}}Q(\bm\uptheta,\bm{v})p_{\bm{V}}(\bm{v}|\bm\uptheta)\ d\bm{v}.
\end{align*}
If the interchange of differentiation and integration is justified we obtain:
\begin{align}
{\bm{g}}(\bm\uptheta)=
\int_{\Omega_{\bm{V}}}\Bigg[\frac{\partial Q(\bm\uptheta,{\bm{v}})}{\partial \bm\uptheta}+Q(\bm\uptheta,{\bm{v}})\frac{\partial \log(p_{{\bm{V}}}({\bm{v}}|\bm\uptheta))}{\partial \bm\uptheta}\Bigg]p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)\ d{\bm{v}}.\label{eq:bias}
\end{align}
\noindent From  (\ref{eq:bias}) we see that
\begin{align}
\label{eq:dieforyou}
\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)=\frac{\partial Q(\bm\uptheta,{\bm{V}})}{\partial \bm\uptheta}\Big|_{\bm\uptheta=\hat{\bm{\uptheta}}_k}+Q(\hat{\bm{\uptheta}}_k,{\bm{V}})\frac{\partial \log[p_{{\bm{V}}}({\bm{V}}|\bm\uptheta)]}{\partial \bm\uptheta}\Big|_{\bm\uptheta=\hat{\bm{\uptheta}}_k},
\end{align}
 is an unbiased measurement of $\bm{g}(\hat{\bm{\uptheta}}_k)$ by construction. 
%Note that in (\ref{eq:dieforyou}) the lower-case letter $\bm{v}$ appearing in (\ref{eq:bias}) has been replaced with upper-case letter $\bm{V}$, the upper-case letter is used a placeholder for future realizations of the random variable. 
The following condition is sufficient for the validity of the interchange of differentiation and integration used in (\ref{eq:bias}).

 \begin{theorem}[{\bf{Interchange of Differentiation and Integration}}](Spall 2003, Theorem 15.1)\nocite{ISSO}. Assume $Q(\bm\uptheta,{\bm{v}})p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)$ and $\partial [Q(\bm\uptheta,{\bm{v}})p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)]/\partial \bm\uptheta$ are continuous on $\mathbb{R}^{p}\times \Omega_{\bm{V}}$. Suppose there exist  two nonnegative integrable functions $q_{0}({\bm{v}})$ and $q_{1}({\bm{v}})$ such that for all pairs $(\bm\uptheta,{\bm{v}})\in \mathbb{R}^p\times \Omega_{\bm{V}}$:
\vspace{-.05in}
\begin{align*}
\left|Q(\bm\uptheta,{\bm{v}})p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)\right|\leq q_{0}({\bm{v}});\ \ \  \left\|\frac{\partial [Q(\bm\uptheta,{\bm{v}})p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)]}{\partial \bm\uptheta}\right\|\leq q_{1}({\bm{v}}).
\end{align*}
\noindent Then:
\begin{align*}
{\bm{g}}(\bm\uptheta)=\frac{\partial}{\partial \bm\uptheta}\int_{\Omega_{\bm{V}}}Q(\bm\uptheta,{\bm{V}})p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)\ d{\bm{v}}=\int_{\Omega_{\bm{V}}}\frac{\partial}{\partial \bm\uptheta}\left[Q(\bm\uptheta,{\bm{V}})p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)\right]\ d{\bm{v}}.
\end{align*}
\end{theorem}
 
 When $\bm{V}$ is a discrete random variable taking the values $1,\dots, N$, a relationship analogous to (\ref{eq:bias}) can be obtained. To see this, let $p_{\bm{V}}(\bm{v}|\bm\uptheta)$ denote the probability mass function (pmf) of $\bm{V}$. In this case, 
% the integral in (\ref{eq:theintegralin}) is replaced with a sum:
 \begin{align}
 \label{eq:frordddas}
{\bm{g}}(\bm\uptheta)=\frac{\partial}{\partial \bm\uptheta}\sum_{\bm{v}=1}^{N}Q(\bm\uptheta,\bm{v})p_{\bm{V}}(\bm{v}|\bm\uptheta).
\end{align}
If $N<\infty$, the interchange of change of summation and differentiation in (\ref{eq:frordddas}) is justified (provided the required derivatives exist). This may not be the case, however, when $N=\infty$ (the sum of the gradients of the individual summands may fail to converge or may converge to something other than $\bm{g}(\bm\uptheta)$). When $N=\infty$, sufficient conditions for the interchange of  differentiation and summation can easily be obtained using Theorem 7.17 in Rudin (1976)\nocite{Rudin1976} (although this theorem pertains only to the case where $\bm\uptheta$ is real, the result of the theorem is easily generalized to the multi-dimensional case by applying the theorem to each entry of the gradient vectors). When the exchange of differentiation and summation in (\ref{eq:frordddas}) is valid,
%
 \begin{align*}
 {\bm{g}}(\bm\uptheta)=  \sum_{\bm{v}=1}^{N}\Bigg[\frac{\partial Q(\bm\uptheta,{\bm{v}})}{\partial \bm\uptheta}+Q(\bm\uptheta,{\bm{v}})\frac{\partial \log[p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)]}{\partial \bm\uptheta}\Bigg]p_{{\bm{V}}}({\bm{v}}|\bm\uptheta).
 \end{align*}
From this,  we deduce that (\ref{eq:dieforyou}) once again represents an unbiased measurement of the gradient.
 
While (\ref{eq:dieforyou}) gives a theoretically valid expression for $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$, it requires information that may not be available. For example, if $p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)$ is unknown we would not be able to compute ${\partial \log{[p_{{\bm{V}}}({\bm{V}}|\bm\uptheta)]}}/{\partial \bm\uptheta}$. However, if $p_{{\bm{V}}}({\bm{v}}|\bm\uptheta)$ is independent of $\bm\uptheta$ (a common assumption) then (\ref{eq:dieforyou}) simplifies to:
\begin{align}
\label{eq:imanIPA}
\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)= \frac{\partial Q(\bm\uptheta,{\bm{V}})}{\partial \bm\uptheta }\Big|_{\bm\uptheta=\hat{\bm{\uptheta}}_k}.
\end{align}
%as the vector-valued random variable with expectation (conditional on $k$ and $\hat{\bm{\uptheta}}_k$) equal to $\bm{g}(\hat{\bm{\uptheta}}_k)$. 
Then, $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ could be obtained through direct measurement of $\partial Q(\bm\uptheta,{\bm{V}})/\partial \bm\uptheta$ evaluated at ${\bm\uptheta=\hat{\bm{\uptheta}}_k}$. In the area of simulation-based optimization, the Robbins--Monro algorithm with $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)=\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ where $\hat{\bm{g}}_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)$ is as in (\ref{eq:imanIPA}) is commonly referred to as the pure IPA algorithm. 

\section[Simultaneous Perturbation SA (SPSA)]{Simultaneous Perturbation SA}
\label{sec:coffee100}

SA is a powerful tool for stochastic optimization. Section \ref{sec:sgfosa} discussed the SG algorithm which used a noisy but unbiased measurement of $\bm{g}(\hat{\bm{\uptheta}}_k)$ to update $\hat{\bm{\uptheta}}_k$. Section \ref{sec:sgfosa} also gave conditions under which a direct measurement of $\partial Q(\bm\uptheta,\bm{V})/\partial \bm\uptheta$ could be used as the noisy unbiased measurement of the gradient. Direct measurement of $\partial Q(\bm\uptheta,\bm{V})/\partial \bm\uptheta$ is certainly a feasible approach in some applications (e.g., Widrow and Stearns 1985). However, measuring $\partial Q(\bm\uptheta,\bm{V})/\partial \bm\uptheta$ is not always possible and is particularly a problem in black-box settings where the form of $Q(\bm\uptheta,\bm{V})$ is unknown. With this motivation, several SA approximate $\bm{g}(\bm\uptheta)$ only using noisy measurements of $Q(\bm\uptheta,\bm{V})$ and, for this reason, these SA algorithms are often said to be {\it{gradient-free}}.


Let us briefly discuss the oldest gradient-free SA method: {\it{finite difference stochastic approximation}} (FDSA). See, for example, Dennis and Schnabel (1989)\nocite{dennisnschnabel1989}. FDSA requires measuring $Q(\bm\uptheta,\bm{V})$ at different values of $\bm\uptheta$. Specifically,
%\begin{align*}
$\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k \hat{\bm{g}}^{\text{FD}}_k(\hat{\bm{\uptheta}}_k)$,
%\end{align*}
where the random vector $\hat{\bm{g}}^{\text{FD}}_k(\hat{\bm{\uptheta}}_k)$ is defined as follows:
\begin{align}
\label{eq:marcella}
\hat{\bm{g}}^{\text{FD}}(\hat{\bm{\uptheta}}_k)\equiv \left[\begin{array}{c}\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k\bm{e}_1,\bm{V}^{1+})-Q(\hat{\bm\uptheta}_k-c_k\bm{e}_1,\bm{V}^{1-})}{2c_k}} \\\vdots \\\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k\bm{e}_p,\bm{V}^{p+})-Q(\hat{\bm\uptheta}_k-c_k\bm{e}_p,\bm{V}^{p-})}{2c_k}}\end{array}\right],
\end{align}
where $\bm{e}_i$ denotes the $i$th standard-basis vector in $\mathbb{R}^p$, $c_k>0$ satisfies $c_k\rightarrow 0$, and where $\bm{V}^{1+},\dots, \bm{V}^{p+}, \bm{V}^{1-},\dots, \bm{V}^{p-}$ denote $2p$ different realizations of $\bm{V}$. The update direction in (\ref{eq:marcella}) is referred to as the two-sided FDSA update direction and requires a total of $2p$ noisy loss function measurements at each iteration (recall that $p$ is the dimension of the parameter space). When $p$ is large and if obtaining noisy loss function measurements is costly, requiring $2p$ noisy loss function measurements per-iteration could be prohibitive (this is also an issue for a one-sided version of the FDSA algorithm requiring $p+1$ noisy loss measurements per-iteration).

The {\it{simultaneous perturbation stochastic approximation}} (SPSA) algorithm (e.g., Spall 1992\nocite{spall1992}; Bhatnagar et al. 2013\nocite{bhatnagaretal2013}) is similar to FDSA but requires only two noisy loss function measurements per iteration (independently of $p$). In SPSA, the gradient approximation in (\ref{eq:marcella}) is replaced with the random vector:
\begin{align}
\label{eq:pocres}
\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)\equiv \left[\begin{array}{c}\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k\bm\Delta_k,\bm{V}^+)-Q(\hat{\bm\uptheta}_k-c_k\bm\Delta_k,\bm{V}^-)}{2c_k\Delta_{k1}}} \\\vdots \\\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k\bm\Delta_k,\bm{V}^+)-Q(\hat{\bm\uptheta}_k-c_k\bm\Delta_k,\bm{V}^-)}{2c_k\Delta_{kp}}}\end{array}\right],
\end{align}
where $\bm\Delta_k=[\Delta_{k1},\dots,\Delta_{kp}]^\top$ is a random vector, $c_k>0$ is a sequence satisfying $c_k\rightarrow 0$, and $\bm{V}^+$ and $\bm{V}^-$ are two different realizations of $\bm{V}$. The SPSA recursion governing $\{\hat{\bm{\uptheta}}_k\}_{k\geq 0}$ is then
%\begin{align*}
$\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)$.
%\end{align*}
By defining $\mathcal{F}_k\equiv \{\hat{\bm{\uptheta}}_0,\dots,\hat{\bm{\uptheta}}_k,\bm\Delta_0,\dots,\bm\Delta_{k-1}\}$, $\bm\upbeta_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)\equiv E[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)-\bm{g}(\hat{\bm{\uptheta}}_k)|\mathcal{F}_k]$, and $\bm\upxi_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)\equiv \hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)-\bm{g}(\hat{\bm{\uptheta}}_k)-\bm\upbeta_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)$,  the connection between the SPSA algorithm and (\ref{eq:youknownothing})--(\ref{eq:tennisey}) becomes apparent. 
%
%Next we make an important observation regarding the bias term $\bm\upbeta_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)$.
%

Let us briefly discuss an important property of $\bm\upbeta_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)$ and $\bm\upxi_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)$, the bias and noise terms associated with the SPSA algorithm. In (\ref{eq:pocres}), the vector $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)$ was obtained by adding a perturbation to $\hat{\bm{\uptheta}}_k$ in two opposite directions and collecting a noisy loss measurement at these new locations. 
%In the noise-free case (i.e., when $\bm\upxi_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)=\bm{0}$), if $\|c_k\bm\Delta_k\|$ is relatively small it may be reasonable to assume that $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)$ is close (in Euclidian distance) to $\bm{g}(\hat{\bm{\uptheta}}_k)$. In the stochastic case, 
 Spall (1992)\nocite{spall1992} derives conditions under which the bias of the gradient estimate decreases w.p.1 as $c_k$ decreases. Spall (1992)\nocite{spall1992} also derives conditions under which 
% there exists a finite vector $\bm{b}$ such that 
 $\bm\upbeta_k(\hat{\bm{\uptheta}}_k^{\text{SP}})=O(c_k^2) $ w.p.1, where $O(\cdot)$ is the standard big-$O$ notation. This result implies that the bias must decrease at least as fast as $c_k^2$ w.p.1. In other words, as the magnitude of the perturbation decreases, the expected update direction approaches the negative gradient of $L(\bm\uptheta)$. In contrast, the noise term $\bm\upxi_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)$ tends to grow as $c_k$ decreases. More specifically, the magnitude of the covariance matrix of $\bm\upxi_k^{\text{SP}}(\hat{\bm{\uptheta}}_k)$ often increases at least as fast as $1/c_k^2$ (e.g., p. 391 in Spall 2003). Here, having $a_k\rightarrow 0$ serves to dampen the effect of the noise's growing variance.
 
 
 \section{Concluding Remarks}
 
 This chapter formally described the stochastic optimization problem and presented the general form of SA algorithms. Through the connection between root-finding and optimization, SA algorithms can be used for stochastic optimization. Although this dissertation focuses on stochastic optimization, the results of Chapters \ref{sec:cyclicseesaw}--\ref{chap:imefficient} also apply to the general root-finding setting (where the update directions are of the form in (\ref{eq:imastandardupdaedirection})) to the extent that the assumptions in Chapters \ref{sec:cyclicseesaw}--\ref{chap:imefficient} remain valid. The following chapter introduces the SA-based algorithm to be the focus of this dissertation. 
 



==> thesis arXiv 2/chapter1pp.tex <==
%!TEX root = root.tex

\chapter{Basic and Generalized Cyclic SA}
\label{chap:descriptionofGCSA}

In the basic cyclic optimization algorithm the parameter vector $\bm\uptheta$ is represented in terms of two subvectors:
\begin{align}
\setstretch{1.5} 
\bm\uptheta=\left[\begin{array}{c}\bm\uptheta^{[{1}]} \\\bm\uptheta^{[{2}]}\end{array}\right]\in \mathbb{R}^{p},
\label{eq:analgoysDRAGON}
\end{align}
\noindent where subvector $\bm\uptheta^{[{1}]}$ has length $p'$ with $0<p'<p$. In other words, if $\bm\uptheta=[\uptau_1,\dots,\uptau_p]^\top$ then $\bm\uptheta^{[{1}]}=[\uptau_1,\dots,\uptau_{p'}]^\top$ and $\bm\uptheta^{[{2}]}=[\uptau_{p'+1},\dots,\uptau_p]^\top$. The idea behind cyclic optimization methods is to alternate between updating one of the subvectors while holding the other fixed, the iterative process continues until a stopping criterion has been satisfied. Since $\bm\uptheta$ is divided into two subvectors we refer to this process as cyclic {\it{seesaw}} optimization due to its back-and-forth nature. In this chapter we introduce the {{cyclic seesaw SA}} algorithm, a cyclic implementation of SA procedures for nonlinear root-finding. This chapter also introduces the generalization to cyclic seesaw SA which will be the focus of this work (see Section \ref{sec:wunderbar}). One extension permitted by the generalization pertains to a version of the algorithm that is not necessarily strictly alternating (not cyclic seesaw). Here, there may be more than two subvectors possibly with shared components and it is known that each will be updated infinitely often as the iteration count grows to infinity. A special case of this extension arises, for example, when at each iteration a random variable dictates which subvector to update. Section \ref{sec:keatonmodasd} formally describes the cyclic seesaw SA algorithm (with two special cases given in Sections \ref{sec:ay} and \ref{sect:cspsa}) and Section \ref{sec:wunderbar} describes the generalized cyclic SA algorithm. Section \ref{sec:cocnremarksGCSA} contains concluding remarks.

\section{Cyclic Seesaw SA}
\label{sec:keatonmodasd}  

We first introduce the following notation: given any vector $\bm{v}\in \mathbb{R}^p$, let the vectors ${\bm{v}}^{(1)}$ and ${\bm{v}}^{(2)}$ be the result of replacing the last $p-p'$ coordinates or the first $p'$ coordinates of ${\bm{v}}$ with zeros, respectively. Specifically,
 \begin{align}
 \setstretch{1.5} 
  \label{eq:electricpulsar}
 \bm{v}^{(1)}=\left[\begin{array}{c}v_1  \\\vdots \\v_{p'}\\{\bm{0}}\end{array}\right]\in \mathbb{R}^p, \ \ \ \bm{v}^{(2)}=\left[\begin{array}{c}{\bm{0}} \\v_{p'+1}  \\\vdots \\v_{p}\end{array}\right]\in\mathbb{R}^p,
 \end{align} 
where $v_i$ denotes the $i$th entry of $\bm{v}$ and $\bm{0}$ denotes a vector of zeros. Thus, for example, $\bm{g}(\bm\uptheta)=\bm{g}^{(1)}(\bm\uptheta)+\bm{g}^{(2)}(\bm\uptheta)$. Using the notation in (\ref{eq:electricpulsar}), the following recursion defines cyclic seesaw SA:
\begin{align}
\bm{{\hat{\uptheta}}}_{k}^{(I)}=\bm{{\hat{\uptheta}}}_{k}-a_{k}^{(1)}\hat{\bm{g}}^{(1)}_k(\hat{\bm\uptheta}_k),\ \ \ \bm{{\hat{\uptheta}}}_{k+1}=\bm{{\hat{\uptheta}}}_{k}^{(I)}-a_{k}^{(2)}\hat{\bm{g}}^{(2)}_k(\hat{\bm\uptheta}_k^{(I)}),\label{eq:propoto2}
\end{align}
where $a_{k}^{(1)}$ and $a_{k}^{(2)}$ are sequences of positive scalars and $\hat{\bm{g}}^{(1)}_k(\hat{\bm\uptheta}_k)$ and $\hat{\bm{g}}^{(2)}_k(\hat{\bm\uptheta}_k^{(I)})$ denote noisy approximations of $\bm{g}^{(1)}(\hat{\bm{\uptheta}}_k)$ and $\bm{g}^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})$, respectively. 
%Note that obtaining $\hat{\bm{g}}^{(1)}(\hat{\bm\uptheta}_k)$ only requires approximating the first $p'$ entries of $\bm{g}(\hat{\bm{\uptheta}}_k)$. Similarly, obtaining $\hat{\bm{g}}^{(2)}(\hat{\bm\uptheta}_k^{(I)})$ only requires approximating the last $p-p'$ entries of $\bm{g}(\hat{\bm{\uptheta}}_k^{({I})})$. 
Throughout our description of the cyclic seesaw algorithm we use the superscript ``$(I)$'' to denote the intermediate step of an iteration, this is done to emphasize the seesaw nature of the algorithm. Using (\ref{eq:tennisey}), (\ref{eq:propoto2}) may also be rewritten as:
\begin{subequations}
\begin{align}
\bm{{\hat{\uptheta}}}_{k}^{(I)}&=\bm{{\hat{\uptheta}}}_{k}-a_{k}^{(1)}\left[{\bm{g}}^{(1)}(\bm{{\hat{\uptheta}}}_{k})+{\bm{\upbeta}}_k^{(1)}(\bm{{\hat{\uptheta}}}_{k})+{\bm{\upxi}}_k^{(1)}(\bm{{\hat{\uptheta}}}_{k})\right],\label{eq:byestablishing0}\\
\bm{{\hat{\uptheta}}}_{k+1}&=\bm{{\hat{\uptheta}}}_{k}^{(I)}-a_{k}^{(2)}\left[{\bm{g}}^{(2)}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upbeta}_k^{(2)}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upxi}_k^{(2)}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})\right].\label{eq:byestablishing}
\end{align}
\end{subequations}
The following section describes the cyclic seesaw SG algorithm, a special case of (\ref{eq:byestablishing0},b) where the gradient estimates are unbiased (see Section \ref{sec:sgfosa}).


\section{Cyclic Seesaw SG}
\label{sec:ay}

The cyclic seesaw SG algorithm produces its updates according to (\ref{eq:propoto2}) by using unbiased noisy gradient measurements to obtain the update directions $\hat{\bm{g}}^{(1)}_k(\hat{\bm\uptheta}_k)$ and $\hat{\bm{g}}^{(2)}_k(\hat{\bm\uptheta}_k^{(I)})$. Specifically, 
%
cyclic seesaw SG recursion is as follows:
%. Recall, however, that the SG noisy gradient measurements satisfy $\bm\upbeta_k^{\text{SG}}(\hat{\bm{\uptheta}}_k)={\bm{\upbeta}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})=\bm{0}$. Thus, cyclic seesaw SG is a special case of (\ref{eq:byestablishing}) where:
% the cyclic seesaw SA algorithm defined by the recursion:
\begin{align}
\bm{{\hat{\uptheta}}}_{k}^{(I)}=\bm{{\hat{\uptheta}}}_{k}-a_{k}^{(1)}\left[\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})\right]^{(1)},\ \ \ \bm{{\hat{\uptheta}}}_{k+1}=\bm{{\hat{\uptheta}}}_{k}^{(I)}-a_{k}^{(2)}\left[\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})\right]^{(2)},
 \label{eq:goonnowharderdinosaur}
\end{align}
where $\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})$ and $\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})$ are the SG estimates of $\bm{g}(\bm\uptheta)$ at $\hat{\bm{\uptheta}}_k$ and $\hat{\bm{\uptheta}}_k^{(I)}$, respectively (see Section \ref{sec:sgfosa}). Because the SG estimates are unbiased (by assumption), there exist vectors ${\bm{\upxi}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})$ and ${\bm{\upxi}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})$ with $E[{\bm{\upxi}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})|\hat{\bm{\uptheta}}_k]=\bm{0}$ and $E[{\bm{\upxi}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})|\hat{\bm{\uptheta}}_k^{(I)}]=\bm{0}$ such that:
\begin{align}
\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})={\bm{g}}(\bm{{\hat{\uptheta}}}_{k})+{\bm{\upxi}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}), \ \ \  \hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})={\bm{g}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upxi}}_k^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)}).
 \label{eq:uglypeppym}
\end{align}
%
Cyclic seesaw SG is then a special case of (\ref{eq:byestablishing0},b) in which the bias terms are zero. It is important to note that the vectors $\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})$ and $\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})$ in (\ref{eq:uglypeppym}) are defined only for theoretical purposes and, in practice, (\ref{eq:goonnowharderdinosaur}) implies it is unnecessary to compute all the entries in $\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k})$ and $\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})$ since several entries are replaced with zeros in (\ref{eq:goonnowharderdinosaur}). The following section introduces the cyclic seesaw SPSA algorithm, another special case of cyclic seesaw SA.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Cyclic Seesaw SPSA}
\label{sect:cspsa}

%
In the SPSA algorithm, two noisy loss function measurements are used to update the vector $\hat{\bm\uptheta}_k$ (see Section \ref{sec:coffee100}). To implement SPSA in a cyclic seesaw manner, one possibility is to replace the noisy gradient estimates in (\ref{eq:propoto2}) with gradient approximations of the form in (\ref{eq:pocres}). In other words, cyclic SPSA could be implemented as follows:
\begin{align}
\bm{{\hat{\uptheta}}}_{k}^{(I)}=\bm{{\hat{\uptheta}}}_{k}-a_{k}^{(1)}[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k)]^{(1)},\ \ \ \bm{{\hat{\uptheta}}}_{k+1}=\bm{{\hat{\uptheta}}}_{k}^{(I)}-a_{k}^{(2)}[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k^{(I)})]^{(2)},
\label{eq:moumousika}
\end{align}
where $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k)$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k^{(I)})$ are noisy estimates of $\bm{g}(\hat{\bm{\uptheta}}_k)$ and $\bm{g}(\hat{\bm{\uptheta}}_k^{(I)})$, respectively, obtained using SPSA (see Section \ref{sec:coffee100}). Specifically,
%
%suppressing the dependence of $Q(\bm\uptheta,\bm{V})$ on $\bm{V}$ for simplicity, one possibility is to let $\hat{\bm{g}}(\hat{\bm{\uptheta}}_k)=\hat{\bm{g}}^{\text{SP}}(\hat{\bm{\uptheta}}_k)$ and $\hat{\bm{g}}(\hat{\bm{\uptheta}}_k^{(I)})=\hat{\bm{g}}^{\text{SP}}(\hat{\bm{\uptheta}}_k^{(I)})$,
%
% where
\begin{align}
\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)&= \left[\begin{array}{c}\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k^{(1)}\bm\Delta_k, \bm{V}^{+}_k)-Q(\hat{\bm\uptheta}_k-c_k^{(1)}\bm\Delta_k, \bm{V}^{-}_k)}{2c_k^{(1)}\Delta_{k1}}} \\\vdots \\ \displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k^{(1)}\bm\Delta_k,\bm{V}^{+}_k)-Q(\hat{\bm\uptheta}_k-c_k^{(1)}\bm\Delta_k,\bm{V}^{-}_k)}{2c_k^{(1)}\Delta_{kp}}}\end{array}\right],
\label{eq:shmasdfg}
\end{align}
for some sequence $\{c_k^{(1)}\}_{k\geq0}$ and random vector $\bm\Delta_k=[\Delta_{k1},\dots,\Delta_{kp}]^\top$, and
\begin{align}
\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})&= \left[\begin{array}{c}\displaystyle{\frac{Q(\hat{\bm\uptheta}_k^{(I)}+c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}^{(I)+}_k)-Q(\hat{\bm\uptheta}_k^{(I)}-c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}^{(I)-}_k)}{2c_k^{(2)}\Delta_{k1}^{(I)}}} \\\vdots \\ \displaystyle{\frac{Q(\hat{\bm\uptheta}_k^{(I)}+c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}^{(I)+}_k)-Q(\hat{\bm\uptheta}_k^{(I)}-c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}^{(I)-}_k)}{2c_k^{(2)}\Delta_{kp}^{(I)}}}\end{array}\right],\label{eq:splice}
\end{align}
for a sequence $\{c_k^{(2)}\}_{k\geq0}$ (not necessarily equal to $\{c_k^{(1)}\}_{k\geq0}$) and a random vector $\bm\Delta_k^{(I)}=[\Delta_{k1}^{(I)},\dots,\Delta_{kp}^{(I)}]^\top$, where $\bm{V}^{+}_k, \bm{V}^{-}_k, \bm{V}^{(I)+}_k, \bm{V}^{(I)-}_k$ denote four different realizations of $\bm{V}$. Note that the definitions of $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})$ given in 
%
%Such a variant of SPSA would require four noisy loss function measurements per iteration (i.e., to obtain $\hat{\bm{\uptheta}}_{k+1}$ given $\hat{\bm{\uptheta}}_k$).
%
(\ref{eq:shmasdfg}) and (\ref{eq:splice}) 
%that computing $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})$
 allow adding a small perturbation to {\it{all}} elements of the vectors $\hat{\bm{\uptheta}}_k$ and $\hat{\bm{\uptheta}}_k^{(I)}$, respectively.  An alternative definition of cyclic seesaw SPSA can be obtained by only perturbing the entries to be updated. This is discussed next.
 
From (\ref{eq:moumousika}) it follows that there is no need to estimate the last $p'$ entries of $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k)$ or the first $p-p'$ entries of $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k^{(I)})$. 
%Furthermore, the vector $[\hat{\bm{g}}^{\text{SP}}_k(\bm\uptheta)]^{(j)}$ can be interpreted as a stochastic estimate of $\bm{g}^{(j)}(\bm\uptheta)$ for $j=1,2$.
%
%Additionally, it is important to note that 
% 
% it is not necessary to perturb all entries of $\hat{\bm{\uptheta}}_k$ in order to estimate the first $p'$ entries of $\hat{\bm{g}}(\hat{\bm{\uptheta}}_k)$. Using this idea, 
 Thus, an alternative definition of cyclic seesaw SPSA can be obtained by setting: 
% $[\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)]^{(1)}=\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)$ where
\begin{align}
%\label{eq:toamosd}
\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)= \left[\begin{array}{c}\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k^{(1)}\bm\Delta_k,\bm{V}_k^+)-Q(\hat{\bm\uptheta}_k-c_k^{(1)}\bm\Delta_k, \bm{V}_k^-)}{2c_k^{(1)}\Delta_{k1}}} \\\vdots \\\displaystyle{\frac{Q(\hat{\bm\uptheta}_k+c_k^{(1)}\bm\Delta_k,\bm{V}_k^+)-Q(\hat{\bm\uptheta}_k-c_k^{(1)}\bm\Delta_k,\bm{V}_k^-)}{2c_k^{(1)}\Delta_{kp'}}}\\ \bm{0}\end{array}\right],\label{eq:howeardspos1}
\end{align}
where $\bm\Delta_k=[\Delta_{k1},\dots,\Delta_{kp'},0,\dots,0]^\top$, and:
%$[\hat{\bm{g}}(\hat{\bm{\uptheta}}_k^{(I)})]^{(2)}=\hat{\bm{g}}^{\text{SP}}(\hat{\bm{\uptheta}}_k^{(I)})$ where
\begin{align}
%\label{eq:samsynocher}
\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})= \left[\begin{array}{c}\bm{0}\\ \displaystyle{\frac{Q(\hat{\bm\uptheta}_k^{(I)}+c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}_k^{(I)+})-Q(\hat{\bm\uptheta}_k^{(I)}-c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}_k^{(I)-})}{2c_k^{(2)}\Delta_{k(p'+1)}^{(I)}}} \\\vdots \\\displaystyle{\frac{Q(\hat{\bm\uptheta}_k^{(I)}+c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}_k^{(I)+})-Q(\hat{\bm\uptheta}_k^{(I)}-c_k^{(2)}\bm\Delta_k^{(I)},\bm{V}_k^{(I)-})}{2c_k^{(2)}\Delta_{kp}^{(I)}}}\end{array}\right],\label{eq:howeardspos2}
\end{align}
where $\bm\Delta_k^{(I)}=[0,\dots,0,\Delta_{k(p'+1)}^{(I)},\dots,\Delta_{kp}^{(I)}]^\top$. 

% In (\ref{eq:toamosd}) and (\ref{eq:samsynocher}) it is only necessary to perturb the entries of the parameter vector that are to be updated. 
%
Regardless of whether $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k)$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm\uptheta}_k^{(I})$ in  (\ref{eq:moumousika}) are obtained according to  (\ref{eq:shmasdfg})--(\ref{eq:splice}) or according to (\ref{eq:howeardspos1})--(\ref{eq:howeardspos2}), the resulting algorithm is a special case of (\ref{eq:byestablishing0},b). To see this, define $\mathcal{F}_k\equiv \{\hat{\bm{\uptheta}}_0,\dots,\hat{\bm{\uptheta}}_k,\bm\Delta_0,\dots,\bm\Delta_{k-1},\bm\Delta_0^{(I)},\dots,\bm\Delta_{k-1}^{(I)}\}$ and $\mathcal{F}_k^{(I)}\equiv \{\mathcal{F}_k, \hat{\bm{\uptheta}}_k^{(I)} , \bm\Delta_{k}\}$.
%\begin{align*}
%\mathcal{F}_k&\equiv \{\hat{\bm{\uptheta}}_0,\dots,\hat{\bm{\uptheta}}_k,\bm\Delta_0,\dots,\bm\Delta_{k-1},\bm\Delta_0^{(I)},\dots,\bm\Delta_{k-1}^{(I)}\},\notag\\
%\mathcal{F}_k^{(I)}&\equiv \{\hat{\bm{\uptheta}}_0,\dots,\hat{\bm{\uptheta}}_k,\hat{\bm{\uptheta}}_k^{(I)},\bm\Delta_0,\dots,\bm\Delta_{k},\bm\Delta_0^{(I)},\dots,\bm\Delta_{k-1}^{(I)}\}.
%\end{align*}
 Then, define the bias terms in (\ref{eq:byestablishing0},b) as follows:
\begin{subequations}
\begin{align}
{\bm{\upbeta}}^{(1)}_k(\hat{\bm{\uptheta}}_k)&=E\left[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)-{\bm{g}}(\hat{\bm{\uptheta}}_k)\Big|\mathcal{F}_k\right]^{(1)},\label{eq:savemebias0}\\
 {\bm{\upbeta}}^{(2)}_k(\hat{\bm{\uptheta}}_k^{(I)})&=E\left[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})-{\bm{g}}^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})\Big|\mathcal{F}_k^{(I)}\right]^{(2)},
\label{eq:savemebias}
 \end{align}
 \end{subequations}
and define the noise terms in (\ref{eq:byestablishing0},b) as follows:
 \begin{subequations}
 \begin{align}
 {\bm{\upxi}}^{(1)}_k(\hat{\bm{\uptheta}}_k)&=\left(\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)-E[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)\Big|\mathcal{F}_k]\right)^{(1)}, \label{eq:savemenoise0}\\
   {\bm{\upxi}}^{(2)}_k(\hat{\bm{\uptheta}}_k^{(I)})&=\left(\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})-E\left[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})\Big|\mathcal{F}_k^{(I)}\right]\right)^{(2)}.
   \label{eq:savemenoise}
\end{align}
 \end{subequations}
We may then write $[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k)]^{(1)}={\bm{g}}^{(1)}(\bm{{\hat{\uptheta}}}_{k})+{\bm{\upbeta}}_k^{(1)}(\bm{{\hat{\uptheta}}}_{k})+{\bm{\upxi}}_k^{(1)}(\bm{{\hat{\uptheta}}}_{k})$ and, similarly, $[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})]^{(2)}={\bm{g}}^{(2)}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upbeta}_k^{(2)}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upxi}_k^{(2)}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})$. Therefore, cyclic seesaw SPSA is a special case of (\ref{eq:byestablishing0},b). The following section introduces the generalized cyclic SA algorithm, the algorithm to be the focus of this dissertation.

\section[Generalized Cyclic SA (GCSA)]{Generalized Cyclic SA}
\label{sec:wunderbar}


While the cyclic seesaw algorithm alternates between updating each of two subvectors of $\bm\uptheta$, it is easy to conceive of an algorithm that does not exhibit this strictly alternating nature. For example, suppose that the vector to update is chosen according to a Bernoulli (i.e., binary) random variable with parameter $q_k$ (``success'' in the Bernoulli trial could mean the first subvector is updated in which case ``failure'' would mean the second subvector is updated). Formally,
\begin{align}
&{\text{Let $\mathcal{X}_k\sim \text{Bernoulli}(q_k)$}},  \notag \\
&{\text{Let $j=1$ if $\mathcal{X}_k=1$ and $j=2$ otherwise}},\notag \\
&\bm{{\hat{\uptheta}}}_{k+1}=\bm{{\hat{\uptheta}}}_{k}-\tilde{a}_{k}^{(j)}\hat{\bm{g}}^{(j)}_k(\hat{\bm\uptheta}_k)\label{eq:beer149}
\end{align}
where $\tilde{a}_k^{(j)}$ is the first unused element of a sequence $\{a_i^{(j)}\}_{i\geq0}$ with $a_i^{(j)}>0$, $q_k$ is a value in the interval $(0,1)$, and where $\mathcal{X}_k\sim \text{Bernoulli}(q_k)$ implies $\mathcal{X}_k$ has a Bernoulli distribution with success probability $q_k$.

Let us draw attention to two important differences between (\ref{eq:propoto2}) and (\ref{eq:beer149}). First, because there is no intermediate step per se in (\ref{eq:beer149}), the superscript ``$(I)$'' is avoided altogether. Second, the deterministic gain $a_k^{(j)}$ in (\ref{eq:propoto2}) has been replaced by the random gain $\tilde{a}_k^{(j)}$. Since the convergence theory for SA procedures typically requires $a_k\rightarrow 0$, using $\tilde{a}_k^{(j)}$ in place of $a_k^{(j)}$ is done with the intention of ensuring that the gain sequence does not become too small too soon. Suppose, for example, that $\mathcal{X}_k=1$ for $k=0,\cdots,99$ and $\mathcal{X}_{100}=0$ so that the first time the second subvector is updated is during iteration 101. 
%Here, $a_{100}^{(2)}$ could be much smaller than $\tilde{a}_{100}^{(2)}=a_0^{(2)}$. 
Setting
\begin{align*}
\bm{{\hat{\uptheta}}}_{101}=\bm{{\hat{\uptheta}}}_{100}-{a}_{100}^{(2)}\ \hat{\bm{g}}^{(2)}_{100}(\hat{\bm\uptheta}_{100})
\end{align*}
in this case might prove disadvantageous since $a_{100}^{(2)}$ could be very small, thus resulting in only a very small modification to the second subvector even when $\|\hat{\bm{g}}^{(2)}_{100}(\hat{\bm\uptheta}_{100})\|$ is not close to zero. This is less of an issue when using $\tilde{a}_k^{(j)}$ since $\tilde{a}_{100}^{(2)}=a_0^{(2)}$, a gain sequence value that is likely much larger than $a_{100}^{(2)}$.
%In contrast, since $\tilde{a}_{100}^{(2)}=a_0^{(2)}$ in the example above, the update in (\ref{eq:beer149}) is equivalent to setting:
%\begin{align*}
%\bm{{\hat{\uptheta}}}_{101}=\bm{{\hat{\uptheta}}}_{100}-{a}_{0}^{(2)}\ \hat{\bm{g}}^{(2)}_{100}(\hat{\bm\uptheta}_{100}).
%\end{align*}
%Here, because $a_0^{(2)}$ is the first element in the gain sequence corresponding to the second subvector, it is likely that $a_0^{(2)}$ is much larger than $a_{100}^{(2)}$. Therefore, a significant modification to the second subvector will be performed depending on the magnitude of $\hat{\bm{g}}^{(2)}_{100}(\hat{\bm\uptheta}_{100})$. 

%Using 
%Then, the first time the last $p'-p$ entries of the parameter vector are updated is during the $100$th iteration. In this case, $\tilde{a}_{100}^{(2)}=a_0^{(2)}$ could be much greater than $a_{100}^{(2)}$. 

As another example of how the cyclic seesaw algorithm might be generalized, the subvectors could be updated according to some predetermined pattern (cyclic seesaw is a particular case). For example, suppose that at each iteration the parameter vector is updated according to the following repeating pattern: two updates to $\bm\uptheta^{[1]}$ followed by a single update to $\bm\uptheta^{[2]}$ and, lastly, two updates to $\bm\uptheta^{[1]}$ (see (\ref{eq:analgoysDRAGON}) for the definition of $\bm\uptheta^{[j]}$). This algorithm could be written as:
\begin{subequations}
\begin{align}
%&\hat{\bm\uptheta}_k^{(I_{1,0})}\equiv\hat{\bm\uptheta}_k,\notag \\
&\bm{{\hat{\uptheta}}}_{k}^{(I_{1,1})}\equiv\bm{{\hat{\uptheta}}}_{k}-{a}_{k}^{(1)}\ \hat{\bm{g}}^{(1)}_k(\hat{\bm\uptheta}_k),\label{eq:believeeyes0}\\
&\bm{{\hat{\uptheta}}}_{k}^{(I_{1,2})}\equiv\bm{{\hat{\uptheta}}}_{k}^{(I_{1,1})}-{a}_{k}^{(1)}\ \hat{\bm{g}}^{(1)}_k\left(\hat{\bm\uptheta}_k^{(I_{1,1})}\right),\label{eq:believeeyes1}\\
&\bm{{\hat{\uptheta}}}_{k}^{(I_{2,1})}\equiv\bm{{\hat{\uptheta}}}_{k}^{(I_{1,2})}-{a}_{k}^{(2)}\ \hat{\bm{g}}^{(2)}_k\left(\hat{\bm\uptheta}_k^{(I_{1,2})}\right),\label{eq:believeeyes2}\\
&\hat{\bm\uptheta}_{k}^{(I_{3,1})}\equiv\bm{{\hat{\uptheta}}}_{k}^{(I_{2,1})}-{a}_{k}^{(1)}\ \hat{\bm{g}}^{(1)}_k\left(\hat{\bm\uptheta}_k^{(I_{2,1})}\right),\label{eq:believeeyes3}\\
&\hat{\bm\uptheta}_{k}^{(I_{3,2})}\equiv\bm{{\hat{\uptheta}}}_{k}^{(I_{3,1})}-{a}_{k}^{(1)}\ \hat{\bm{g}}^{(1)}_k\left(\hat{\bm\uptheta}_k^{(I_{3,1})}\right),\label{eq:believeeyes4}\\
&\hat{\bm{\uptheta}}_{k+1}= \hat{\bm\uptheta}_{k}^{(I_{3,2})}.
\label{eq:believeeyes}
\end{align}
\end{subequations}
Another way to visualize (\ref{eq:believeeyes0}--f) is given below:
\begin{align}
\hat{\bm{\uptheta}}_k\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} {{\hat{\bm\uptheta}_k^{(I_{1,1})}}}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} \hat{\bm\uptheta}_k^{(I_{1,2})}\overset{(2)}{\xrightarrow{\hspace*{0.8cm}}}\hat{\bm\uptheta}_k^{(I_{2,1})}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} \hat{\bm\uptheta}_k^{(I_{3,1})}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} {\underbrace{\hat{\bm\uptheta}_{k+1}}_{=\hat{\bm\uptheta}_k^{(I_{3,2})}}},\label{eq:lifetime}
%{\xrightarrow{\hspace*{0.8cm}}} \hat{\bm\uptheta}_k^{(I_{3,1})}\overset{(1)}
\end{align}
where the numbers above the arrows indicate which subvector was updated. In (\ref{eq:lifetime}) there are three main update ``blocks'': the first block consists of two updates to the first subvector (lines (\ref{eq:believeeyes0},b)), the second block consists of a single update to the second subvector (line (\ref{eq:believeeyes2})), and the third block consists of two more updates to the second subvector (lines (\ref{eq:believeeyes3},e)). Next we provide a slight generalization of  (\ref{eq:believeeyes0}--f) to allow for any general (deterministic) pattern for selecting the subvector to update. We begin by giving the following formal definition of what constitutes a ``block'' of subvector updates.
%(the superscripts above the arrows indicate which subvector was updated). 


\begin{definition}
\label{def:block}
 Let a block of subvector updates be defined as a {\it{maximal consecutive sequence of updates on the same subvector}}. 
 \end{definition}
 
Let $s\geq 1$ denote the number of blocks in a single iteration (in the previous example we have $s=3$) and let $n(m)\geq 1$ denote the number of updates in the $m$th block for $m=1,\dots,s$ (in the previous example, $n(1)=2$, $n(2)=1$, and $n(3)=2$). Then, the vectors of the form $\hat{\bm{\uptheta}}_k^{(I_{m,i})}$ in (\ref{eq:believeeyes0}--f) can be interpreted as the vector obtained during the $m$th block of the $(k+1)$st iteration after having performed exactly $i\geq 0$ updates within the block. Note that this interpretation 
%of $\hat{\bm{\uptheta}}_k^{(I_{m,i})}$
 implies $\hat{\bm{\uptheta}}_k^{(I_{m,n(m)})}=\hat{\bm{\uptheta}}_k^{(I_{m+1,0})}$ when $m<s$.  Including this observation in (\ref{eq:lifetime}):\label{def:intermediate}
 \begin{align*}
{\underbrace{\hat{\bm{\uptheta}}_k}_{=\hat{\bm{\uptheta}}_k^{(I_{1,0})}}}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} {{\hat{\bm\uptheta}_k^{(I_{1,1})}}}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} {\underbrace{\hat{\bm\uptheta}_k^{(I_{1,2})}}_{=\hat{\bm{\uptheta}}_k^{(I_{2,0})}}}\overset{(2)}{\xrightarrow{\hspace*{0.8cm}}}{\underbrace{\hat{\bm\uptheta}_k^{(I_{2,1})}}_{=\hat{\bm{\uptheta}}_k^{(I_{3,0})}}}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} \hat{\bm\uptheta}_k^{(I_{3,1})}\overset{(1)}{\xrightarrow{\hspace*{0.8cm}}} {\underbrace{\hat{\bm\uptheta}_{k+1}}_{=\hat{\bm\uptheta}_k^{(I_{3,2})}}}.
%{\underbrace{\hat{\bm\uptheta}_k^{(I_{3,2})}}_{=\hat{\bm\uptheta}_{k+1}}}.
\end{align*}
While at first it may seem convoluted to assign two different labels to the same vector, having $\hat{\bm{\uptheta}}_k^{(I_{m,n(m)})}=\hat{\bm{\uptheta}}_k^{(I_{m+1,0})}$ for $m<s$ serves to significantly simplify the presentation of the generalized cyclic SA algorithm of which (\ref{eq:beer149}) and (\ref{eq:believeeyes0}--f) are special cases.

An alternative way to write the algorithm in (\ref{eq:believeeyes0}--f) is as follows:
\begin{align}
&\bm{F}_k\equiv \left[{a}_{k}^{(1)}\ \hat{\bm{g}}^{(1)}_k(\hat{\bm\uptheta}_k)+{a}_{k}^{(2)}\ \hat{\bm{g}}^{(2)}_k\left(\hat{\bm\uptheta}_k^{(I_{1,2})}\right)+\sum_{i=1}^3{a}_{k}^{(1)}\ \hat{\bm{g}}^{(1)}_k\left(\hat{\bm\uptheta}_k^{(I_{i,1})}\right)\right]/a_k,\notag \\
&\hat{\bm\uptheta}_{k+1}=\hat{\bm\uptheta}_k-a_k\bm{F}_k,\label{eq:william}
\end{align}
for some sequence $\{a_i\}_{i\geq 0}$ with $a_i>0$.
%Note that expression in (\ref{eq:william}) is a special case of (\ref{eq:formof}) where ${\bm{d}}_k(\hat{\bm{\uptheta}}_k)=\bm{F}_k/a_k$. 
Similarly, the algorithm in (\ref{eq:beer149}) can also be written in the form $\hat{\bm\uptheta}_{k+1}=\hat{\bm\uptheta}_k-a_k\bm{F}_k$ after redefining the vector $\bm{F}_k$. Specifically, the algorithm in (\ref{eq:beer149}) can be written as follows:
\begin{align}
&{\text{Let $\mathcal{X}_{k}\sim \text{Bernoulli}(q_k)$}},\notag \\
&{\text{Let $j=1$ if $\mathcal{X}_{k}=1$ and $j=2$ otherwise}},\notag \\
&\bm{F}_k\equiv \left[\tilde{a}_{k}^{(j)}\hat{\bm{g}}^{(j)}_k(\hat{\bm\uptheta}_k)\right]/a_k,\notag\\
&\bm{{\hat{\uptheta}}}_{k+1}=\bm{{\hat{\uptheta}}}_{k}-a_k\bm{F}_k.\label{eq:beerabove}
\end{align}
In fact, (\ref{eq:beerabove}) is a variant of (\ref{eq:william}) in which $s=1$ (there is only one block per iteration), $n(1)=1$ (there is only one update within the block), and the subvector to update within the block is selected at random. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In general, it is possible to conceive of a vector $\bm{F}_k$ with a more general form than that in (\ref{eq:william}) or (\ref{eq:beerabove}). The number of blocks in an iteration of (\ref{eq:believeeyes0}--f), for example, could be a random variable, $s_k$, depending on the iteration number. The number of updates within a block could also be a random variable, $n_k(m)$, depending on the iteration number as well as on the block number. Moreover, the choice of which subvector to update during the $m$th block could also be a random variable, $j_k(m)$, depending on $k$. These generalizations are captured by the generalized cyclic SA algorithm introduced next. 

Let $\{\mathcal{S}_j\}_{j=1}^d$ be (not necessarily disjoint) subsets of $\mathcal{S}\equiv \{1,\dots,p\}$ satisfying:
\begin{align}
\label{eq:notexclusive}
\bigcup_{j=1}^d\mathcal{S}_j=\mathcal{S}.
\end{align}
Next, for $j=1,\dots,d$ and any vector $\bm{v}=[v_1,\dots,v_p]^\top\in \mathbb{R}^p$ define the vector $\bm{v}^{(j)}$, with $i$th entry denoted by ${v}^{(j)}_i$, as follows:
\begin{align}
\label{eq:alonesong}
{v}^{(j)}_i=
\begin{cases} v_i &\mbox{if } i \in \mathcal{S}_j,  \\ 
0 & \mbox{otherwise, }  \end{cases} 
\end{align}
this is simply a generalization of the notation used in (\ref{eq:electricpulsar}) to the case where there are $d$ subvectors possibly with shared components. Note that it is possible that $\sum_{j=1}^d\bm{g}^{(j)}(\bm\uptheta)\neq\bm{g}(\bm\uptheta)$ since $\{\mathcal{S}_j\}_{j=1}^d$ are not necessarily disjoint. The generalized cyclic stochastic approximation (GCSA) algorithm is described next.

\begin{algorithm}[p]                     
\caption{Generalized Cyclic Stochastic Approximation (GCSA)}          
\label{findme}                          
\begin{algorithmic} [1]                   % enter the algorithmic environment
\setstretch{1.5} 
\REQUIRE    $\hat{\bm{\uptheta}}_0$ and $\{a_k^{(j)}\}_{k\geq 0}$ for $j=1,\dots,d$. Set $k=0$.
%\STATE{Set $k=0$}.
\WHILE{stopping criterion has not been reached}
         \STATE{Let $s_k\in \mathbb{Z}^+$ be a random variable, where $\mathbb{Z}^+$ denotes the positive integers.
%          that is bounded uniformly in $k$.
          }
         \FOR{$m=1,\dots,s_k$}
         \STATE{Let $j_k(m)\in \{1,\dots, d\}$ be a random variable, where $d$ is defined above (\ref{eq:notexclusive}) (recall $d$ is the number of subvectors that can be updated).
%          such that $P(j_k(m)=j)=q_{k}(m,j)\neq 0$, where $P(\mathcal{E})$ denotes the probability of the event $\mathcal{E}$. 
%         and $\sum_{j=1}^dP(j_k(m)=j)=1$, where $P(\mathcal{E})$ denotes the probability of the event $\mathcal{E}$.
         } 
         \STATE{Let $n_k(m)\in \mathbb{Z}^+$ be a random variable.}
%         \label{eq:line55}
	\FOR{$i=1,\dots,n_k(m)$}\label{line:lineme}
	\STATE{Define:\label{eq:indianindinorange}
	\begin{align*}
	\hat{\bm\uptheta}_k^{(I_{m,i})}\equiv \hat{\bm\uptheta}_k&- \sum_{z=1}^{m-1}\sum_{\ell=0}^{n_k(z)-1} \left[\tilde{A}_{k}(z)\ \hat{\bm{g}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)\right]-\sum_{\ell=0}^{i-1} \left[\tilde{A}_{k}(m)\ \hat{\bm{g}}^{(j_k(m))}_k\left(\hat{\bm\uptheta}_k^{(I_{m,\ell})}\right)\right],
	\end{align*}
	where $\tilde{A}_{k}(m)\equiv\sum_{j=1}^d\chi\{j_k(m)=j\}\tilde{a}_k^{(j)}$\label{eq:attaritapo}, $\tilde{a}_k^{(j)}$ is the first unused element of the predetermined sequence $\{a_k^{(j)}\}_{k\geq0}$, $\chi \{\mathcal{E}\}$ denotes the indicator function of the event $\mathcal{E}$, and $\sum_{i=a}^b (\cdot)_i=0$ whenever $b<a$.   A mathematical definition of the random sequence $\tilde{a}_k^{(j)}$ is given in (\ref{eq:saropian}) and Figure \ref{fig:answerscully} gives a visual representation of the process through which $\tilde{a}_k^{(j)}$ is updated.  
	}
	\ENDFOR \label{line:lineme2}
	 \ENDFOR
	 \STATE{Let:
	 \begin{align*}
%	 \label{eq:pheobee}
	 \hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k^{(I_{m,i})}{\text{ with $m=s_k$ and $i=n_k(s_k)$}}.
	 \end{align*}
	 }
	\STATE{set $k=k+1$}
\ENDWHILE

\end{algorithmic}

\end{algorithm}

Using the notation in (\ref{eq:alonesong}), the idea behind GCSA is as follows: given the current parameter estimate, $\hat{\bm{\uptheta}}_k$, a decision is first made on which of its coordinates to update by selecting the coordinates in one of the sets $\mathcal{S}_1,\dots,\mathcal{S}_d$ according to a random variable. The number of blocks, number of updates within each block, and the subvector to update within each block are also random variables. After $\hat{\bm{\uptheta}}_{k+1}$ has been obtained, the process is repeated until a stopping criterion is reached. The process needed to update $\hat{\bm{\uptheta}}_k$ to $\hat{\bm{\uptheta}}_{k+1}$ will constitute an {\it{iteration}} of GCSA. Figure \ref{eq:rextickles} gives a representation of the components of an iteration of GCSA and Algorithm \ref{findme} provides an outline of GCSA. 
%Note that the algorithms in  (\ref{eq:william}) and (\ref{eq:beerabove}) are special cases of GCSA. 



%
\begin{figure}[t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
   

% 1 block
\node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[width=12mm]{Graphics/cubewhitethin-eps-converted-to.pdf}};
    \draw[->, ultra thick] (0.95,0)--(1.7,0);
    \node at (0,1.2) {\small{Block 1}};
    
    % 2 block
	\begin{scope}[xshift=+75pt]
 	  \node[inner sep=0pt] (russell) at (0,0)
  	  {\includegraphics[width=12mm]{Graphics/cubewhitethin-eps-converted-to.pdf}};
	 \draw[->, dotted, ultra thick] (0.95,0)--(2.25,0);
	 \node at (0,1.2) {\small{Block 2}};
	 
		% m block
		\begin{scope}[xshift=+90pt]
 		\node[inner sep=0pt] (russell) at (0,0)
  		{\includegraphics[width=12mm]{Graphics/cubewhitethin-eps-converted-to.pdf}};
		\draw[->, dotted, ultra thick] (0.95,0)--(2.25,0);
		\node at (0,1.2) {\small{Block $m$}};
		\draw[->, ultra thick] (0,-0.85)--(0,-1.85);
		\node[align=center] at (0,-2.9) {{Update the entries of $\bm\uptheta$}\\ {with indices in the set $\mathcal{S}_{j_k(m)}$}\\ {a total of $n_k(m)$ times.}\\};
		
			% s_k block
			\begin{scope}[xshift=+90pt]
 			\node[inner sep=0pt] (russell) at (0,0)
  			{\includegraphics[width=12mm]{Graphics/cubewhitethin-eps-converted-to.pdf}};
			\node at (0,1.2) {\small{Block $s_k$}};
			
			\end{scope} 
		
   		\end{scope}  
		
	\end{scope}  

\end{tikzpicture}
%
%
\caption[The components of an iteration of GCSA]{The components of the $(k+1)$st iteration of the GCSA algorithm (Algorithm \ref{findme}). The numbers $j_k(m)$, $n_k(m)$, and $s_k$ are allowed to be random variables. Once the value of $j_k(m)$ has been obtained, the entries to update are determined by the indices in $\mathcal{S}_{j_k(m)}$. The updates performed within the $m$th block correspond to lines \ref{line:lineme}--\ref{line:lineme2} of Algorithm \ref{findme}. 
%Note that GCSA is synchronous in nature since only one subvector may be updated at any given time. 
%In addition, note that the algorithms of (\ref{eq:believeeyes}) and (\ref{eq:beerabove}) are special cases of the GCSA.
%Here, the value $j_k(m)$ is allowed to be a random variable. The $m$th block is in charge of updating the entries of the parameter vector that lie in the set $S_{j_k(m)}$. The number of updates within block $m$, namely $n_k(m)$, is allowed to be a random variable.
}
\label{eq:rextickles}
\end{figure}
%



Let us define the sequence $\tilde{a}_k^{(j)}$ in Algorithm \ref{findme} more precisely.
% is set to be equal to the first unused element of the sequence $\{a_k^{(j)}\}_{k\geq0}$. More precisely, 
First, define:
%$\upvarphi_k^{(j)}$ be defined as follows:
\begin{align}
\label{eq:wheretheasaredefinedd}
\upvarphi_k^{(j)}\equiv\sum_{i=0}^k \chi\left\{\left(\sum_{m=1}^{s_i}\chi \{j_i(m)=j\}\right)>0\right\}-1,
\end{align}
%for each $j$.
%
%
%
%
 for each $j$. In other words, to compute $\upvarphi_k^{(j)}$ one must subtract one from the number of iterations up to and including iteration $k+1$ that use the sequence $\{a_i^{(j)}\}_{i\geq0}$.
 %
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 								TIKZ figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
 \begin{tikzpicture}
  
  
  \definecolor{newblue}{RGB}{41, 67, 86}
 
  \definecolor{mycoloring}{RGB}{183,208,225}
   \definecolor{mynewcoloring}{RGB}{215,230,244}
     \definecolor{mygrey}{RGB}{238, 243, 246}
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % LEFT PART
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      
% GRID
\fill[mynewcoloring] (-2.4,-2.4) rectangle (2.4,1.2);

%\fill[mycoloring] (-2.4,-2.4) rectangle (-1.2,-1.2);
\fill[mycoloring] (-1.2,-2.4) rectangle (1.2,-1.2);
%\fill[mycoloring] (1.2,-2.4) rectangle (2.4,-1.2);

\fill[mygrey] (-1.2,-4.8) rectangle (0,-2.4);
\fill[mygrey] (0,-3.6) rectangle (1.2,-2.4);
\fill[mygrey] (1.2,-6) rectangle (2.4,-2.4);

\draw[step=1.2cm,white,  line width=3pt] (-2.4,-6) grid (2.4,1.2);

% SELECTED FOR USE
\node[align=center] at (0,2.7) {Entries $\mathcal{S}_2$ and $\mathcal{S}_3$ are updated\\ when obtaining $\hat{\bm{\uptheta}}_{k+1}$ from $\hat{\bm{\uptheta}}_k$.};

\draw[->,ultra thick] (-0.6,1.95) -- (-0.6,1.45);
\draw[->,ultra thick] (0.6,1.95) -- (0.6,1.45);

% BIG RECTANGLE
\draw[newblue, ultra thick] (-2.63,-2.35) rectangle (2.6,-1.25);

% ARROWS
\draw[->,ultra thick] (-3.4,-1.8) -- (-2.9,-1.8);

% ARROW LABELS
\node at (-3.85,-1.75) {$\tilde{a}_k^{(j)}$};

%%%% SEQUENCES
% MAIN Row:
\node at (-1.8,-1.8) {$a_0^{(1)}$};
\node at (-0.6,-1.8) {$a_2^{(2)}$};
\node at (0.6,-1.8) {$a_1^{(3)}$};
\node at (1.8,-1.8) {$a_3^{(4)}$};

% BOTTOM Rows (COLUMN 2):
\node at (-0.6,-3) {${a_1^{(2)}}$};
\node at (-0.6,-4.2) {${a_0^{(2)}}$};

% BOTTOM Rows (COLUMN 3):
\node at (0.6,-3) {${a_0^{(3)}}$};

% BOTTOM Rows (COLUMN 4):
\node at (1.8,-3) {${a_2^{(4)}}$};
\node at (1.8,-4.2) {${a_1^{(4)}}$};
\node at (1.8,-5.4) {${a_0^{(4)}}$};

% TOP Rows (COLUMN 1):
\node at (-1.8,-0.6) {$a_1^{(1)}$};
\node at (-1.8,0.6) {$\vdots$};

% TOP Rows (COLUMN 2):
\node at (-0.6,-0.6) {$a_3^{(2)}$};
\node at (-0.6,0.6) {$\vdots$};

% TOP Rows (COLUMN 3):
\node at (0.6,-0.6) {$a_2^{(3)}$};
\node at (0.6,0.6) {$\vdots$};

% TOP Rows (COLUMN 4):
\node at (1.8,-0.6) {$a_4^{(4)}$};
\node at (1.8,0.6) {$\vdots$};

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % RIGHT PART
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{scope}[xshift=10pt]
% GRID
\fill[mynewcoloring] (3.6,-2.4) rectangle (8.4,1.2);

\fill[mygrey] (4.8,-6) rectangle (6,-2.4);
\fill[mygrey] (6,-4.8) rectangle (7.2,-2.4);
\fill[mygrey] (7.2,-6) rectangle (8.4,-2.4);

%\fill[mycoloring] (3.6,-2.4) rectangle (8.4,-1.2);
%\fill[mycoloring] (4.8,-3.6) rectangle (7.2,-2.4);

\draw[step=1.2cm, white, line width=3pt] (3.6,-6) grid (8.4,1.2);

% BIG RECTANGLE
\draw[newblue, ultra thick] (3.37,-2.35) rectangle (8.6,-1.25);

% ARROWS
\draw[->,ultra thick] (9.35,-1.8) -- (8.85,-1.8);

% ARROW LABELS
\node at (10,-1.75) {$\tilde{a}_{k+1}^{(j)}$};

%%%% SEQUENCES
% MAIN Row:
\node at (4.2,-1.8) {$a_0^{(1)}$};
\node at (5.4,-1.8) {$a_3^{(2)}$};
\node at (6.6,-1.8) {$a_2^{(3)}$};
\node at (7.8,-1.8) {$a_3^{(4)}$};

% BOTTOM Rows (COLUMN 2):
\node at (5.4,-3) {${a_2^{(2)}}$};
\node at (5.4,-4.2) {${a_1^{(2)}}$};
\node at (5.4,-5.4) {${a_0^{(2)}}$};

% BOTTOM Rows (COLUMN 3):
\node at (6.6,-3) {${a_1^{(3)}}$};
\node at (6.6,-4.2) {${a_0^{(3)}}$};

% BOTTOM Rows (COLUMN 4):
\node at (7.8,-3) {${a_2^{(4)}}$};
\node at (7.8,-4.2) {${a_1^{(4)}}$};
\node at (7.8,-5.4) {${a_0^{(4)}}$};

% TOP Rows (COLUMN 1):
\node at (4.2,-0.6) {$a_1^{(1)}$};
\node at (4.2,0.6) {$\vdots$};

% TOP Rows (COLUMN 2):
\node at (5.4,-0.6) {$a_4^{(2)}$};
\node at (5.4,0.6) {$\vdots$};

% TOP Rows (COLUMN 3):
\node at (6.6,-0.6) {$a_3^{(3)}$};
\node at (6.6,0.6) {$\vdots$};

% TOP Rows (COLUMN 4):
\node at (7.8,-0.6) {$a_4^{(4)}$};
\node at (7.8,0.6) {$\vdots$};

% SHIFT DOWN

\node[align=center] at (6,3) {Once $\hat{\bm{\uptheta}}_{k+1}$ has been obtained,\\ shift queues 2 and 3 down\\ and begin the new iteration.};

\draw[->,ultra thick] (5.4,1.95) -- (5.4,1.45);
\draw[->,ultra thick] (6.6,1.95) -- (6.6,1.45);
\end{scope}



 \end{tikzpicture}
 \caption[The process through which $\tilde{a}_k^{(j)}$ is updated]{This is an illustration of the process through which $\tilde{a}_k^{(j)}$ is updated. For $j=1,\dots, 4$, the $j$th column of each of the two ``tables'' above represents a queue containing the used and unused elements of $\{a_i^{(j)}\}_{i\geq0}$. 
% In the example above, the sequence $\{a_k^{(1)}\}_{k\geq0}$ has not been used implying that $\tilde{a}_k^{(1)}=a_0^{(1)}$, the other three sequences have all been used at least once.
 In the example above, initially  $\tilde{a}_k^{(1)}=a_0^{(1)}$, $\tilde{a}_k^{(2)}=a_2^{(2)}$, $\tilde{a}_k^{(3)}=a_1^{(3)}$, $\tilde{a}_k^{(4)}=a_3^{(4)}$. Then, the subvectors with entries in the sets $\mathcal{S}_2$ and $\mathcal{S}_3$ are updated when obtaining $\hat{\bm{\uptheta}}_{k+1}$ from $\hat{\bm{\uptheta}}_k$. Consequently,
 % Since $a_2^{(2)}$ and $a_1^{(3)}$ are used when obtaining $\hat{\bm{\uptheta}}_{k+1}$ from $\hat{\bm{\uptheta}}_k$, 
 $\tilde{a}_{k+1}^{(1)}=a_0^{(1)}$, $\tilde{a}_{k+1}^{(2)}=a_3^{(2)}$, $\tilde{a}_{k+1}^{(3)}=a_2^{(3)}$, and $\tilde{a}_{k+1}^{(4)}=a_3^{(4)}$. 
%  Note that the gain sequence(s) used when obtaining $\hat{\bm{\uptheta}}_{k+1}$ from $\hat{\bm{\uptheta}}_k$ depend on the subvector(s) updated. Therefore, $\tilde{a}_{k+1}^{(j)}$ always depends on which subvectors were updated during the previous iteration.
  }
  \label{fig:answerscully}
\end{figure}
Then, for $k+1\geq 0$ the value of $\tilde{a}_{k+1}^{(j)}$ satisfies the following equation:
\begin{align}
\label{eq:saropian}
\tilde{a}_{k+1}^{(j)}&=a_0^{(j)}+\sum_{i=0}^k \chi\{\upvarphi_k^{(j)}\geq i\}(a_{i+1}^{(j)}-a_{i}^{(j)}).
\end{align}
Note that $\tilde{a}_0^{(j)}=a_0^{(j)}$ for all $j$ since $\sum_{a}^b(\cdot)=0$ if $a>b$. Note also that if the sequence $\{a_i^{(j)}\}_{i\geq 0}$ is not used during the $(k+1)$st iteration, that is if $j_k(m)\neq j$ for all $m$, then $\tilde{a}_{k+1}^{(j)}$ will be equal to $\tilde{a}_k^{(j)}$. This shows that $\tilde{a}_{k+1}^{(j)}$ and the indicator function $\chi\{j_k(m)\neq j\}$ may be {\it{dependent random variables}} (with the exception of the case where $\tilde{a}_{k}^{(j)}$ is a deterministic function of $k$, as in the case of (\ref{eq:william})).
% while the variables $\tilde{a}_{k}^{(j)}$ and $\chi \{j_k(m)\neq j\}$ can be assumed to be {\it{independent random variables}} (provided dependence between these variables is not intentionally introduced). 
 

The expression for $\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k^{(I_{s_k,n_k(s_k)})}$ in the GCSA algorithm (Algorithm \ref{findme}) is equivalent to the recursion:
\begin{align}
\hat{\bm\uptheta}_{k+1}= \hat{\bm\uptheta}_k-a_k\bm{F}_k,\text{ where }\bm{F}_k\equiv 
%\sum_{z=1}^{s_k-1}\sum_{\ell=0}^{n_k(z)-1} \left[\tilde{A}_{k}(z)\ \hat{\bm{g}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)\right]+\sum_{\ell=0}^{n_k(s_k)-1} \left[\tilde{A}_{k}(s_k)\ \hat{\bm{g}}^{(j_k(s_k))}_k\left(\hat{\bm\uptheta}_k^{(I_{s_k,\ell})}\right)\right]\notag\\
\left[ \sum_{z=1}^{s_k}\sum_{\ell=0}^{n_{k}(z)-1} \tilde{A}_{k}(z)\ \hat{\bm{g}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)\right]/a_k,\label{eq:hand}
\end{align}
and where $a_k>0$. Therefore, an iteration of the GCSA algorithm can be written in the general form $\hat{\bm\uptheta}_{k+1}=\hat{\bm\uptheta}_k-a_k\bm{F}_k$ (the two algorithms defined by (\ref{eq:william}) and (\ref{eq:beerabove}) are special cases of (\ref{eq:hand})). Although (\ref{eq:hand}) resembles the general SA update in (\ref{eq:formof}), existing results on convergence of SA algorithms are not directly applicable to GCSA due to the increased complexity of $\bm{F}_k$ over $\bm{Y}_k$, the typical SA update direction.

%
%
% the vector $\bm{F}_k$ is not necessarily 
%The following chapter presents a theorem on the convergence w.p.1 of the iterates of the GCSA algorithm.


\section{Concluding Remarks}
\label{sec:cocnremarksGCSA}

This chapter described the GCSA algorithm for stochastic optimization via SA, the  iterative algorithm for updating the parameter vector $\hat{\bm{\uptheta}}_k$ that will be the focus of this dissertation. The basic idea behind GCSA is to divide the vector of parameters into $d$ (possibly overlapping) subvectors. Then, at each time a decision is made regarding which subvector to update (this decision can be made according to a random variable or may be governed by a deterministic selection pattern). The subvector updates are performed using SA-based update directions (in general, it is impossible to guarantee that the update direction is a descent direction due to the presence of the noise and bias terms described in Section \ref{sec:dummieyouask}). In the GCSA algorithm, each subvector has an associated gain sequence that is a deterministic function of $k$ and is used to scale the update direction. Although the gain sequences for the different subvectors may be different, the convergence theory in the following chapter will require that all gain sequences converge to zero at the same rate.






  


==> thesis arXiv 2/chapter2.tex <==
%!TEX root = root.tex

\chapter{Convergence of GCSA}
\label{sec:cyclicseesaw}


This chapter derives conditions for the convergence w.p.1 of the GCSA iterates. Section \ref{sec:rewrite} first rewrites the GCSA algorithm as a stochastic time-dependent process. Section \ref{sec:12or15miles} then provides a detailed analysis of the process from Section \ref{sec:rewrite}. Section \ref{sec:convo} states the main theorem for this chapter (Theorem \ref{thm:hoeshoo}). Section \ref{sec:specialitay} states two corollaries regarding special cases of GCSA. Section \ref{sec:discussconvergence} discusses the validity of the assumptions of Theorem \ref{thm:hoeshoo}. Lastly, Section \ref{sec:concremarksconvergence} contains concluding remarks.

\section{Rewriting the GCSA Recursion}
\label{sec:rewrite}
The theory behind the convergence of GCSA relies on rewriting the algorithm as a stochastic time-dependent process. Loosely speaking, this section first rewrites
%
a realization of GCSA
%
 as a multi-dimensional, {{continuous}}, time-dependent function.
%
This continuous time-dependent function is then shown to satisfy a time-dependent version of the GCSA recursion in (\ref{eq:hand}), a fact which
% The two time-dependent recursions
will play a crucial role in the development of the convergence theory for GCSA in Sections \ref{sec:12or15miles} and \ref{sec:convo}.  The aforementioned time-dependent {\it{continuous function}} and a related time-dependent {\it{step function}} are constructed next.
%
%Constructing the two time-dependent versions of (\ref{eq:hand}) requires first rewriting the expression for $\bm{F}_k$. This is done next.
%

We begin by defining the following time-dependent {\it{step function}}:
\begin{align}
\bar{\bm{Z}}_{0}(t)\equiv \begin{cases}  \hat{\bm{\uptheta}}_k &\mbox{if } t\in[t_{k},t_{k+1}){\text{ for }} k\geq 0,  \\ 
{\bar{\bm{Z}}_{0}}(t_0) &\mbox{if } t\leq t_0,
 \end{cases} 
 \label{eq:daviddaas}
\end{align}
%
 where $t_{k}\equiv \sum_{i=0}^{k-1}a_{i}$ for $k\geq 0$ and where $a_k>0$ is a deterministic sequence satisfying $a_k\rightarrow 0$ (Section \ref{sec:12or15miles} imposes other assumptions on $a_k$ relating it to the gain sequences $a_k^{(j)}$ from Algorithm \ref{findme}).
% 
  Now, the time-dependent {\it{continuous function}} discussed in this section's opening paragraph
% 
  will be defined as:
%
\begin{align}
\label{eq:anlogouskartmannedg}
\bm{Z}_0(t)&\equiv \frac{(t_{k+1}-t)}{a_{k}}\bar{\bm{Z}}_0(t_k)+\frac{(t-t_k)}{a_{k}}\bar{\bm{Z}}_0(t_{k+1})
%
\end{align}
 for $t\in[t_k,t_{k+1}]$, and $\bm{Z}_0(t)\equiv\bm{Z}_0(t_0)$ for $t\leq t_0$. The function $\bm{Z}_0(t)$ is then simply an interpolation of $\bar{\bm{Z}}_0(t)$ at the interpolation points $\{t_k\}_{k\geq 0}$ (see Figure \ref{fig:zeevszeebar}). The subindex ``0'' is used in anticipation of modified versions of $\bar{\bm{Z}}_0(t)$ and $\bm{Z}_0(t)$ to be introduced in Section \ref{sec:12or15miles}. Next we rewrite the GCSA recursion in (\ref{eq:hand}) by decomposing $\bm{F}_k$ into several terms, after which the resulting expression is used to construct a time-dependent analogue to (\ref{eq:hand}) involving $\bm{Z}_0(t)$.
 

By adding and subtracting select terms (effectively adding zero) to the definition of $\bm{F}_k$ in (\ref{eq:hand}) and using the fact that $\hat{\bm{g}}_k(\bm\uptheta)= {\bm{g}}(\bm\uptheta)+{\bm{\upbeta}}_k(\bm\uptheta)+{\bm{\upxi}}_k(\bm\uptheta)$ (see Section \ref{sec:dummieyouask}), the recursion in (\ref{eq:hand}) can first be rewritten as:
%
\begin{align}
\label{eq:paved}
\hat{\bm\uptheta}_{k+1}=\hat{\bm\uptheta}_k&-\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1} \tilde{A}_{k}(m)\left[\bm\upbeta^{(j_k(m))}_k\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)+\bm\upxi^{(j_k(m))}_k\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right]\notag\\
&-\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1} \tilde{A}_{k}(m)\left[ {\bm{g}}^{(j_k(m))}\left(\hat{\bm\uptheta}_k^{\left(I_{m,i}\right)}\right)- {\bm{g}}^{(j_k(m))}(\hat{\bm\uptheta}_k)\right]\notag\\
&-\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1} \tilde{A}_{k}(m)\ {\bm{g}}^{(j_k(m))}(\hat{\bm\uptheta}_k).
\end{align}
Next,
%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 								TIKZ figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\begin{tikzpicture}
  
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
  \definecolor{mygray2}{gray}{0.8}
    
    % Axes
    \draw[mygray2, ultra thick] (-.5,0)  -- (5.8,0);
    \draw[mygray2, ultra thick] (0,-.5) -- (0,4.5);
    \node at (0.01,4.8) {$\uptheta$};
    \node at (6.95,0) {$t$};
     \node at (-0.70,0.3) {$\uptheta={0}$};
    
    % Propagation
    \draw[->,ultra thick] (5.75,0) -- (6.25,0) -- (6.75,0) ;
    
    % Waves
     \node at (.75,-.3) {$t_0=0$};
     \node at (2.5,-.3) {$t_1$};
     \node at (4,-.3) {$t_2$};
     \node at (4.8,-.3) {$t_3$};
     \node at (5.3,-.3) {$t_4$};
     
     \draw[help lines, mynewcoloring] (2.5,0) -- (2.5,4);

     \draw[ultra thick,dotted, mynewcoloring] (-.5,1)  -- (0,1); 
     \draw[ultra thick, dotted, mynewcoloring] (0,1)  -- (2.5,4);
     \draw[ultra thick, dotted, mynewcoloring] (2.5,4)  -- (4,3);
     \draw[ultra thick, dotted, mynewcoloring] (4,3)  -- (4.8,2);
     \draw[ultra thick, dotted, mynewcoloring] (4.8,2)  -- (5.3,4);
     

     \draw[ultra thick, mynewcoloring] (-.25,1)  -- (2.5,1); %
     \draw[ultra thick, mynewcoloring] (2.5,4) -- (4,4); %
     \draw[ultra thick, mynewcoloring] (4,3) -- (4.8,3); %
      \draw[ultra thick, mynewcoloring] (4.8,2) -- (5.3,2); %
      \draw[ultra thick, mynewcoloring] (5.3,4)  -- (5.75,4); %

     \draw[help lines, mynewcoloring] (4,0) -- (4,3);     
     \draw[help lines, mynewcoloring] (4.8,0) -- (4.8,2);
     \draw[help lines, mynewcoloring] (5.3,0) -- (5.3,4);   
      
      % Function Labels
      \node at (3.25,4.4) {$\bar{Z}_0(t)$};
      \node[rotate=51] at (1,2.8) {$Z_0(t)$};
   
   \draw[->] (-.6,1.6)--(-.1,1.1);
   \node at (-0.9,1.9) {$\hat{{\uptheta}}_0$};
   
   \draw[->] (1.9,4.6)--(2.4,4.1);
   \node at (1.6,4.9) {$\hat{{\uptheta}}_1$};
   
   \draw[->] (4.7,4.6)--(5.2,4.1);
   \node at (4.4,4.9) {$\hat{{\uptheta}}_4$};
    
    \node at (0,1) {\textbullet};
    \node at (2.5,4) {\textbullet};
    \node at (4,3) {\textbullet};
    \node at (4.8,2) {\textbullet};
    \node at (5.3,4) {\textbullet};
    
       
  \end{tikzpicture}
\caption[The difference between $\bar{\bm{Z}}_0(t)$ and $\bm{Z}_0(t)$.]{The difference between $\bar{Z}_0(t)$ and $Z_0(t)$, special cases of $\bar{\bm{Z}}_0(t)$ and $\bm{Z}_0(t)$ where both functions are real-valued. In general, $\bar{\bm{Z}}_0(t_k)=\bm{Z}_0(t_k)=\hat{\bm{\uptheta}}_k$.}
\label{fig:zeevszeebar}
\end{figure}
%
%
%
for $j=1,\dots, d$ define the random variables:
%
\begin{align}
\label{eq:tinkelpan}
x_k(j)\equiv \left(\frac{\tilde{a}_{k}^{(j)} }{a_{k}}\right)\sum_{m=1}^{s_k}\chi\{j_k(m)=j\}n_k(m).
\end{align}
%
 Assuming $\upmu_k(j)\equiv E[x_k(j)]$ exists 
% with $|\upmu_k(j)|<\infty$ 
and is finite and that $\upmu(j)\equiv \lim_{k\rightarrow \infty} \upmu_k(j)$ exists and is finite (these assumptions will be discussed in Section \ref{sec:discussconvergence}), define:
%
\begin{align}
\bm{h}_k(\bm\uptheta)\equiv \sum_{j=1}^d \upmu_k(j)\bm{g}^{(j)}(\bm\uptheta), \ \ \ \bm{h}(\bm\uptheta)\equiv \sum_{j=1}^d \upmu(j)\bm{g}^{(j)}(\bm\uptheta).\label{eq:unrealantartica}
\end{align}
%
By adding and subtracting $a_k\bm{h}(\hat{\bm{\uptheta}}_k)$ from the right-hand side of (\ref{eq:paved}):
\begin{align}
\hat{\bm\uptheta}_{k+1}=\hat{\bm\uptheta}_k&-a_k\bm{h}(\hat{\bm{\uptheta}}_k)-a_k\Bigg[\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1} \left(\frac{\tilde{A}_{k}(m) }{a_{k}}\right){\bm{g}}^{(j_k(m))}(\hat{\bm\uptheta}_k)-\bm{h}(\hat{\bm{\uptheta}}_k)\Bigg]\notag\\
&-a_k\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1} \left(\frac{\tilde{A}_{k}(m) }{a_{k}}\right)\left[\bm\upbeta_k^{(j_k(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)+\bm\upxi_k^{(j_k(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right]\notag\\
%
&-a_{k}\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1}\left(\frac{\tilde{A}_{k}(m)}{a_{k}}\right)\left[ {\bm{g}}^{(j_k(m))}\left(\hat{\bm\uptheta}_k^{\left(I_{m,i}\right)}\right)- {\bm{g}}^{(j_k(m))}(\hat{\bm\uptheta}_k)\right].
\label{eq:pandabear}
\end{align}
Thus, when $\upmu_k(j)$ and $\upmu(j)$ exist and are finite, (\ref{eq:pandabear}) is equivalent to the GCSA recursion from (\ref{eq:hand}). Next we derive a time-dependent version of (\ref{eq:pandabear}).

We begin by defining the following terms:
\begin{subequations}
\begin{align}
\bar{\bm{B}}_0(t_k)\equiv&\ \sum_{r=0}^{k-1} a_r\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1} \left(\frac{\tilde{A}_{r}(m) }{a_{r}}\right)\bm\upbeta_r^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right),\label{eq:pulcritud0}\\
\bar{\bm{M}}_0(t_k)\equiv&\ \sum_{r=0}^{k-1} a_r\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1} \left(\frac{\tilde{A}_{r}(m) }{a_{r}}\right)\bm\upxi_r^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right),\label{eq:pulcritud1}\\
{\bar{\bm{N}}}_0(t_k)\equiv&\ \sum_{r=0}^{k-1} a_r\Bigg[\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1} \left(\frac{\tilde{A}_{r}(m) }{a_{r}}\right){\bm{g}}^{(j_r(m))}(\hat{\bm\uptheta}_r)-h(\hat{\bm{\uptheta}}_r)\Bigg],\label{eq:pulcritud2}\\
\bar{\bm{W}}_0(t_k)\equiv&\ \sum_{r=0}^{k-1} a_{r}\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1}\left(\frac{\tilde{A}_{r}(m)}{a_{r}}\right)\left[ {\bm{g}}^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{\left(I_{m,i}\right)}\right)- {\bm{g}}^{(j_r(m))}(\hat{\bm\uptheta}_r)\right].\label{eq:pulcritud}
\end{align}
\end{subequations}
%
Then, using the notation from  (\ref{eq:pulcritud0}--d), an equivalent way to write (\ref{eq:pandabear}) is:
\begin{align}
\bar{\bm{Z}}_0(t_{k+1})=&\ \bar{\bm{Z}}_0(t_{0})-\bar{\bm{B}}_0(t_{k+1})-\bar{\bm{M}}_0(t_{k+1})\notag\\
&-\bar{\bm{N}}_0(t_{k+1})-\bar{\bm{W}}_0(t_{k+1})-\sum_{i=0}^ka_i\bm{h}(\bar{\bm{Z}}_0(t_i)).\label{eq:excited}
%
\end{align}
The expression in (\ref{eq:excited}) lays the foundation for constructing the continuous and time-dependent version of the GCSA recursion (\ref{eq:pandabear}). Specifically,
%
in a manner analogous to (\ref{eq:daviddaas}) let $\bar{\bm{B}}_0(t)$, $\bar{\bm{M}}_0(t)$, $\bar{\bm{N}}_0(t)$, and $\bar{\bm{W}}_0(t)$ be step functions on the interval $[t_k,t_{k+1})$ and, in a manner analogous to (\ref{eq:anlogouskartmannedg}),
let $\bm{B}_0(t)$, $\bm{M}_0(t)$, $\bm{N}_0(t)$, and $\bm{W}_0(t)$ denote their respective interpolation functions.
%
Then, using $t_0=0$:
\begin{align}
\label{eq:sandsss}
{\bm{Z}}_0(t)=&\ {\bm{Z}}_0(0)-{\bm{B}}_0(t)-{\bm{M}}_0(t)-{\bm{N}}_0(t)-{\bm{W}}_0(t)
-\int_{0}^t{\bm{h}}(\bar{\bm{Z}}_0(s))\ ds.
\end{align}
Alternatively, replacing the integrand (\ref{eq:sandsss}) with $\bm{h}(\bm{Z}_0(s))$ we obtain:
\begin{align}
\label{eq:levelred222}
{\bm{Z}}_0(t)=&\ {\bm{Z}}_0(0)-{\bm{B}}_0(t)-{\bm{M}}_0(t)-{\bm{N}}_0(t)-{\bm{W}}_0(t)
-\int_{0}^t{\bm{h}}({\bm{Z}}_0(s))\ ds +{\bm{\upzeta}}_{0}(t),
\end{align}
where $\bm\upzeta_0(t)$ is a vector representing the error introduced by using ${\bm{h}}({\bm{Z}}_0(s))$ in place of ${\bm{h}}(\bar{\bm{Z}}_0(s))$. Equation (\ref{eq:levelred222}) represents a continuous and time-dependent version of the GCSA recursion.
%
The following section proves a few lemmas regarding the GCSA algorithm when treated as the stochastic time-dependent, continuous process in (\ref{eq:levelred222}). 

\section{Analyzing the GCSA Recursion}
\label{sec:12or15miles}



This section proves several results regarding a set of shifted versions of (\ref{eq:sandsss}) and (\ref{eq:levelred222}). Specifically, 
%
define the {\it{shift functions}}:
\begin{align}
\label{eq:gochoire}
 \bar{\bm{Z}}_k(t)\equiv{\bar{\bm{Z}}}_0(t_k+t), \ \ \ \bm{Z}_k(t)\equiv{\bm{Z}}_0(t_k+t), 
 \end{align}
 and the {\it{shift-increment functions}}:
 \begin{subequations}
 \begin{align} 
\bm{B}_k(t)\equiv{\bm{B}}_0(t_k+t)-{\bm{B}}_0(t_k),\ \ \ \bm{M}_k(t)\equiv{\bm{M}}_0(t_k+t)-{\bm{M}}_0(t_k),\label{eq:easychair0}\\
\bm{N}_k(t)\equiv{\bm{N}}_0(t_k+t)-{\bm{N}}_0(t_k),\ \ \ \bm{W}_k(t)\equiv{\bm{W}}_0(t_k+t)-{\bm{W}}_0(t_k).\label{eq:easychair}
\end{align}
\end{subequations}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 								TIKZ figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
 \begin{tikzpicture}
  
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
  \definecolor{mygray2}{gray}{0.8}
  \definecolor{mygreen}{RGB}{80, 135, 96}

    \draw[mygray2, ultra thick] (-0.5,0)  -- (4,0);
    \draw[mygray2, ultra thick] (0,-.5) -- (0,4.5);
    
    % Set 1
    
     \draw[ultra thick, mynewcoloring] (-.5,1)  -- (0,1); 
     \draw[ultra thick, mynewcoloring] (0,1)  -- (2,4);
      \draw[ultra thick, mynewcoloring] (2,4)  -- (3,3);
      \draw[ultra thick, mynewcoloring] (3,3)  -- (3.5,3.5);
      
      \draw[->,ultra thick] (3.5,0) -- (4.5,0) ;
            
     \draw[help lines, mynewcoloring] (2,0) -- (2,4);
     \draw[help lines, mynewcoloring] (3,0) -- (3,3);
     \draw[help lines, mynewcoloring] (3,0) -- (3,3);
   
     \node at (0.01,4.8) {$\uptheta$};
     \node at (4.75,0) {$t$};
         \node at (-0.70,0.3) {$\uptheta={0}$};
     \node at (.75,-.3) {$t_0=0$};
     \node at (2,-.3) {$t_1$};
     \node at (3,-.3) {$t_2$};
     \node at (-2.75,1.5) {${Z}_1(t)$};
     \node at (4.25,3.65) {$Z_0(t)$}; 
      \node at (-2.75,0) {${B}_1(t)$};  
      \node at (4.25,1.9) {$B_0(t)$}; 


     \draw[ultra thick,dotted, mynewcoloring] (-2.5,1)  -- (-2,1); 
     \draw[ultra thick, dotted,mynewcoloring] (-2,1)  -- (0,4);
     \draw[ultra thick, dotted, mynewcoloring] (0,4)  -- (1,3);     
     \draw[ultra thick, dotted, mynewcoloring] (1,3)  -- (1.5,3.4);
     
    
    \draw[->] (-0.6,4.6)--(-0.1,4.1);
    \node at (-0.9,4.9) {$\hat{{\uptheta}}_1$};
    
    \draw[->] (1.4,4.6)--(1.9,4.1);
    \node at (1.1,4.9) {$\hat{{\uptheta}}_1$};
     
     % Set 2
     
      \draw[ultra thick, mygreen] (-.5,0)  -- (0,0); 
      \draw[ultra thick, mygreen] (0,0)  -- (2,0.5); 
      \draw[ultra thick, mygreen] (2,0.5)  -- (3,2.5); 
      \draw[ultra thick, mygreen] (3,2.5)  -- (3.5,2); 
      
      \draw[ultra thick,dotted,mygreen] (-2.5,-0.5)  -- (-2,-0.5);
      \draw[ultra thick,dotted,mygreen] (-2,-0.5)  -- (0,0);
      \draw[ultra thick,dotted,mygreen] (0,0)  -- (1,2);
      \draw[ultra thick,dotted,mygreen] (1,2)  -- (1.5,1.5);
        
     \node at (0,1) {\textbullet};
     \node at (2,4) {\textbullet}; 
     \node at (3,3) {\textbullet};
          
     \node at (-2,1) {\textbullet};
     \node at (0,4) {\textbullet}; 
     \node at (1,3) {\textbullet};
     

      \node at (2,0.5) {\textbullet};
      \node at (3,2.5) {\textbullet};
      
      \node at (-2,-0.5) {\textbullet};
      \node at (0,0) {\textbullet};
      \node at (1,2) {\textbullet};
      
  \end{tikzpicture}
  \caption[Comparing $\bm{Z}_0(t)$ to $\bm{Z}_1(t)$ and $\bm{B}_0(t)$ to $\bm{B}_1(t)$.]{Comparing $\bm{Z}_0(t)$ to $\bm{Z}_1(t)$ and $\bm{B}_0(t)$ to $\bm{B}_1(t)$ for the case where all functions have real-valued output. The variables in (\ref{eq:easychair0},b) are obtained by shifting a function up/down and to the left so that $\bm{B}_k(t_0)=\bm{M}_k(t_0)=\bm{N}_k(t_0)=\bm{W}_k(t_0)=\bm{0}$. In contrast, the functions in (\ref{eq:gochoire}) are obtained solely via left-shifts so that $ \bar{\bm{Z}}_k(t_0)=\bm{Z}_k(t_0)=\hat{\bm{\uptheta}}_k$.}
  \label{fig:ufosite}
\end{figure} 
(Figure \ref{fig:ufosite} illustrates the difference between a shift function and a shift-increment function.)
% 
%
Using the notation from (\ref{eq:gochoire}) and (\ref{eq:easychair0},b), ${\bm{Z}}_k(t)$ satisfies:
%
\begin{align}
\label{eq:bondok}
{\bm{Z}}_k(t)=&\ {\bm{Z}}_k(0)-{\bm{B}}_k(t)-{\bm{M}}_k(t)-{\bm{N}}_k(t)-{\bm{W}}_k(t)
-\int_{0}^t{\bm{h}}(\bar{\bm{Z}}_k(s))\ ds.
\end{align}
%
Alternatively, replacing the integrand (\ref{eq:bondok}) with $\bm{h}(\bm{Z}_k(s))$:
\begin{align}
\label{eq:levelred}
{\bm{Z}}_k(t)=&\ {\bm{Z}}_k(0)-{\bm{B}}_k(t)-{\bm{M}}_k(t)-{\bm{N}}_k(t)-{\bm{W}}_k(t)
-\int_{0}^t{\bm{h}}({\bm{Z}}_k(s))\ ds +{\bm{\upzeta}}_{k}(t),
\end{align}
for a vector $\bm\upzeta_k(t)$ representing the error introduced by using ${\bm{h}}({\bm{Z}}_k(s))$ in place of ${\bm{h}}(\bar{\bm{Z}}_k(s))$.  Equation (\ref{eq:levelred}) is similar to equation (2.3.3) in Kushner and Clark (1978)\nocite{kushnclark1978}, though (\ref{eq:levelred}) is significantly more complex.
%
This section proves several lemmas pertaining to terms appearing in (\ref{eq:bondok}) and (\ref{eq:levelred}). These lemmas will then be used in Section \ref{sec:convo} to prove this chapter's main convergence theorem. Pages \pageref{chap:fun}-- \pageref{def:lastpage} contain a compilation of frequently used notation (including a section with GCSA-specific notation) which may be used as a quick reference.




The results in this section make use of Kolmogorov's Extension Theorem (\O ksendal 2003, Theorem 2.1.5)\nocite{oksendal2003}, which guarantees that any realization of GCSA can be seen as a random variable on a probability space $(\Omega,\mathcal{F},P)$, where $\Omega$ is the sample space, $\mathcal{F}$ is the $\upsigma$-field and $P$ is a probability measure. In other words, each $\upomega\in \Omega$ is assumed to determine (via some unknown function) an entire realization of GCSA. Thus, for example, the random sets $\{\tilde{A}_k^{(j_k(m))}\}_{k}$, $\{\hat{\bm\uptheta}_k^{(I_{m,i})}\}_{k,m,i}$, $\{\bm\upxi_k^{(j_k(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})\}_{k,m,i}$, and $\{\bm\upbeta_k^{(j_k(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})\}_{k,m,i}$ are fully determined by $\upomega$. 
%
  Next, we introduce a set of assumptions to be used throughout this section. Throughout these assumptions let $\upomega$ be as defined above.

\begin{DESCRIPTION}
%
\item[A0] Let $a_{k}>0$ and $a_k^{(j)}>0$ for all $k$ and $j$. Let $\sum_{k=0}^{\infty}a_{k}=\infty$ and $\sum_{k=0}^{\infty}a_{k}^2<\infty$. Next, let $E[\tilde{a}_k^{(j)}/a_k]\rightarrow r_j$ with $0\leq r_j<\infty$. Additionally, let there exist a set $\Omega_0\subset\Omega$ with $P(\Omega_0)=1$ such that $\tilde{a}_k^{(j)}/a_k\rightarrow r_j$ for all $\upomega\in\Omega_0$.  
\item [A1]  Let $s_k$ and $n_k(m)$ be bounded uniformly over $k$, $m$, and $\upomega$.  \label{cond:conditiona1}
\item[A2] Assume $\upmu_k(j)= E[x_k(j)]$ exists for all $k$ and $j$ and is finite (i.e., $\upmu_k(j)<\infty$) and that $\upmu(j)= \lim_{k\rightarrow \infty} \upmu_k(j)$ exists and is finite  ($x_k(j)$, $\upmu_k(j)$, and $\upmu(j)$ were first introduced in pp. \pageref{eq:tinkelpan}--\pageref{eq:unrealantartica}).
%
Additionally, define:
\begin{align*}
C_k(j)\equiv \sum_{m=1}^{s_k}\chi\{j_k(m)=j\}n_k(m),\ \ \ S_k\equiv \sum_{j=1}^dE\left[\frac{\tilde{a}_k^{(j)}}{a_k}\right](C_k(j)-E[C_k(j)]),
\end{align*}
and let $E[S_kS_\ell]=0$ for $k\neq \ell$. Furthermore, let $\tilde{a}_k^{(j)}$ and $C_k(j)$ be independent.
%
\item[A3] Let ${\bm{g}}(\bm\uptheta)$ be a continuous  function (i.e., $L(\bm\uptheta)$ is continuously differentiable).
\item[A4] For $k\geq0$, $m\leq s_k$, $i\leq n_k(m)$, let there exist a set $\Omega_1\subset\Omega$ with $P(\Omega_1)=1$ and a scalar $0<R_1(\upomega)<\infty$ such that the set $\{\hat{\bm\uptheta}_k^{(I_{m,i})}\}_{k,m,i}$ is contained within a $p$-dimensional ball of radius $R_1(\upomega)$ centered at the origin for all $\upomega\in\Omega_1$.  \label{cond:conditiona4}
\item[A5] For $k\geq0$, $m\leq s_k$, $i\leq n_k(m)$, let there exist a set $\Omega_2\subset\Omega$ with $P(\Omega_2)=1$ and a scalar $0<R_2(\upomega)<\infty$ such that the set $\{\bm\upbeta_k^{(j_k(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})\}_{k,m,i}$ is contained within a $p$-dimensional ball of radius $R_2(\upomega)$ centered at the origin for all $\upomega\in\Omega_2$.
%
Additionally, let $\bm\upbeta_k^{(j_k(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})$ converge to ${\bm{0}}$ w.p.1 as $k\rightarrow\infty$.
\item[A6] Define $\bm{D}_r\equiv \sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1} \left(\frac{\tilde{A}_{r}(m) }{a_{r}}\right)\bm\upxi^{(j_r(m))}_r\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right)$.
%
Assume for all $\upvarepsilon>0$ we have $ \lim_{k\rightarrow \infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}\bm{D}_{r}\Big\|\geq \upvarepsilon\right)=0$.
%
\item [A7] Let $\bm{\uptheta^{\ast}}$ be a locally asymptotically stable (in the sense of Lyapunov) solution of the differential equation:
\begin{align}
\label{eq:ode}
\dot{\bm{Z}}(t)\equiv\frac{d {\bm{Z}}(t)}{d t}=- \sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bm{Z}(t))
\end{align}
with domain of attraction $DA(\bm{\uptheta^{\ast}})$. 
\item[A8] There is a compact subset $A$ of $DA(\bm{\uptheta^{\ast}})$ such that $\bm{{\hat{\uptheta}}}_{k} \in A$ infinitely often (here compactness is defined using the Euclidean topology).
\end{DESCRIPTION}

The validity of A0--A8 will be discussed 
%
in Sections \ref{sec:specialitay} and \ref{sec:discussconvergence}. We note that while $a_k$ is not used by the GCSA algorithm, it serves as a representation of the rate at which ${a}_k^{(j)}$ decreases. Following are several lemmas regarding the set of functions $\{{\bm{Z}}_{k}(t)\}_{k\geq0}$.  Throughout all proofs
%
 any unspecified probabilistic arguments are meant to hold w.p.1.

\begin{lemma}
\label{claim:brey}
Assume A0 and A1 hold. Using the definition of $x_k(j)$ in (\ref{eq:tinkelpan}) let: 
\begin{align}
\label{eq:apoint}
X_k\equiv \sum_{j=1}^dx_k(j).
\end{align}
 Then, there exists a constant $0<R_3(\upomega)<\infty$ such that $|X_k|<R_3(\upomega)$ for all $\upomega\in \Omega_3$ and all $k\geq 0$.
\end{lemma}

\begin{proof}
 By A1 it follows that $s_k$ and $n_k(m)$ are bounded (uniformly in $k$, $m$, and $\upomega$). Next, A0 (using the fact that $\tilde{a}_k^{(j)}/a_k\rightarrow r_j$ w.p.1 where $0\leq r_j<\infty$) implies that for $\upomega\in \Omega_0$ the sequence $\{\tilde{a}_k^{(j)}/a_k\}_{k\geq 0}$ is bounded in magnitude by a constant that depends on $\upomega$ but is independent of $k$. Combining this with the definition of $x_k(j)$ given in (\ref{eq:tinkelpan}) and the fact that $d<\infty$ yields the desired result.
\end{proof}


\begin{lemma}
\label{claim:trompeta} Assume condition A4 holds. Then, w.p.1 the set $\{\bm{Z}_k(t)\}_{k\geq0}$ is a set of continuous functions that are bounded over $t$ uniformly in $k$.
\end{lemma}

\begin{proof}
A direct consequence of condition A4 is that $\{\hat{\bm\uptheta}_k\}_{k\geq 0}$ must be a bounded set (although the magnitude of the bound may be a function of $\upomega$). Since $\bm{Z}_0(t)$ was obtained by interpolating the vectors $\{\hat{\bm\uptheta}_k\}_{k\geq 0}$ then $\bm{Z}_0(t)$ must be bounded uniformly over $t\in\mathbb{R}$ w.p.1. Since $\bm{Z}_k(t)$ is obtained by performing a sequence of left-shifts on $\bm{Z}_0(t)$, all functions in $\{\bm{Z}_k(t)\}_{k\geq 0}$ must be bounded uniformly in $k$ and $t$ w.p.1. Additionally, these functions are clearly continuous by construction (the functions are linear interpolations of bounded vectors). 
\end{proof}

The next lemma relies on the concept of the ``equicontinuity'' of set of functions. This concept  and two related concepts are defined next.

\begin{definition}
\label{def:newspaperchaingg}
A set $\{\bm{\uprho}_k(t)\}_{k\geq0}$ of functions from $\mathbb{R}$ to $\mathbb{R}^p$ is said to be {\it{equicontinuous}} at $t$ if for all $k$ and $\upepsilon>0$ there exists a $\updelta(t,\upepsilon)$ such that $\|\bm{\uprho}_k(t)-\bm{\uprho}_k(s)\|<\upepsilon$ if $|t-s|<\updelta(t,\upepsilon)$.  If the set of functions is equicontinuous at every $t$ it is said to be {\it{point-wise equicontinuous}}. The set of functions is said to be {\it{uniformly equicontinuous}} over a set $\mathcal{S}\subset \mathbb{R}$ if for all $k\geq 0$, $t\in \mathcal{S}$, and $\upepsilon>0$ there exists a $\updelta(\upepsilon)$ such that $\|\bm{\uprho}_k(t)-\bm{\uprho}_k(s)\|<\upepsilon$ whenever $|t-s|<\updelta(\upepsilon)$ and $s\in \mathcal{S}$ (note that $\updelta(\upepsilon)$ depends neither on $k$ nor on $t$).
\end{definition}


\begin{lemma}
\label{claim:loan}
 Assume conditions A0, A1, and A5 hold and for any finite $T>0$ define $I_{T}\equiv[-T,T]$. Then, the following statements hold for all $\upomega$ in a set w.p.1 and any finite $T>0$. The set $\{{\bm{B}}_{k}(t)\}_{k\geq0}$ is a set of functions, each of which is uniformly continuous over $ I_T$ (note that at this point we are not claiming equicontinuity). Additionally, the functions in $\{{\bm{B}}_{k}(t)\}_{k\geq0}$ are bounded over $t\in I_T$ uniformly in $k$. Furthermore, $\bm{B}_{k}(t)\rightarrow \bm{0}$ uniformly over $t\in I_T$ as $k\rightarrow \infty$. The former statements imply $\{{\bm{B}}_{k}(t)\}_{k\geq0}$ is uniformly equicontinuous over $ I_T$.
\end{lemma}

\begin{proof}
%
First, we prove that $\{\bm{B}_k(t)\}_{k\geq 0}$ is bounded over $t\in I_T$ uniformly in $k$. First and foremost, using the fact that all gain sequences are nonnegative (condition A0), the definition of $\tilde{A}_{r}(m)$ given in Algorithm \ref{findme}, and the definition of $\bar{\bm{B}}_0(t_k)$ in (\ref{eq:pulcritud0}) along with the triangle inequality gives rise to the following inequality:
\begin{align}
\label{eq:mussel}
\|\bar{\bm{B}}_0(t_k)\|\leq \sum_{r=0}^{k-1} a_r\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1} \left(\frac{\tilde{A}_{r}(m) }{a_{r}}\right)\left\|\bm\upbeta_r^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right)\right\|.
\end{align}
Under A5, for all $\upomega\in\Omega_2$  there exists a constant $R_2(\upomega)$ such that the term $\|\bm\upbeta_k^{(j_k(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\|$ is bounded above by $R_2(\upomega)$.
%
Then, from (\ref{eq:mussel}) we have:
\begin{align*}
%
\|\bar{\bm{B}}_0(t_{k+1})-\bar{\bm{B}}_0(t_{k})\|&\leq a_k\sum_{m=1}^{s_k}\sum_{i=0}^{n_k(m)-1} \left(\frac{\tilde{A}_{k}(m) }{a_{k}}\right)R_2(\upomega)\notag\\
&= a_kX_kR_2(\upomega)
\end{align*}
%
for all $\upomega\in\Omega_2$, where $X_k$ was defined in (\ref{eq:apoint}).
%
 Using the result from Lemma \ref{claim:brey} we obtain the bound $|X_k|<R_3(\upomega)$ for $\upomega \in \Omega_3$, which implies:
\begin{align}
\label{eq:soeur}
\|\bar{\bm{B}}_0(t_{k+1})-\bar{\bm{B}}_0(t_{k})\|\leq a_kR_2(\upomega)R_3(\upomega)
\end{align}
for all $\upomega\in\Omega_2\cap\Omega_3$ (note that $P({\Omega_2}\cap{\Omega_3})=1$).
%
Because $\bm{B}_0(t)$ is a piecewise-linear interpolation of $\bar{\bm{B}}_0(t)$ at the points $\{t_k\}_{k\geq0}$,
%
it follows from (\ref{eq:soeur}) that for $t\in\mathbb{R}$:
\begin{align}
\label{eq:santiagokorman}
\|\bm{B}_k(t)\|=\|\bm{B}_0(t_k+t)-\bm{B}_0(t_k)\|\leq |t|R_2(\upomega)R_3(\upomega).
\end{align}
The inequality in (\ref{eq:santiagokorman}) implies that each function in $\{\bm{B}_k(t)\}_{k\geq0}$ is bounded in magnitude by $TR_2(\upomega)R_3(\upomega)$ for $t\in I_T$ and $\upomega\in\Omega_2\cap\Omega_3$ (independently of $k$).
%

Observe now that $\bm{B}_k(t)$ is continuous by construction. Since any continuous function on a compact set is uniformly continuous on that set, for each $k$ the function ${\bm{B}}_k(t)$ is uniformly continuous on $I_T$ (Rudin 1976, Theorem 4.19)\nocite{Rudin1976}. So far, we have proven that the functions in the set $\{\bm{B}_k(t)\}_{k\geq 0}$ are bounded uniformly (in $k$) for $t\in I_T$ and that, for each $k$, the function $\bm{B}_k(t)$ is uniformly continuous over $t\in I_T$. Next, we show $\bm{B}_k(t)$ converges to the zero vector uniformly over $t\in I_T$. 

By the last part of A5 (the convergence of the bias vector to zero), there exists a set $\Omega_4\subset\Omega$ with $P(\Omega_4)=1$ such that for any $\upomega\in\Omega_4$ and any $\upepsilon>0$ there exists a finite constant $K_1(\upomega,\upepsilon)$ such that $\|\bm\upbeta_k^{(j_k(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})\|\leq \upepsilon$
%
whenever $k\geq K_1(\upomega,\upepsilon)$. Therefore, using (\ref{eq:santiagokorman}) with $R_2(\upomega)$ replaced by $\upepsilon$ yields the bound:
\begin{align}
\label{eq:danceheart}
\|\bm{B}_k(t)\|=\|\bm{B}_0(t_k+t)-\bm{B}_0(t_k)\|\leq \upepsilon|t|R_3(\upomega),
\end{align}
provided $t_k+t > t_{K_1(\upomega,\upepsilon)}$. Note that having $k> K_1(\upomega, \upepsilon)$ does not guarantee that $t_k+t > t_{K_1(\upomega,\upepsilon)}$ since $t$ may be negative. However, by condition A0 (using the fact that $\sum_{k=0}^\infty a_k=\infty$) there exists a finite constant $K_2(T,K_1(\upomega,\upepsilon))$ with $K_2(T,K_1(\upomega,\upepsilon))\geq K_1(\upomega,\upepsilon)$ such that for $k\geq K_2(T,K_1(\upomega,\upepsilon))$ and $t\in I_T$ we have $t_k+t\geq t_k-T\geq t_{K_1(\upomega,\upepsilon)}$.
%\begin{align*}
%t_k+t\geq t_k-T\geq t_{K_1(\upomega,\upepsilon)}.
%\end{align*}
In other words, if $k$ is large enough (at least as large as $K_2(T,K_1)$), the value $t_k+t$ can also be made large enough so that the interpolated bias term at time $t_k+t$ is arbitrarily small. Let $k\geq K_2(T,K_1)$ and $t\in I_T$. Then, (\ref{eq:danceheart}) with $|t|$ replaced by $T$ implies:
\begin{align}
\label{eq:blonsky}
\left\|{\bm{B}}_k(t)\right\|=\left\|{\bm{B}}_0(t_k+t)-{\bm{B}}_0(t_k)\right\|\leq  \upepsilon TR_3(\upomega)
\end{align}
provided $\upomega \in \Omega_3\cap\Omega_4$. Since $K_1(\upomega,\upepsilon)$ and $K_2(T,K_1(\upomega,\upepsilon))$ do not depend on $t$ and since $\upepsilon$ can be taken to be as small as desired, ${\bm{B}}_k(t)$ converges uniformly (in $t$) to the zero vector for $t\in I_T$ and $\upomega\in\Omega_3\cap\Omega_4$ (note that $P(\Omega_3\cap\Omega_4)=1$). The fact that $\{{\bm{B}}_{k}(t)\}_{k\geq0}$ is uniformly equicontinuous for $t\in I_T$ now follows in a similar manner to the proof of Theorem 7.24 in Rudin (1976)\nocite{Rudin1976}.
\end{proof}

      
      The following lemma will be useful for 
%      studying the set
      establishing some important properties regarding 
     the set $\{\bm{M}_k(t)\}_{k\geq0}$.

\begin{lemma}[Kushner and Clark 1978, Lemma 2.2.1]
\label{lem:opportunityxyz}
\nocite{kushnclark1978}
Let $\bm{\uprho}_k$ be a vector-valued random variable. For $t_k=\sum_{r=0}^{k-1}a_r$ define
% For $t\in[0,\infty)$ let $\bm{F}(t)$ be the piecewise linear interpolation of 
%$\{\sum_{i=0}^{k-1}a_i\bm{f}_i\}$ with interpolation intervals $\{a_k\}_{k\geq0}$. Specifically,  
$\bm{R}(t_k)\equiv \sum_{r=0}^{k-1}a_r\bm{\uprho}_r$ . For $t\in[0,\infty)$ let $\bm{R}(t)$ be the piecewise linear interpolation of $\{\bm{R}(t_k)\}_{k\geq 0}$. Additionally, for $t\in(-\infty,0]$ let $\bm{R}(t)\equiv \bm{R}(t_0)$. Assume:
\begin{align*}
 \lim_{k\rightarrow \infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}\bm{\uprho}_{r}\Big\|\geq \upvarepsilon\right)=0.
\end{align*}
Then, $\bm{R}(t)$ is uniformly continuous over $t\in \mathbb{R}$ w.p.1 and $\sum_{k=0}^\infty a_k\bm{\uprho}_k<\infty$ w.p.1.
\end{lemma}

The statement of the following Lemma is similar to the statement of Lemma \ref{claim:loan} with the exception that it pertains to $\{{\bm{M}}_{k}(t)\}_{k\geq0}$. The proof of the following lemma, however, is fundamentally different from the proof of Lemma \ref{claim:loan}.

%\begin{corollary}
%Money.
%\end{corollary}


      
\begin{lemma}
\label{claim:travaille}
 Assume conditions A0 and A6 hold and for any finite $T>0$ let $ I_T$ be defined as in Lemma \ref{claim:loan}. Then, the following statements hold for all $\upomega$ in a set w.p.1 and any finite $T>0$. The set $\{{\bm{M}}_{k}(t)\}_{k\geq0}$ is a set of functions each of which is uniformly continuous over $ I_T$. Additionally, the functions in $\{{\bm{M}}_{k}(t)\}_{k\geq0}$ are bounded over $t\in I_T$ uniformly in $k$. Furthermore, $\bm{M}_{k}(t)\rightarrow \bm{0}$ uniformly over $t\in I_T$ as $k\rightarrow \infty$. The former statements imply $\{{\bm{M}}_{k}(t)\}_{k\geq0}$ is uniformly equicontinuous over $ I_T$.
\end{lemma}


\begin{proof} 
%As in the proof of Lemma \ref{claim:loan} we show that Lemma \ref{claim:travaille} holds when $ I_T$ is replaced with $I_T$. 
By letting $\bm{\uprho}_r=\bm{D}_r$ and $\bm{R}(t)=\bm{M}_0(t)$ in Lemma \ref{lem:opportunityxyz}, condition A6 
%and the fact that $\bm{M}_0(t_k)=\bar{\bm{M}}_0(t_k)$ 
implies that $\bm{M}_0(t)$ is uniformly continuous for $t\in\mathbb{R}$. Moreover, due to the manner in which $\bm{M}_k(t)$ can be obtained from $\bm{M}_0(t)$ (i.e., via shifting) we obtain the uniform continuity of $\bm{M}_k(t)$ for $t\in\mathbb{R}$ and, therefore, over $t\in I_T$. The fact that $\{\bm{M}_{k}(t)\}_{k\geq 0}$ is bounded over $t\in I_T$ uniformly in $k$ also follows from Lemma \ref{lem:opportunityxyz} as is shown next.

%Let $t_\ast \in [0,T]$ be such that $t_{n_2}=t_{n_1}+t_\ast$ for some nonnegative integers $n_1$ and $n_2$ with $n_2\geq n_1+1$. Then,
First, using the definition of $\bar{\bm{M}}_0(t_k)$ (see (\ref{eq:pulcritud1})) along with the definition of $\bm{M}_k(t)$ (see (\ref{eq:easychair0})) it follows that for any two nonnegative integers $n_1$ and $n_2$ satisfying $n_2\geq n_1+1$ the following holds:
%\begin{align*}
%\left\|\bm{M}_k(t)\right\|&=\left\|\bm{M}_0(t_k+t)-\bm{M}_0(t_k)\right\|\\
%&\leq \left\|\sum_{}\right\|
%\end{align*}
%note that if $t_m\leq t_n$:
\begin{align*}
%\bm{M}_{n_1}(t_\ast)&=
\bm{M}_0(t_{n_2})-\bm{M}_0(t_{n_1})=\bar{\bm{M}}_0(t_{n_2})-\bar{\bm{M}}_0(t_{n_1})= \sum_{r=n_1}^{n_2-1}a_r\bm{D}_r
%\label{eq:sopor}
\end{align*}
(recall that $\bm{D}_r$ was defined in condition A6). 
%Similarly, if $t_\ast\in [-T,0]$ is such that $t_{n_2}=t_{n_1}+t_\ast$ for some nonnegative integers $n_1$ and $n_2$ then:
%\begin{align*}
%\bm{M}_{n_1}(t_\ast)&=-[\bm{M}_0(t_{n_1})-\bm{M}_0(t_{n_2})]=-[\bar{\bm{M}}_0(t_{n_1})-\bar{\bm{M}}_0(t_{n_2})]= -\sum_{r={n_2}}^{n_1-1}a_r\bm{D}_r.
%%\label{eq:sopo}
%\end{align*}
Next, condition A6, Lemma \ref{lem:opportunityxyz}, and the Cauchy criterion for convergence (Rudin 1976, Theorem 3.11) imply that for any $\upepsilon>0$ there exists a constant $K_1(\upomega,\upepsilon)$ such that for $n_1, n_2\geq K_1(\upomega,\upepsilon)$:
% each of the sums in (\ref{eq:sopor}) and (\ref{eq:sopo}) has a magnitude that is upper-bounded by $\upepsilon >0$ when $n,k\geq K_1(\upomega,\upepsilon)$. In other words, 
 \begin{align}
 \label{eq:whowbuabuu}
 \Big\| \sum_{r=n_1}^{n_2-1}a_r\bm{D}_r\Big\|<\upepsilon
% \ \ \ \Big\|\sum_{r=n_2}^{n_1-1}a_r\bm{D}_r\Big\|<\upepsilon
 \end{align}
 for all $\upomega$ in a set of probability one. Therefore, $\|\bm{M}_0(t_{n_2})-\bm{M}_0(t_{n_1})\|<\upepsilon$.
 %
 In general, 
% for any $t$ a bound similar to (\ref{eq:whowbuabuu}) can be derived. Specifically, condition A0 (using the fact that $\sum_{k=0}^\infty a_k=\infty$) implies there exists an $n_\ast\geq 0$ such that $t_{n_\ast}\leq t_k+t\leq t_{n_\ast+1}$. Additionally, 
 for each $t\in I_T$ it follows from condition A0 (using the fact that $\sum_{k=0}^\infty a_k=\infty$) that
%if $t\in I_T$ is such that $t_n=t_k+t$ then 
there exists a constant $K_2(\upomega,\upepsilon,T)$ such that if $k\geq K_2(\upomega,\upepsilon,T)$ then:
\begin{align}
\label{eq:spyplanesssarc}
t_{n}\leq t_k+t\leq t_{n+1}
\end{align}
 for some $n\geq K_1(\upomega,\upepsilon)$ (the value of $n$ depends on $k$ and on $t$ although this dependance has been omitted for simplicity since it does not impact our arguments). Next, note that (\ref{eq:whowbuabuu}) with $n_1=n$ and $n_2=n+1$ implies that $\|\bm{M}_0(t_{n+1})-\bm{M}_0(t_{n})\|<\upepsilon$. 
% Since $\bm{M}_k(t)=\bm{M}_0(t_n+t_\ast)-\bm{M}_0(t_n)$ 
 Combining this with (\ref{eq:spyplanesssarc}) it follows that $\|\bm{M}_k(t)\|=\|\bm{M}_0(t_k+t)-\bm{M}_0(t_n)\|<\upepsilon$ whenever $t\in I_T$ and $k\geq K_2(\upomega,\upepsilon,T)$.
%
%at the interpolation points $t_n=t_k+t$ (provided $t\in I_T$).
%
% Because $\bm{M}_k(t)$ is a continuous piecewise-linear interpolation at these interpolation points, its magnitude must be bounded by $\upepsilon$ for all $t\in I_T$ such that $t$ is between two interpolation points provided $k\geq K_3(\upomega,\upepsilon,T)$. By A0 (using the fact that $a_k\rightarrow 0$) we can extend this conclusion to all $t\in I_T$.  
 Since $K_2(\upomega,\upepsilon,T)$ does not depend on $t$, $\bm{M}_k(t)$ must be bounded over $t\in I_T$ uniformly in $k$. Furthermore, since $\upepsilon$ can be arbitrarily small we also obtain the desired convergence of $\bm{M}_k(t)\rightarrow \bm{0}$ uniformly over $t\in I_T$. The uniform equicontinuity of $\{{\bm{M}}_{k}(t)\}_{k\geq0}$ follows immediately (see the end of the proof of Lemma \ref{claim:loan}).
\end{proof}

 The statement of the following lemma is similar to the statements of Lemmas \ref{claim:loan} and \ref{claim:travaille} with the exception that it pertains to the set $\{{\bm{N}}_{k}(t)\}_{k\geq0}$. Part of the proof of the following lemma is a combination of the proofs of Lemmas \ref{claim:loan} and \ref{claim:travaille} and, consequently, some details have been omitted. 


%\subsection[On \texorpdfstring{$\{{\bm{N}}_{k}(t)\}_{k\geq0}$}{} %
%      ]{On \texorpdfstring{$\{{\bm{N}}_{k}(t)\}_{k\geq0}$}{} %
%      }
\begin{lemma}
\label{claim:marseille}
 Assume conditions A0--A4 hold and for any finite $T>0$ let $ I_T$ be defined as in Lemma \ref{claim:loan}. Then, the following statements hold for all $\upomega$ in a set w.p.1 and any finite $T>0$. The set $\{{\bm{N}}_{k}(t)\}_{k\geq0}$ is a set of functions each of which is uniformly continuous over $ I_T$. Additionally, the functions in $\{{\bm{N}}_{k}(t)\}_{k\geq0}$ are bounded over $t\in I_T$ uniformly in $k$. Furthermore, $\bm{N}_{k}(t)\rightarrow \bm{0}$ uniformly over $t\in I_T$ as $k\rightarrow \infty$. The former statements imply $\{{\bm{N}}_{k}(t)\}_{k\geq0}$ is uniformly equicontinuous over $ I_T$.
%
\end{lemma}

\begin{proof}
% As in the proof of Lemma \ref{claim:loan} we show that Lemma \ref{claim:marseille} holds when $ I_T$ is replaced with $I_T$. 
 First, rewrite the expression for $\bar{\bm{N}}_0(t_k)$ given in (\ref{eq:pulcritud2}) as follows:
\begin{align}
\bar{\bm{N}}_0(t_k)
%&=\sum_{r=0}^{k-1}a_r \left[\sum_{j=1}^dx_r(j)\bm{g}^{(j)}(\hat{\bm{\uptheta}}_r)-\bm{h}(\hat{\bm{\uptheta}}_r)\right]\notag\\
%&=\sum_{r=0}^{k-1}a_r \left[\sum_{j=1}^dx_r(j)\bm{g}^{(j)}(\hat{\bm{\uptheta}}_r)-\sum_{i=1}^d \upmu(j)\bm{g}^{(j)}(\bm\hat{\bm{\uptheta}}_r)\right]\notag\\
&=\sum_{r=0}^{k-1}a_r\left[\sum_{j=1}^d(x_r(j)-\upmu_r(j)+\upmu_r(j)-\upmu(j))\bm{g}^{(j)}(\hat{\bm{\uptheta}}_r)\right]=\sum_{r=0}^{k-1}a_r\bm\upnu_r,\label{eq:votedownsimb}
\end{align}
where $\bm\upnu_r\equiv\sum_{j=1}^d(x_r(j)-\upmu_r(j)+\upmu_r(j)-\upmu(j))\bm{g}^{(j)}(\hat{\bm{\uptheta}}_r)$ with $x_r(j)$, $\upmu_r(j)$, and $\upmu(j)$ defined in on pp. \pageref{eq:tinkelpan}--\pageref{eq:unrealantartica}. Using A0 (the fact that $\tilde{a}_k^{(j)}/a_k\rightarrow r_j$ w.p.1), A1, A2, A3, and A4, equation (\ref{eq:votedownsimb}) implies that $\bm\upnu_r$ is bounded in magnitude w.p.1 (for $\upomega\in\Omega_0\cap \Omega_1$) uniformly over $r$. Therefore, w.p.1 there exists a constant $R_4(\upomega)$ satisfying $\|\bm\upnu_r\|\leq R_4(\upomega)$ for $\upomega$ in a  set w.p.1. Then, via a derivation similar to that of (\ref{eq:santiagokorman}) it is possible to show that $\|\bm{N}_k(t)\|=\|\bm{N}_0(t_k+t)-\bm{N}_0(t_k)\|\leq |t|R_4(\upomega)$.
% By noting that
%\begin{align*}
%\|\bm{N}_k(t)\|=\|\bm{N}_0(t_k+t)-\bm{N}_0(t_k)\|\leq |t|R_4(\upomega).
%%&\|\bm{N}_0(t)-\bm{N}_0(t_k)\|= \left\|\left(\frac{t-t_k}{a_k}\right)[\bar{\bm{N}}_0(t_{k+1})-\bar{\bm{N}}_0(t_k)]\right\|\leq (t-t_k)R_4(\upomega)
%\end{align*}
This implies $\{\bm{N}_k(t)\}_{k\geq0}$ is bounded over $t\in I_T$ uniformly in $k$.

 Because $\bm{N}_k(t)$ is a continuous function on $I_T$ it is clear that $\bm{N}_k(t)$ must also be uniformly continuous on $I_T$. It remains to show that  $\bm{N}_k(t)$ converges to the zero vector uniformly over $t\in I_T$. We begin by rewriting the expression for the vector $\bm\upnu_r$ appearing in (\ref{eq:votedownsimb}). First,
%
 using the last part of condition A2:
%  we obtain the equation:
\begin{align}
x_r(j)-\upmu_r(j)=&\ E\left[\frac{\tilde{a}_r^{(j)}}{a_r}\right](C_r(j)-E[C_r(j)])\notag\\
&+\left(\frac{\tilde{a}_r^{(j)}}{a_r}-E\left[\frac{\tilde{a}_r^{(j)}}{a_r}\right]\right)C_r(j).\label{eq:pinottnoiress}
\end{align}
Using (\ref{eq:pinottnoiress}) let us express $\bm\upnu_r$ as $\bm\upnu_r= \bm\upnu_r'+\bm\upnu_r''$, where
\begin{align*}
\bm\upnu_r'&\equiv \sum_{j=1}^dE\left[\frac{\tilde{a}_r^{(j)}}{a_r}\right](C_r(j)-E[C_r(j)])\bm{g}^{(j)}(\hat{\bm{\uptheta}}_r),\notag\\
\bm\upnu_r''&\equiv \sum_{j=1}^d\left[\upeta_r(j)C_r(j)+\upmu_r(j)-\upmu(j)\right]\bm{g}^{(j)}(\hat{\bm{\uptheta}}_r),
\end{align*}
and $\upeta_k(j)\equiv{\tilde{a}_k^{(j)}}/{a_k}-E[{\tilde{a}_k^{(j)}}/{a_k}]$. Note that A0 implies $\upeta_k(j)\rightarrow 0$ w.p.1. Therefore,
% for any $\upepsilon>0$ and $k$ large enough: $0\leq |T_k(j)|<\upepsilon$.
%for some scalar $T_k(j,\upepsilon)$ with magnitude less than $\upepsilon$. 
since $C_k(j)$ is bounded (a consequence of condition A1) it follows that $\upeta_k(j)C_k(j)\rightarrow 0$ w.p.1. Next we study the asymptotic properties of $\bm\upnu_r'$ and $\bm\upnu_r''$.

Conditions A2, A3, and A4 along with the fact that $\upeta_k(j)C_k(j)\rightarrow 0$ w.p.1 imply $\bm\upnu_r''\rightarrow \bm{0}$ w.p.1.
%\begin{align}
%\label{eq:tagg}
%{\text{$\bm\upnu_r''\rightarrow \bm{0}$ w.p.1.}} 
%\end{align}
The term $\bm\upnu_r'$, on the other hand, cannot be assumed to converge. However, it is possible to show $\sum_{k=0}^{\infty}a_{k}\bm{\upnu}_k'<\infty$, which we do next. Using the definition of $S_r$ given in condition A2,
%\begin{align*}
%S_r\equiv \sum_{j=1}^dE\left[\frac{\tilde{a}_r^{(j)}}{a_r}\right](C_r(j)-E[C_r(j)]).
%\end{align*}
conditions A0 and A1 imply that for a fixed $k$ the sequence $\{\sum_{r=k}^{m}a_rS_r\}_{m\geq k}$ (indexed by $m$)
%\begin{align*}
%\left\{\sum_{r=k}^{m}a_rS_r\right\}_{m\geq k}
%\end{align*}
is a martingale sequence. An implication of p. 315 in Doob (1953)\nocite{doob1953} is the following:
\begin{align}
P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}S_r\Big\|\geq \upvarepsilon\right)&\leq\upvarepsilon^{-2}E\Big\|\sum_{r=k}^\infty a_{r}{S_r}\Big\|^2=\upvarepsilon^{-2}\sum_{r=k}^\infty a_{r}^{2}\Var{(S_r)},
\label{eq:ranchie2}
\end{align}
where equality holds by condition A2 (the fact that $E[S_kS_\ell]=0$ for $k\neq \ell$).
%
Moreover, since the $C_k(j)$ are bounded uniformly in $k$ and $j$ (condition A1) and since the sequence $E[{\tilde{a}_k^{(j)}}/{a_k}]$ converges (condition A0), the sequence $S_k$ must be bounded uniformly in $k$. Therefore, there exists an $\upsigma^2>0$ such that $\Var{(S_k)}\leq \upsigma^2$ for all $k$. Then, (\ref{eq:ranchie2}) along with condition A0 
%(using the fact that $\sum_{k=0}^\infty a_k^2<\infty$) 
implies:
\begin{align*}
\lim_{k\rightarrow\infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}S_r\Big\|\geq \upvarepsilon\right)\leq \lim_{k\rightarrow\infty}\frac{\upsigma^2}{\upvarepsilon^{2}}\sum_{r=k}^\infty a_{r}^{2}=0.
\end{align*}
Then, 
%\begin{align*}
%\lim_{k\rightarrow\infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}S_r\Big\|\geq \upvarepsilon\right)
%= 0.
%\end{align*}
Lemma \ref{lem:opportunityxyz} implies:
\begin{align*}
\sum_{k=0}^{\infty}a_{k}\sum_{j=1}^dE\left[\frac{\tilde{a}_k^{(j)}}{a_k}\right](C_k(j)-E[C_k(j)])=\sum_{k=0}^{\infty}a_{k}S_k<\infty{\text{ w.p.1.}}
\end{align*}
Furthermore, since $\|\bm{g}^{(j)}(\hat{\bm{\uptheta}}_k)\|$ is bounded w.p.1 (conditions A3 and A4): 
\begin{align}
\label{eq:saxophone2}
\sum_{k=0}^{\infty}a_{k}\sum_{j=1}^dE\left[\frac{\tilde{a}_k^{(j)}}{a_k}\right](C_k(j)-E[C_k(j)])\bm{g}^{(j)}(\hat{\bm{\uptheta}}_k)=\sum_{k=0}^{\infty}a_{k}\bm{\upnu}_k'<\infty.
\end{align}



Following the ideas in the proofs of Lemmas \ref{claim:loan} and \ref{claim:travaille}, equation (\ref{eq:saxophone2}) and the fact that $\bm\upnu_k''\rightarrow \bm{0}$ w.p.1 can be used to show that $\bm{N}_{k}(t)$ converges to the zero vector uniformly over $t\in I_T$. Specifically, the term $\bm{\upnu}_r'$ can be related to the term $\bm{D}_r$ appearing in condition A6 and $\bm\upnu_r''$ can be related to the term:
\begin{align*}
\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1} \left(\frac{\tilde{A}_{r}(m) }{a_{r}}\right)\left\|\bm\upbeta_r^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right)\right\|
\end{align*}
appearing in (\ref{eq:mussel}).
%
 Once again, the uniform equicontinuity of $\{{\bm{N}}_{k}(t)\}_{k\geq0}$ follows immediately (see the proof of Lemma \ref{claim:loan}).
 \end{proof}
 
  The statement of the following lemma is similar to the statements of Lemmas \ref{claim:loan}, \ref{claim:travaille}, and \ref{claim:marseille}, with the exception that it pertains to the set $\{{\bm{W}}_{k}(t)\}_{k\geq0}$.
 

\begin{lemma}
\label{claim:dasmaitien}
 Assume conditions A0, A1, and A3--A6 hold and for any finite $T>0$ let $ I_T$ be defined as in Lemma \ref{claim:loan}. Then, the following statements hold for all $\upomega$ in a set w.p.1 and any finite $T>0$. 
% The set $\{{\bm{N}}_{k}(t)\}_{k\geq0}$ is a set of functions each of which is uniformly continuous over $ I_T$
 The set $\{{\bm{W}}_{k}(t)\}_{k\geq0}$ is a set of functions each of which is uniformly continuous over $ I_T$. Additionally, the functions in $\{{\bm{W}}_{k}(t)\}_{k\geq0}$ are bounded over $t\in I_T$ uniformly in $k$. Furthermore, $\bm{W}_{k}(t)\rightarrow \bm{0}$ uniformly over $t\in I_T$ as $k\rightarrow \infty$. The former statements imply $\{{\bm{W}}_{k}(t)\}_{k\geq0}$ is uniformly equicontinuous over $ I_T$.
%
\end{lemma}

\begin{proof}
%As in the proof of Lemma \ref{claim:loan} we show that Lemma \ref{claim:marseille} holds when $ I_T$ is replaced with $I_T$. 
% As in the previous claims, the uniform continuity of each ${\bm{W}}_{k}(t)$ function on finite intervals follows by definition. 
 First we prove the boundedness part of the lemma.  Recall the definition of $\bar{\bm{W}}_0(t_k)$ in (\ref{eq:pulcritud}) (we include it here for convenience):
\begin{align}
\label{eq:blackriverriverse}
\bar{\bm{W}}_0(t_k)= \sum_{r=0}^{k-1} a_{r}\sum_{m=1}^{s_r}\sum_{i=0}^{n_r(m)-1}\left(\frac{\tilde{A}_{r}(m)}{a_{r}}\right)\left[ {\bm{g}}^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{\left(I_{m,i}\right)}\right)- {\bm{g}}^{(j_r(m))}(\hat{\bm\uptheta}_r)\right].
\end{align}
Conditions A3 and A4 imply all terms of the form ${\bm{g}}^{(j)}(\cdot)$ in (\ref{eq:blackriverriverse}) are bounded in magnitude by a constant $R_5(\upomega)$ for all $\upomega\in \Omega_1$. Thus, using Lemma \ref{claim:brey} and following a derivation similar to that of (\ref{eq:santiagokorman}) we obtain that $\|\bm{W}_k(t)\|=\|\bm{W}_0(t_k+t)-\bm{W}_0(t_k)\|\leq |t|R_3(\upomega)R_5(\upomega)$.
%\begin{align*}
%\|\bm{W}_k(t)\|=\|\bm{W}_0(t_k+t)-\bm{W}_0(t_k)\|\leq 2|t|R_3(\upomega)R_5(\upomega).
%\end{align*}
For $t\in I_T$ this implies $\|\bm{W}_k(t)\|\leq TR_3(\upomega)R_5(\upomega)$.
%\begin{align*}
%\|\bm{W}_k(t)\|\leq TR_3(\upomega)R_5(\upomega).
%\end{align*}
Thus, $\{{\bm{W}}_{k}(t)\}_{k\geq0}$ is bounded uniformly in $k$ for $t\in I_T$. The uniform continuity of each ${\bm{W}}_{k}(t)$ function on finite (i.e., closed and bounded) intervals follows by the continuity of ${\bm{W}}_{k}(t)$. 
%Next we show ${\bm{W}}_{k}(t)$ converges to the zero vector uniformly over $t\in I_T$.
Next we show uniform convergence of $\bm{W}_{k}(t)$ to zero.

First recall that $\hat{\bm\uptheta}_k^{(I_{m,i})}$ satisfies:
\begin{align}
\label{eq:romanee}
	\hat{\bm\uptheta}_k^{(I_{m,i})}=&\ \hat{\bm\uptheta}_k- \sum_{z=1}^{m-1}\sum_{\ell=0}^{n_k(z)-1} \left[\tilde{A}_{k}(z)\ \hat{\bm{g}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)\right]-\sum_{\ell=0}^{i-1} \left[\tilde{A}_{k}(m)\ \hat{\bm{g}}^{(j_k(m))}_k\left(\hat{\bm\uptheta}_k^{(I_{m,\ell})}\right)\right]
\end{align}
(Line \ref{eq:indianindinorange} of Algorithm \ref{findme}). Next, recall that $\hat{\bm{g}}^{(j_k(z))}_k(\hat{\bm\uptheta}_k^{(I_{z,\ell})})$ can be written as the sum ${\bm{g}}^{(j_k(z))}(\hat{\bm\uptheta}_k^{(I_{z,\ell})})+{\bm{\upbeta}}^{(j_k(z))}_k(\hat{\bm\uptheta}_k^{(I_{z,\ell})})+{\bm{\upxi}}^{(j_k(z))}_k(\hat{\bm\uptheta}_k^{(I_{z,\ell})})$.
%the terms $\hat{\bm{g}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)$ in (\ref{eq:romanee}) can be written as follows:
%
%\begin{align*}
%\hat{\bm{g}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)={\bm{g}}^{(j_k(z))}\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)+{\bm{\upbeta}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)+{\bm{\upxi}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right).
%\end{align*}
%
%where 
%that is we can rewrite the noisy gradient observations in terms of the true gradient, a bias term, and a noise term. 
Furthermore, ${\bm{g}}^{(j_k(z))}(\hat{\bm\uptheta}_k^{(I_{z,\ell})})$ and ${\bm{\upbeta}}^{(j_k(z))}_k(\hat{\bm\uptheta}_k^{(I_{z,\ell})})$ are bounded w.p.1 (conditions A3--A5). Therefore, using condition A0 (the implication that $\tilde{a}_k^{(j)}\rightarrow 0$  w.p.1 for all $j$) and condition A1 we rewrite (\ref{eq:romanee}) as follows:
\begin{align}
\hat{\bm\uptheta}_k^{(I_{m,i})}=&\ \hat{\bm\uptheta}_k- \sum_{z=1}^{m-1}\sum_{\ell=0}^{n_k(z)-1} \tilde{A}_{k}(z)\ {\bm{\upxi}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)-\sum_{\ell=0}^{i-1} \tilde{A}_{k}(m)\ {\bm{\upxi}}^{(j_k(m))}_k\left(\hat{\bm\uptheta}_k^{(I_{m,\ell})}\right)+ \bm{T}_k,\label{eq:digerrootoros}
\end{align}
where $\bm{T}_k$ is a vector such that $\bm{T}_k\rightarrow \bm{0}$ w.p.1. Additionally, condition A6 and Lemma \ref{lem:opportunityxyz} imply $\sum_{k=0}^\infty a_k\bm{D}_k<\infty$ w.p.1. Therefore, 
 \begin{align}
\sum_{z=1}^{m-1}\sum_{\ell=0}^{n_k(z)-1} \left[\tilde{A}_{k}(z)\ {\bm{\upxi}}^{(j_k(z))}_k\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)\right]+\sum_{\ell=0}^{i-1} \left[\tilde{A}_{k}(m)\ {\bm{\upxi}}^{(j_k(m))}_k\left(\hat{\bm\uptheta}_k^{(I_{m,\ell})}\right)\right]\rightarrow \bm{0}{\text{ w.p.1}}\label{eq:casakakk}
\end{align}
(this is a consequence of Theorem 3.11 in Rudin 1976\nocite{Rudin1976}, also known as the Cauchy criterion for convergence). Using (\ref{eq:digerrootoros}) and (\ref{eq:casakakk}) and we can write $\hat{\bm\uptheta}_k^{(I_{m,i})}=\hat{\bm{\uptheta}}_k+\bm{T}'_k$, where $\bm{T}'_k$ is a vector such that $\bm{T}'_k\rightarrow \bm{0}$ w.p.1 as $k\rightarrow \infty$. Consequently, condition A3 implies $\|{\bm{g}}^{(j_r(m))}(\hat{\bm\uptheta}_r^{\left(I_{m,i}\right)})- {\bm{g}}^{(j_r(m))}(\hat{\bm\uptheta}_r)\|\rightarrow 0$ w.p.1
%\begin{align*}
%\left\|{\bm{g}}^{(j_r(m))}\left(\hat{\bm\uptheta}_r^{\left(I_{m,i}\right)}\right)- {\bm{g}}^{(j_r(m))}(\hat{\bm\uptheta}_r)\right\|\rightarrow 0{\text{ w.p.1}}
%\end{align*}
as $r\rightarrow \infty$ uniformly in $m$ and $i$.
%
Then, via a derivation similar to that of (\ref{eq:blonsky}) it follows that $\left\|{\bm{W}}_0(t_k+t)-{\bm{W}}_0(t_k)\right\|\leq T R_3(\upomega) \upepsilon$
%\begin{align*}
%\left\|{\bm{W}}_0(t_k+t)-{\bm{W}}_0(t_k)\right\|\leq T R_3(\upomega) \upepsilon
%\end{align*}
for $k$ large enough and $t\in I_T$. 
%Therefore, we have proven uniform convergence of $\bm{W}_k(t)$ to the zero vector on finite intervals. 
Uniform equicontinuity then follows (see the end of the proof of Lemma \ref{claim:loan}).
\end{proof}


\begin{lemma}
\label{claim:musicaxyz} Assume conditions A2--A4 hold and for any finite $T>0$ let $ I_T$ be defined as in Lemma \ref{claim:loan}. Then, the following statements hold for all $\upomega$ in a set w.p.1 and any finite $T>0$. 
%Then, the following statements hold for all $\upomega$ in a set w.p.1. 
The set of functions $\{\int_0^t\bm{h}(\bar{\bm{Z}}_k(s))\ ds\}_{k\geq0}$ is bounded over $t\in I_T$ uniformly in $k$. Furthermore, $\{\int_0^t\bm{h}(\bar{\bm{Z}}_k(s))\ ds\}_{k\geq0}$ is uniformly equicontinuous over $ I_T$.
\end{lemma}

\begin{proof}
%As in the proof of Lemma \ref{claim:loan} we show that Lemma \ref{claim:travaille} holds when $ I_T$ is replaced with $I_T$. 
Recall from (\ref{eq:unrealantartica}) that $\bm{h}(\bm\uptheta)= \sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bm\uptheta)$.
%\begin{align*}
%h(\bm\uptheta)= \sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bm\uptheta).
%\end{align*}
Then,
\begin{align}
\label{eq:buhai}
\int_0^t\bm{h}(\bar{\bm{Z}}_k(s))\ ds=\int_0^t \sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bar{\bm{Z}}_k(s))\ ds.
\end{align}
Since $\bm{g}^{(j)}(\bar{\bm{Z}}_k(t))$ is bounded w.p.1 uniformly over $k$ and $t$ (conditions A3 and A4) and since $\upmu(j)$ must be bounded uniformly in $j$ (condition A2), then the magnitude of the integrand in (\ref{eq:buhai}) must be bounded uniformly over $t$ by some constant $R_6(\upomega)$ for $\upomega$ in a set w.p.1. Thus, the boundedness part of the lemma follows for $t\in I_T$. Next, for $t_1, t_2\in I_T$ with $t_1<t_2$:
%Therefore, if $t\in I_T$ then $\|\int_0^t\bm{h}(\bar{\bm{Z}}_k(s))\ ds\|\leq T R_6(\upomega)$.
%\begin{align*}
%\left\|\int_0^t\bm{h}(\bar{\bm{Z}}_k(s))\ ds\right\|\leq T R_6(\upomega).
%\end{align*}
%This gives the uniform (over $k$) boundedness on $I_T$. The uniform equicontinuity of $\int_0^t\bm{h}(\bar{\bm{Z}}_k(s))\ ds$ follows immediately since:
\begin{align*}
\left\|\int_0^{t_2}\bm{h}(\bar{\bm{Z}}_k(s))\ ds-\int_0^{t_1}\bm{h}(\bar{\bm{Z}}_k(s))\ ds\right\|&\leq \int_{t_1}^{t_2}\left\|\bm{h}(\bar{\bm{Z}}_k(s))\right\|\ ds\leq |t_2-t_2|R_6(\upomega)
\end{align*}
independently of $k$. Therefore, the desired equicontinuity also follows.
\end{proof}

%The statements of Claims \ref{claim:trompeta}--\ref{claim:musicaxyz} all consider $t\in  I_T$.
 The following Lemma presents a result similar to that of Lemmas \ref{claim:trompeta}--\ref{claim:musicaxyz} for the set of functions $\{{\bm{Z}}_k(t)\}_{k\geq0}$ with one important modification: parts of the result are now shown to hold for all $t\in \mathbb{R}$ rather than only for $t\in  I_T$.

%\subsection[On the boundedness and equicontinuity of \texorpdfstring{$\{{\bm{Z}}_k(t)\}_{k\geq0}$}{}]{On the boundedness and equicontinuity\\ of \texorpdfstring{$\{{\bm{Z}}_k(t)\}_{k\geq0}$}{}%
%}

\begin{lemma}
\label{claim:sinuses}
 Assume conditions A0--A6 hold. Then, the functions in the set $\{{\bm{Z}}_k(t)\}_{k\geq0}$ are bounded over $t\in \mathbb{R}$ uniformly in $k$ w.p.1. Additionally, $\{{\bm{Z}}_k(t)\}_{k\geq0}$ is uniformly equicontinuous for $t\in \mathbb{R}$ w.p.1.
%  and has compact closure for $t\in\mathbb{R}$ w.p.1 (here, compactness is defined in terms of the topology of uniform convergence on closed and bounded intervals).
\end{lemma}


\begin{proof}
The desired uniform boundedness was proven in Lemma \ref{claim:trompeta}. Next, recall from (\ref{eq:bondok}) that:
\begin{align*}
{\bm{Z}}_k(t)=&\ {\bm{Z}}_k(0)-{\bm{B}}_k(t)-{\bm{M}}_k(t)-{\bm{N}}_k(t)-{\bm{W}}_k(t)-\int_{0}^t{\bm{h}}(\bar{\bm{Z}}_k(s))\ ds.
\end{align*}
%Since the sum of a finite number of uniformly equicontinuous functions is uniformly equicontinuous,
Here, Lemmas \ref{claim:loan}--\ref{claim:musicaxyz} and the fact that $\bm{Z}_k(t)$ is a shifted version of $\bm{Z}_0(t)$ imply that $\{{\bm{Z}}_k(t)\}_{k\geq0}$ is a set of uniformly equicontinuous functions for $t\in \mathbb{R}$. 
\end{proof}


 

\begin{lemma}
\label{claim:windowsxyz}
Assume conditions A0--A6 hold and for any finite $T>0$ let $ I_T$ be defined as in Lemma \ref{claim:loan}. Then, for any finite $T>0$ it follows that $\bm\upzeta_k(t)\rightarrow \bm{0}$ (recall $\bm\upzeta_k(t)$ was defined in (\ref{eq:levelred})) w.p.1 uniformly over $t\in  I_T$ as $k\rightarrow \infty$.
\end{lemma}

\begin{proof}
%As in the proof of Lemma \ref{claim:loan} we show that Lemma \ref{claim:travaille} holds when $ I_T$ is replaced with $I_T$. 
We remind the reader that any unspecified probabilistic arguments are meant w.p.1. The vector $\bm\upzeta_k(t)$ can be written as:
\begin{align}
\label{eq:haloodst}
\bm\upzeta_k(t)&=\int_{0}^t{\bm{h}}({\bm{Z}}_k(s))\ ds-\int_{0}^t{\bm{h}}(\bar{\bm{Z}}_k(s))\ ds\notag\\
%&=\int_{0}^t\left[{\bm{h}}({\bm{Z}}_k(s))-{\bm{h}}(\bar{\bm{Z}}_k(s))\right]\ ds\notag\\
&=\int_0^t \sum_{j=1}^d\upmu(j)\left[\bm{g}^{(j)}({\bm{Z}}_k(s))-\bm{g}^{(j)}(\bar{\bm{Z}}_k(s))\right]\ ds.
\end{align}
%By condition A3 we know $\bm{g}(\bm\uptheta)$ is a continuous function of $\bm\uptheta$. Furthermore, 
By condition A4, the vectors $\bar{\bm{Z}}_k(s)$ and ${\bm{Z}}_k(s)$ must lie in a $p$-dimensional ball of radius $R_1(\upomega)$ for all $\upomega\in\Omega_1$. Let $\Theta(\upomega)\subset \mathbb{R}^p$ denote the closure (using the Euclidean topology) of the aforementioned ball. Then, condition A3 implies $\bm{g}(\bm\uptheta)$ is uniformly continuous over $\bm\uptheta\in \Theta(\upomega)$. In other words, 
%if $\bar{\bm{Z}}_k(s)$ and ${\bm{Z}}_k(s)$ lie in the aforementioned compact set and are also close enough (in Euclidian norm), then 
for any $\upepsilon>0$ there exists a $\updelta_1(\upomega,\upepsilon)>0$ such that $\|\bm{g}^{(j)}({\bm{Z}}_k(s))-\bm{g}^{(j)}(\bar{\bm{Z}}_k(s))\|<\upepsilon$ if $\|\bar{\bm{Z}}_k(s)-{\bm{Z}}_k(s)\|<\updelta_1(\upomega,\upepsilon)$.
%
Next, Lemma \ref{claim:sinuses} implies $\{\bm{Z}_k(t)\}_{k\geq0}$ is uniformly equicontinuous w.p.1 on $I_T$. Therefore, for $t_1,t_2\in I_T$ and any $\upepsilon>0$, there exists a $\updelta_2(\upepsilon,T,\upomega)>0$ such that $\|{\bm{Z}}_k(t_2)-{\bm{Z}}_k(t_1)\|<\updelta_1(\upomega,\upepsilon)$
%\begin{align*}
%\|{\bm{Z}}_k(t_2)-{\bm{Z}}_k(t_1)\|<\upepsilon
%\end{align*}
whenever $|t_2-t_1|<\updelta_2(\upepsilon,T,\upomega)$ independently of $k$. Next, note that for any $\updelta_2(\upepsilon, T,\upomega)>0$ and $s\in I_T$ it is possible to take $k$ large enough (independently of $t$) so that $t_m\leq t_k+s\leq t_{m+1}$ where $t_{m+1}-t_m=a_m<\updelta_2(\upepsilon, T,\upomega)$ (this follows from condition A0). Then, for large enough $k$ and $s\in I_T$ we have $\|{\bm{Z}}_k(s)-\bar{\bm{Z}}_k(s)\|\leq \|{\bm{Z}}_k(t_{m+1})-{\bm{Z}}_k(t_m)\|<\updelta_1(\upepsilon,\upomega)$ and,
%\begin{align*}
%\|{\bm{Z}}_k(s)-\bar{\bm{Z}}_k(s)\|<\upepsilon.
%\end{align*} 
%In other words, $\|{\bm{Z}}_k(s)-\bar{\bm{Z}}_k(s)\|$ can be made small as small as desired by simply making $k$ large whenever $s\in I_T$.
 therefore, $\|\bm{g}^{(j)}({\bm{Z}}_k(s))-\bm{g}^{(j)}(\bar{\bm{Z}}_k(s))\|<\upepsilon$ for all $s\in I_T$. Consequently,
%  the integrand in (\ref{eq:haloodst}) can be made as small as desired (in magnitude) by taking $k$ to be large provided $t\in I_T$. Therefore, 
  the maximum possible norm of the integral in (\ref{eq:haloodst}) for $t\in I_T$ is $\upepsilon T$, where $\upepsilon>0$ can be as small as desired provided $k$ is large (precisely how large is independent of $t$).
%
Thus, we have proven the desired uniform (in $t$) convergence to the zero vector.
\end{proof}



\section[A Convergence Theorem for GCSA]{A Convergence Theorem for GCSA}
\label{sec:convo}

We are now ready to prove the following theorem for convergence of the GCSA algorithm. Once again, all unspecified probabilistic arguments in the statement of the theorem as well as in its proof are meant w.p.1.

\begin{theorem}
\label{thm:hoeshoo} 
Let $\hat{\bm{\uptheta}}_k$ denote the GCSA iterates of Algorithm \ref{findme} and assume conditions A0--A6 hold. Then, there exists a subsequence 
%
$\{\bm{Z}_{k_i}(t)\}_{i\geq1}$ of $\{\bm{Z}_{k}(t)\}_{k\geq0}$ 
%
and a bounded (w.p.1) function $\bm{Z}(t)$ such that $\bm{Z}_{k_i}(t)\rightarrow \bm{Z}(t)$ uniformly over $t\in I_T$ for any finite $T>0$ as $i\rightarrow \infty$ ($I_T$ was defined in Lemma \ref{claim:loan}).
%
% such that $\bm{Z}_{k_i}(t)\rightarrow \bm{Z}(t)$ uniformly for $t\in I_T$ for any finite $T>0$ as $i\rightarrow \infty$. 
%
%compact closure under the topology of uniform convergence over finite intervals. 
The aforementioned limit function, 
%if $\bm{Z}(t)$ denotes the limit of a converging subsequence $\{\bm{Z}_{k_i}(t)\}_{i\geq0}$, then 
$\bm{Z}(t)$, satisfies the ODE in (\ref{eq:ode}). If in addition conditions A7 and A8 hold (i.e., if A0--A8 hold) then ${\bm{\bm{{\hat{\uptheta}}}}}_{k}\rightarrow {\bm\uptheta^{\ast}}$ w.p.1.
\end{theorem}

\begin{proof}The proof of this theorem consists of three main steps:

\begin{DESCRIPTION}
\item[Step 1:] Show that A0--A6 imply that for $t\in \mathbb{R}$ the functions $\{{\bm{Z}_{k}(t)\}}_{k\geq0}$ are bounded uniformly in $k$, and $\{{\bm{Z}_{k}(t)\}}_{k\geq0}$  is uniformly equicontinuous.
%
\item[Step 2:] Given Step 1, the Arzel\`a--Ascoli Theorem implies that the sequence $\{\bm{Z}_k(t)\}_{k\geq0}$ must have 
%compact closure (under the topology of uniform convergence over closed and bounded intervals) as a function of $t\in \mathbb{R}$ and, therefore, 
a subsequence $\{\bm{Z}_{k_i}(t)\}_{i\geq 1}$ that converges to some bounded function $\bm{Z}(t)$ uniformly over $t\in I_T$ for any finite $T>0$ as $i\rightarrow \infty$. This step consists of showing that $\bm{Z}(t)$ must satisfy the ODE in condition A7.
%\item The next step is to show the error term $\bm\zeta_{k}(t)$  converges to zero uniformly on finite intervals w.p.1.
\item[Step 3:]  Using the asymptotic stability condition (condition A7) along with A8 show that $\bm{{\hat{\uptheta}}}_{k}$ must converge to $\bm\uptheta^\ast$.
\end{DESCRIPTION}
 Step 1 was completed in Lemma \ref{claim:sinuses}. Step 2 is an implication of  Lemmas \ref{claim:loan}--\ref{claim:dasmaitien}, \ref{claim:sinuses}, and \ref{claim:windowsxyz} as is shown next. Using the
 Arzel\`a--Ascoli Theorem (Kushner and Clark 1978, p. 20)\nocite{kushnclark1978} 
 along with the fact that $\bm{Z}_k(t)$ is a shifted version of $\bm{Z}_0(t)$
% we know the set has compact closure for $t\in\mathbb{R}$. In other words, $\bm{Z}_k(t)$ has a subsequence with a limiting function, say $\bm{Z}(t),$ which lies in the closure of $\{\bm{Z}_k(t)\}_{k\geq0}$ for $t\in \mathbb{R}$ (recall that the topology used to define closure is that of uniform convergence on closed and bounded intervals).
 it follows that there exists a subsequence $\{\bm{Z}_{k_i}(t)\}_{i\geq 1}$ and a bounded (w.p.1) function $\bm{Z}(t)$ such that $\bm{Z}_{k_i}(t)\rightarrow \bm{Z}(t)$ uniformly over $t\in I_T$ for any finite $T>0$ as $i\rightarrow \infty$. 
% Additionally, using the fact that $\bm{Z}_k(t)$ is a shifted version of $\bm{Z}_0(t)$, it follows that $\bm{Z}_{k_i}(t)\rightarrow \bm{Z}(t)$ uniformly on any closed and bounded interval.
% (see the end of the proof of Lemma \ref{claim:sinuses}). 
 Then, by (\ref{eq:levelred}) in conjunction with Lemmas \ref{claim:loan}--\ref{claim:dasmaitien} and \ref{claim:windowsxyz} (using the convergence to zero of the different functions) it follows that $\bm{Z}(t)$ satisfies:
%  the following expression:
\begin{align*}
\bm{Z}(t)= \lim_{i\rightarrow\infty}\bm{Z}_{k_i}(t)
%=&\ \lim_{i\rightarrow \infty}\left[{\bm{Z}}_{k_i}(0)-{\bm{B}}_{k_i}(t)-{\bm{M}}_{k_i}(t)-{\bm{N}}_{k_i}(t)-{\bm{W}}_{k_i}(t) -\int_{0}^t{\bm{h}}({\bm{Z}}_{k_i}(s))\ ds +{\bm{\upzeta}}_{k_i}(t)\right]\\
= {\bm{Z}}(0)-\lim_{i\rightarrow \infty}\int_{0}^t{\bm{h}}({\bm{Z}}_{k_i}(s))\ ds,
\end{align*}
for $t\in I_T$.
% Since $\{\bm{Z}_{k}(t)\}_{k\geq0}$ is uniformly equicontinuous on finite intervals, any limiting subsequence converges uniformly on $I_T$. 
Due to the uniform convergence of $\bm{Z}_{k_i}(t)$ on $I_T$ and using the continuity of $\bm{g}(\bm\uptheta)$, it follows that:
\begin{align}
\label{eq:alexgotseidankee}
\bm{h}({\bm{Z}}_{k_i}(t))\rightarrow  \sum_{j=1}^d\upmu(j)\bm{g}^{(j)}({\bm{Z}}(t))=\bm{h}({\bm{Z}}(t)){\text{ w.p.1}}
\end{align}
uniformly over $t\in I_T$ as $i\rightarrow \infty$. Using the uniform convergence in (\ref{eq:alexgotseidankee}) along with Lebesgue's dominated convergence theorem implies:
\begin{align}
\label{eq:ansdgwichtdil}
\bm{Z}(t)&= {\bm{Z}}(0)-\int_{0}^t\bm{h}({\bm{Z}}(s))\ ds
\end{align}
for $t\in I_T$. Because $T>0$ is arbitrary, (\ref{eq:ansdgwichtdil}) holds for all $t$. Therefore,
%\begin{align*}
%{\bm{Z}}(t)={\bm{Z}(0)}&-\int_{0}^{t}\bm{g}^{(1)}(\bm{Z}(t))+r\bm{g}^{(2)}(\bm{Z}(t))\ ds
%\end{align*}
%which in turn implies:
\begin{align*}
%\label{eq:cello}
\dot{\bm{Z}}(t)&=-\sum_{j=1}^d\upmu(j)\bm{g}^{(j)}({\bm{Z}}(t)),
\end{align*}
which is the ODE in (\ref{eq:ode}).
 %
% follows from Lemmas \ref{claim:loan}--\ref{claim:dasmaitien}, \ref{claim:sinuses}, and \ref{claim:windowsxyz} (see the discussion at the end of Section \ref{sec:12or15miles}). 
 The remainder of the proof (Step 3) is now identical to the last part of the proof of Theorem 2.3.1 in Kushner and Clark (1978). Therefore, only a brief outline of Step 3 is included below.

%Throughout the remainder of this proof (Step 3) all unspecified probabilistic arguments are meant w.p.1.
 By condition A8, we know there exists a subsequence $\{\bm{{\hat{\uptheta}}}_{k_i}\}_{i\geq1}$ such that $\bm{{\hat{\uptheta}}}_{k_i}\in A$ for all $i\geq 1$. Furthermore, by Step 2 we can assume without loss of generality that $\bm{Z}_{k_i}(t)\rightarrow\bm{Z}(t)$ where $\bm{Z}(t)$ satisfies the ODE in condition A7. Additionally, since $\bm{Z}_{k_i}(0)=\bm{{\hat{\uptheta}}}_{k_i}\in A$ where $A$ is a compact set then $\bm{Z}(0)\in A$ by construction. Because $\bm\uptheta^\ast$
 is an assymptotically stable (in the sense of Lyapunov) solution to the differential equation (\ref{eq:ode}), we know $ \lim_{t\rightarrow \infty}\bm{Z}(t)=\bm\uptheta^\ast$.
%  \begin{align*}
%% \lim_{t\rightarrow \infty}\bm{Z}(t)=\bm\uptheta^\ast.
% \end{align*}
The stability properties of $\bm\uptheta^\ast$ then guarantee $\bm{{\hat{\uptheta}}}_{k}\rightarrow\bm\uptheta^\ast$ (see Kushner and Clark 1978, pp. 42--43).
\end{proof}

\begin{corollary}
\label{eq:idamagedittarantatan}
If the conditions of Theorem \ref{thm:hoeshoo} hold, then the sequence $\{\hat{\bm\uptheta}_k^{(I_{m,i})}\}$ of Algorithm \ref{findme} converges to $\bm\uptheta^\ast$ w.p.1 uniformly in $m$ and $i$ as $k\rightarrow \infty$.
\end{corollary}
 \begin{proof}
 This result follows immediately from Theorem \ref{thm:hoeshoo} along with the comment below (\ref{eq:casakakk}).
%
 \end{proof}
 The following section obtains Corollaries to Theorem \ref{thm:hoeshoo} pertaining to two special cases of the GCSA algorithm.
 
 \section[Two Special Cases of GCSA]{Two Special Cases of GCSA}
 \label{sec:specialitay}
 
 
 Theorem \ref{thm:hoeshoo} gave convergence conditions for the GCSA algorithm, two special cases of which were discussed in Section \ref{sec:wunderbar} (see (\ref{eq:beer149}) and (\ref{eq:beerabove})). In (\ref{eq:beerabove}), for example, the parameter vector was partitioned into two subvectors; at each iteration the subvector to update was chosen at random. A generalization of (\ref{eq:beerabove}) is obtained by partitioning $\bm\uptheta$ into $d$ subvectors. The resulting generalization of (\ref{eq:beerabove}) is presented in Algorithm \ref{beastwasdone} below. For simplicity, it is assumed the sets $\mathcal{S}_1,\dots,\mathcal{S}_d$ in (\ref{eq:notexclusive}) satisfy:
\begin{align}
\label{eq:scurry}
\bigcup_{i=1}^d\mathcal{S}_i=\mathcal{S}, \ \ \ \bigcap_{i=1}^d\mathcal{S}_i=\emptyset.
\end{align}
%
In order to study the behavior of Algorithm \ref{beastwasdone} we first prove two lemmas that are useful for understanding the behavior of the sequence $\tilde{a}_k^{(j)}/a_k$, a sequence whose relevance stems from condition A0 in Theorem \ref{thm:hoeshoo} (also note that this ratio affects the value of $\bm{h}(\bm\uptheta)$ through (\ref{eq:tinkelpan})). The following lemma gives sufficient conditions for the convergence w.p.1 of $\tilde{a}_k^{(j)}/a_k$.
% regarding the random sequence ${\tilde{a}_{k}^{(j)}}/{a_{k}}$.
%The following lemma gives sufficient conditions for the convergence w.p.1 of ${\tilde{a}_{k}^{(j)}}/{a_{k}}$.
 \begin{algorithm}[!t]                     
\caption{Randomized Subvector Selection}          
\label{beastwasdone}                          
\begin{algorithmic} [1]                   % enter the algorithmic environment
\setstretch{1.5} 
\REQUIRE    $\hat{\bm{\uptheta}}_0$, $\{a_k^{(j)}\}_{k\geq 0}$ for $j=1,\dots,d$, and let $\mathcal{S}_1,\dots, \mathcal{S}_d$ be such that (\ref{eq:scurry}) holds. Set $k=0$.
%\STATE{Set $k=0$}.
\WHILE{stopping criterion has not been reached}
  \STATE{Let $j_k$ be a random variable with $P(j_k=j)=q(j)\neq0$ and $\sum_{j=1}^d q(j)=1$.}
	\STATE{Define:
	\begin{align*}
%	\label{eq:kidstogether}
	\hat{\bm\uptheta}_{k+1}\equiv&\ \hat{\bm\uptheta}_k-\tilde{a}_k^{(j_{k})}\hat{\bm{g}}^{(j_{k})}(\hat{\bm{\uptheta}}_k).
	\end{align*}}
	\STATE{set $k=k+1$}
\ENDWHILE
\end{algorithmic}
\end{algorithm}


\begin{lemma}
\label{lem:devil}
%(This lemma uses the notation of Algorithm \ref{findme}.) Assume $q_k(m,j)>0$ does not depend on $k$ or $m$, thus we write $q(j)$ in place of $q_k(m,j)$.
Consider the setting of Algorithm \ref{beastwasdone}. Assume $a_k>0$ and that $a_k^{(j)}>0$ is a monotonically decreasing sequence with $a_k^{(j)}\rightarrow 0$. In addition, assume there exists a function $\uprho(j,q)$ with domain $\{1,\dots,j\}\times [0,1]$ and range in $\mathbb{R}$ such that if $\upepsilon>0$ is small enough that $0\leq q(j)\pm\upepsilon\leq 1$ then:
\begin{align*}
\lim_{k\rightarrow \infty}\frac{a^{(j)}_{\floor{k(q(j)-\upepsilon)}}}{a_{k}}=\uprho (j,q(j)-\upepsilon), \ \ \ \lim_{k\rightarrow \infty}\frac{a^{(j)}_{\ceil{k(q(j)+\upepsilon)}}}{a_{k}}=\uprho (j,q(j)+\upepsilon),
\end{align*}
 ($\floor{\cdot}$ and $\ceil{\cdot}$ denote the floor and ceiling functions, respectively). Assume there exist a constant $C<\infty$ such that $0<\uprho (j, q(j)\pm \upepsilon)<C$. Finally, let:
\begin{align*}
\lim_{\upepsilon\rightarrow 0}\uprho (j, q(j)\pm \upepsilon)=\uprho (j, q(j))\in [\uprho (j, q(j)+\upepsilon),\uprho (j, q(j)-\upepsilon)].
\end{align*}
% $\uprho (j, q(j))\in [\uprho (j, q(j)+\upepsilon),\uprho (j, q(j)-\upepsilon)]$ and that $\lim_{\upepsilon\rightarrow 0}\uprho (j, q(j)\pm \upepsilon)=\uprho (j, q(j))$. 
%for $\upepsilon$ small enough. 
Then, $\tilde{a}_k^{(j)}/a_k\rightarrow \uprho (j,q(j))$ w.p.1 with $0<\uprho (j,q(j))<C$.
\end{lemma}
\begin{proof}
Throughout this proof all unspecified probabilistic arguments are meant to hold w.p.1. From (\ref{eq:saropian}) we know that for $k>0$:
\begin{align}
\tilde{a}_{k+1}^{(j)}
%&=a_0^{(j)}+\sum_{i=0}^k \mathcal{X}\left\{\frac{A_k^{(j)}}{k}\geq \frac{i}{k}\right\}(a_{i+1}^{(j)}-a_{i}^{(j)})\notag\\
&=a_0^{(j)}+\sum_{i=0}^k \chi\left\{\frac{\upvarphi_k^{(j)}}{k}-q(j)\geq \frac{i}{k}-q(j)\right\}(a_{i+1}^{(j)}-a_{i}^{(j)}),\label{eq:pianofortee}
\end{align}
where $0\leq \upvarphi_k^{(j)}\leq k$ was defined in (\ref{eq:wheretheasaredefinedd}). Furthermore, the strong law of large numbers implies that $\upvarphi_k^{(j)}/k-q(j)\rightarrow 0$ w.p.1 as $k\rightarrow \infty$. This implies (w.p.1) that for all $\upepsilon>0$ there exists an $N(\upepsilon)$ such that $|{\upvarphi_k^{(j)}}/{k}-q(j)|<\upepsilon$
%\begin{align*}
%\left|\frac{A_k^{(j)}}{k}-q(j)\right|<\upepsilon
%\end{align*}
for $k\geq N(\upepsilon)$ (the constant $N(\upepsilon)$ depends on $\upomega$ although the dependence has been omitted for simplicity). Therefore,
%Note that if $A_k^{(j)}/k-q(j)<\upepsilon$ then $\mathcal{X}\{{A_k^{(j)}}/{k}-q(j)\geq {i}/{k}-q(j)\}=0$ for all $i$ such that $i/k-q(j)\geq \upepsilon$. Equivalently:
\begin{align}
\label{eq:samuraislicemetan}
\chi\left\{\frac{\upvarphi_k^{(j)}}{k}-q(j)\geq \frac{i}{k}-q(j)\right\}=
\begin{cases} 
0 &\mbox{if } {\text{$k\geq N(\upepsilon)$ and $i\geq \ceil{k(\upepsilon+q(j))}$}},\\
1 & \mbox{if } {\text{$k\geq N(\upepsilon)$ and $i\leq \floor{k(q(j)-\upepsilon)}$}}.
 \end{cases} 
\end{align}
%
Equation (\ref{eq:samuraislicemetan}) implies $\tilde{a}_{k+1}^{(j)}\in[a^{(j)}_{ \ceil{k(\upepsilon+q(j))}}, a^{(j)}_{\floor{k(q(j)-\upepsilon)}+1}]$ for $k\geq N(\upepsilon)$. Therefore:
%
\begin{align}
\tilde{a}_{k}^{(j)}\in\left[a_{\ceil{k(q(j)+\upepsilon)-(q(j)+\upepsilon)}}^{(j)},a_{\floor{k(q(j)-\upepsilon)-(q(j)-\upepsilon)}+1}^{(j)}\right]\label{eq:jing}
\end{align}
for $k$ large. From (\ref{eq:jing}) it follows that for large $k$ and $\upepsilon>0$ small enough that $0\leq q(j)\pm\upepsilon\leq 1$:
%Note that for $\upepsilon>0$ small enough, $\tilde{I}_k^{(j)}(\upepsilon)\subset [a^{(j)}_{\ceil{k(q(j)+\upepsilon)}},a^{(j)}_{\floor{k(q(j)-\upepsilon)}}]$. Therefore,
\begin{align*}
\frac{\tilde{a}_{k}^{(j)}}{a_k}\in \left[\frac{a^{(j)}_{\ceil{k(q(j)+\upepsilon)}}}{a_k},\frac{a^{(j)}_{\floor{k(q(j)-\upepsilon)}}}{a_k}\right].
\end{align*}
Therefore, ${\tilde{a}_{k}^{(j)}}/{a_k}$ must approach the interval $I(\upepsilon)\equiv [\uprho (j, q(j)+\upepsilon),\uprho (j, q(j)-\upepsilon)]$ as $k$ grows (i.e., the distance between ${\tilde{a}_{k}^{(j)}}/{a_k}$ and its closest point in the interval $I(\upepsilon)$ approaches zero).
%\begin{align*}
% I_T(\upepsilon)\equiv\lim_{k\rightarrow \infty}\left[\frac{a^{(j)}_{\ceil{k(q(j)+\upepsilon)}}}{a_k},\frac{a^{(j)}_{\floor{k(q(j)-\upepsilon)}}}{a_k}\right]=[\uprho (j, (q(j)+\upepsilon)),\uprho (j, q(j)-\upepsilon)].
%\end{align*}
Because ${I}(\upepsilon)$ contains the point $\uprho (j, q(j))$ for all $\upepsilon>0$ small enough (by assumption) and because the length of ${I}(\upepsilon)$ decreases as $\upepsilon$ decreases,
%Thus, for any $\updelta>0$ and $k$ large enough $\tilde{a}_{k}^{(j)}/a_k$ is within $\updelta$ of $ I_T(\upepsilon)$. Furthermore, by assumption ${I}(\upepsilon)$ contains $\uprho (j, q(j))$. Since $\updelta$ and $\upepsilon$ can be taken as small as desired, 
the sequence $\tilde{a}_{k}^{(j)}/a_k$ must converge w.p.1 to $0<\uprho (j, q(j))<C$.
\end{proof}

Let us comment on the assumptions of Lemma \ref{lem:devil}. The first requirement is that $q(j)>0$ depends neither on $k$ nor on $m$. In other words, when selecting the coordinates to update from one of the sets $\mathcal{S}_1,\dots,\mathcal{S}_d$, we require the probability of selecting $\mathcal{S}_j$ to be independent of the iteration and block numbers.
% Of course, in some applications the user may be able control these probabilities. In general, we must keep in mind that this condition is sufficient but not necessary for the lemma's result to hold.
 The remaining assumptions are satisfied for sequences of the form $a_k^{(j)}=a^{(j)}/(k+A^{(j)}+1)^\upalpha$ and $a_k=a/(k+1)^\upalpha$ where $a^{(j)}>0$, $a>0$, $A^{(j)}>0$, and $0<\upalpha$. To see this, note that $\lim_{k\rightarrow \infty} a^{(j)}_k/a_k=a^{(j)}/a$ and that:
% $\lim_{k\rightarrow \infty} a^{(j)}_k/a_k=a^{(j)}/a$ and
\begin{align*}
\lim_{k\rightarrow \infty}\frac{a^{(j)}_{\floor{ck}}}{a_{k}^{(j)}}=\lim_{k\rightarrow \infty}\left(\frac{k+1}{\floor{ck}+A^{(j)}+1}\right)^\upalpha=\frac{1}{c^\upalpha},
\end{align*}
for $c>0$. The last limit can be computed by using $c_k$ as an upper bound for $\floor{ck}$, using $ck-1$ as a lower bound for $\floor{ck}$, and observing that both the upper and lower bounds result in the same limit: $1/c^\upalpha$. Therefore, $\lim_{k\rightarrow \infty}{a^{(j)}_{\floor{ck}}}/{a_{k}}=a^{(j)}/a c^\upalpha$. Similarly, it is possible to show $\lim_{k\rightarrow \infty}{a^{(j)}_{\ceil{ck}}}/{a_{k}}=a^{(j)}/(a c^\upalpha)$. In the notation of Lemma \ref{lem:devil}: $\uprho (j,q(j)-\upepsilon)=a^{(j)}/[a (q(j)-\upepsilon)^\upalpha]$ for small $\upepsilon>0$ and $\uprho (j,q(j)+\upepsilon)=a^{(j)}/[a (q(j)+\upepsilon)^\upalpha]$. Then, all the conditions of Lemma \ref{lem:devil} are satisfied with $0<\uprho (j,q(j))=a^{(j)}/(aq(j)^\upalpha)<\infty$.

Lemma \ref{lem:devil} gave conditions for the convergence w.p.1 of $\tilde{a}_k^{(j)}/a_k$. It is also of interest to derive conditions for the convergence of $E[\tilde{a}_k^{(j)}/a_k]$ (condition A0). For this we first define the concept of uniform integrability.

\begin{definition}
\label{def:unifintegrable}
[Chung 2001\nocite{chung2001}]
Given a sequence $\mathcal{X}_k$ of random variables, the set $\{\mathcal{X}_k\}_{k\geq0}$ is said to be {\it{uniformly integrable}} if and only if:
\begin{align*}
\lim_{n\rightarrow \infty}\int_{|\mathcal{X}_k|> n}|\mathcal{X}_k|\ dP=0{\text{ uniformly in $k$.}}
\end{align*}
\end{definition}

%The following lemma uses the notion of uniform integrability to provide sufficient conditions for the convergence of $E[\tilde{a}_k^{(j)}/a_k]$.

\begin{lemma}
\label{lem:lemmylime}
Assume $a_k^{(j)}>0$ and $a_k>0$ are both strictly monotonically decreasing sequences and that all the assumptions of Lemma \ref{lem:devil} hold. Furthermore, let $\upepsilon>0$ be such that $q(j)-\upepsilon>0$ and assume $e^{-2\upepsilon^2k}/a_k\rightarrow 0$ as $k\rightarrow \infty$ (this last assumption holds when $a_k$ satisfies condition A0). Then, $E[\tilde{a}_k^{(j)}/a_k]\rightarrow \uprho (j,q(j))$.
\end{lemma}
\begin{proof}
%
For each $j=1,\dots, d$ we will show that the set $\{\tilde{a}_k^{(j)}/a_k\}_{k\geq 0}$ is uniformly integrable. Then, the result will follow from  Lemma \ref{lem:devil} along with Theorem 4.5.4 in Chung (2001)\nocite{chung2001}, which states that $E[\tilde{a}_k^{(j)}/a_k]\rightarrow \uprho (j,q(j))$ if the set $\{\tilde{a}_k^{(j)}/a_k\}_{k\geq 0}$ is uniformly integrable and $\tilde{a}_k^{(j)}/a_k\rightarrow \uprho (j,q(j))$ w.p.1.

For each $j$ define $\mathcal{X}_k^{(j)}\equiv\tilde{a}_k^{(j)}/a_k>0$ and $n_i\equiv a_0^{(j)}/a_i$. Then, $n_i\rightarrow \infty$ as $i\rightarrow \infty$. Furthermore, for each $i\geq 0$ and any probability measure $P$:
\begin{align}
\label{eq:anothgerway}
\int_{\mathcal{X}_k^{(j)}> n_i} \mathcal{X}_k^{(j)}\ dP\leq \sup_{k\geq 0}\left\{\int_{\mathcal{X}_k^{(j)}> n_i} \mathcal{X}_k^{(j)}\ dP\right\}.
\end{align}
Using the fact that $a_k$ and $a_k^{(j)}$ are both monotonically-decreasing sequences of strictly positive numbers, for each $k$ we have:
%can bound the integral on the right-hand side of (\ref{eq:anothgerway}) as follows:
\begin{align*}
\int_{\mathcal{X}_k^{(j)}> n_i} \mathcal{X}_k^{(j)}\ dP\leq P(\mathcal{X}_k^{(j)}> n_i)\frac{a_0^{(j)}}{a_k}.
\end{align*}
Combining this bound with (\ref{eq:anothgerway}):
\begin{align}
\int_{\mathcal{X}_k^{(j)}> n_i} \mathcal{X}_k^{(j)}\ dP&\leq  \sup_{k\geq 0}\left\{P(\mathcal{X}_k^{(j)}> n_i)\frac{a_0^{(j)}}{a_k}\right\}
%&=a_0^{(j)}\sup_{k\geq 0}\left\{\frac{P(\tilde{a}_k^{(j)}/a_k> a_0^{(j)}/a_i)}{a_k}\right\}\notag\\
%&=a_0^{(j)}\sup_{k\geq i}\left\{\frac{P(\tilde{a}_k^{(j)}/a_k> a_0^{(j)}/a_i)}{a_k}\right\}\notag\\
= a_0^{(j)}\sup_{k\geq i}\left\{\frac{P(\mathcal{X}_k^{(j)}> n_i)}{a_k}\right\}.
\label{eq:lepainabongout}
\end{align}
%To simplify the analysis of the asymptotic behavior of (\ref{eq:lepainabongout}), n
%
%Next we obtain an upper bound for $P(\mathcal{X}_k^{(j)}> n_i)$. 
%
Because $a_{\floor{k(q(j)-\upepsilon)}}^{(j)}/a_k\rightarrow \uprho (j,(q(j)-\upepsilon))$ (by assumption), for each $\updelta>0$ there exists an $N(\updelta)>0$ such that $a_{\floor{k(q(j)-\upepsilon)}}^{(j)}/a_k<\uprho (j,q(j)-\upepsilon)+\updelta$
% $|a_{\floor{k(q(j)-\upepsilon)}}^{(j)}/a_k-\uprho (j,q(j)-\upepsilon)|<\updelta$ for 
whenever $k\geq N(\updelta)$. 
% In particular, for $k\geq N(\updelta)$ we have $a_{\floor{k(q(j)-\upepsilon)}}^{(j)}/a_k<\uprho (j,q(j)-\upepsilon)+\updelta$.
  Let $M(\updelta)>0$ be such that $\uprho (j,q(j)-\upepsilon)+\updelta<a_0^{(j)}/a_i$ for $i\geq M(\updelta)$ ($M(\updelta)$ exists because $a_i$ is monotonically decreasing). Then, for $k\geq i\geq \max\{M(\updelta),N(\updelta)\}$:
\begin{align*}
%\label{eq:jackiebackie}
\frac{a_{\floor{k(q(j)-\upepsilon)}}^{(j)}}{a_k}<\uprho (j,q(j)-\upepsilon)+\updelta\leq \frac{a_0^{(j)}}{a_i}=n_i.
\end{align*}
%Since ${\tilde{a}_k^{(j)}}/{a_k}> {a_{\floor{k(q(j)-\upepsilon)}}^{(j)}}/{a_k}$, (\ref{eq:jackiebackie}) implies ${\tilde{a}_k^{(j)}}/{a_k}> {a_{\floor{k(q(j)-\upepsilon)}}^{(j)}}/{a_k}$ whenever ${\tilde{a}_k^{(j)}}/{a_k}> a_0^{(j)}/{a_i}$. 
We then have the following bound when $k\geq i\geq \max\{M(\updelta),N(\updelta)\}$: 
\begin{align}
\label{eq:hoeffdingsboundme}
P(\mathcal{X}_k^{(j)}> n_i)\leq P\left(\frac{\tilde{a}_k^{(j)}}{a_k}> \frac{a_{\floor{k(q(j)-\upepsilon)}}^{(j)}}{a_k}\right)=P(\tilde{a}_k^{(j)}> a^{(j)}_{\floor{k(q(j)-\upepsilon)}}).
\end{align}
The term $P(\tilde{a}_k^{(j)}> a^{(j)}_{\floor{k(q(j)-\upepsilon)}})$ can be computed exactly. We do this next.

From (\ref{eq:pianofortee}) we can see that $\tilde{a}_k^{(j)}$ will be strictly greater than $a^{(j)}_{\floor{k(q(j)-\upepsilon)}}$ if the sequence $\{a_k^{(j)}\}_{k\geq0}$ has been used strictly less than $\floor{k(q(j)-\upepsilon)}$ times by the time $\tilde{a}_k^{(j)}$ is computed (this is due to the strictly monotonically decreasing nature of $a_k^{(j)}$). 
The number of times $\{a_k^{(j)}\}_{k\geq0}$ has been used can be modeled using a Binomial random variable with ``success'' probability $q(j)$. Therefore,
% with $k$ trials and probability $q(j)$ of success during each trial:
\begin{align}
\label{eq:hoeffdingsboundmeNEXT}
P(\tilde{a}_k^{(j)}> a^{(j)}_{\floor{k(q(j)-\upepsilon)}})&=\sum_{i=0}^{\floor{k(q(j)-\upepsilon)}-1} {{k}\choose{i}}q(j)^i (1-q(j))^{k-i}.
%&\leq \sum_{i=0}^{\floor{k(q(j)-\upepsilon)}} {{k}\choose{i}}q(j)^i (1-q(j))^{k-i}.
\end{align}
 Since $\floor{k(q(j)-\upepsilon)}-1\leq k(q(j)-\upepsilon)$, Hoeffding's inequality (e.g., Hoeffding 1963\nocite{hoeffding}) allows us to further bound the probability in (\ref{eq:hoeffdingsboundmeNEXT}) as follows:
\begin{align}
\label{eq:elleguteleriz}
P(\tilde{a}_k^{(j)}> a^{(j)}_{\floor{k(q(j)-\upepsilon)}})\leq e^{-2\upepsilon^2k}.
\end{align}
Combining (\ref{eq:hoeffdingsboundme}) with (\ref{eq:elleguteleriz}) yields $P(\mathcal{X}_k^{(j)}> n_i)\leq e^{-2\upepsilon^2k}$ for  $i\geq \max\{M(\updelta),N(\updelta)\}$ and $k\geq i$. Combining this bound with (\ref{eq:lepainabongout}) yields (for large values of $i$ and $k$):
\begin{align*}
\int_{\mathcal{X}_k^{(j)}> n_i} \mathcal{X}_k^{(j)}\ dP&\leq  a_0^{(j)}\sup_{k\geq i}\left\{\frac{e^{-2\upepsilon^2k}}{a_k}\right\}.
\end{align*}
Since $e^{-2\upepsilon^2k}/a_k\rightarrow 0$ (by assumption), we know that $\sup_{k\geq i}\{{e^{-2\upepsilon^2k}}/{a_k}\}\rightarrow 0$ as $i\rightarrow \infty$. Therefore, the set $\{\mathcal{X}_k\}_{k\geq 0}$ is uniformly integrable and Theorem 4.5.4 in (Chung 2001) implies $E[\tilde{a}_k^{(j)}/a_k]\rightarrow \uprho (j,q(j))$ as desired.
\end{proof}

% ********
%Next, assume $q_{k,m}(j)=q_{}(j)$ does not depend on $k$ or $m$, that $n_k(m)$ are i.i.d. over $m$ and independent of $s_k$,that $E[s_k]\rightarrow s$ and that $E[n_k(m)]\rightarrow n$. 

%%%%%%%%%%%%%%%%%%%%%%

The following corollary gives sufficient conditions for the iterates of Algorithm \ref{beastwasdone} to converge w.p.1 to $\bm\uptheta^\ast$, that is for $\hat{\bm{\uptheta}}_k\rightarrow \bm\uptheta^\ast$ w.p.1.


 
\begin{corollary}
\label{thm:hoeshoo49488} 
Let ${\bm{\bm{{\hat{\uptheta}}}}}_{k}$ be defined by according to Algorithm \ref{beastwasdone} and assume the following conditions hold:
\begin{DESCRIPTION}
\item[A0$'$] Let $a_{k}>0$, $a_k^{(j)}>0$, $ \sum_{k=0}^{\infty}a_{k}=\infty$ and $ \sum_{k=0}^{\infty}a_{k}^2<\infty$. Additionally, assume the conditions of Lemmas {\ref{lem:devil}} and \ref{lem:lemmylime} hold with $0<\uprho (j,q(j))<\infty$.
%\item[A2$'$]  Assume the sequences values ${a_k^{(j)}}$ and ${a_k}$ are chosen independently of $\mathcal{F}_k$.
%\item[A2$'$] The same as A2.
%\item[A4$'$] The same as A4.
%\item[A5$'$] The same as A5.
\item[A4$'$] For $k\geq0$, let there exist a set $\Omega_1\subset\Omega$ with $P(\Omega_1)=1$ and a scalar $0<R_1(\upomega)<\infty$ such that the set $\{\hat{\bm\uptheta}_k\}_{k\geq 0}$ is contained within a $p$-dimensional ball of radius $R_1(\upomega)$ centered at the origin for all $\upomega\in\Omega_1$.
\item[A5$'$] For $k\geq0$, let there exist a set $\Omega_2\subset\Omega$ with $P(\Omega_2)=1$ and a scalar $0<R_2(\upomega)<\infty$ such that the set $\{\bm\upbeta_k^{(j_k)}(\hat{\bm\uptheta}_k)\}_{k}$ is contained within a $p$-dimensional ball of radius $R_2(\upomega)$ centered at the origin for all $\upomega\in\Omega_2$.
%The set $\left\{\bm\upbeta\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right\}_{k, m, i}$ where $k\geq 0$, $m\leq s_k$ and $i\leq n_k(m)$ is bounded w.p.1. 
Furthermore, let $\bm\upbeta_k^{(j_k)}(\hat{\bm\uptheta}_k)\rightarrow {\bm{0}}$ w.p.1.
%
%The set $\left\{\bm\upbeta^{(j_k)}(\hat{\bm\uptheta}_k)\right\}_{k\geq0}$ is bounded w.p.1. Furthermore, $\bm\upbeta^{(j_k)}(\hat{\bm\uptheta}_k)\rightarrow {\bm{0}}$ w.p.1 as $k\rightarrow \infty$.
\item[A6$'$] $\bm{D}_r\equiv \left(\frac{\tilde{a}_r^{(j_r)}}{a_r}\right)\bm\upxi_r^{(j_r)}(\hat{\bm\uptheta}_r)$
%\begin{align*}
%\bm{Y}_r\equiv \left(\frac{\tilde{a}_r^{(j_r)}}{a_r}\right)\bm\upxi^{(j_r)}(\hat{\bm\uptheta}_r)
%\end{align*}
and $\lim_{k\rightarrow \infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}\bm{D}_{r}\Big\|\geq \upvarepsilon\right)=0$ for $\upvarepsilon>0$.
% there exists a $T>0$ such that:
%\begin{align*}
% \lim_{k\rightarrow \infty}P\left(\sup_{m\geq k}\Big\|\sum_{i=k}^{m}a_{r}\bm{Y}_{r}\Big\|\geq \upvarepsilon\right)=0.
%\end{align*}
\item [A7$'$] Let $\bm{\uptheta^{\ast}}$ be a locally asymptotically stable (in the sense of Lyapunov) solution of the differential equation:
\begin{align}
\label{eq:ode333}
\dot{\bm{Z}}(t)=- \sum_{j=1}^dq(j)\uprho (j,q(j))\bm{g}^{(j)}(\bm{Z}(t))=-\bm{\Lambda}\bm{g}(\bm{Z}(t)),
\end{align}
where $\bm\Lambda$ is a diagonal matrix with $i$th diagonal entry $\Lambda_{ii}=q(j)\uprho (j,q(j))$ where $j$ is such that $i\in \mathcal{S}_j$. Let (\ref{eq:ode333}) have domain of attraction $DA(\bm{\uptheta^{\ast}})$. 
\item[A3$'$ and A8$'$] The same as A3 and A8, respectively.
%\item[A8$'$] The same as A8.
\end{DESCRIPTION}
 Then, ${\bm{\bm{{\hat{\uptheta}}}}}_{k}\rightarrow {\bm\uptheta^{\ast}}$ w.p.1.
\end{corollary}


\begin{proof}
 We will show that conditions A0$'$ and A3$'$--A8$'$ imply A0--A8, the result will then follow from Theorem \ref{thm:hoeshoo}. First, note that A0$'$ along with the results from Lemmas {\ref{lem:devil}} and \ref{lem:lemmylime} imply that A0 holds with $r_j=\uprho (j,q(j))$. Additionally, condition A1 is satisfied because $s_k=1$ and $n_k(m)=1$. Next we show that condition A2 is satisfied. First, note that $x_k(j)=\chi\{j_k=j\}(\tilde{a}_k^{(j)}/a_k)$. Therefore, $\upmu_k(j)=E[\chi\{j_k=j\}(\tilde{a}_k^{(j)}/a_k)]$. However, because $\chi\{j_k=j\}$ and $\tilde{a}_k^{(j)}$ are independent in Algorithm \ref{beastwasdone}, $\upmu_k(j)=q(j)E[\tilde{a}_k^{(j)}/a_k]$
%\begin{align*}
%\upmu_k(j)=E[\mathcal{X}\{j_k=j\}(\tilde{a}_k^{(j)}/a_k)]=q(j)E[\tilde{a}_k^{(j)}/a_k]
%\end{align*}
so that $\lim_{k\rightarrow \infty} \upmu_k(j)= q(j)\uprho (j,q(j))$. Then, the first part of A2 holds with $\upmu(j)=q(j)\uprho (j,q(j))$. Next, for Algorithm \ref{beastwasdone} we have $S_r=\sum_{j=1}^dE[\tilde{a}_r^{(j)}/a_r](\chi\{j_r=j\}-q(j))$. Therefore, by the independence of the variables $\{j_k\}_{k\geq 0}$, we see that the rest of condition A2 holds. Since A3$'$--A8$'$ are simply versions of A3--A8 rewritten in terms of the notation of Algorithm \ref{beastwasdone}, it follows that conditions A3--A8 are automatically satisfied. Therefore, the conclusion of Theorem \ref{thm:hoeshoo} holds.
\end{proof}



  Another special case of the GCSA algorithm pertains to the case where $\hat{\bm{\uptheta}}_k$ is updated via a deterministic subvector update pattern. This is described in Algorithm \ref{kirkey}. The basic idea is that the number of updates made during an iteration is a constant, $s$, and the $m$th block consists of $n(m)$ updates to subvector $j(m)$. In Algorithm \ref{kirkey} the variables $s$, $n(m)$, and $j(m)$ are deterministic (cyclic seesaw is a special case). The following corollary gives conditions for the convergence of the iterates of Algorithm \ref{kirkey}.
%  Here, $s_k=s$ does not depend on $k$ and $j(m)$ and $n(m)$ are deterministic functions of $m=1,\dots,s$.
 \begin{algorithm}[!t]                     
\caption{Deterministic Pattern for Coordinate Selection}      
\label{kirkey}                
\begin{algorithmic} [1]                  % enter the algorithmic environment
\setstretch{1.5} 
\REQUIRE    $\hat{\bm{\uptheta}}_0$, $\{a_k^{(j)}\}_{k\geq 0}$ for $j=1,\dots,d$, and let $\mathcal{S}_1,\dots, \mathcal{S}_d$ be such that (\ref{eq:scurry}) holds. Set $k=0$.
%\STATE{Set $k=0$}.
\WHILE{stopping criterion has not been reached}
         \STATE{Let $s\in \mathbb{Z}^+$ be a finite integer-valued constant.}\label{line:brothermove}
         \FOR{$m=1,\dots,s$}
         \STATE{Let $j(m)\in\{1,\dots,d\}$ and let $n(m)\in \mathbb{Z}^+$ be a finite integer.}
%         \STATE{Let $n(m)\in \mathbb{Z}^+$ be a finite integer.}
%         \label{eq:line5}
%	\STATE{Define $ \hat{\bm{\uptheta}}_k^{(1,0)}\equiv \hat{\bm{\uptheta}}_k$.}
	\FOR{$i=1,\dots,n(m)$}
	\STATE{Define:
	\begin{align*}
	\hat{\bm\uptheta}_k^{(I_{m,i})}\equiv&\ \hat{\bm\uptheta}_k- \sum_{z=1}^{m-1}\sum_{\ell=0}^{n(z)-1} \left[{a}_{k}^{(j(z))}\ \hat{\bm{g}}^{(j(z))}\left(\hat{\bm\uptheta}_k^{(I_{z,\ell})}\right)\right]-\sum_{\ell=0}^{i-1} \left[{a}_{k}^{(j(m))}\ \hat{\bm{g}}^{(j(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,\ell})}\right)\right]
	\end{align*}
	}
%	where $\tilde{a}_k^{(j)}$ is the first unused element of a sequence $\{a_k^{(j)}\}_{k\geq0}$.}
	\ENDFOR
	 \ENDFOR
	 \STATE{Let $\hat{\bm{\uptheta}}_{k+1}\equiv\hat{\bm{\uptheta}}_k^{(I_{m,i})}$ {\text{ with $m=s$ and $i=n(s)$}}.
	 }
	\STATE{set $k=k+1$}
\ENDWHILE
\end{algorithmic}
\end{algorithm}



\begin{corollary}
\label{thm:hoeshooHarry} 
Let ${\bm{\bm{{\hat{\uptheta}}}}}_{k}$ be defined as in Algorithm \ref{kirkey}. Assume the following hold:
\begin{DESCRIPTION}
\item[A0$''$] Let $a_{k}>0$, $a_k^{(j)}>0$, $ \sum_{k=0}^{\infty}a_{k}=\infty$ and $ \sum_{k=0}^{\infty}a_{k}^2<\infty$. Additionally, assume ${a}_k^{(j)}/a_k\rightarrow r_j$ with $0<r_j<\infty$.
%
\item[A4$''$] For $k\geq0$, $m\leq s$ ($s$ is defined in Line \ref{line:brothermove} of Algorithm \ref{kirkey}), $i\leq n(m)$, let there exist a set $\Omega_1\in\Omega$ with $P(\Omega_1)=1$ and a scalar $0<R_1(\upomega)<\infty$ such that the set $\{\hat{\bm\uptheta}_k^{(I_{m,i})}\}_{k,m,i}$ is contained within a $p$-dimensional ball of radius $R_1(\upomega)$ centered at the origin for all $\upomega\in\Omega_1$.
\item[A5$''$] For $k\geq0$, $m\leq s$, $i\leq n(m)$, let there exist a set $\Omega_2\in\Omega$ with $P(\Omega_2)=1$ and a scalar $0<R_2(\upomega)<\infty$ such that the set $\{\bm\upbeta_k^{(j(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})\}_{k,m,i}$ is contained within a $p$-dimensional ball of radius $R_2(\upomega)$ centered at the origin for all $\upomega\in\Omega_2$.
%The set $\left\{\bm\upbeta\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right\}_{k, m, i}$ where $k\geq 0$, $m\leq s_k$ and $i\leq n_k(m)$ is bounded w.p.1. 
Furthermore, let $\bm\upbeta_k^{(j(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})\rightarrow {\bm{0}}$ w.p.1 uniformly in $m$ and $i$.
\item[A6$''$] Define $\bm{D}_r\equiv \sum_{m=1}^{s}\sum_{i=0}^{n(m)-1} \left(\frac{{a}_{r}^{(j(m))} }{a_{r}}\right)\bm\upxi^{(j(m))}_r\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right)$.
%\begin{align*}
%\bm{Y}_r= \sum_{m=1}^{s}\sum_{i=0}^{n(m)-1} \left(\frac{{a}_{r}^{(j(m))} }{a_{r}}\right)\bm\upxi^{(j(m))}\left(\hat{\bm\uptheta}_r^{(I_{m,i})}\right)
%\end{align*}
Assume for all $\upvarepsilon>0$ we have $\lim_{k\rightarrow \infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}\bm{D}_{r}\Big\|\geq \upvarepsilon\right)=0$.
% there exists a $T>0$ such that:
%\begin{align*}
% \lim_{k\rightarrow \infty}P\left(\sup_{m\geq k}\Big\|\sum_{i=k}^{m}a_{r}\bm{Y}_{r}\Big\|\geq \upvarepsilon\right)=0.
%\end{align*}
\item [A7$''$] $\bm{\uptheta^{\ast}}$ is a locally asymptotically stable (in the sense of Lyapunov) solution of:
% the differential equation:
\begin{align}
\label{eq:leghearhere}
\dot{\bm{Z}}(t)=- \sum_{j=1}^d\left[r_j\sum_{m=1}^s\chi\{j(m)=j\}n(m)\right]\bm{g}^{(j)}(\bm{Z}(t))=-\bm\Lambda\bm{g}(\bm{Z}(t)),
\end{align}
%where:
%\begin{align*}
%\upmu(j)=r_j\sum_{m=1}^s\mathcal{X}\{j(m)=j\}n(m)
%\end{align*}
where the $i$th diagonal entry of $\bm\Lambda$ equals $\Lambda_{ii}=r_j\sum_{m=1}^s\chi\{j(m)=j\}n(m)$
%\begin{align*}
%\Lambda_{ii}=r_j\sum_{m=1}^s\mathcal{X}\{j(m)=j\}n(m)
%\end{align*}
\label{eq:professiedadadna}
where $j$ is such that $i\in \mathcal{S}_j$. Let (\ref{eq:leghearhere}) have domain of attraction $DA(\bm{\uptheta^{\ast}})$.
\item[A3$''$ and A8$''$] The same as A3 and A8, respectively.
%\item[A8$''$] The same as A8.
\end{DESCRIPTION}
 Then, ${\bm{\bm{{\hat{\uptheta}}}}}_{k}\rightarrow {\bm\uptheta^{\ast}}$ w.p.1.
\end{corollary}

\begin{proof}
 Because all gain sequences are deterministic (not random), condition A0$''$ implies A0. Additionally, since $s_k=s<\infty$ and since $n_k(m)=n(m)$ is a bounded deterministic function of $m$, then condition A1 is also satisfied. Next, note that for Algorithm {\ref{kirkey}}:
\begin{align*}
\upmu_k(j)=\left(\frac{{a}_{k}^{(j)} }{a_{k}}\right)\sum_{m=1}^{s}\chi\{j(m)=j\}n(m).
\end{align*}
Here, $\upmu_k(j)$ is a deterministic quantity since the subvector to update (and hence the indicator random variables in the previous equation) are deterministic functions of $m$. Since $a_k^{(j)}/a_k\rightarrow r_j$ then $\upmu(j)=r_j\sum_{m=1}^{s}\chi\{j(m)=j\}n(m)$. Thus, the first part of A2 holds. The second part of A2 holds since $S_r=0$ for all $r$. Because A3$''$--A8$''$ are versions of A3--A8 that have been rewritten in terms of Algorithm \ref{kirkey}, we have shown conditions A0--A8 are satisfied. 
%Therefore, the conclusion of Theorem \ref{thm:hoeshoo} holds and $\hat{\bm{\uptheta}}_k\rightarrow \bm\uptheta^\ast$ w.p.1.
\end{proof}


The following section discusses the validity of conditions A0--A8.

 \section[On the Convergence Conditions]{On the Convergence Conditions}
 \label{sec:discussconvergence}

Sections \ref{sec:12or15miles}--\ref{sec:specialitay} presented conditions for the convergence of the GCSA algorithm (conditions A0--A8).
% as well as for the convergence of two special cases of GCSA. 
 It is worthwhile to note that conditions A0--A8 closely resemble those in Kushner and Clark (1978) for the convergence of SA procedures. This is not surprising given that the proof of Theorem \ref{thm:hoeshoo} is based on principles similar to those in the proof of Theorem 2.3.1 in Kusher and Clark (1978) \nocite{kushnclark1978}. This section comments on the validity of A0--A8.
% and highlights the differences and similarities between A0--A8 and other conditions commonly imposed throughout the SA literature.
 
%  This section comments on the feasibility of conditions A0--A8 for the convergence of the GCSA iterates (see Theorem \ref{thm:hoeshoo}).
 
{\underline{\it{Condition A0}}}. Requiring $a_k>0$ and $a_k^{(j)}>0$ is a reasonable assumption when one has complete control over the specific form of the gain sequences (in the deterministic steepest descent algorithm, having the gain sequences be strictly positive guarantee that the update direction is in fact a descent direction). Furthermore, the requirement that $\sum_{k=0}^\infty a_k=\infty$ and $\sum a_k^2<\infty$ is easily satisfied by sequences of the form $a_k=a/(1+k+A)^\upalpha$ where $a>0$ and $A>0$ and where $0.5< \upalpha\leq 1$ (the non-convergence and square summability for series associated with $a_k$ is a long-standing requirement in SA). 
%
%Generally, SA algorithms require the use of decreasing gain sequences to counteract the effects of the noise in the gradient measurements. As we discuss next, the assumptions of condition A0 imply $a_k^{(j)}\rightarrow 0$ at an $O(a_k)$ rate.
%
% and $a_k^{(j)}=a^{(j)}/(1+k+A^{(j)})^\upalpha$ for some strictly positive constants $a$, $a^{(j)}$, $A$, $A^{(j)}$, and $0<\upalpha<1$. 
 %

Another assumptions in condition A0 is that the sequence $\tilde{a}_k^{(j)}/a_k$ converges in expectation and w.p.1 of to some finite, strictly positive constant. Because $\tilde{a}_k^{(j)}/a_k$ must converge (in a stochastic sense) to a non-zero constant for all $j$, all gain sequences must converge to zero at the same rate (in a stochastic sense). For Algorithm \ref{beastwasdone} (randomized subvector selection), Lemmas \ref{lem:devil} and \ref{lem:lemmylime} give conditions under which $\tilde{a}_j^{(j)}/a_k$ converges w.p.1 and in expectation to a finite constant. For Algorithm \ref{kirkey}, it suffices to have $a_k^{(j)}=a^{(j)}/(k+A^{(j)}+1)^\upalpha$ and $a_k=a/(k+1)^\upalpha$, where $a^{(j)}>0$, $a>0$, $A^{(j)}>0$, and $0<\upalpha\leq 1$ ($\upalpha$ must be the same for all $j$). It is important to note that the sequence $a_k$ is not used by the GCSA algorithm. Rather, $a_k$ serves only as a representation of the rate at which ${a}_k^{(j)}$ decreases. It is important to note that the requirement in condition A0 that $r_j$ be strictly positive is introduced only to guarantee that $\sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bm\uptheta)=\bm{0}$ only when $\bm{g}(\bm\uptheta)=\bm{0}$. This implies that the only way in which the ODE in (\ref{eq:ode}) is equal to zero is if $\bm{Z}(t)=\bm\uptheta^\ast$. Note that if the sets $\mathcal{S}_1,\dots,\mathcal{S}_d$ overlap, it is still possible that the only solution to $\sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bm\uptheta)=\bm{0}$ occurs at $\bm\uptheta=\bm\uptheta^\ast$ even when some of the $\upmu(j)$ are equal to zero (this occurs provided $\sum_{j=1}^d\upmu(j)\bm{g}^{(j)}(\bm\uptheta)=\bm\Lambda\bm{g}(\bm\uptheta)$ for some positive definite diagonal matrix $\bm\Lambda$). 


{\underline{\it{Conditions A1 and A2}}}. Condition A1 requires that the number of blocks within the $k$ iteration, $s_k$, and the number of updates within each block, $n_k(m)$, be uniformly bounded over $k$, $m$, and $\upomega$. A special case where A1 holds is when a hard bound is imposed on $s_k$ and $n_k(m)$, as in the case of Algorithms \ref{beastwasdone} and \ref{kirkey}. Additionally, both these algorithms were shown to satisfy condition A2, which imposes a restriction on how $s_j$ and $n_j(m)$ relate to $s_i$ and $n_i(m)$ for $i\neq j$.


\label{page:onconditionA4444}{\underline{\it{Conditions A3 and A4}}}. Despite the fact that the gradient of $L(\bm\uptheta)$ is not explicitly used by the GCSA algorithm, the convergence theory of Section \ref{sec:convo} requires the existence of $\bm{g}(\bm\uptheta)$ and its continuity, a fact which may be hard to verify. Condition A4 is also difficult to verify in practice. Here, it is assumed that the algorithm's iterates are bounded w.p.1 (see Figure \ref{fig:spheres}). While the boundedness of the iterates is a common assumption throughout the SA, it remains somewhat controversial 
%since it imposes a condition on the iterates themselves 
(e.g., Benveniste et al. 1990, p. 46)\nocite{benveniste1990}. 
Kushner and Clark (1978)\nocite{kushnclark1978}, however, mention that this boundedness is not necessarily a strong assumption since one typically imposes bounds on $\bm\uptheta$ in practice.
% Such bounds could be enforced by projecting the iterates onto a bounded region, effectively turning the optimization problem into a constrained stochastic optimization problem. 
 Projected versions of GCSA could be the subject of future work and, with this in mind, the following quote seems fitting: 
%
\begin{quote}
There is no general scheme for showing $P(Q) = 1$ [the iterates of a realization are bounded w.p.1]. There are, however, problem-specific techniques for special problem classes. . . . One way to escape the boundedness issue is to alter the algorithm by projecting the iterates back onto a prescribed, large bounded set whenever they exit from the same. The trade-off is that the limiting ODE becomes more complicated. It is now confined to the said set and thus involves a ``reflection at the boundary'' of the same in an appropriate sense. (Borkar 1998\nocite{borkar1998}, on an asynchronous SA algorithm related to GCSA).
\end{quote}
\label{page:quotepage}

\begin{figure}[!t]
\centering
 \raisebox{1em}{\begin{tikzpicture}

\definecolor{mynewcoloring}{RGB}{102, 128, 153}
 \definecolor{mygreen}{RGB}{80, 135, 96}

\def\R{2.5} % sphere radius
\def\angEl{15} % elevation angle

\foreach \t in {0} { \DrawBackLatitudeCircle[\R]{\t} }
%\foreach \t in {-60} { \DrawBackLongitudeCircle[\R]{\t} }%

%\DrawLatPlane[\R]{-20}%

\coordinate (a) at (0,1.5);
\coordinate (b) at (1,-1,1);
\coordinate (c) at (-0.9,-1.5,1);
\coordinate (d) at (-1.4,1.7,0);

\coordinate (O) at (0,0);
\coordinate (r1) at (-3.25,0,0);
\coordinate (r2) at (-4.25,0,0);

\draw[->,ultra thick] (r2)--(r1);
\node at (-4.35,0,0)[left] {Ball of radius $R_1(\upomega)$};
\draw[help lines] (O)--(a);
\draw[help lines] (O)--(b);
\draw[help lines] (O)--(c);
\draw[help lines] (O)--(d);

\fill[black] (a) circle[radius=2pt] node[right] {\ $\hat{\bm{\uptheta}}_{4}$};
\fill[black] (b) circle[radius=2pt] node[right] {\ $\hat{\bm{\uptheta}}_{10}$};
\fill[black] (c) circle[radius=2pt] node[right] {\ $\hat{\bm{\uptheta}}_{8}^{(I_{4,3})}$};
\fill[black] (d) circle[radius=2pt] node[right] {\ $\hat{\bm{\uptheta}}_{5}^{(I_{1,5})}$};
\fill[black] (O) circle[radius=2pt] node[right] {\ Origin};



\foreach \t in {0} { \DrawFrontLatitudeCircle[\R]{\t} }
%\foreach \t in {-60} { \DrawFrontLongitudeCircle[\R]{\t} }

\draw[ultra thick] (0,0) circle (\R);
\end{tikzpicture}}
\caption[Condition A4 on the boundedness of the iterates]{Condition A4 states that the iterates produced by a single realization of GCSA must be contained within a ball of radius $R_1(\upomega)<\infty$ for $\upomega\in \Omega_1$}
\label{fig:spheres}
\end{figure}



{\underline{\it{Condition A5}}}. 
%This condition requires  $\{\bm\upbeta_{k}^{(j(m))}(\hat{\bm{\uptheta}}_k^{(I_{m,i})})\}_{k,m,i}$ to be bounded w.p.1 and that the bias terms $\bm\upbeta_k^{(j_k(m))}(\hat{\bm\uptheta}_k^{(I_{m,i})})$ converge to ${\bm{0}}$ w.p.1 uniformly in $m$ and $i$. 
When the GCSA update directions are obtained using SG-type measurements, all bias terms are identically zero and condition A5 would automatically be satisfied. For the cyclic seesaw SPSA algorithm, Spall (1992)\nocite{spall1992} gives conditions under which the bias term is bounded (w.p.1) and converges to zero. In a manner analogous to Lemma 1 in Spall (1992)\nocite{spall1992} and under similar conditions (after a natural adaptation for the cyclic setting) it can be shown that the bias terms of the GCSA algorithm satisfy  A5.


{\underline{\it{Condition A6}}}. This condition restricts the relationship between $a_k$ and $\bm{D}_k$, a vector which represents the ``total noise'' of the $(k+1)$st iteration of GCSA (see the statement of condition A6 for a the precise definition of $\bm{D}_k$). Let us give an example of when condition A6 holds. Assume that for each $k\geq0$ the sequence  $\{\sum_{r=k}^m a_r \bm{D}_r\}_{m\geq k}$ (indexed by $m$) is a martingale sequence, that $E\|\bm{D}_k\|^2<\infty$, and that $E[\bm{D}_i^\top\bm{D}_j]=0$ for $i\neq j$. Then, by a relation on p. 315 in Doob (1953)\nocite{doob1953} we obtain the following inequality:
\begin{align}
\lim_{k\rightarrow\infty}P\left(\sup_{m\geq k}\Big\|\sum_{r=k}^{m}a_{r}\bm{D}_{r}\Big\|\geq \upvarepsilon\right)&\leq\lim_{k\rightarrow\infty}\upvarepsilon^{-2}\sum_{r=k}^\infty a_{r}^{2}E\|\bm{D}_{r}\|^2.\label{eq:ranch}
\end{align}
If in addition  we assume $\sum_{k=1}^\infty a_k^2<\infty$ and $E\|\bm{D}_{k}\|^2<\upsigma^2$ for some finite $\upsigma^2>0$, then the limit of the upper bound in (\ref{eq:ranch}) is equal to zero and A6 holds. Requiring the noise term to have a bounded variance could be a reasonable assumption when the update directions are obtained using SG-based gradient measurements. However, it is not always reasonable to assume the noise has bounded variance. For example, for the SPSA algorithm (which is a special case of GCSA) it is often the case that the variance of $\bm{D}_k$ grows at a rate proportional to $1/c_k^2$ (recall $c_k\rightarrow 0$). Therefore, in order for the limit in the upper bound of (\ref{eq:ranch}) to be zero, it would be necessary to have $a_k$ and $c_k$ satisfy $\sum_{k=1}^\infty a_k^2/c_k^2<\infty$ (see, for example, Spall 2003, p. 183)\nocite{ISSO}\label{page:anotherpagereffs}. 
%In general, there needs to be a delicate balance between $a_k$, $a_k^{(j)}$, and $\bm{Y}_k$, in order for the GCSA algorithm's iterates to converge w.p.1.
%\begin{align*}
%\lim_{k\rightarrow\infty}P\left(\sup_{m\geq k}\Big\|\sum_{i=k}^{m}a_{i}^{(j)}\bm{\upxi}_{i}^{(j)}\Big\|\geq \upvarepsilon\right)&\leq \lim_{k\rightarrow\infty}\frac{\upsigma^2p}{\upvarepsilon^{2}}\sum_{i=k}^\infty(a_{i}^{(j)})^{2}
%\end{align*}
%it is clear that the limit in (\ref{eq:ranch}) is zero by the Cauchy criterion for convergence (Rudin, 1976, Theorem 3.11).

{\underline{\it{Conditions A7 and A8}}}. Since the premise of stochastic optimization is that the function $L(\bm\uptheta)$ and its gradient are unknown, conditions A7 and A8 are likely to be impossible to verify in practice. Nevertheless, it is impractical to attempt to derive convergence conditions for an optimization algorithm without imposing restrictions on the properties of the function to minimize. Informally, conditions A7 and A8 force $\hat{\bm{\uptheta}}_k$ be inside the domain of attraction of $\bm\uptheta^\ast$ with enough frequency (for infinitely many $k$) that the iterates begin to benefit from the asymptotic stability of $\bm\uptheta^\ast$, which results in $\hat{\bm{\uptheta}}_k\rightarrow \bm\uptheta^\ast$ w.p.1. A few observations regarding the ODE in condition A7 are given next.

Understanding the ODE in (\ref{eq:ode}) requires understanding the terms $\upmu(j)$ (defined on p. \pageref{eq:tinkelpan}). When ${\tilde{a}_{k}^{(j)}}/{a_{k}}$ is independent of $s_k$, $n_k(m)$, and $j_k(m)$ (a valid assumption for Algorithms \ref{beastwasdone} and \ref{kirkey}),
%\begin{align*}
%\upmu_k(j)=&\ \left(\frac{\tilde{a}_{k}^{(j)} }{a_{k}}\right) \times [\text{\# times entries $S_j$ are updated during iteration $k+1$}].
%\end{align*}
%Therefore, then the 
$\upmu(j)$ can be rewritten as:
\begin{align*}
\upmu(j)=&\ r_j \times [\text{asymptotic average \# times entries $\mathcal{S}_j$ are updated per-iteration}].
\end{align*}
By construction, $\upmu(j)>0$ for all $j$. Thus, there exists a diagonal matrix $\bm\Lambda$ with strictly positive diagonal entries (determined by the $\upmu(j)$) such that:
\begin{align}
\label{eq:goodnewspillsconpaint}
\dot{\bm{Z}}(t)=- \bm\Lambda\bm{g}(\bm{Z}(t))
\end{align} 
(see p. \pageref{eq:ode333} and p. \pageref{eq:professiedadadna} for two special cases of $\bm\Lambda$). The ODE in (\ref{eq:goodnewspillsconpaint}) is a slight variation of the ODE that arises in the standard SA algorithm from (\ref{eq:formof}), where $\bm\Lambda=\bm{I}$ (see, for example, Spall 2003, Chapter 7)\nocite{ISSO}. 

%On the other hand, (\ref{eq:goodnewspillsconpaint}) is in fact quite similar to the ODE that arises when studying several adaptive SA algorithms (Benveniste et al. 2012, Section 3.2). 

At this point one might wonder whether $\bm\uptheta^\ast$, a minimizer of $L(\bm\uptheta)$, is necessarily a stable solution to (\ref{eq:goodnewspillsconpaint}). The answer, unfortunately, is no. While $\bm{Z}(t)=\bm\uptheta^\ast$ is certainly an {\it{equilibrium}} point of (\ref{eq:goodnewspillsconpaint}) (and hence a solution to (\ref{eq:goodnewspillsconpaint})), it is entirely possible for $\bm{Z}(t)=\bm\uptheta^\ast$ not to be a {\it{stable}} equilibrium point of (\ref{eq:goodnewspillsconpaint}) even when $L(\bm\uptheta)$ is differentiable for all degrees of differentiation) and $\bm\Lambda=\bm{I}$ (e.g., Absil and Kurdyka 2006, Proposition 2)\nocite{ansilandkurd2006}. Thus, condition A7 is not automatically satisfied when $\bm\uptheta^\ast$ is a minimizer of $L(\bm\uptheta)$. We will note, however, that if $\bm\uptheta^\ast$ is a Lyapunov stable solution to $\dot{\bm{Z}}(t)=-\bm{g}(\bm{Z}(t))$, if the entries of $\bm\Lambda$ have finite magnitudes, and if the smallest eigenvalue of $\bm\Lambda$ is strictly positive (more generally, if the smallest real part of an eigenvalue is strictly positive), then $\bm\uptheta^\ast$ is also a Lyapunov stable solution to (\ref{eq:goodnewspillsconpaint}) (e.g., Benveniste et al. 1990, pp. 111--112)\nocite{benveniste1990}. Therefore, asking for $\bm\uptheta^\ast$ to be a stable solution of (\ref{eq:goodnewspillsconpaint}) is not a stronger condition than the corresponding stability assumption when $\bm\Lambda=\bm{I}$.

% The results of this chapter are concerned with showing convergence w.p.1 of the GCSA iterates to a zero of $\bm{g}(\bm\uptheta)$. 
 
 In general, it is impossible to know whether there is a unique solution to $\bm{g}(\bm\uptheta)=\bm{0}$. However, if $\bm\uptheta^{\ast,1}$ and $\bm\uptheta^{\ast,2}$ denote two distinct zeros of the gradient, it is impossible for both vectors to satisfy A7 and A8. Therefore, the GCSA iterates will converge to whichever of $\bm\uptheta^{\ast,1}$ and $\bm\uptheta^{\ast,2}$ (if any) satisfies both A7 and A8. Based on the idea in  Kushner and Clark (1978, p.39)\nocite{kushnclark1978}, however, condition A8 could be relaxed to allow all zeros of the gradient to be contained within some set that is stable (in the sense of Lyapunov), which would result in the GCSA algorithm's iterates converging to the aforementioned set w.p.1. This, however, would not guarantee convergence to a zero of $\bm{g}(\bm\uptheta)$.
% to allow ``cycling'' in the SA iterates. Essentially, the authors suggest generalizing the stability condition



\section{Concluding Remarks}
\label{sec:concremarksconvergence}

 This chapter gave a theorem for the convergence of the GCSA algorithm (Theorem \ref{thm:hoeshoo}) as well as two corollaries pertaining to special cases of GCSA (Corollaries \ref{thm:hoeshoo49488} and \ref{thm:hoeshooHarry}). The proof of Theorem \ref{thm:hoeshoo} is based on the proof of Theorem 2.3.1 in Kushner and Clark (1978)\nocite{kushnclark1978} which, in turn, is based on the ODE-based method for proving convergence of SA algorithms that was introduced by Ljung (1977)\nocite{ljung1977}. The time-dependent recursion in (\ref{eq:levelred}), which describes the evolution of the GCSA iterates, is similar to equation (2.3.3) in Kushner and Clark (1978)\nocite{kushnclark1978} although we point out that (\ref{eq:levelred}) is significantly more complex. As a result, some of the conditions of Theorem \ref{thm:hoeshoo} 
 % conditions A0--A8 
 resemble the conditions of Kushner and Clark's Theorem 2.3.1.\nocite{kushnclark1978}
 
 
 
 In contrast to this chapter's focus on convergence w.p.1 of the GCSA iterates, the following chapter focuses on the asymptotic normality of the normalized iterates from Algorithm \ref{kirkey}, a special case of GCSA in which the subvector to update is selected according to a deterministic pattern (see, for example, the algorithm specified by (\ref{eq:believeeyes0}--f), which is a special case of Algorithm \ref{kirkey}).









==> thesis arXiv 2/chapter3.tex <==
%!TEX root = root.tex

\chapter{Asymptotic Normality of GCSA}
\label{sec:ROC}
%\chaptermark{Rate of Convergence}

When applicable, asymptotic normality results can be used to construct approximate confidence regions for the SA iterates, to compute the relative efficiency between two SA algorithms by comparing their asymptotic mean squared errors (e.g., Spall 1992)\nocite{spall1992}, or even to define the rate of convergence of the vector-valued random sequence $\hat{\bm{\uptheta}}_k$.
%to simply serve as a performance guarantee.
% Additionally, because the sequence $\hat{\bm{\uptheta}}_k$ of SA iterates is a vector-valued random variable, 
Fabian (1968)\nocite{fabian1968}, a seminal paper in the SA literature, provides conditions for the asymptotic normality of the iterates of SA algorithms (after an appropriate centering and scaling). Fabian's theorem (Fabian 1968, Theorem 2.2)\nocite{fabian1968}, gives conditions under which there exists a constant $\upbeta>0$ such that $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$ has a limiting multivariate normal distribution with a theoretically computable mean and covariance. 
%Indeed, obtaining a result on asymptotic normality has practical and theoretical applications.
 One of the assumptions from Fabian's theorem, however, 
% makes an critical assumption 
 is too strong for the GCSA algorithm. Specifically, Fabian (1968, Assumption 2.2.1)\nocite{fabian1968} requires a matrix that affects the mean and covariance matrix in the limiting distribution of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$ to be symmetric. Section \ref{sec:genfabiangenfabian} generalizes Fabian's result by relaxing the symmetry assumption of the aforementioned matrix. The resulting generalization 
% 
%  This chapter provides a generalization of Fabian's theorem which relaxes the symmetry assumption of a matrix that affects the mean and covariance matrix in the limiting distribution of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$. Our generalization 
%  
  expands the theorem's applicability to include a broader range of SA algorithms of practical interest (see Appendix \ref{sec:fabiansecgeneralize}) including a special case of GCSA.


The remainder of this chapter is organized as follows. First, Section \ref{sec:reviewfabian} reviews Fabian's theorem and its connection to SA algorithms. Then, Section \ref{subsec:primadonna} explains the nature of the incompatibility between Fabian's theorem and the GCSA algorithm. Section \ref{sec:genfabiangenfabian} provides a generalization of Fabian's theorem which is used in Section \ref{sec:upperpotomacshell} to derive an asymptotic normality result for a special case of GCSA. Section \ref{sec:bonestrailseason} comments on the validity of the assumptions in Section \ref{sec:upperpotomacshell}. Lastly, Section \ref{sec:dontmeanthings} contains concluding remarks.


%\section[Mode and Rate of Convergence for Random Sequences]{Mode and Rate of Convergence\\ for Random Sequences}
%\label{sec:probability}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Their rate of convergence, on the other hand, will be related to the convergence in distribution of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$ for some constant $\upbeta>0$, this constant is not to be confused with $\bm\upbeta_k(\hat{\bm{\uptheta}}_k)$. 



\section[Reviewing Fabian's Theorem]{Reviewing Fabian's Theorem}
\label{sec:reviewfabian}

%Fabian (1968) provided an asymptotic normality result with application to SA algorithms for nonlinear root-finding. 
This section briefly reviews Fabian's result on asymptotic normality.
% and clarifies the nature of its connection to SA procedures.

% We also illustrate why Fabian's result needs to be generalized in order to be applicable to cyclic stochastic optimization. Fabian's asymptotic normality result is the following theorem.

\begin{theorem}
[Fabian 1968, Theorem 2.2 or ``Fabian's Theorem''\nocite{fabian1968}]
\label{thm:fabian}
%All probabilistic arguments are meant to hold w.p.1 unless stated otherwise.
 For $k\geq 1$, let $\bm{V}_k$, $\bm{W}_k$, $\bm{T}_k$, and $\bm{T}$ be vectors in $\mathbb{R}^p$, and let $\bm\Gamma_k$, $\bm\Phi_k$, $\bm\Sigma$, $\bm\Gamma$, $\bm\Phi$, and $\bm{P}$ be matrices in $\mathbb{R}^{p\times p}$. Let $\bm{W}_k$ satisfy the recursion: 
\begin{align}
\label{eq:alien}
\bm{W}_{k+1}=(\bm{I}-k^{-\upalpha}\bm\Gamma_k)\bm{W}_k+\frac{\bm{T}_k}{k^{\upalpha+\upbeta/2}}+\frac{\bm\Phi_k\bm{V}_k}{k^{(\upalpha+\upbeta)/2}}.
%\bm{U}_{k+1}=(\bm{I}-k^{-\upalpha}\bm\Gamma_k)\bm{U}_k+k^{-\upalpha-\upbeta/2}\bm{T}_k+k^{-(\upalpha+\upbeta)/2}\bm\Phi_k\bm{W}_k.
\end{align}
Additionally, let $\mathcal{F}_k$ be a non-decreasing sequence of $\upsigma$-fields and assume there exists a set $\mathcal{S}$ such that $\mathcal{F}_k\subset \mathcal{S}$ for all $k$. Assume the following conditions hold:
%\begin{align*}
%&{\text{$\bm{U}_k$, $\bm{V}_k$, $\bm{T}_k$, and $\bm{T}$ be vectors in $\mathbb{R}^p$,}}\\
%&{\text{$\bm\Gamma_k$, $\bm\Phi_k$, $\bm\Sigma$, $\bm\Gamma$, $\bm\Phi$, and $\bm{P}$ be matrices in $\mathbb{R}^{p\times p}$.}}
%\end{align*} 
\begin{DESCRIPTION}
\item[B0] $\bm\Gamma_k$, $\bm\Phi_{k-1}$, and $\bm{V}_{k-1}$ are $\mathcal{F}_k$-measurable. 
\item[B1]$\bm\Gamma_k\rightarrow\bm\Gamma$ w.p.1 where $\bm\Gamma=\bm{P}\bm\Lambda\bm{P}^\top$ for some real orthogonal matrix $\bm{P}$ and a diagonal matrix $\bm\Lambda$ with strictly positive eigenvalues (an important implication is that the matrix $\bm\Gamma$ must be symmetric).
%this implies $\bm\Gamma=\bm{P}\bm\Lambda\bm{P}^\top$ for an orthogonal matrix $\bm{P}$ and a diagonal matrix $\bm\Lambda$ with strictly positive eigenvalues.
\item[B2] $\bm\Phi_k\rightarrow \bm\Phi$ w.p.1.
\item[B3] Either $\bm{T}_k\rightarrow \bm{T}$ w.p.1 or $E\|\bm{T}_k-\bm{T}\|\rightarrow 0$.
\item[B4] $E[\bm{V}_k|\mathcal{F}_k]=\bm{0}$ and there exists $C$ such that $C>\|E[\bm{V}_k\bm{V}_k^\top|\mathcal{F}_k]-\bm\Sigma\|\rightarrow 0$.
%\begin{center}
%$\bm\Gamma_k\rightarrow\bm\Gamma$, $\bm\Phi_k\rightarrow \bm\Phi$, either $\bm{T}_k\rightarrow \bm{T}$ or $E\|\bm{T}_k-\bm{T}\|\rightarrow 0$, $E[\bm{W}_k|\mathcal{F}_k]=\bm{0}$,\\
% and there exists a constant $C$ such that $C>\|E[\bm{W}_k\bm{W}_k^\top|\mathcal{F}_k]-\bm\Sigma\|\rightarrow 0$.
%\end{center}
\item[B5] $\upsigma_{k,r}^2\equiv E\chi\{\|\bm{V}_k\|^2\geq rk^\upalpha\}\|\bm{V}_k\|^2$ (recall $\chi\{\mathcal{E}\}$ denotes the indicator function of the event $\mathcal{E}$). For every $r>0$ assume that one of the following holds:
%\begin{align*}
%\label{eq:foreveryr}
\begin{enumerate}[label=(\roman*)]
\item $\lim_{k\rightarrow \infty}\upsigma_{k,r}^2=0$.
\item $\upalpha=1$ and $\lim_{n\rightarrow \infty}n^{-1}\sum_{k=1}^n\upsigma^2_{k,r}=0$.
\end{enumerate}
%\end{align*}
\item[B6] Let $\uplambda\equiv \min_i{\{\Lambda_{ii}\}}$ where $\Lambda_{ii}$ is the $i$th diagonal entry of $\bm\Lambda$. Let $\upalpha$ and $\upbeta$ be constants such that $0<\upalpha\leq 1$ and $0\leq \upbeta$. Define $\upbeta_+\equiv\upbeta$ if $\upalpha=1$ and $\upbeta_+\equiv 0$ otherwise. Let $\upbeta_+<2\uplambda$.
\label{page:scratchless}
\end{DESCRIPTION}
%\begin{align*}
%\upbeta_+\equiv
%\begin{cases} \upbeta &\mbox{if } \upalpha=1,\\ 
%0 & \mbox{if } \upalpha\neq1,
%\end{cases} 
%\end{align*}
 Then, the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$ is a multivariate normal random variable with mean $(\bm\Gamma-(\upbeta_+/2)\bm{I})^{-1}\bm{T}$ and covariance matrix $\bm{PQP}^\top$, where the $(i,j)$th entry of $\bm{Q}$ is equal to $(\bm{P}^\top\bm{\Phi}\bm\Sigma\bm\Phi^\top\bm{P})_{ij}(\Lambda_{ii}+\Lambda_{jj}-\upbeta_+)^{-1}$ with $(\bm{P}^\top\bm{\Phi}\bm\Sigma\bm\Phi^\top\bm{P})_{ij}$ denoting the $(i,j)$th entry of the matrix $\bm{P}^\top\bm{\Phi}\bm\Sigma\bm\Phi^\top\bm{P}$.
\end{theorem}

Let us discuss the connection between Fabian's theorem (Theorem \ref{thm:fabian}) and stochastic optimization.
% is apparent through a rewriting of the standard SA update
%The connection between Theorem \ref{thm:fabian} and stochastic optimization is apparent through a rewriting of the standard SA update. We show this next.
 Consider a stochastic optimization algorithm that produces updates according to (\ref{eq:youknownothing}). Writing $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$ as in (\ref{eq:tennisey}) 
% yields:
%. Then,
%\begin{align}
%\label{eq:focus}
%\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\left({\bm{g}}(\hat{\bm{\uptheta}}_k)+{\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)\right).
%\end{align}
%L
and letting $\bm{W}_k= \hat{\bm{\uptheta}}_k-\bm\uptheta^\ast$, the algorithm in (\ref{eq:youknownothing}) can be rewritten as follows:
% and subtracting $\bm\uptheta^\ast$ from both sides of (\ref{eq:focus}):
\begin{align}
\label{eq:husseinbolt}
\bm{W}_{k+1}=\bm{W}_k-a_k\left({\bm{g}}(\hat{\bm{\uptheta}}_k)+{\bm{\upbeta}}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k(\hat{\bm{\uptheta}}_k)\right).
\end{align}
Asssume  $L(\bm\uptheta)$ is twice continuously differentiable and denote its Hessian matrix by
%, the recursion in (\ref{eq:husseinbolt}) can be written in the form of (\ref{eq:alien}). To see this, first let 
$\bm{H}(\bm\uptheta)$.
% denote the Hessian of $L(\bm\uptheta)$.
Then, using Taylor's theorem we may write $\bm{g}(\hat{\bm{\uptheta}}_k)=\tilde{\bm{H}}_k(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$,
%\begin{align}
%\label{eq:refeemee}
%\bm{g}(\hat{\bm{\uptheta}}_k)=\tilde{\bm{H}}_k(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast),
%\end{align}
where the $i$th row of $\tilde{\bm{H}}_k$ is equal to the $i$th row of $\bm{H}(\bm\uptheta)$ evaluated at $\bm\uptheta=(1-\uplambda_i)\hat{\bm{\uptheta}}_k+\uplambda_i\bm\uptheta^\ast$ for some $\uplambda_i\in[0,1]$ which depends on $\hat{\bm{\uptheta}}_k$.
% Because $\bm{g}(\bm\uptheta^\ast)=\bm{0}$, equation (\ref{eq:refeemee}) implies $\bm{g}(\hat{\bm{\uptheta}}_k)=\tilde{\bm{H}}_k(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$.
%If $L(\bm\uptheta)$ is twice continuously differentiable, then using Taylor's theorem we can write $\bm{g}(\bm\uptheta)=\bm{g}(\bm\uptheta^\ast)+\bm{H}(\overline{\bm\uptheta})(\bm\uptheta-\bm\uptheta^\ast)$ where $\bm{H}(\bm\uptheta)$ is the Hessian of $L(\bm\uptheta)$ and, informally, $\overline{\bm\uptheta}=(1-\ell)\bm\uptheta-\ell\bm\uptheta^\ast$ for some $\ell\in[0,1]$. (If we want to be more formal, each row of $\bm{H}(\overline{\bm\uptheta})$ will have a corresponding value of $\ell$.) 
By expanding $\bm{g}(\hat{\bm{\uptheta}}_k)$ around $\bm\uptheta^\ast$ in this way, we can rewrite (\ref{eq:husseinbolt}) in the following manner:\label{page:thispagehello}
\begin{align}
\bm{W}_{k+1}
%&=\bm{W}_k-a_k\left(\tilde{\bm{H}}_k\bm{W}_k+{\bm{\upbeta}}(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}(\hat{\bm{\uptheta}}_k)\right)\notag\\
&=\left(\bm{I}-k^{-\upalpha}k^{\upalpha}a_k\tilde{\bm{H}}_k\right)\bm{W}_k-\frac{k^{\upalpha+\upbeta/2}a_k\bm\upbeta_k(\hat{\bm{\uptheta}}_k)}{k^{\upalpha+\upbeta/2}}-\frac{k^{(\upalpha+\upbeta)/2}a_k\bm\upxi_k(\hat{\bm{\uptheta}}_k)}{k^{(\upalpha+\upbeta)/2}}.
\label{eq:crownuni}
\end{align}
%where $\overline{\bm\uptheta}_k=(1-\ell)\hat{\bm{\uptheta}}_k-\ell\bm\uptheta^\ast$ for some $\ell\in[0,1]$ (once again, recall we are committing an abuse of notation here). 
Letting $\bm\Gamma_k=k^{\upalpha}a_k\tilde{\bm{H}}_k$, $\bm\Phi_k=\bm{I}$, $\bm{T}_k=-k^{\upalpha+\upbeta/2}a_k\bm\upbeta_k(\hat{\bm{\uptheta}}_k)$, and $\bm{V}_k=-k^{(\upalpha+\upbeta)/2}a_k\bm\upxi_k(\hat{\bm{\uptheta}}_k)$,
%\begin{align}
%\label{eq:zoidberg}
%\bm\Gamma_k=k^{\upalpha}a_k\tilde{\bm{H}}_k,\ \bm\Phi_k=\bm{I},\ \bm{T}_k=k^{\upalpha+\upbeta/2}a_k\bm\upbeta(\hat{\bm{\uptheta}}_k),{\text{ and }} \bm{V}_k=k^{(\upalpha+\upbeta)/2}a_k\bm\upxi(\hat{\bm{\uptheta}}_k)
%\end{align}
it follows that (\ref{eq:crownuni}), and therefore (\ref{eq:youknownothing}), can be rewritten in the form of (\ref{eq:alien}). Consequently, Fabian's theorem can be used to derive conditions for the asymptotic normality of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$ when $\hat{\bm{\uptheta}}_k$ is obtained via the general SA recursion in  (\ref{eq:youknownothing}).
%The validity of B0--B6 has been explored throughout the literature for different SA algorithms (e.g., Spall 1992, Ruppert 1985, 
%

Undoubtedly, Fabian's theorem is already applicable to a variety of SA algorithms (see, for example, Zhou and Hu 2014,  Kar et al. 2013, Hu et al. 2012, and Zorin et al. 2000 to name a few recent applications). However, a critical assumption in Fabian's theorem is that $\bm\Gamma_k\rightarrow \bm\Gamma$ w.p.1 for some real, positive definite matrix $\bm\Gamma$ (condition B1). This assumption 
%introduces an important limitation, the nature of which we review next.
%
%In general, attempting to write the GCSA algorithm in the form of (\ref{eq:alien}) 
gives rise to an important complication
% the nature of which is explored in the following section.
when attempting to write the GCSA algorithm in the form of (\ref{eq:alien}); the nature of this complication is explored in the following section. 
%The following section  
%Here, a key observation is that if $\hat{\bm{\uptheta}}_k\rightarrow \infty$


\section[A Limitation of Fabian's Theorem]{A Limitation of Fabian's Theorem}
%\section{Relating GCS to Theorem \ref{thm:generalizefabian}}
\label{subsec:primadonna}
In this section we explore an issue that arises when attempting to write the recursion for the GCSA algorithm (see Line \ref{eq:indianindinorange} of Algorithm \ref{findme}) in the form of (\ref{eq:alien}), the recursion in Fabian's theorem. The nature of this issue is simple: the matrix $\bm\Gamma$ from condition B1 cannot generally be assumed to be symmetric for the GCSA algorithm, thus assumption B1 is not always satisfied and Fabian's theorem is not applicable. Using a simple example, we first explain why $\bm\Gamma$ cannot be assumed to be symmetric for the GCSA algorithm. Then, we discuss why it is not always possible to redefine $\bm\Gamma_k$, $\bm{T}_k$, $\bm{\Phi}_k$, and $\bm{V}_k$ in such a way that $\bm\Gamma$ (the limit w.p.1 of $\bm\Gamma_k$) is symmetric. Finally, we propose a slight generalization of Fabian's theorem that would allow for treatment of the special case of the GCSA algorithm where the subvector to update is selected according to a deterministic pattern (see, for example, the algorithm defined by (\ref{eq:william})).

Let us begin by rewriting the cyclic seesaw SA algorithm (a special case of GCSA) in the form of (\ref{eq:alien}). Recall that cyclic seesaw SA satisfies:
\begin{align}
\label{eq:santa}
\bm{{\hat{\uptheta}}}_{k+1}=\bm{{\hat{\uptheta}}}_{k}-a_{k}^{(1)}\hat{\bm{g}}_k^{(1)}(\hat{\bm\uptheta}_k)-a_{k}^{(2)}\hat{\bm{g}}_k^{(2)}(\hat{\bm\uptheta}_k^{(I)}),
\end{align}
where $\hat{\bm{\uptheta}}_k^{(I)}$ is defined in (\ref{eq:propoto2}). If $L(\bm\uptheta)$ is twice continuously differentiable then expanding $\bm{g}(\hat{\bm{\uptheta}}_k)$ around $\bm\uptheta^\ast$ and $\bm{g}(\hat{\bm{\uptheta}}_k^{(I)})$ around $\hat{\bm{\uptheta}}_k$:
\begin{align*}
\bm{g}^{(1)}(\hat{\bm{\uptheta}}_k)&=\bm{J}^{(1)}(\overline{\bm\uptheta}_k)(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast),\notag\\
\bm{g}^{(2)}(\hat{\bm{\uptheta}}_k)&=\bm{J}^{(2)}(\overline{\bm\uptheta}_k)(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast),\notag\\
\bm{g}^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})&=\bm{g}^{(2)}(\hat{\bm{\uptheta}}_k)+\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})(\hat{\bm{\uptheta}}_k^{(I)}-\hat{\bm{\uptheta}}_k),
\end{align*}
%
where $\bm{J}^{(j)}(\bm\uptheta)$ is the Jacobian of $\bm{g}^{(j)}(\bm\uptheta)$ with respect to $\bm\uptheta$,
% $\overline{\bm\uptheta}_k$ is a vector ``between'' $\hat{\bm{\uptheta}}_k$ and $\bm\uptheta^\ast$, and $\overline{\bm\uptheta}_k^{(I)}$ is a vector ``between'' $\hat{\bm{\uptheta}}_k^{(I)}$ and $\hat{\bm{\uptheta}}_k$. 
% To be more precise,
  the $i$th row of $\bm{J}^{(j)}(\overline{\bm\uptheta}_k)$ is equal to the $i$th row of $\bm{J}^{(j)}(\bm\uptheta)$ evaluated at $\bm\uptheta=(1-\uplambda_i)\hat{\bm{\uptheta}}_k+\uplambda_i\bm\uptheta^\ast$ for some $\uplambda_i\in[0,1]$ which depends on $\hat{\bm{\uptheta}}_k$, and the $i$th row of $\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})$ is the $i$th row of $\bm{J}^{(2)}(\bm\uptheta)$ with $\bm\uptheta=(1-\uplambda_i)\hat{\bm{\uptheta}}_k^{(I)}+\uplambda_i\hat{\bm{\uptheta}}_k$ for some $\uplambda_i\in[0,1]$ which depends on $\hat{\bm{\uptheta}}_k^{(I)}$. We now rewrite (\ref{eq:santa}) as:
%   as follows:
\label{page:betweenersow}
\begin{align}
\bm{{\hat{\uptheta}}}_{k+1}=&\ \bm{{\hat{\uptheta}}}_{k}-a_{k}^{(1)}\bm{J}^{(1)}(\overline{\bm\uptheta}_k)(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)-a_{k}^{(2)}\bm{J}^{(2)}(\overline{\bm\uptheta}_k)(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)-a_{k}^{(2)}\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})(\hat{\bm{\uptheta}}_k^{(I)}-\hat{\bm{\uptheta}}_k)\notag\\
&-a_k^{(1)}\left({\bm{\upbeta}}_k^{(1)}(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}_k^{(1)}(\hat{\bm{\uptheta}}_k)\right)-a_k^{(2)}\left({\bm{\upbeta}}_k^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})+{\bm{\upxi}}_k^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})\right).\label{eq:buckwild}
\end{align}
Using (\ref{eq:propoto2}) it follows that $-(\hat{\bm{\uptheta}}_k^{(I)}-\hat{\bm{\uptheta}}_k)/a_k^{(1)}=\bm{g}^{(1)}(\hat{\bm{\uptheta}}_k)+{\bm{\upbeta}}^{(1)}_k(\hat{\bm{\uptheta}}_k)+{\bm{\upxi}}^{(1)}_k(\hat{\bm{\uptheta}}_k)$. Combining this last observation with (\ref{eq:buckwild}) and using (\ref{eq:tennisey}), the cyclic seesaw SA algorithm can be written in the form of (\ref{eq:alien}) by letting $\bm{W}_k=\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast$, 
%
\begin{subequations}
\begin{align}
\bm\Gamma_k=&\ {k^\upalpha}\left[a_k^{(1)}\bm{J}^{(1)}(\overline{\bm\uptheta}_k)+ a_k^{(2)}\bm{J}^{(2)}(\overline{\bm\uptheta}_k)\right],\label{eq:shmee0}\\
\bm{T}_k=& -{k^{\upalpha+\upbeta/2}}\Big[a_k^{(1)}\bm{\bm{\upbeta}}_k^{(1)}(\hat{\bm\uptheta}_k)+a_k^{(2)}\bm{\upbeta}_k^{(2)}(\hat{\bm\uptheta}_k^{(I)})-a_k^{(1)}a_k^{(2)}\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})\bm{g}^{(1)}(\hat{\bm\uptheta}_k)\notag\\
&-a_k^{(1)}a_k^{(2)}\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})\bm{\upbeta}_k^{(1)}(\hat{\bm\uptheta}_k)-a_k^{(1)}a_k^{(2)}E\Big(\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})\bm{\upxi}_k^{(1)}(\hat{\bm\uptheta}_k)\Big|\mathcal{F}_k\Big)\Big],\label{eq:shmee1}\\
\bm{V}_k=& - k^{(\upalpha+\upbeta)/2}\Big[a_k^{(1)}\bm{\upxi}_k^{(1)}(\hat{\bm\uptheta}_k)+a_k^{(2)}\bm{\upxi}_k^{(2)}(\hat{\bm\uptheta}_k^{(I)})+a_k^{(1)}a_k^{(2)}E\Big(\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})\bm{\upxi}_k^{(1)}(\hat{\bm\uptheta}_k)\Big|\mathcal{F}_k\Big)\notag\\
&-a_k^{(1)}a_k^{(2)}\bm{J}^{(2)}(\overline{\bm\uptheta}_k^{(I)})\bm{\upxi}^{(1)}_k(\hat{\bm\uptheta}_k)\Big],\label{eq:shmee}
\end{align}
\end{subequations}
where $\mathcal{F}_k\equiv \{\hat{\bm{\uptheta}}_0, \hat{\bm{\uptheta}}_0^{(I)},\hat{\bm{\uptheta}}_1, \hat{\bm{\uptheta}}_1^{(I)}, \dots, \hat{\bm{\uptheta}}_k\}$, and letting $\bm\Phi_k=\bm{I}$.
% In other words, cyclic seesaw SA is a special case of the recursion in Theorem \ref{thm:fabian}.

In general, the matrix $\bm\Gamma_k$ in (\ref{eq:shmee0}) cannot be assumed to converge to a symmetric matrix w.p.1. To see this consider the case where $k^\upalpha a_k^{(1)}\rightarrow a^{(1)}$, $k^\upalpha a_k^{(2)}\rightarrow a^{(2)}$, and $\bm{J}^{(j)}(\hat{\bm{\uptheta}}_k)\rightarrow \bm{J}^{(j)}(\bm\uptheta^\ast)$ w.p.1 (e.g., when $L(\bm\uptheta)$ is twice continuously differentiable and $\hat{\bm{\uptheta}}_k\rightarrow \bm\uptheta^\ast$ w.p.1). Then,
\begin{align}
\label{eq:lookatme}
\bm\Gamma_k\rightarrow \bm\Gamma=a^{(1)}\bm{J}^{(1)}(\bm\uptheta^\ast)+a^{(2)}\bm{J}^{(2)}(\bm\uptheta^\ast){\text{ w.p.1.}}
\end{align}
%Moreover, if
%If $a^{(1)}=a^{(2)}=a>0$ then $\bm\Gamma=a\bm{H}(\bm\uptheta^\ast)$; it is not unusual for this matrix to be positive definite. However, whenever 
If $a^{(1)}=a^{(2)}=a>0$ then $\bm\Gamma=a\bm{H}(\bm\uptheta^\ast)$ is clearly a symmetric matrix. This is not generally the case, however, when $a^{(1)}\neq a^{(2)}$ (an exception being the case where $L(\bm\uptheta)$ is linearly separable in $\bm\uptheta^{(1)}$ and $\bm\uptheta^{(2)}$). Because there is no {\it{unique}} way to define the variables $\bm\Gamma_k$, $\bm{T}_k$, $\bm{\Phi}_k$, and $\bm{V}_k$ in (\ref{eq:alien}), it may be tempting to think that it is always possible to redefine these variables so that $\bm\Gamma$ is symmetric. Next we show that such a redefinition often leads to very strong assumptions on $\hat{\bm{\uptheta}}_k$.

%Therefore, condition B1 is not satisfied for cyclic seesaw SA (let alone for the GCSA algorithm) and Theorem \ref{thm:fabian} is not applicable. 



%Let us take a look at the definition of $\bm\Gamma_k$ in (\ref{eq:shmee}). Theorem \ref{thm:fabian} requires $\bm\Gamma_k$ to converge w.p.1 to a strictly positive definite matrix $\bm\Gamma$. 
%Furthermore, recall that if $\bm\Gamma$ is not symmetric then



Suppose an SA algorithm can be written in the form of (\ref{eq:alien}) and that all of the conditions of Fabian's theorem are satisfied {\it{with the exception that $\bm\Gamma$ is not symmetric}}. 
%
% by giving an example illustrating the issues that arise when attempting to redefine $\bm\Gamma_k$, $\bm{T}_k$, $\bm{\Phi}_k$, and $\bm{V}_k$. 
%
For simplicity, let us consider a special case where writing the algorithm in the form of (\ref{eq:alien}) can be done by letting $\upbeta\neq 0$, $\bm{T}_k=\bm{T}$, $\bm\Phi_k=\bm{I}$, and $\bm\Gamma_k=\bm\Gamma$ where $\bm\Gamma$ is not symmetric (note that we are assuming that $\bm{T}_k$, $\bm{\Phi}_k$, and $\bm{\Gamma}_k$ do not depend on $k$). 
% Then,
%\begin{align}
%\label{eq:crommer}
%\bm{W}_{k+1}=(\bm{I}-k^{-\upalpha}\bm\Gamma)\bm{W}_k+\frac{\bm{T}}{k^{\upalpha+\upbeta/2}}+\frac{\bm{V}_k}{k^{(\upalpha+\upbeta)/2}}.
%\end{align}
Now, assume the matrices $\bm\Gamma_k'$, $\bm\Phi_k'$ and vectors $\bm{T}_k'$, $\bm{V}_k'$ provide an alternative way to write the SA algorithm in the form of (\ref{eq:alien}). Furthermore, assume that $\bm\Gamma_k'$ converges w.p.1 to a positive definite matrix. Then, since
\label{eq:anotherpagerefgoeshere}
\begin{align*}
\bm{W}_{k+1}=&\ (\bm{I}-k^{-\upalpha}\bm\Gamma_k')\bm{W}_k+\frac{\bm{T}}{k^{\upalpha+\upbeta/2}}+\frac{\bm{V}_k}{k^{(\upalpha+\upbeta)/2}}+k^{-\upalpha}(\bm\Gamma_k'-\bm\Gamma)\bm{W}_k,
\end{align*}
 it is known that either $\bm{T}_k'$ must depend on $(\bm\Gamma'_k-\bm\Gamma)\bm{W}_k$ or $\bm\Phi_k'\bm{V}_k'$ must depend on $(\bm\Gamma_k'-\bm\Gamma)\bm{W}_k$. However, the assumptions Fabian's theorem imposes on $\bm{T}_k'$, $\bm\Phi_k'$, and $\bm{V}_k'$ are typically incompatible with the term $k^{\upbeta/2}(\bm\Gamma'_k-\bm\Gamma)\bm{W}_k$. Say, for example, that we let $\bm\Phi_k'=\bm{I}$, $\bm{V}_k'=\bm{V}_k$, and $\bm{T}_k'=\bm{T}+k^{\upbeta/2}(\bm\Gamma'_k-\bm\Gamma)\bm{W}_k$.
% \begin{align*}
% \bm{T}_k'=\bm{T}+k^{\upbeta/2}(\bm\Gamma'_k-\bm\Gamma)\bm{W}_k.
% \end{align*}
 Here, having $\bm{T}_k'$ converge to some finite vector $\bm{T}'$ w.p.1 (as required by B3) would impose a priori conditions on the stochastic rate at which $\hat{\bm{\uptheta}}_k$ converges to $\bm\uptheta^\ast$. However, such a condition violates the very purpose of Fabian's theorem, which is to establish such a rate of convergence.
% , converges to the zero vector. 
 Alternatively, having $\bm\Phi_k'\bm{V}_k'=\bm{V}_k+k^{(\upbeta-\upalpha)/2}(\bm\Gamma_k'-\bm\Gamma)\bm{W}_k$ does not lead to an appropriate definition of $\bm\Phi_k'$ and $\bm{V}_k'$
% to incorporate the term $(\bm\Gamma_k'-\bm\Gamma)\bm{W}_k$ into the definition of $\bm{V}_k'$ would not be appropriate 
 given the restriction that $\bm{V}_k'$ must have mean zero conditionally on $\mathcal{F}_k$. 
%
By simply generalizing the theorem to relax the symmetry condition on $\bm\Gamma$ we avoid the need for imposing additional restrictions on $\hat{\bm{\uptheta}}_k$. Next we propose a generalization of Fabian's theorem that will allow us to show asymptotic normality for a special case of the GCSA algorithm.
 

Note that in (\ref{eq:lookatme}) we have
% present the same issue when attempting to use Theorem \ref{thm:fabian}, namely,
  $\bm\Gamma=\bm{A}\bm{H}(\bm\uptheta^\ast)$, where $\bm{A}$ is a diagonal matrix with $i$th diagonal entry equal to $a^{(1)}$ if $i\leq p'$ and with $i$th diagonal entry equal to $a^{(2)}$ if $i>p'$. While $\bm\Gamma=\bm{A}\bm{H}(\bm\uptheta^\ast)$ is not generally real symmetric and positive definite as required by Fabian's condition B1 (an exception being the case where $L(\bm\uptheta)$ is linearly separable in $\bm\uptheta^{(1)}$ and $\bm\uptheta^{(2)}$), it is entirely possible for this matrix to have strictly positive eigenvalues and be real-diagonalizable (i.e., $\bm{S}^{-1}\bm{AH(\bm\uptheta^\ast)S}=\bm\Lambda$ for a nonsingular real matrix $\bm{S}$ and a positive definite diagonal matrix $\bm\Lambda$); the following proposition formalizes this observation.
%   and may have strictly positive eigenvalues (i.e., $\bm\Lambda$ has strictly positive diagonal entries). 
 

\begin{proposition}
\label{prop:sandpipercrossing}
Let $\bm{A}$ and $\bm{H}(\bm\uptheta^\ast)$ be real square matrices. Additionally, let $\bm{A}$ be a diagonal matrix with strictly positive diagonal entries. Finally, let  $\bm{H}(\bm\uptheta^\ast)$ be symmetric and positive definite (a common assumption in minimization problems). Then, there exist a nonsingular real matrix $\bm{S}$ and a positive definite diagonal matrix $\bm\Lambda$ such that $\bm{S}^{-1}\bm{AH(\bm\uptheta^\ast)S}=\bm\Lambda$.
\end{proposition}
\begin{proof}
Because $\bm{A}$ and $\bm{H}(\bm\uptheta^\ast)$ are both real and positive definite, Corollary 2.5.14 in Horn and Johnson (2010) implies there exist real, symmetric, positive definite matrices $\bm{A}^{1/2}$ and $\bm{H}(\bm\uptheta^\ast)^{1/2}$ such that $\bm{A}=\bm{A}^{1/2}\bm{A}^{1/2}$ and $\bm{H}(\bm\uptheta^\ast)=\bm{H}(\bm\uptheta^\ast)^{1/2}\bm{H}(\bm\uptheta^\ast)^{1/2}$. Therefore, 
%we can compute the positive definite square root of each and write 
$\bm{AH(\bm\uptheta^\ast)}=\bm{A}^{1/2}\bm{A}^{1/2}\bm{H}(\bm\uptheta^\ast)^{1/2}\bm{H}(\bm\uptheta^\ast)^{1/2}$. By multiplying the previous equation on the right by $\bm{I}=\bm{A}^{1/2}\bm{A}^{-1/2}$, we have:
\begin{align*}
\bm{AH(\bm\uptheta^\ast)}&=\bm{A}^{1/2}[\bm{H}(\bm\uptheta^\ast)^{1/2}\bm{A}^{1/2}]^\top[\bm{H}(\bm\uptheta^\ast)^{1/2}\bm{A}^{1/2}]\bm{A}^{-1/2}.
%=\bm{A}^{1/2}{\underbrace{(\bm{H}(\bm\uptheta^\ast)^{1/2}\bm{A}^{1/2})^\top(\bm{H}(\bm\uptheta^\ast)^{1/2}\bm{A}^{1/2})}_{\equiv \bm{M}}}\bm{A}^{-1/2}.
%\label{eq:yoogieoo}
\end{align*}
Define $\bm{M}\equiv \bm{H}(\bm\uptheta^\ast)^{1/2}\bm{A}^{1/2}$. Then, $\bm{M}^\top\bm{M}$ is a positive definite real symmetric matrix. Thus,  Corollary 2.5.14 in Horn and Johnson (2010) once again implies that
%Furthermore, all positive definite matrices are diagonalizable. $\bm{M}\succ 0$ 
we can write $\bm{M}=\bm{P}_0\bm\Lambda\bm{P}_0^{-1}$ for a nonsingular real orthogonal matrix $\bm{P}_0$ and a diagonal matrix, $\bm\Lambda$, with strictly positive eigenvalues. Then, $\bm{AH(\bm\uptheta^\ast)}= \bm{S\Lambda S}^{-1}$ with $\bm{S}=\bm{A}^{1/2}\bm{P}_0$. Note that while $\bm{S}$ is a real matrix, it is not necessarily an orthogonal matrix (i.e., $\bm{S}^{-1}$ is not necessarily equal to $\bm{S}^\top$), this follows from the fact that $\bm{S}^{-1}=\bm{P}_0^\top\bm{A}^{-1/2}$ and $\bm{S}^\top=\bm{P}_0^\top\bm{A}^{1/2}$ so that having $\bm{S}^{-1}=\bm{S}^\top$ would imply $\bm{A}^{-1/2}=\bm{A}^{1/2}$, which is only true of $\bm{A}=\bm{I}$.
% we can rewrite (\ref{eq:yoogieoo}) as $\bm{AH(\bm\uptheta^\ast)}=\bm{A}^{1/2}\bm{S}_0\bm\Lambda\bm{S}_0^{-1}\bm{A}^{-1/2}= \bm{S\Lambda S}^{-1}$.
\end{proof}


It follows from Proposition \ref{prop:sandpipercrossing} that generalizing Condition B1 in Fabian's theorem to allow $\bm\Gamma$ to be any real diagonalizable matrix with strictly positive eigenvalues (i.e., $\bm{S}^{-1}\bm{AH(\bm\uptheta^\ast)S}=\bm\Lambda$ with $\bm{S}$ and $\bm\Lambda$ defined as in Proposition \ref{prop:sandpipercrossing}) would allow for treatment of the cyclic seesaw SA algorithm. Furthermore, Section \ref{sec:upperpotomacshell} shows that the proposed generalization to Fabian's theorem would also allow for treatment of Algorithm \ref{kirkey} (deterministic pattern for coordinate selection), a special case of the GCSA algorithm (Algorithm \ref{findme}).

 In the following section we provide a generalization of Fabian's theorem which is slightly more general than the extension suggested by Proposition \ref{prop:sandpipercrossing}. The generalization only requires that $\bm\Gamma=\bm{SUS}^{-1}$ for a real non-singular matrix $\bm{S}$ and a real {{upper triangular}} matrix $\bm{U}$ with strictly positive diagonal entries (here $\bm\Gamma$ is said to be upper-triangularizable). Appendix \ref{sec:fabiansecgeneralize} discusses how the generalization to Fabian's theorem expands the theorem's applicability to include other SA algorithms (aside from Algorithm \ref{kirkey}) of practical interest.



\section{Generalizing Fabian's Theorem}
\label{sec:genfabiangenfabian}

This section contains
% states two lemmas pertaining to the process in (\ref{eq:alien}) which are used to derive 
 a generalization to Fabian's theorem derived by replacing condition B1 with a slightly weaker assumption.  Specifically, for $\bm{W}_k$ and $\upbeta$ defined as in (\ref{eq:alien}) we show $k^{\upbeta/2}\bm{W}_k$ converges in distribution to a multivariate normal random variable under conditions B0, B2--B6, and a relaxed version of B1. Following the proof of Fabian's theorem (Fabian 1968), we begin by showing that $k^{\upbeta/2}\bm{W}_k$ is asymptotically normally distributed if and only if a much simpler process is also asymptotically normally distributed. After showing that the simpler process does, in fact, converge in distribution to a multivariate normal random variable, the parameters of its asymptotic distribution will uniquely determine the parameters of the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$. Next we introduce some notation and the generalized version of condition B1.

  Throughout this Chapter $M_{ij}$ and $M_{k(i,j)}$ denote the $(i,j)$th entries of the matrices $\bm{M}$ and $\bm{M}_k$, respectively, and ${v}_i$ and $v_{k(i)}$ denote the $i$th entries of the vectors $\bm{v}$ and $\bm{v}_k$, respectively. Furthermore, $k\geq 1$ denotes a strictly positive integer; $\xrightarrow{\text{\ dist\ }}$ means convergence in distribution; $\bm{V}_k$, $\bm{W}_k$, $\bm{T}_k$, and $\bm{T}$ are vectors in $\mathbb{R}^p$; $\bm\Gamma_k$, $\bm\Phi_k$, $\bm\Sigma$, $\bm\Gamma$, $\bm\Phi$, and $\bm{P}$ are matrices in $\mathbb{R}^{p\times p}$; and $\mathcal{N}(\bm\upmu,\bm{M})$ denotes a multivariate normal random variable with mean $\bm\upmu$ and covariance $\bm{M}$. Furthermore, throughout this section we assume the recursion for ${\bm{W}}_k$ given in (\ref{eq:alien}) satisfies the following conditions:
  \begin{DESCRIPTION}
\label{apge:definematrixindices}
\item[B1$'$] There exists an {\it{upper triangular}} matrix $\bm{U}\in \mathbb{R}^{p\times p}$ with strictly positive eigenvalues and a nonsingular $\bm{S}\in \mathbb{R}^{p\times p}$ such that $\bm\Gamma_k\rightarrow \bm\Gamma=\bm{S}\bm{U}\bm{S}^{-1}$ w.p.1.
\item[B6$'$] Define $\uplambda\equiv \min_i{\{U_{ii}\}}$. Let $\upalpha$ and $\upbeta$ be constants such that $0<\upalpha\leq 1$ and $0\leq \upbeta$. Define $\upbeta_+\equiv\upbeta$ if $\upalpha=1$ and $\upbeta_+\equiv 0$ otherwise. Then, $\upbeta_+<2\uplambda$.
\item[B0$'$ \& B2$'$--B5$'$]  The same as B0 and B2--B5, respectively.
\end{DESCRIPTION}
%
Conditions B0$'$ and B2$'$--B6$'$ are identical to the conditions of Fabian's theorem (note that B6$'$ is obtained by rewriting B6 in the notation of B1$'$). On the other hand, B1$'$ is the relaxed version of Fabian's  corresponding condition (condition B1 in Theorem \ref{thm:fabian}) requiring symmetry of $\bm\Gamma$. As discussed in the comment following Proposition \ref{prop:sandpipercrossing}, any real square matrix with real eigenvalues satisfies B1$'$. The following Theorem is our generalization to Fabian's theorem based on conditions B1$'$--B6$'$.


  \begin{theorem}[A Generalization of Fabian's Theorem]
  \label{thm:generalizefabian} 
  Assume the recursion for ${\bm{W}}_k$ given in (\ref{eq:alien}) satisfies B0$'$--B6$'$. Then, the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$ is a multivariate normal random variable with mean $\bm{S}\bm\upnu$ and covariance matrix $\bm{SQS}^\top$, where the entries of $\bm\upnu$ are the unique solution to:
\begin{align}
 \label{eq:okayfine}
 \upnu_i\equiv (\tilde{{U}}_{ii})^{-1}\tilde{{T}}_i-\Bigg[(\tilde{{U}}_{ii})^{-1}\sum_{j=i+1}^p \tilde{U}_{ij}\upnu_j\Bigg]
% \upnu^{[i]}\equiv  (\tilde{{U}}^{[i,i]})^{-1}\Bigg[\tilde{{T}}^{[i]}-\sum_{j=i+1}^p \tilde{U}^{[i,j]}\upnu^{[j]}\Bigg].
 \end{align}
with  $\tilde{\bm{T}}\equiv \bm{S}^{-1}\bm{T}$ and $\tilde{\bm{U}}\equiv \bm{U}-(\upbeta_+/2)\bm{I}$; and the entries of $\bm{Q}$ are the unique solution to:
\begin{align}
\label{eq:nolookback}
Q_{ij}=\frac{[\bm{S}^{-1}\bm{\Phi\Sigma\Phi}^\top(\bm{S}^{-1})^\top]_{ij}}{\tilde{U}_{ii}+\tilde{U}_{jj}}-\Bigg[\frac{\sum_{\ell=j+1}^{p} \tilde{U}_{j\ell}\ Q_{i\ell}+\sum_{\ell=i+1}^{p} \tilde{U}_{i\ell}\ Q_{\ell j}}{\tilde{U}_{ii}+\tilde{U}_{jj}}\Bigg].
%Q^{[i,j]}=\frac{\tilde{\Sigma}^{[i,j]}-\sum_{\ell=j+1}^{p} \tilde{U}^{[j,\ell]}Q^{[i,\ell]}-\sum_{\ell=i+1}^{p} \tilde{U}^{[i,\ell]}Q^{[\ell,j]}}{\tilde{U}^{[i,i]}+\tilde{U}^{[j,j]}}.
\end{align}
%with $\tilde{\bm\Sigma}\equiv \bm{S}^{-1}\bm{\Phi\Sigma\Phi}^\top(\bm{S}^{-1})^\top$.
 Using (\ref{eq:nolookback}), $Q_{ij}$ is a function of the elements of the set $\{Q_{mn}\}_{(m,n)\in \mathcal{G}}$ where $\mathcal{G}$ is the set of $(m,n)$ tuples such that either $m\geq i+1$ and $n\geq j+1$, $m=i$ and $n\geq j+1$, or $m\geq i+1$ and $n=j$. Therefore, the entries of $\bm{Q}$ can be computed sequentially beginning with $Q_{pp}$, for which (\ref{eq:nolookback}) gives a solution. Similarly, the entries of $\bm\upnu$ can be computed beginning with $\upnu_p$, for which (\ref{eq:okayfine}) gives a solution.
\end{theorem}

\begin{proof}
(Although the following proof is complete, a more detailed proof of the theorem can be found in Appendix \ref{sec:fabiansecgeneralize}). In order to compute the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$ we begin by constructing the following process:
\begin{align*}
%\label{eq:linkssfton}
\tilde{\bm{W}}_{k}=(k-1)^{\upbeta/2}\bm{S}^{-1}\bm{W}_k,
\end{align*}
where $\bm{S}$ is the matrix from B1$'$. Here, using Slutsky's theorem it follows that if $\tilde{\bm{W}}_k\xrightarrow{\text{\ dist\ }}\mathcal{N}(\bm\upmu,\bm{M})$,
% has an asymptotically normal distribution with mean $\bm\upmu$ and covariance matrix $\bm{M}$
 then $k^{\upbeta/2}\bm{W}_k\xrightarrow{\text{\ dist\ }}\mathcal{N}(\bm{S}\bm\upmu,\bm{SM S}^\top)$.
%  must have an asymptotically normal distribution with mean $\bm{S}\bm\upmu$ and covariance matrix $\bm{SM S}^\top$.
   Thus, proving that the process $\tilde{\bm{W}}_k$ is asymptotically normally distributed (with certain mean vector and covariance matrix) is sufficient for computing the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$. Moreover, after some algebraic manipulation it can be shown that:
\begin{align}
\label{eq:graham3884}
 \tilde{\bm{W}}_{k+1}=&\ (\bm{I}-k^{-\upalpha}\tilde{\bm{\Gamma}}_k)\tilde{\bm{W}}_k+\frac{\bm{S}^{-1}\bm{T}_k}{k^\upalpha}+\frac{\bm{S}^{-1}\bm\Phi_k\bm{V}_k}{k^{\upalpha/2}},
\end{align}
 where $\tilde{\bm{W}}_{1}=\bm{0}$, 
\begin{align*}
%\label{eq:equis2222s}
\tilde{\bm\Gamma}_k\equiv \left(\frac{k}{k-1}\right)^{\upbeta/2}\bm{S}^{-1}\bm\Gamma_k\bm{S}-\left[\left(\frac{k}{k-1}\right)^{\upbeta/2}-1\right]k^\upalpha\bm{I},
\end{align*}
and $\tilde{\bm\Gamma}_k\rightarrow \tilde{\bm{U}}= \bm{U}-(\upbeta_+/2)\bm{I}$ w.p.1 so that $\tilde{\bm{W}}_k$ is a special case of (\ref{eq:alien}). Using the same arguments as those in Fabian (1968, proof of Theorem 2.2) it can be shown that replacing ${\bm{T}}_k$ with ${\bm{T}}$ and $\bm\Phi_k$ with $\bm\Phi$  in (\ref{eq:graham3884}) does not change the asymptotic distribution of $\tilde{\bm{W}}_k$ (this result is not immediate due to the recursive nature of $ \tilde{\bm{W}}_{k}$). Therefore, in order to show that $\tilde{\bm{W}}_k$ is asymptotically normally distributed we may assume, without loss of generality (w.l.o.g.), that ${\bm{T}}_k={\bm{T}}$ and $\bm\Phi_k=\bm\Phi$ so that:
\begin{align}
\label{eq:jaredboothsssd}
 \tilde{\bm{W}}_{k+1}=(\bm{I}-k^{-\upalpha}\tilde{\bm{\Gamma}}_k)\tilde{\bm{W}}_k+k^{-\upalpha}\tilde{\bm{T}}+k^{-\upalpha/2}\tilde{\bm{V}}_k,
\end{align}
where $\tilde{\bm{T}}= \bm{S}^{-1}\bm{T}$ and $\tilde{\bm{V}}_k\equiv \bm{S}^{-1}\bm{\Phi V}_k$. Next, we relate the asymptotic distribution of $\tilde{\bm{W}}_k$, as described by (\ref{eq:jaredboothsssd}), to that of an even simpler process. 

Consider the process:
\begin{align}
\label{eq:norahjoness772}
 \tilde{\bm{W}}_{k+1}'=(\bm{I}-k^{-\upalpha}\tilde{\bm{\Gamma}}_k)\tilde{\bm{W}}_k'+k^{-\upalpha/2}\tilde{\bm{V}}_k,
\end{align}
obtained by removing the term $k^{-\upalpha}\tilde{\bm{T}}$ from (\ref{eq:jaredboothsssd}). Lemma 4.2 (Fabian 1967) implies $\tilde{\bm{W}}_k-\tilde{\bm{W}}_k'\rightarrow\bm\upnu$ w.p.1, where the entries of $\bm\upnu$ are given in (\ref{eq:okayfine}).
%\begin{align}
%\label{eq:okayfine}
%\upnu^{[i]}\equiv (\tilde{{U}}^{[i,i]})^{-1}\Bigg[\tilde{{T}}^{[i]}-\sum_{j=i+1}^p \tilde{U}^{[i,j]}\upnu^{[j]}\Bigg].
%\end{align} 
The significance of this observation is that if $\tilde{\bm{W}}_{k}'\xrightarrow{\text{\ dist\ }}\mathcal{N}(\bm\upmu,\bm{M})$,
% converges in distribution to a multivariate normal random variable with mean $\bm\upmu$ and covariance $\bm{M}$, 
 then $\tilde{\bm{W}}_{k}\xrightarrow{\text{\ dist\ }}\mathcal{N}(\bm\upmu+\bm\upnu,\bm{M})$. 
% must converge in distribution to a multivariate normal random variable with mean $\bm\upmu+\bm\upnu$ and covariance $\bm{M}$. 
% 
% Therefore, deriving the asymptotic distribution of $\tilde{\bm{W}}_{k}'$ is sufficient for deriving the asymptotic distribution of $\tilde{\bm{W}}_{k}$ and, therefore, of $k^{\upbeta/2}\bm{W}_k$. 
 At this point, the same arguments as those in Fabian (1968, proof of Theorem 2.2) can be used to show the following two results:
 \begin{enumerate}
 \item Replacing $\tilde{\bm{\Gamma}}_k$ with $\tilde{\bm{U}}$ in (\ref{eq:norahjoness772}) does not change the asymptotic distribution of $\tilde{\bm{W}}_k'$ which depends on the limit (w.p.1) of $\tilde{\bm{\Gamma}}_k$ but not on $\tilde{\bm{\Gamma}}_k$ itself. Therefore, w.l.o.g. we may assume that $\tilde{\bm{\Gamma}}_k=\tilde{\bm{U}}$ so that:
 \begin{align}
\label{eq:utildenew}
 \tilde{\bm{W}}_{k+1}'=(\bm{I}-k^{-\upalpha}\tilde{\bm{U}})\tilde{\bm{W}}_k'+k^{-\upalpha/2}\tilde{\bm{V}}_k.
\end{align} 

 
 \item The characteristic function of the asymptotic distribution of $\tilde{\bm{W}}_{k}'$ evaluated at $\bm{t}\in \mathbb{R}^p$ depends on $\bm{t}$, $\upalpha$, $\tilde{\bm{U}}$, and on $\tilde{\bm{\Sigma}}\equiv \lim_{k\rightarrow \infty}\text{cov}[\tilde{\bm{V}}_k|\mathcal{F}_k]$ but is independent of other aspects of the distribution of $\tilde{\bm{V}}_k$ (provided conditions B0$'$--B6$'$ hold).  Therefore, we may assume w.l.o.g. that the vectors $\tilde{\bm{V}}_k$ are i.i.d. $\mathcal{N}(\bm{0},\tilde{\bm{\Sigma}})$.
%  and that $\tilde{\bm{V}}_k$ is independent of $\mathcal{F}_k$.
 \end{enumerate}
%A consequence of point No. 1 above is that computing the asymptotic distribution of $\bm{W}_k'$, defined by recursion (\ref{eq:utildenew}), is sufficient for computing the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$.
 Next we derive the asymptotic distribution of the process $\tilde{\bm{W}}_k'$ in (\ref{eq:utildenew}).
% is asymptotically normally distributed with mean and covariance depending on $\tilde{\bm{U}}$ and $\tilde{\bm{\Sigma}}$.

First, note that $\tilde{\bm{\Sigma}}=\bm{S}^{-1}\bm{\Phi\Sigma\Phi}^\top(\bm{S}^{-1})^\top$ by condition B4$'$. Next, by point 2 in the previous paragraph we may assume w.l.o.g. that the vectors $\tilde{\bm{V}}_k$ are i.i.d. $\mathcal{N}(\bm{0},\tilde{\bm{\Sigma}})$. Consequently, the distribution of $\tilde{\bm{W}}_k'$ from (\ref{eq:utildenew}) must be a multivariate normal random variable with mean zero (since $\tilde{\bm{W}}_1'=\bm{0}$) and covariance $\bm{Q}_k\equiv E[\tilde{\bm{W}}_{k}'(\tilde{\bm{W}}_{k}')^\top]$
% From (\ref{eq:utildenew}), $\bm{Q}_k$ 
which satisfies:
\begin{align*}
Q_{k+1(ij)}=&\ \left(1-k^{-\upalpha}\left[\tilde{U}_{ii}+\tilde{U}_{jj}-k^{-\upalpha} \tilde{U}_{ii}\hspace{.2em} \tilde{U}_{jj}\right]\right)Q_{k(ij)}\notag\\
&-k^{-\upalpha}\left[\sum_{\ell=j+1}^{p} \tilde{U}_{j\ell}\hspace{.2em} Q_{k(i\ell)}+\sum_{\ell=i+1}^{p} \tilde{U}_{i\ell}\hspace{.2em} Q_{k(\ell j)}\right]+k^{-\upalpha}\tilde{\Sigma}_{ij}\notag\\
&+k^{-2\upalpha}\sum_{\ell=i}^p \tilde{U}_{i\ell}\sum_{s=j+1}^p\tilde{U}_{js}\hspace{.2em} Q_{\ell s}+k^{-2\upalpha}\sum_{\ell=i+1}^p \tilde{U}_{i\ell}\hspace{.2em} \tilde{U}_{jj}\hspace{.2em} Q_{\ell j}.
%Q^{[i,j]}_{k+1}=&\ \left(1-k^{-\upalpha}\left[\tilde{U}^{[i,i]}+\tilde{U}^{[j,j]}-k^{-\upalpha} \tilde{U}^{[i,i]}\tilde{U}^{[j,j]}\right]\right)Q^{[i,j]}_k\notag\\
%&-k^{-\upalpha}\left[\sum_{\ell=j+1}^{p} \tilde{U}^{[j,\ell]}Q^{[i,\ell]}_k+\sum_{\ell=i+1}^{p} \tilde{U}^{[i,\ell]}Q^{[\ell,j]}_k\right]+k^{-\upalpha}\tilde{\Sigma}^{[i,j]}\notag\\
%&+k^{-2\upalpha}\sum_{\ell=i}^p \tilde{U}^{[i,\ell]}\sum_{s=j+1}^p\tilde{U}^{[j,s]}Q^{[\ell,s]}+k^{-2\upalpha}\sum_{\ell=i+1}^p \tilde{U}^{[i,\ell]}\tilde{U}^{[j,j]}Q^{[\ell,j]}.
%%Q^{[i,j]}_{k+1}=&\ (1-k^{-\upalpha}[\tilde{U}^{[i,i]}+\tilde{U}^{[j,j]}-o(1)])Q^{[i,j]}_k\notag\\
%%&-k^{-\upalpha}\left[\sum_{\ell=j+1}^{p} \tilde{U}^{[j,\ell]}Q^{[i,\ell]}_k+\sum_{\ell=i+1}^{p} \tilde{U}^{[i,\ell]}Q^{[\ell,j]}_k-o(1)-\tilde{\Sigma}^{[i,j]}\right].
\end{align*}
 Here, Lemma 4.2 in Fabian (1967) implies $\bm{Q}\equiv \lim_{k\rightarrow \infty}\bm{Q}_k$ is a matrix whose entries are the unique solution to (\ref{eq:nolookback}).
% \begin{align}
%\label{eq:nolookback}
%Q^{[i,j]}=\frac{\tilde{\Sigma}^{[i,j]}-\sum_{\ell=j+1}^{p} \tilde{U}^{[j,\ell]}Q^{[i,\ell]}-\sum_{\ell=i+1}^{p} \tilde{U}^{[i,\ell]}Q^{[\ell,j]}}{\tilde{U}^{[i,i]}+\tilde{U}^{[j,j]}}.
%\end{align}
Therefore, $\tilde{\bm{W}}_k'\xrightarrow{\text{\ dist\ }}\mathcal{N}(\bm{0},\bm{Q})$ which implies ${\bm{W}}_{k}\xrightarrow{\text{\ dist\ }}\mathcal{N}(\bm{S}\bm\upnu,\bm{S}\bm{Q}\bm{S}^\top)$.
% converges in distribution to a multivariate normal random variable with mean zero and covariance matrix $\bm{Q}$.
\end{proof}


Note that if $\bm\Gamma$ is real symmetric then the terms in square brackets in (\ref{eq:okayfine}) and (\ref{eq:nolookback}) disappear since $\tilde{\bm{U}}$ may be taken to be a diagonal matrix. This implies that when $\bm\Gamma$ is a real and symmetric matrix (as in Fabian's theorem) then:
\begin{align}
\label{eq:fishytailshastrain}
\bm{S}\bm\upnu=\bm{S}\tilde{\bm{U}}^{-1}\tilde{\bm{T}}=\bm{S}[\bm{U}-(\upbeta_+/2)\bm{I}]^{-1}\bm{S}^{-1}\bm{T}=(\bm\Gamma-(\upbeta_+/2)\bm{I})^{-1}\bm{T}.
\end{align}
%where we have used the fact that $\bm{S}[\bm{U}-(\upbeta_+/2)\bm{I}]^{-1}\bm{S}^{-1}=\left(\bm{S}[\bm{U}-(\upbeta_+/2)\bm{I}]\bm{S}^{-1}\right)^{-1}$. 
The mean vector in (\ref{eq:fishytailshastrain}) is the same as the mean of the asymptotic distribution in Fabian's theorem (Theorem \ref{thm:fabian}). Similarly, when $\bm{U}$ is a diagonal matrix, we can assume $\bm{S}=\bm{P}$ for some orthogonal matrix $\bm{P}$ and
% $\bm{S}$ can be assumed to be equal to an orthogonal matrix $\bm{P}$ and 
 (\ref{eq:nolookback}) reduces to $Q_{ij}=(\bm{P}^\top\bm{\Phi}\bm\Sigma\bm\Phi^\top\bm{P})_{ij}(U_{ii}+U_{jj}-\upbeta_+)^{-1}$ as in Fabian's theorem.



\section{Asymptotic Normality of Algorithm \ref{kirkey}}
\label{sec:upperpotomacshell}
This section gives a set of conditions for the asymptotic normality of the normalized iterates from Algorithm \ref{kirkey} (a special case of GCSA).
%which are based on conditions B0$'$--B6$'$. 
%
%  the recursion from Theorem \ref{thm:generalizefabian}.
%
%Consider the setting of Algorithm \ref{kirkey} (Deterministic Pattern for Coordinate Selection). This is Then, t
First, following a derivation similar to that of (\ref{eq:buckwild}), Algorithm \ref{kirkey} may be written as:
%the iterates of Algorithm \ref{kirkey} can be shown to satisfy the following recursion:
% a derivation similar to that of (\ref{eq:buckwild}),
%  the iterates of Algorithm \ref{kirkey} 
%%  can be shown to satisfy the following recursion:
%satisfy:
\begin{align}
 \hat{\bm{\uptheta}}_{k+1}=&\ \hat{\bm\uptheta}_k-\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}(\overline{\bm\uptheta}_k)(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)\notag\\
 &+\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right)[\bm\Delta_{\bm{g}}^{(I_{z,\ell})}+\bm\Delta_{\bm{\upbeta}}^{(I_{z,\ell})}+\bm\Delta_{\bm{\upxi}}^{(I_{z,\ell})}]\notag\\
 &-\sum_{z=1}^{s}\sum_{\ell=0}^{n_(z)-1} {a}_{k}^{(j(z))} {\bm{\upbeta}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\right)\notag\\
 &-\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} {\bm{\upxi}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\right),\label{eq:eleafanimalstrees}
\end{align}
where $\hat{\bm{\uptheta}}_k$ denotes an iterate of Algorithm \ref{kirkey} and
%In relation to this equation, define
\begin{subequations}
\begin{align}
 \bm\Delta_{\bm{g}}^{(I_{z,\ell})}\equiv&\ \sum_{m=1}^{z-1}\sum_{i=0}^{n(m)-1} \left[ {a}_{k}^{(j(m))} {\bm{g}}^{(j(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right]+\sum_{i=0}^{\ell-1} \left[ {a}_{k}^{(j(z))}{\bm{g}}^{(j(z))}\left(\hat{\bm\uptheta}_k^{(I_{z,i})}\right)\right],\label{eq:futuramasohs0}\\
 \bm\Delta_{\bm\upbeta}^{(I_{z,\ell})}\equiv&\ \sum_{m=1}^{z-1}\sum_{i=0}^{n_k(m)-1} \left[ {a}_{k}^{(j(m))} {\bm{\upbeta}}_k^{(j(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right]+\sum_{i=0}^{\ell-1} \left[ {a}_{k}^{(j(z))} {\bm{\upbeta}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{(I_{z,i})}\right)\right],\label{eq:futuramasohs1}\\
 \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\equiv&\ \sum_{m=1}^{z-1}\sum_{i=0}^{n_k(m)-1} \left[ {a}_{k}^{(j(m))} {\bm{\upxi}}_k^{(j(m))}\left(\hat{\bm\uptheta}_k^{(I_{m,i})}\right)\right]+\sum_{i=0}^{\ell-1} \left[ {a}_{k}^{(j(z))} {\bm{\upxi}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{(I_{z,i})}\right)\right].\label{eq:futuramasohs}
\end{align}
\end{subequations}
Then, in a manner analogous to (\ref{eq:shmee0}--c) we let $\upalpha>0$, $\upbeta\geq 0$, $\bm{W}_k=\hat{\bm{\uptheta}}_k=\bm\uptheta^\ast$, and let $\mathcal{F}_k$ be the sigma field generated by $\{\hat{\bm{\uptheta}}_\ell\}_{\ell=0}^k$ as well as by any random variables generated  by the algorithm in the production of $\hat{\bm{\uptheta}}_k$. Additionally,
let 
%$\bm{T}_k$ be: 
\begin{align}
\bm{T}_k=& \ - k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} {\bm{\upbeta}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\right)\notag\\
&+k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right)[\bm\Delta_{\bm{g}}^{(I_{z,\ell})}+\bm\Delta_{\bm{\upbeta}}^{(I_{z,\ell})}]\notag\\
&+k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} E\Big[\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big|\mathcal{F}_k\Big],
\label{eq:goingcrazyhim}
\end{align}
let $\bm\Phi_k=\bm{I}$, let $\bm{V}_k$ be given by
\begin{align}
\bm{V}_k=&\ -k^{(\upalpha+\upbeta)/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} {\bm{\upxi}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\right)\notag\\
&+k^{(\upalpha+\upbeta)/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\notag\\
&-k^{(\upalpha+\upbeta)/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} E\Big[\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big|\mathcal{F}_k\Big],
\label{eq:othingcoodsd}
\end{align}
and let
\begin{align}
\bm\Gamma_k=k^\upalpha\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}(\overline{\bm\uptheta}_k).
\label{eq:pantyponcho}
\end{align}
With this notation, the recursion in (\ref{eq:eleafanimalstrees}) defining an iteration of Algorithm \ref{kirkey} can be written in the form of (\ref{eq:alien}), the recursion of Theorem \ref{thm:generalizefabian}. 

Because (\ref{eq:eleafanimalstrees}) is a special case of (\ref{eq:alien}), conditions B0$'$--B6$'$ would be sufficient for the asymptotic normality of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$ when $\hat{\bm{\uptheta}}_k$ denotes an iterate of Algorithm \ref{kirkey}. In practice, however, the validity of conditions B0$'$--B6$'$ (or of the slightly stronger conditions B0--B6) can be difficult to verify for {\it{any}} algorithm which may be written in the form of (\ref{eq:alien}). 
%
%Typically, the usefulness of conditions B0$'$--B6$'$ stems from the fact that the conditions may appear to be 
%reasonable 
%
In the case of Algorithm \ref{kirkey} this is complicated by the fact that the terms $\bm\Gamma_k$, $\bm{T}_k$, $\bm{\Phi}_k$, and $\bm{V}_k$ have more complex forms than the corresponding variables for classical SA algorithms (compare the definitions below (\ref{eq:crownuni}) to (\ref{eq:goingcrazyhim})--(\ref{eq:pantyponcho})). 
%
%Therefore, for Algorithm \ref{kirkey} even understanding whether B0$'$--B6$'$ are {\it{reasonable}} assumptions is difficult.
%
 In an effort to obtain a set of conditions that are easier to understand than B0$'$--B6$'$, this section derives a set of conditions which imply B0$'$--B6$'$ hold for Algorithm \ref{kirkey}. To do this, we first present a useful lemma related to condition B5$'$.
%
%Before stating conditions for the asymptotic normality of the iterates from Algorithm \ref{kirkey} we present a useful lemma which is related to condition B5$'$.


\begin{lemma}
\label{lem:piccardo}
Let $\bm{V}_k$ be a vector-valued sequence with $\bm{V}_k= \sum_{i=1}^N\bm{\Psi}_k(i)$, where $N$ is an integer such that $2\leq N<\infty$ and $\bm{\Psi}_k(i)$ denotes a vector-valued random variable.
%so that 
%\begin{align*}
%\bm{\Psi}_k= \bm{A}_k+\bm{B}_k.
%\end{align*}
Additionally,
%For each $k$ and $i\neq j$, let $\bm{\Psi}_k(i)$ and $\bm{\Psi}_k(j)$ be independent random variables. Furthermore, for all $k$ let $E[\bm{\Psi}_k(i)]=\bm{0}$ and $E\|\bm{\Psi}_k(i)\|^2\leq c_i$ for some finite constant $c_i$.
%
% each with mean zero. Furthermore, assume there exist constants $0<a,b<\infty$ such that $E\|\bm{A}_k\|^2\leq a$ and $E\|\bm{B}_k\|^2\leq b$. 
% 
% Finally, 
 for some $\upalpha>0$ and for every $r>0$ let the values $\upsigma_{k,r}^2(i)\equiv E\chi \{\|\bm{\Psi}_k(i)\|^2\geq rk^\upalpha\}\|\bm{\Psi}_k(i)\|^2$ satisfy
%\begin{enumerate}[label=(\roman*)]
$\lim_{k\rightarrow \infty}\upsigma_{k,r}^2(i)=0$ for all $i$.
% \item $\upalpha=1$ and $\lim_{n\rightarrow \infty}n^{-1}\sum_{k=1}^n\upsigma^2_{k,r}(i)=0$ for all $i$.
%\end{enumerate}
%for $\bm{V}_k= \bm{A}_k,\bm{B}_k$ (one of the two conditions must hold for both $\bm{A}_k$ and $\bm{B}_k$). 
Then, the sequence $\upsigma_{k,r}^2\equiv E\chi\{\|\bm{V}_k\|^2\geq rk^\upalpha\}\|\bm{V}_k\|^2$ also satisfies $\lim_{k\rightarrow \infty}\upsigma_{k,r}^2=0$.
\end{lemma}
\begin{proof}
For simplicity, we assume $N=2$ so that $\bm{V}_k=\bm\Psi_k(1)+\bm\Psi_k(2)$ (the proof for $N>2$ is essentially identical).
%(the proof for $N>2$ is a trivial generalization).
% We wish to prove the same holds for $\bm{V}_k=\bm\Psi_k$. 
First,
% note the following:
%\begin{align*}
%%\label{eq:zeldacsezelda}
%\upsigma_{k,r}^2=E\chi\{\|\bm{V}_k\|^2\geq rk^\upalpha\}\|\bm{V}_k\|^2=\int_{\|\bm{V}_k\|\geq \sqrt{rk^\upalpha}} \|\bm{V}_k\|^2\ dP,
%\end{align*}
%where $P$ denotes the joint probability measure of $\bm\Psi_k(1)$ and $\bm\Psi_k(2)$. 
%The goal is to show that either (i) or (ii) holds when $\upsigma_{k,r}^2(i)$ is replaced by $\upsigma_{k,r}^2$ (see B5$'$ or B5). 
%
%We begin by upper-bounding the integrand in (\ref{eq:zeldacsezelda}).
%
% However, 
 using the triangle inequality we know $\|\bm{V}_k\|\leq \|\bm{\Psi}_k(1)\|+\|\bm{\Psi}_k(2)\|$. Therefore, in order to have $\|\bm{V}_k\|\geq \sqrt{rk^\upalpha}$ at least one of $\|\bm{\Psi}_k(1)\|$ or $\|\bm{\Psi}_k(2)\|$ must be greater or equal to $\sqrt{rk^\upalpha}/2$, which implies:
 \begin{align*}
 \chi\{\|\bm{V}_k\|\geq \sqrt{rk^\upalpha}\}\|\bm{V}_k\|\leq\sum_{i=1}^2 2\chi\{\|\bm{\Psi}_k(i)\|\geq \sqrt{rk^\upalpha}/2\}\|\bm{\Psi}_k(i)\|
% \notag\\
% &+2\chi\{\|\bm{\Psi}_k(2)\|\geq \sqrt{rk^\upalpha}/2\}\|\bm{\Psi}_k(2)\|
 \end{align*}
(recall that $\chi\{\mathcal{E}\}$ is the indicator function of the event $\mathcal{E}$). Equivalently,
  \begin{align}
  \label{eq:masstwilighteffext}
 \chi\{\|\bm{V}_k\|^2\geq {rk^\upalpha}\}\|\bm{V}_k\|\leq\sum_{i=1}^2 2\chi\{\|\bm{\Psi}_k(i)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(i)\|.
 \end{align}
 Taking the square on both sides of (\ref{eq:masstwilighteffext}) gives:
   \begin{align}
& \chi\{\|\bm{V}_k\|^2\geq {rk^\upalpha}\}\|\bm{V}_k\|^2\leq \sum_{i=1}^2 4\chi\{\|\bm{\Psi}_k(i)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(i)\|^2\notag\\
 &+8\chi\{\|\bm{\Psi}_k(1)\|^2\geq {rk^\upalpha}/4\}\chi\{\|\bm{\Psi}_k(2)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(1)\|\|\bm{\Psi}_k(2)\|.
 \label{eq:ffrustratingg}
 \end{align}
Taking the expectation on both sides of (\ref{eq:ffrustratingg}) and using the definition of $\upsigma_{k,r}^2$:
 \begin{align}
&\upsigma_{k,r}^2\leq  \sum_{i=1}^2 4E\Big[\chi\{\|\bm{\Psi}_k(i)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(i)\|^2\Big]\notag\\
&+8E\Big[\chi\{\|\bm{\Psi}_k(1)\|^2\geq {rk^\upalpha}/4\}\chi\{\|\bm{\Psi}_k(2)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(1)\|\|\bm{\Psi}_k(2)\|\Big].
\label{eq:kriganwreckgerudo}
\end{align}
By assumption, however, $\lim_{k\rightarrow \infty}E\left[\chi\{\|\bm{\Psi}_k(i)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(i)\|^2\right]= 0$. Therefore, (\ref{eq:kriganwreckgerudo}) becomes:
  \begin{align}
  \label{eq:cawcawsquak}
\upsigma_{k,r}^2\leq o(1)+8E\Big[\chi\{\|\bm{\Psi}_k(1)\|^2\geq {rk^\upalpha}/4\}\chi\{\|\bm{\Psi}_k(2)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(1)\|\|\bm{\Psi}_k(2)\|\Big],
\end{align}
where $o(\cdot)$ denotes the standard little-$o$ notation. Next, using the Cauchy--Schwarz inequality:
\begin{align}
&E\Big[\chi\{\|\bm{\Psi}_k(1)\|^2\geq {rk^\upalpha}/4\}\chi\{\|\bm{\Psi}_k(2)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(1)\|\|\bm{\Psi}_k(2)\|\Big]\leq\notag\\
&\left(E\Big[\chi\{\|\bm{\Psi}_k(1)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(1)\|^2\Big]\right)^{1/2}\left(E\Big[\chi\{\|\bm{\Psi}_k(2)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(2)\|^2\Big]\right)^{1/2}.
\label{eq:onceagainherewegooooo}
\end{align}
Once again, since $\lim_{k\rightarrow \infty}E\left[\chi\{\|\bm{\Psi}_k(i)\|^2\geq {rk^\upalpha}/4\}\|\bm{\Psi}_k(i)\|^2\right]= 0$, combining (\ref{eq:cawcawsquak}) and (\ref{eq:onceagainherewegooooo}) implies $\upsigma_{k,r}^2=o(1)$, as desired.
%
\end{proof} 




The following theorem gives conditions for the asymptotic normality of the normalized iterates from Algorithm \ref{kirkey}.

\begin{theorem}
\label{thm:fnogg}
%All probabilistic arguments are meant to hold w.p.1 unless stated otherwise.
Let $\hat{\bm{\uptheta}}_k$ be generated according to Algorithm \ref{kirkey}. Additionally, let $\mathcal{F}_k$ denote the sigma field generated by $\{\hat{\bm{\uptheta}}_\ell\}_{\ell=0}^k$ as well as by any random variables generated  by the algorithm in the production of $\hat{\bm{\uptheta}}_k$. Let $\bm{W}_k=\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast$, let $\upbeta$, $\upalpha$, $\bm\Gamma_k$, $\bm{T}_k$, $\bm\Phi_k$, and $\bm{V}_k$ be defined as in (\ref{eq:goingcrazyhim})--(\ref{eq:pantyponcho}) and assume these variables have real-valued entries. Additionally, assume the following conditions hold:
%\begin{align*}
%&{\text{$\bm{U}_k$, $\bm{V}_k$, $\bm{T}_k$, and $\bm{T}$ be vectors in $\mathbb{R}^p$,}}\\
%&{\text{$\bm\Gamma_k$, $\bm\Phi_k$, $\bm\Sigma$, $\bm\Gamma$, $\bm\Phi$, and $\bm{P}$ be matrices in $\mathbb{R}^{p\times p}$.}}
%\end{align*} 
\begin{DESCRIPTION}
\item[C0] $L(\bm\uptheta)$ is twice continuously differentiable, $\bm{H}(\bm\uptheta)$ (the Hessian of $L(\bm\uptheta)$) has bounded entries (i.e., $\bm{g}(\bm\uptheta)$ is Lipschitz continuous), and $\hat{\bm\uptheta}_k^{(I_{z,i})}\rightarrow \bm\uptheta^\ast$ w.p.1 uniformly over $z$ and $i$.
\item[C1] For each $j$,  $a_k^{(j)}>0$ and $k^\upalpha {a}_k^{(j)}\rightarrow r_j<\infty$.
\item[C2] There exists  an upper triangular matrix $\bm{U}\in \mathbb{R}^{p\times p}$ with strictly positive eigenvalues and a nonsingular matrix $\bm{S}\in \mathbb{R}^{p\times p}$ such that
\begin{align}
\label{eq:macnealhuh}
\bm\Gamma\equiv \sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)} \bm{J}^{(j(z))}(\bm\uptheta^\ast)=\bm{SUS}^{-1},
%\sum_{j=1}^d q_jr_j\bm{J}^{(j)}(\bm\uptheta^\ast)=
\end{align}
where $\bm{J}^{(j)}(\bm\uptheta)$ denotes the Jacobian of $\bm{g}^{(j)}(\bm\uptheta)$.
\item[C3] $\upbeta$ and $\upalpha$ satisfy $0<\upbeta\leq \upalpha$. Additionally, for all $j$ there exist a finite vector $\bm{b}^{(j)}\in \mathbb{R}^p$ such that $k^{\upbeta/2}{\bm{\upbeta}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\rightarrow \bm{b}^{(j(z))}$ w.p.1 uniformly over $z$ and $i$.
%\begin{description}
%\item[(a)] $k^{\upbeta/2}{\bm{\upbeta}}^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\rightarrow \bm{b}^{(j(z))}$ w.p.1
%\item[(b)] $k^{\upbeta/2}E[{\bm{\upbeta}}^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)]\rightarrow \bm{b}^{(j(z))}$.
%\end{description}
%One of the following holds:
%\begin{description}
%\item[(a)] $\upbeta<\upalpha$ and $k^{\upbeta/2}{\bm{\upbeta}}^{(j)}(\hat{\bm{\uptheta}}_k)\rightarrow \bm{b}^{(j)}$ w.p.1 for all $j$ where $\bm{b}^{(j)}\in \mathbb{R}^p$ is finite.
%\item[(b)] $\upbeta= \upalpha$ and $\bm\upbeta^{(j)}(\hat{\bm{\uptheta}}_k)=\bm{0}$ for all $j$ and $k$ so that $k^{\upbeta/2}{\bm{\upbeta}}^{(j)}(\hat{\bm{\uptheta}}_k)\rightarrow \bm{b}^{(j)}=\bm{0}$.
%\end{description}
\item[C4] For all $z$ and $i$,
% the vector ${\bm{\upxi}}^{(j)}(\hat{\bm{\uptheta}}_k)$ is independent of $\mathcal{F}_k$, of ${}\mathcal{X}\{j_k=j\}$, and of $\{\bm\upbeta^{(i)}(\hat{\bm{\uptheta}}_\ell)\}_{\ell,i}$ for $\ell=1,\dots, k$ and $i=1,\dots, d$.
%%and of all bias terms up to (and including) the bias produced during the $k$th iteration. 
%We write ${\bm{\upxi}}^{(j)}(\hat{\bm{\uptheta}}_k)={\bm{\upxi}}^{(j)}_k$. 
  $E\left[{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\Big|\hat{\bm\uptheta}_k^{(I_{z,i})}\right]=\bm{0}$.
%   and the vectors $\{{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\}_{z,i}$ are conditionally uncorrelated (i.e., their conditional covariance matrix is the zero matrix) given $\mathcal{F}_k$ (see p. \pageref{pageref:melclts} for a weaker condition).
%Additionally, ${\bm{\upxi}}^{(j)}_k$ and ${}\mathcal{X}\{j_k=j\}$ are independent random variables.
\item[C5]  For all $z$ there exists a constant $C>0$ and a matrix $\bm\Sigma^{(j)}$ such that one of the following holds w.p.1 (convergence is meant uniformly over $i$):
\begin{enumerate}[label=(\roman*)]
\item $\upbeta=\upalpha$, $C>\|E[{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)[{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)]^\top|\mathcal{F}_k]-\bm\Sigma^{(j(z))}\|\rightarrow 0$.
\item $\upbeta<\upalpha$, $C>\|k^{\upbeta-\upalpha}E[{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)[{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)]^\top|\mathcal{F}_k]-\bm\Sigma^{(j(z))}\|\rightarrow 0$.
\end{enumerate}
Additionally, if $\bm{v}_1$ and $\bm{v}_2$ are two different elements of $\{{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\}_{z,i}$, then one of the following holds w.p.1:
\begin{enumerate}[label=(\roman*)]
\setcounter{enumi}{2}
\item C5-(i) holds and $C>\|E[\bm{v}_1\bm{v}_2^\top|\mathcal{F}_k]\|\rightarrow 0$.
\item C5-(ii) holds and $C>\|k^{\upbeta-\upalpha}E[\bm{v}_1\bm{v}_2^\top|\mathcal{F}_k]\|\rightarrow 0$.
\end{enumerate}
%
% are conditionally uncorrelated (i.e., their conditional covariance matrix is the zero matrix) given $\mathcal{F}_k$ (see p. \pageref{pageref:melclts} for a weaker condition).
%
% and the vectors $\{{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\}_{z,i}$ are conditionally uncorrelated (i.e., their conditional covariance matrix is the zero matrix) given $\mathcal{F}_k$ (see p. \pageref{pageref:melclts} for a weaker condition).
\item[C6] $\bm\Sigma\equiv \sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)}^2 {\bm\Sigma}^{(j(z))}$ is a positive definite matrix.
\item[C7] For each $z=1,\dots, s$ and $i=1,\dots, n(z)$ one of the following holds:
\begin{enumerate}[label=(\roman*)]
\item$\upbeta=\upalpha$ and B5-(i) holds with $\bm{V}_k$ replaced by ${\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)$.
\item $\upbeta<\upalpha$ and B5-(i) holds with $\bm{V}_k$ replaced by $k^{(\upbeta-\upalpha)/2}{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)$.
\end{enumerate}
% For $0< \upalpha\leq 1$ define $\upsigma_{k,r,z}^2\equiv E{\mathcal{X}}\{\|{\bm{\upxi}}^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\|^2\geq rk^\upalpha\}\|{\bm{\upxi}}^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\|^2$ does not depend on $i$. For every $r>0$ and $z=1,\dots,s$ either:
%\begin{align}
%\label{eq:foreveryr}
%{\text{$\lim_{k\rightarrow \infty}\upsigma_{k,r,z}^2=0$ or $\upalpha=1$ and $\lim_{n\rightarrow \infty}n^{-1}\sum_{k=1}^n\upsigma^2_{k,r,z}=0$.}}
%\end{align}
\item[C8] The same as B6$'$.
\end{DESCRIPTION}
%
Then, 
%using the notation from Theorem \ref{thm:generalizefabian} we can let:
%\begin{align*}
%\bm\Gamma
%\end{align*}
the asymptotic distribution of $k^{\upbeta/2}\bm{W}_k$ is a multivariate normal random variable with mean $\bm{S}\bm\upnu$ and covariance matrix $\bm{SQS}^\top$, where the entries of $\bm\upnu$ are the unique solution to (\ref{eq:okayfine})
% \begin{align*}
%\Delta_{k}^{[i]}\rightarrow\upnu^{[i]}=  (\tilde{{U}}^{[i,i]})^{-1}\left[\tilde{{T}}^{[i]}-\sum_{j=i+1}^p \tilde{U}^{[i,j]}\upnu^{[j]}\right],
%\end{align*}
with $\tilde{\bm{T}}=-\bm{S}^{-1}\left[\sum_{z=1}^{s}\sum_{\ell=0}^{n_(z)-1}r_{j(z)}\bm{b}^{(j(z))}\right]$ and $\tilde{\bm{U}}=\bm{U}-(\upbeta_+/2)\bm{I}$, and the entries of $\bm{Q}$ are the unique solution to (\ref{eq:nolookback}) with $\tilde{\bm{U}}$ defined as above and $\bm\Phi=\bm{I}$.
% \begin{align*}
%Q^{[i,j]}_{k+1}=&\ (1-k^{-\upalpha}[\tilde{U}^{[i,i]}+\tilde{U}^{[j,j]}])Q^{[i,j]}_k-k^{-\upalpha}\left[\sum_{\ell=1}^{j-1} \tilde{U}^{[j,\ell]}Q^{[i,\ell]}_k+\sum_{\ell=i+1}^{p} \tilde{U}^{[i,\ell]}Q^{[\ell,j]}_k\right]\notag\\
%&+k^{-\upalpha}\left[o(1)+\tilde{\Sigma}^{[i,j]}\right].
%\end{align*}
%with $\tilde{\bm{U}}$ as above and $\tilde{\bm{\Sigma}}=\bm{S}^{-1}\bm{\Sigma}(\bm{S}^{-1})^\top$.
\end{theorem}


\begin{proof}
We show that conditions B0$'$--B6$'$ hold. The result then follows from Theorem \ref{thm:generalizefabian}. First, note that condition B0$'$ holds by the definition of $\bm\Phi_k$, $\bm{\Gamma}_k$, $\bm{V}_k$, and $\mathcal{F}_k$. Next, we show that B1$'$ holds. First, by C0 and C1:
\begin{align*}
\lim_{k\rightarrow \infty}\bm\Gamma_k&=\lim_{k\rightarrow \infty}k^\upalpha\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}(\overline{\bm\uptheta}_k)=\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)}\bm{J}^{j(z)}(\bm\uptheta^\ast){\text{ w.p.1.}}
\end{align*}
Then, C2 guarantees B1$'$ holds with $\bm\Gamma$ equal to the matrix in (\ref{eq:macnealhuh}). The fact that B2$'$ holds follows immediately from the fact that $\bm\Phi_k=\bm{I}$ for all $k$, so that $\bm\Phi$ in B1$'$ is equal to the identity matrix. Next we show that B3$'$ holds.

First, using C1 and C3 it follows that
\begin{align}
- \lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} {\bm{\upbeta}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\right)=-\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1}r_{j(z)}\bm{b}^{(j(z))}{\text{ w.p.1.}}
\label{eq:timetowos}
\end{align}
Next, C0, C1, and C3 imply that
\begin{align}
&\lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right)[\bm\Delta_{\bm{g}}^{(I_{z,\ell})}+\bm\Delta_{\bm{\upbeta}}^{(I_{z,\ell})}]\notag\\
&=\lim_{k\rightarrow \infty} k^{\upalpha +\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} O(k^\upalpha) \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right)o(k^\upalpha)\notag\\
&=\bm{0}{\text{ w.p.1.}}
\label{eq:mosestron}
\end{align}
Lastly, by C0 (the boundedness of $\bm{H}(\bm\uptheta)$), C1, C3 (using $0<\upbeta\leq \upalpha$), and C5:
\begin{align}
&\lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\Bigg\|\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} E\Big[\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big|\mathcal{F}_k\Big]\Bigg\|\notag\\
%&\leq \lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \Big\|E\Big[\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big|\mathcal{F}_k\Big]\Big\|\notag\\
&\leq \lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \left(E\Big[\Big\|\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big\|^2\Big|\mathcal{F}_k\Big]\right)^{1/2}\notag\\
&\leq\lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} O(k^{\upalpha})\left(E\left[\Big\|\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right)\Big\|^2\Big\| \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big\|^2\Big|\mathcal{F}_k\right]\right)^{1/2}\notag\\
&\leq \lim_{k\rightarrow \infty}k^{\upalpha+\upbeta/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1}O(k^{\upalpha})\Big[E\Big\| \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big\|^2\Big|\mathcal{F}_k\Big]^{1/2}\notag\\
&={0}{\text{ w.p.1}},
\label{eq:listeningtozeldeeee}
\end{align}
where the first inequality in (\ref{eq:listeningtozeldeeee}) follows from the triangle inequality and the fact that $\|E[\bm{v}]\|^2\leq E\|\bm{v}\|^2$ for $\bm{v}\in \mathbb{R}^p$ so that $\|E[\bm{v}]\|\leq \sqrt{E\|\bm{v}\|^2}$, the third inequality follows from the submultplicativity of the Frobenius norm ($\|\cdot\|$ applied to a matrix is the Frobenius norm), and the last inequality follows from the boundedness of the the Hessian (which implies the boundedness of $\bm{J}^{(j)}(\bm\uptheta)$). 
% H\"older's inequality (Chung 2001) and 
%
Thus, the definition of $\bm{T}_k$ in (\ref{eq:goingcrazyhim}) along with (\ref{eq:timetowos})--(\ref{eq:listeningtozeldeeee}) imply
\begin{align}
\bm{T}_k\rightarrow -\sum_{z=1}^{s}\sum_{\ell=0}^{n_(z)-1}r_{j(z)}\bm{b}^{(j(z))}{\text{ w.p.1.}}
\label{eq:nobrothersand}
\end{align}
This implies B3$'$ holds with $\bm{T}$ defined as in the right-hand side of (\ref{eq:nobrothersand}). Next we show B4$'$ holds. 

That $E[\bm{V}_k|\mathcal{F}_k]=\bm{0}$ follows immediately from C4. Next we show that there exists a constant $C'<\infty$ such that $C'>\|E[\bm{V}_k\bm{V}_k^\top|\mathcal{F}_k]-\bm\Sigma\|\rightarrow 0$, where $\bm\Sigma$ is as in C6. 
%In order to show this, we rewrite the expression for $\bm{V}_k$ in (\ref{eq:othingcoodsd}) as $\bm{V}_k=\bm{N_1}+\bm{N}_2$ with
%\begin{align*}
%\bm{N}_1=
%\end{align*}
%where 
First, 
%by C0 (the boundedness of the Hessian),
by C1, C4, and C5:
% we know that 
\begin{align}
\label{eq:avatarparticulatsfs}
C_1>\Bigg\|\Var{\Bigg[k^{(\upalpha+\upbeta)/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} {\bm{\upxi}}_k^{(j(z))}\left(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\right)\Bigg|\mathcal{F}_k\Bigg]}-\bm\Sigma\Bigg\|\rightarrow 0,
\end{align}
for some constant $C_1<\infty$. (Note that the vector inside the variance in the previous equation has mean zero by the first part of condition C4. Therefore, its variance is equal to its second moment matrix.)  Next, by the definition of $\bm\Delta_{\bm\upxi}^{(\cdot)}$ in (\ref{eq:futuramasohs}) and using conditions C0, C1, and C5 it follows that there must exist a constant $C_2<\infty$ such that:
\begin{align}
\label{eq:doughiesloon}
C_2>\Bigg\|\Var{\Bigg[k^{(\upalpha+\upbeta)/2}\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} {a}_{k}^{(j(z))} \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Bigg|\mathcal{F}_k\Bigg]}\Bigg\|\rightarrow 0.
\end{align}
%
%along with (\ref{eq:avatarparticulatsfs}) and the definition of $\bm{V}_k$
%
From (\ref{eq:avatarparticulatsfs}) we see that the second moment matrix of the first line of (\ref{eq:othingcoodsd}) is bounded and converges to $\bm\Sigma$. Additionally, (\ref{eq:doughiesloon}) says that the second moment matrix of the last two lines of (\ref{eq:othingcoodsd}) is bounded and converges to the zero matrix. Furthermore, any cross-term expectation involving a summand from the first line of (\ref{eq:othingcoodsd}) and a summand from the second or third line of (\ref{eq:othingcoodsd}) is also bounded and converges to the zero matrix due to the fact that:
%Next, by C5:
% (the boundedness of the second moments of the noise terms):
\begin{align*}
k^{\upbeta-\upalpha} O(k^{-\upalpha})\left(E\Big\|{\bm{\upxi}}_k^{(j(z))}\Big(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\Big)\Big|\mathcal{F}_k\Big\|^2\right)^{1/2}\left(E\Big\|{\bm{\upxi}}_k^{(j(m))}\Big(\hat{\bm\uptheta}_k^{\left(I_{m,i}\right)}\Big)\Big|\mathcal{F}_k\Big\|^2\right)^{1/2}=o(1),
%\notag\\
%&=k^{\upbeta-\upalpha}{\text{trace}}\Big\{E\Big[{\bm{\upxi}}_k^{(j(z))}\Big(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\Big){\bm{\upxi}}_k^{(j(z))}\Big(\hat{\bm\uptheta}_k^{\left(I_{z,\ell}\right)}\Big)\Big|\mathcal{F}_k\Big]^\top\Big\}\notag\\
%&\times O(k^{-2\upalpha}){\text{trace}}\Big\{E\Big[{\bm{\upxi}}_k^{(j(m))}\Big(\hat{\bm\uptheta}_k^{\left(I_{i,i}\right)}\Big){\bm{\upxi}}_k^{(j(m))}\Big(\hat{\bm\uptheta}_k^{\left(I_{m,i}\right)}\Big)\Big|\mathcal{F}_k\Big]^\top\Big\}\notag\\
%
%\left( \bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}-E\Big[\bm{J}^{(j(z))}\left(\overline{\bm\uptheta}_k^{(I_{z,\ell})}\right) \bm\Delta_{\bm\upxi}^{(I_{z,\ell})}\Big|\mathcal{F}_k\Big]\right)
\end{align*}
a consequence of C5. In conclusion, $E[\bm{V}_k\bm{V}_k^\top|\mathcal{F}_k]$ is equal to the sum of finite number of bounded matrices, most of which converge to the zero matrix w.p.1 except for one matrix (the matrix in the variance of equation \ref{eq:avatarparticulatsfs}) which converges to $\bm\Sigma$ w.p.1. Therefore, there exists a constant $C'<\infty$ such that $C'>\|E[\bm{V}_k\bm{V}_k^\top|\mathcal{F}_k]-\bm\Sigma\|\rightarrow 0$ and B4$'$ holds.

It remains to show that B5$'$ and B6$'$ hold. First, conditions C0 and C7 imply $\bm{V}_k$ 
%is the (finite) sum of several terms, each of which satisfies B5-(i). Then, 
satisfies the conditions of Lemma \ref{lem:piccardo}. Therefore, by Lemma \ref{lem:piccardo} the vector $\bm{V}_k$ satisfies B5-(i) (a special case of B5$'$). Lastly, since C8 and B6$'$ are identical, condition B6$'$ is automatically satisfied. Since we have shown that conditions C0--C8 imply B0$'$--B6$'$ are satisfied, the conclusion of Theorem \ref{thm:generalizefabian} holds and the desired result follows from said theorem.
%It follows that $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)$ is asymptotically normally distributed with the desired mean and covariance.
\end{proof}




\section[On the Conditions for Normality]{On the Conditions for Normality}
\label{sec:bonestrailseason}

Theorem \ref{thm:fnogg} stated a set of conditions for the asymptotic normality of the scaled iterates from Algorithm \ref{kirkey} (conditions C0--C8). This section discusses the validity of these conditions. 

{\underline{\it{Condition C0}}}. One of the assumptions of this condition is that the Hessian of $L(\bm\uptheta)$, $\bm{H}(\bm\uptheta)$, must be bounded uniformly over $\bm\uptheta$. This is certainly a stronger assumption than condition A0 which only requires $L(\bm\uptheta)$ to be twice-continuously differentiable. 
%The boundedness of the Jacobian
 Condition C0 also assumes that $\hat{\bm\uptheta}_k^{(I_{z,i})}\rightarrow \bm\uptheta^\ast$ w.p.1 uniformly over $z$ and $i$, this assumption is satisfied under the conditions of Theorem \ref{thm:hoeshoo} (see Corollary \ref{eq:idamagedittarantatan}). 

{\underline{\it{Condition C1}}}. Note that this condition is a special case of the assumption from A0$''$ requiring $a_k^{(j)}/a_k\rightarrow r_j$ (condition C1 replaces $a_k$ with $k^{-\upalpha}$). As discussed in Section \ref{sec:discussconvergence}, C1 would be satisfied by sequences of the form $a_k^{(j)}=a^{(j)}/(1+k+A^{(j)})^\upalpha$ where $a^{(j)}$ and $A^{(j)}$ are both strictly-positive constants. 

{\underline{\it{Condition C2}}. This condition requires $\bm\Gamma=\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)} \bm{J}^{(j(z))}(\bm\uptheta^\ast)
$
%\begin{align*}
%\bm\Gamma=\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)} \bm{J}^{(j(z))}(\bm\uptheta^\ast)
%\end{align*}
to be equal to $\bm{SUS}^{-1}$ where $\bm{S}$ and $\bm{U}$ are both real matrices and $\bm{U}$ is positive-definite and upper-triangular. In order to discuss whether this is a reasonable assumption, note that $\bm{J}^{(j)}(\bm\uptheta^\ast)\in \mathbb{R}^{p\times p}$ is a matrix formed by taking $\bm{H}(\bm\uptheta^\ast)$ and replacing the rows in the set $\mathcal{S}_j$, as defined in (\ref{eq:notexclusive}), with zeros. If $\bm{H}(\bm\uptheta^\ast)$ is positive definite, one situation in which C2 holds is when $r_j>0$ for all $j$ and the $\mathcal{S}_j$ are disjoint sets (it is important to note that having this sets be disjoint is not a necessary condition). Then,
\begin{align}
\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)} \bm{J}^{(j(z))}(\bm\uptheta^\ast)=\sum_{j=1}^d r_j d_j\bm{J}^{(j)}(\bm\uptheta^\ast)
\label{eq:parisorny}
\end{align}
where $d_j= \sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1}{}\chi\{j(z)=j\}$. The variable $d_j$ represents the (deterministic) number of times the $j$th subvector is updated during the $k$th iteration. Provided $r_jd_j>0$, (\ref{eq:parisorny}) can be rewritten as follows:
\begin{align}
\label{eq:sensorypinetree}
\sum_{j=1}^d r_j d_j\bm{J}^{(j)}(\bm\uptheta^\ast)=\bm{\Lambda}\bm{H}(\bm\uptheta^\ast),
\end{align}
where the matrix $\bm{\Lambda}$ is a positive definite diagonal matrix with $i$th diagonal entry equal to $r_jd_j$ where $j$ satisfies $i\in \mathcal{S}_j$ (recall that in this example $i$ lies in $\mathcal{S}_j$ for exactly one $j$ since the sets $\mathcal{S}_j$ are disjoint). Then, as proven in Proposition \ref{prop:sandpipercrossing}, condition C2 holds. Note that having $r_jd_j>0$ implies that $k^\upalpha a_k^{(j)}\rightarrow r_j>0$ and that each subvector must be updated at least once per iteration.

{\underline{\it{Condition C3}}. In the case where the noisy gradient estimates in Algorithm \ref{kirkey} are obtained in using the SG estimates (see, for example, Section \ref{sec:ay}) the bias term is equal to zero. Therefore, in this case we can assume ${\bm{\upbeta}}^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)=\bm{0}$ so that C3 holds with $\bm{b}^{(j(z))}=\bm{0}$. When the noisy gradient estimates are obtained in an SPSA manner (see, for example, Section \ref{sect:cspsa}) the bias terms ${\bm{\upbeta}}^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)$ cannot be assumed to be equal to the zero vector. However, analogous conditions to those of Proposition 2 in Spall (1992)\nocite{spall1992} (after an natural adaptation for the setting of Algorithm \ref{kirkey}) can be used to show that the bias terms satisfy  C3 when the noisy gradient updates are obtained in the manner of (\ref{eq:shmasdfg})--(\ref{eq:splice}) or in the manner of (\ref{eq:howeardspos1})--(\ref{eq:howeardspos2}).


{\underline{\it{Condition C4}}. The mean-zero assumption of the noise terms is a common assumption throughout the SA literature. The assumption essentially requires the conditional mean of the noise term (conditional on $\hat{\bm\uptheta}_k^{(I_{z,i})}$) to be absorbed into the bias term ${\bm{\upbeta}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)$. Condition C3 would then require the conditional mean of the noise terms to converge to the zero vector.


{\underline{\it{Condition C5}}. Condition C5 allows for two possible scenarios. The first case, C5-(i), requires the noise vectors to have a bounded conditional covariance matrix which converges w.p.1. A simple scenario in which this holds is when the noise vectors are based on independent multivariate Gaussians with mean vector equal to zero and covariance matrix equal to $\bm{I}$. Condition C5-(ii), on the other hand, allows the noise terms to have a growing (in magnitude) conditional covariance matrix. The amount of growth, however, must be proportional to $k^{\upalpha-\upbeta}$. This condition is well suited for algorithms such as SPSA where the conditional covariance of the noise grows as $k\rightarrow \infty$ (e.g., Spall 1992)\nocite{spall1992}. Conditions C5-(iii) and C5-(iv) are similar to C5-(i) and C5-(ii), respectively. Loosely speaking, C5-(iii) requires any two different noise vectors to be asymptotically uncorrelated while C5-(iv) allows the magnitude of the correlation to increase at a rate proportional to $k^{\upalpha-\upbeta}$. One scenario where conditions C5-(iii) and C5-(iv) are satisfied is when the noise terms are independent of each other. Section \ref{sec:hannahashley} gives an example of where the noise terms are not independent but where C5-(iv) holds.


{\underline{\it{Condition C6}}}. This condition requires $\bm\Sigma=\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)} {\bm\Sigma}^{(j(z))}$
%\begin{align*}
%\bm\Sigma=\sum_{z=1}^{s}\sum_{\ell=0}^{n(z)-1} r_{j(z)} {\bm\Sigma}^{(j(z))}
%\end{align*}
to be positive definite. Let us give an example of when this condition may hold. If the sets $\mathcal{S}_j$ are disjoint (i.e., that the subvectors to update do not overlap) then with $d_j$ defined as in (\ref{eq:sensorypinetree}): 
\begin{align*}
\bm\Sigma=\sum_{j=1}^d r_j d_j\bm{\Sigma}^{(j)}
\end{align*}
(note that each matrix $\bm{\Sigma}^{(j)}$ has zeros in the columns and rows whose indices are not in $\mathcal{S}_j$). If the submatrix of $\bm{\Sigma}^{(j)}$ formed by taking the rows and columns with indices $\mathcal{S}_j$ is positive definite (i.e., assume the limiting conditional covariance matrix of the nonzero entries of $\bm\upxi_k^{(j)}$ is positive definite, a reasonable assumption) and if we also assume $r_jd_j>0$ then $\bm\Sigma$ would be a block-diagonal positive definite matrix and C6 would be satisfied. Having $r_jd_j>0$ requires each subvector to be updated at least once per iteration and $k^\upalpha a_k^{(j)}\rightarrow r_j>0$.

{\underline{\it{Conditions C7 and C8}}}. Conditions C7 and C8 are assumptions that are often applied to non-cyclic SA algorithms. C7 pertains to the uniform integrability of the squared magnitude of $\{{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)\}$ or $k^{(\upbeta-\upalpha)/2}{\bm{\upxi}}_k^{(j(z))}\big(\hat{\bm\uptheta}_k^{(I_{z,i})}\big)$ (see Definition \ref{def:unifintegrable}). A sufficient condition for C7 to hold is if the traces of the covariance matrices of the a noise terms are bounded uniformly over $k$. Condition C8 is impossible to verify in practice although we note that C8 is essentially identical to condition B6 of Fabian's theorem (see p. \pageref{page:scratchless}).





\section{Concluding Remarks}
\label{sec:dontmeanthings}

This chapter presented a generalization of Fabian's theorem (see Theorem 2.2 in Fabian 1968 or Theorem \ref{thm:fabian} in this dissertation)\nocite{fabian1968}. The resulting generalization (Theorem \ref{thm:generalizefabian}) was used to prove the asymptotic normality of the normalized iterates form Algorithm \ref{kirkey} (a few additional applications of Theorem \ref{thm:generalizefabian} are discussed in Appendix \ref{sec:fabiansecgeneralize}). Attempting to use Theorem \ref{thm:generalizefabian} to derive an asymptotic normality result for Algorithm \ref{beastwasdone} gives rise to a critical complication.
% which we review here. 
 First, note that when $L(\bm\uptheta)$ is twice continuously differentiable then:
%
%%Furthermore,  $\bm{M}_k^{(j_k(z))}\rightarrow \bm{0}$ w.p.1. Thus, it would suffice for $s_k$, $n_k(z)$, and $k^\upalpha\tilde{A}_{k}(z)$ to be bounded w.p.1 for $\bm\Gamma_k$ to converge. 
%A more precise analysis will be performed later in this section (see the proof of Theorem \ref{thm:gcssanormal}).
%where $M_k^{(j_k(z))}$ is such that:
%\begin{align*}
%\bm{J}^{(j_k(z))}(\overline{\bm\uptheta}_k)=\bm{J}^{(j_k(z))}(\overline{\overline{\bm\uptheta}}_k)+M_k^{(j_k(z))}.
%\end{align*}
%Then,
\begin{align}
\label{eq:noealnavyyard}
 \hat{\bm{\uptheta}}_{k+1}=&\ \hat{\bm\uptheta}_k-\tilde{a}_{k}^{(j_k)} \bm{J}^{(j_k)}(\overline{\bm\uptheta}_k)(\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast)- \tilde{a}_{k}^{(j_k)} {\bm{\upbeta}}_k^{(j_k)}(\hat{\bm{\uptheta}}_k)- \tilde{a}_{k}^{(j_k)} {\bm{\upxi}}_k^{(j_k)}(\hat{\bm{\uptheta}}_k),
 \end{align}
%
 where $\hat{\bm{\uptheta}}_k$ denotes an iterate from Algorithm \ref{beastwasdone} and where the $i$th row of $\bm{J}^{(j)}(\overline{\bm\uptheta}_k)$ is equal to the $i$th row of $\bm{J}^{(j)}(\bm\uptheta)$ evaluated at $\bm\uptheta=(1-\uplambda_i)\hat{\bm{\uptheta}}_k+\uplambda_i\bm\uptheta^\ast$ for some $\uplambda_i\in[0,1]$ which depends on $\hat{\bm{\uptheta}}_k$. Then, (\ref{eq:noealnavyyard}) may be written in the form of (\ref{eq:alien}) by letting $\bm{W}_k=\hat{\bm{\uptheta}}_k-\bm\uptheta^\ast$, $\bm\Gamma_k=k^\upalpha\tilde{a}_{k}^{(j_k)} \bm{J}^{(j_k)}(\overline{\bm\uptheta}_k)$, $\bm{T}_k=-k^{\upalpha+\upbeta/2}\tilde{a}_{k}^{(j_k)} {\bm{\upbeta}}_k^{(j_k)}(\hat{\bm{\uptheta}}_k)$, $\bm\Phi_k=\bm{I}$, and $\bm{V}_k=-k^{(\upalpha+\upbeta)/2}\tilde{a}_{k}^{(j_k)} {\bm{\upxi}}_k^{(j_k)}(\hat{\bm{\uptheta}}_k)$. Note, however, that $\bm\Gamma_k$ does not converge w.p.1 to any matrix since the random variable $j_k$ does not converge. Therefore, Theorem \ref{thm:generalizefabian} cannot be used to derive an asymptotic normality result for (\ref{eq:noealnavyyard}) for this definition of $\bm\Gamma_k$. Moreover, as discussed in pp. \pageref{eq:anotherpagerefgoeshere}--\pageref{prop:sandpipercrossing}, it is not generally possible to find an alternate definition of $\bm\Gamma_k$ (along with a redefinition of $\bm{T}_k$, $\bm{\Phi}_k$, and $\bm{V}_k$) so that all of the conditions of Fabian's conditions hold without imposing more assumptions on $\hat{\bm{\uptheta}}_k$. Future research could consider combining Algorithm \ref{kirkey} with iterate averaging, which may lead to the asymptotic normality of the normalized iterates.







==> thesis arXiv 2/chapter4.tex <==
%!TEX root = root.tex

\chapter[Generalizations: Non-Cyclic Behavior]{Generalizations:\\ Non-Cyclic Behavior}
\label{sec:gen1}
\chaptermark{First Generalizations}

In this section, we provide conditions for the convergence of a non-seesaw generalization of CSG and CSPSA to a minimizer $\bm\uptheta^\ast$ of $L(\bm\uptheta)$. In these generalizations it is assumed that each subvector will be updated infinitely often (i.o.) w.p.1. While a strictly alternating (strictly seesaw) algorithm satisfies the assumption of updating each subvector i.o., the assumption allows for more general behavior. For example, if at each step a choice of whether to update the first subvector or the second is made according to a $\text{Bernoulli}(p)$ distribution with $0<p<1$ then the i.o. assumption will also be satisfied.

First we clarify that  our generalization to non-seesaw behavior {\it{includes}}, as a particular case, the cyclic seesaw case as discussed in the opening paragraph of this section. We will be assuming each subvector is updated i.o. w.p.1. For example, the sequence of updates could look something like:
\begin{align}
\label{eq:newnot}
\bm\uptheta(0){\overset{j_0}{\longrightarrow}}\bm\uptheta(1)\overset{j_1}{\longrightarrow} \bm\uptheta(2)\overset{j_2}{\longrightarrow} \bm\uptheta(3)\overset{j_3}{\longrightarrow} \cdots
\end{align}
%For simplicity we deviate from our usual notation involving ``intermediate'' updates and use the following instead:
%\begin{align}
%\bm{{\hat{\uptheta}}}_{0}{\overset{j_0}{\longrightarrow}} \bm{{\hat{\uptheta}}}_{1}\overset{j_1}{\longrightarrow} \bm{{\hat{\uptheta}}}_{2}\overset{j_2}{\longrightarrow} \bm{{\hat{\uptheta}}}_{3}\overset{j_3}{\longrightarrow} \cdots
%\end{align}
where $j_k\in\{0,1\}$. Eqn. (\ref{eq:newnot}) will be taken to mean that $\bm\uptheta(k+1)$ was obtained from $\bm\uptheta(k)$ by updating its $j_k$th subvector (recall $j_k$ will either be 1 or 2 to indicate whether the first or second subvector is updated). At each subiterateion, a decision is made to update the first or the second subvectors of the current estimate. As an example, consider the following sequence:
%To further clarify the change of notation, consider the following sequence generated with our usual (cyclic) notation: 
%Such a situation still assumes the existence of a global clock which keeps track of iteration number, namely $k$. 
%\begin{align*}
%\bm{{\hat{\uptheta}}}_{0}\rightarrow \bm{{\hat{\uptheta}}}_{0}^{(I)}\rightarrow \bm{{\hat{\uptheta}}}_{1}\rightarrow \bm{{\hat{\uptheta}}}_{1}^{(I)}\rightarrow\cdots
%\end{align*}
%In the new notation we would simply have:
\begin{align}
\label{eq:sampseq}
\bm\uptheta(0){\overset{1}{\longrightarrow}} \bm\uptheta(1)\overset{2}{\longrightarrow}\bm\uptheta(2)\overset{1}{\longrightarrow} \bm\uptheta(3)\overset{2}{\longrightarrow} \cdots,
\end{align}
the alternating behavior of the $j_k$'s indicates a cyclic seesaw algorithm was used so that:
\begin{align*}
\bm\uptheta(0)=\bm{{\hat{\uptheta}}}_{0},\ \ \bm\uptheta(1)=\bm{{\hat{\uptheta}}}_{0}^{(I)},\ \ \bm\uptheta(2)=\bm{{\hat{\uptheta}}}_{1},\ \ \bm\uptheta(3)=\bm{{\hat{\uptheta}}}_{1}^{(I)}, \cdots
\end{align*}
so that (\ref{eq:sampseq}) is equivalent to:
\begin{align}
\label{eq:simto}
\bm{{\hat{\uptheta}}}_{0}{{\longrightarrow}} \bm{{\hat{\uptheta}}}_{0}^{(I)}{\longrightarrow}\bm{{\hat{\uptheta}}}_{1}{\longrightarrow}\bm{{\hat{\uptheta}}}_{1}^{(I)}{\longrightarrow} \cdots,
\end{align}
Because the generalization discussed in this section does not imply a strictly alternating sequence of updates, another realization could look something like:
\begin{align}
\label{eq:posca}
\bm\uptheta(0){\overset{1}{\longrightarrow}} \bm\uptheta(1)\overset{1}{\longrightarrow} \bm\uptheta(2)\overset{2}{\longrightarrow} \bm\uptheta(3)\overset{2}{\longrightarrow} \cdots,
\end{align}
such a sequence will be represented in the equivalent notation:
\begin{align*}
\bm\uptheta(0)=\bm{{\hat{\uptheta}}}_{0},\ \bm\uptheta(1)=\bm{{\hat{\uptheta}}}_{0}^{(I)_1},\ \bm\uptheta(2)=\bm{{\hat{\uptheta}}}_{0}^{(I)_2}, \bm\uptheta(3)=\bm{{\hat{\uptheta}}}_{1}
\end{align*}
so that similar to the equivalence between (\ref{eq:sampseq}) and (\ref{eq:simto}), we can rewrite (\ref{eq:posca}) as:
\begin{align}
\label{eq:pazaak}
\bm{{\hat{\uptheta}}}_{0}{{\longrightarrow}} \bm{{\hat{\uptheta}}}_{0}^{(I)_1}{\longrightarrow}\bm{{\hat{\uptheta}}}_{0}^{(I)_2}{\longrightarrow}\bm{{\hat{\uptheta}}}_{1}{\longrightarrow} \cdots,
\end{align}
Note that the assumption of updating each subvector i.o. does not imply there is a particular cyclic seesaw pattern and the original notion of intermediate steps is lost.  In general, we will say an iteration is complete as soon as all subvectors have been updated at least once; during the $k$th iteration $\bm{{\hat{\uptheta}}}_{k}$ is obtained via a sequence of updates beginning at $\bm{{\hat{\uptheta}}}_{k-1}$. In the previous sequence we see that during the first iteration, the first subvector was updated twice while the second subvector was only updated once. However, by assumption both subvectors will (eventually) be updated infinitely often w.p.1. 


The proof of convergence  of this method in the setting where each coordinate is updated i.o. w.p.1 is identical to that of Theorem 1. The following sections discuss the generalization in more detail.
\section{Generalization of CSG  to Non-Seesaw Behavior}
\label{subsec:alternatingSG1}

The values $\bm{{\hat{\uptheta}}}_{k}$ in this generalized algorithm obey the following recursion:
\begin{align}
\label{eq:gencsg}
&\bm\uptheta({k+1})=\bm\uptheta(k)-a_{n_k}^{(j_k)}{\bm{Y}}^{(j_k)}(\bm\uptheta(k)),\\
&\bm\uptheta(0)=\bm{{\hat{\uptheta}}}_{0},\\
& \bm{{\hat{\uptheta}}}_{k} {\textnormal{ is defined recursively (see below),}}
\end{align}
where $n_k$ denotes the number of times subvector $j_k$ has been updated by time $k$ (recall that $j_k\in\{0,1\}$ when there are only two subvectors). While $j_k$ allows us to keep track of what gain sequence to use, $n_k$ tells us which element of that gain sequence is required (recall there are two gain sequences corresponding to the two subvectors). Furthermore, $\bm{{\hat{\uptheta}}}_{k}$ is defined recursively: given that $\bm{{\hat{\uptheta}}}_{k}=\bm\uptheta(m_1)$ for some nonnegative integer $m_1$, we have $\bm{{\hat{\uptheta}}}_{k+1}=\bm\uptheta(m_2)$ if $m_2$ is an integer strictly greater than $m_1$  and the sequence:
\begin{align*}
j_{m_1},\ j_{m_1+1},\ j_{m_1+2}, \cdots, j_{m_2}
\end{align*}
is the shortest sequence for $j_k$ beginning at $k=m_1$ that contains at least one $0$ and one $1$. In other words, given that $\bm{{\hat{\uptheta}}}_{k}=\bm\uptheta(m_1)$, the next iterate $\bm{{\hat{\uptheta}}}_{k+1}$ will be determined as soon as each subvector has been updated at least once. Because of this definition, it is possible for the number of subiterations to vary between iterations.

The following theorem states that under the same conditions of theorem 1 we can prove convergence of this generalization of CSG.

\noindent{\bf{Theorem 4}}: Let conditions A0--A4 hold. Furthermore, assume $E[{\bm{Y}}(\bm\uptheta)|\bm\uptheta]={\bm{g}}(\bm\uptheta)$ for all $\bm\uptheta$. Then, the generalization of the CSG algorithm given by eqn.(\ref{eq:gencsg}) to the case where each subvector is updated i.o. w.p.1 (i.e., $j_k=0$ i.o. and $j_k=2$ i.o. w.p.1) converges to $\bm\uptheta^{\ast}$ w.p.1.

\noindent{\it{Proof:}} As usual, all probabilistic arguments will be assumed to hold w.p.1. Given that each coordinate will be updated infinitely often, we know that (w.p.1) a realization:
\begin{align*}
\bm{{\hat{\uptheta}}}_{0}{\overset{j_0}{\longrightarrow}} \bm{{\hat{\uptheta}}}_{1}\overset{j_1}{\longrightarrow} \bm{{\hat{\uptheta}}}_{2}\overset{j_2}{\longrightarrow} \bm{{\hat{\uptheta}}}_{3}\overset{j_3}{\longrightarrow} \cdots
\end{align*}
will have $j_k=1$ infinitely often and $j_k=2$ infinitely often.  Adapting the proof of theorem 1 to the notation in eqn. (\ref{eq:gencsg}) we have:
\begin{align*}
E\left[f(\bm\uptheta(k+1))-f(\bm\uptheta(k))|\bm\uptheta(k)\right]\leq &-{\bm{f'}}(\bm\uptheta(k))^\top\bm{g}^{(j_k)}(\bm\uptheta(k))\left(a_{n_k}^{(j_k)}-b_3\cdot (a_{n_k}^{(j_k)})^2\right)\\
&+b_4\cdot(a_{n_k}^{j_k})^2(1+f(\bm\uptheta(k)).
\end{align*}
Now, we also make another natural adaptation of the notation from the proof of Theorem 1:
\begin{align*}
a_0\equiv a_{n_0}^{(j_0)}, \ a_1\equiv a_{n_1}^{(j_1)}, \ a_2\equiv a_{n_2}^{(j_2)}, \ a_3\equiv a_{n_3}^{(j_3)}, \ \cdots
\end{align*}
and:
\begin{align*}
\upvarphi_k\equiv \upvarphi(\bm\uptheta(k))\equiv\bm{f'}(\bm\uptheta(k))^\top\bm{g}^{(j_k)}(\bm\uptheta(k))
\end{align*}
Using our previous notation for $W_{k}$ and $\upalpha_k$ we derive (in the same manner as in the proof of theorem 1) the inequality:
\begin{align*}
E[W_{k+1}-W_k|\bm\uptheta(k)]\leq -\upalpha_k\upvarphi_k
\end{align*}
 so that $W_k$ is eventually (for $k$ large enough) a nonnegative supermartingale. As before, this implies $f(\bm\uptheta(k))$ has a finite limit. The rest of the proof is identical to that of Theorem 1. \hfill $\Box$
% similarly to ACC-2014, we have:
% \begin{align*}
% &\sum_{j_k=1}\upalpha_{k}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
% +&\sum_{j_k=0}\upalpha_{k}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(2)}(\bm{{\hat{\uptheta}}}_{k})<\infty.
% \end{align*}
%From this we obtain that $\bm{{\hat{\uptheta}}}_{k}\rightarrow \bm\uptheta^\ast$. 

While this proof also applies to the CSG algorithm we present it as a generalization in the hope that the underlying ideas will be made clearer by addressing the cyclic case first. Since we have proven convergence under the same conditions as those required in Theorem 1, the corollary to said theorem still applies.

\section{Generalization of CSPSA  to Non-Seesaw Behavior}
\label{subsec:alternatingSPSA}

Similarly to section \ref{subsec:alternatingSG1}, here we consider a generalized version of CSPSA where the assumption is that each subvector will be updated i.o. w.p.1. Similar to eq. (\ref{eq:gencsg}) this generalization of CSPSA is given by:
\begin{align}
\label{eq:gencspsa}
&\bm\uptheta(k+1)=\bm\uptheta(k)-a_{n_k}^{(j_k)}\left[{\bm{g}}^{(j_k)}(\bm\uptheta(k))+{\bm{\upbeta}_k^{(j_k)}}+{\bm{\upxi}_k^{(j_k)}}\right],\\
&\bm\uptheta(0)= \bm{{\hat{\uptheta}}}_{0},\\
& \bm{{\hat{\uptheta}}}_{k} {\textnormal{ is defined recursively (see below).}}
\end{align}
As in section \ref{subsec:alternatingSG1}, $n_k$ represents the number of times subvector $j_k$ has been updated by time $k$ and $\bm{{\hat{\uptheta}}}_{k}$ is obtained from $\bm{{\hat{\uptheta}}}_{k-1}$ as soon as each subvector has been updated at least once.
%a_{k}^{(2)}\left({\bm{g}}^{(2)}(\bm{{\hat{\uptheta}}}_{k}^{(I)})+{\bm{\upbeta}_{k}^{(2)}}+{\bm{\upxi}_{k}^{(2)}}\right)


To prove the convergence of this generalized version of SPSA we introduce a set of conditions that is very similar to the $A$ conditions (see for section \ref{sec:ay} for notation definition):
\begin{description} 
\item[C0] ${\bm{H}}(\bm\uptheta)$ has bounded entries for all $\bm\uptheta$,
\item[C1] $ \sum_{k=0}^{\infty}\left(a_{k}^{(j)}\right)^{2}<\infty$, $\sum_{k=0}^{\infty}a_{k}^{(j)}=\infty$,
\item[C2] $f(\bm\uptheta)\geq0$, $f(\bm\uptheta^{\ast})=0$, $f(\bm\uptheta)\rightarrow \infty$ as $\|\bm\uptheta\|\rightarrow \infty$,
\item[C3] ${\displaystyle{\inf_{\upvarepsilon<\|\bm\uptheta-\bm\uptheta^{\ast}\|<1/\upvarepsilon}}}{\bm{f'}}(\bm\uptheta)^\top\overline{{\bm{g}}}^{(j)}(\bm\uptheta)>0$, ${\bm{f'}}(\bm\uptheta)^\top\overline{{\bm{g}}}^{(j)}(\bm\uptheta)\geq0$ where $\overline{\bm{g}}^{(j)}(\bm\uptheta)$ is defined as:
\begin{align*}
\overline{\bm{g}}^{(j)}(\bm\uptheta)\equiv E[\hat{\bm{g}}^{(j)}|\bm\uptheta]=\bm{g}^{(j)}(\bm\uptheta)+E[\bm\upbeta^{(j)}|\bm\uptheta],
\end{align*}
\item[C4] $\|{\bar{\bm{g}}}^{(j)}(\bm\uptheta)\|^{2}+E[\|{\bm{\upxi}}^{(j)}(\bm\uptheta)\|^{2}|\bm\uptheta]\leq b_{1}(1+f(\bm\uptheta))+b_{2}{\bm{f'}}(\bm\uptheta)^\top\bar{{\bm{g}}}^{(j)}(\bm\uptheta)$ for constants $b_{1}$ and $b_{2}$; without loss of generality, these constants are assumed to be strictly positive,
%\item[C5] Assume $\{\bm\upbeta_{k}^{(j)}\}$ is bounded w.p.1 and $\bm\upbeta_{k}^{(j)}\rightarrow {\bm{0}}$ w.p.1 for $j=1,2$.
\end{description}
Sigma al
Conditions C0--C2 are identical to A0--A2 while C3 and C4 are modified versions of A3 and A4. 

\noindent{\bf{Theorem 5}}: Let conditions C0--C5 hold. Then, the generalization of the CSPSA algorithm given by eqn.(\ref{eq:gencsg}) to the case where each subvector is updated i.o. w.p.1 (i.e., $j_k=0$ i.o. and $j_k=2$ i.o. w.p.1) converges to $\bm\uptheta^{\ast}$ w.p.1.\\

\noindent {\it{Proof:}} First we have:
\begin{align*}
&E[f(\bm\uptheta(k+1))-f(\bm\uptheta(k))|\bm\uptheta(k)]=-a_{n_k}^{(j_k)}\bm{f'}(\bm\uptheta(k))^\top\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\\
%&-a_{n_k}^{(j_k)}\bm{f'}(\bm\uptheta(k))^\top E\big[\bm{\upbeta}^{(j_k)}_k\big|\bm\uptheta(k)\big]\\
%E[f(\bm\uptheta(k+1))|\bm\uptheta(k)]-f(\bm\uptheta(k))\\
%&=-a_{n_k}^{(j_k)}E\Big[{\bm{f'}}(\bm\uptheta(k))^\top\left({\bm{g}}^{(j_k)}(\bm\uptheta(k))+{\bm{\upbeta}_{k}^{(j_k)}}+{\bm{\upxi}_{k}^{(j_k)}}\right)\Big|\bm\uptheta(k)\Big]\\
%&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2E\left[\bm{Y}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k){\bm{Y}}^{(j_k)}(\bm\uptheta(k))\Big|\bm\uptheta(k)\right]\\
&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\\
%&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2E\left[\bm{\upbeta}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)\bm{\upbeta}^{(j_k)}(\bm\uptheta(k))\big|\bm\uptheta(k)\right]\\
&+\frac{1}{2}\left(a_{n_k}^{(j_k)}\right)^2E\left[\bm{\upxi}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)\bm{\upxi}^{(j_k)}(\bm\uptheta(k))\big|\bm\uptheta(k)\right]
%&+\left(a_{n_k}^{(j_k)}\right)^2\bm{g}^{(j_k)}(\bm\uptheta(k))^\top\bm{H}(\bar{\bm\uptheta}_k)E\left[\bm{\upbeta}^{(j_k)}_k\big|\bm\uptheta(k)\right] 
\end{align*}
where $\bar{\bm\uptheta}_k=\uplambda\bm\uptheta(k)+(1-\uplambda)\bm\uptheta(k+1)$ for some $\uplambda\in[0,1]$. By C0 and C4 we have the following inequality:
\begin{align*}
&E[f(\bm\uptheta(k+1))-f(\bm\uptheta(k))|\bm\uptheta(k)]\leq-a_{n_k}^{(j_k)}\bm{f'}(\bm\uptheta(k))^\top\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\\
&+\frac{c}{2}\cdot\left(a_{n_k}^{(j_k)}\right)^2\left[b_1(1+f(\bm\uptheta(k)))+b_2\bm{f'}(\bm\uptheta(k))^\top\bar{\bm{g}}^{(j_k)}(\bm\uptheta(k))\right]
\end{align*}
%\begin{align*}
%E[f(\bm{{\hat{\uptheta}}}_{k}^{(I)})-f(\bm{{\hat{\uptheta}}}_{k})|\bm{{\hat{\uptheta}}}_{k}]\leq&-a_k^{(1)}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
%&+\frac{c}{2}\cdot\left(a_{k}^{(1)}\right)^2\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
%&+\frac{c}{2} E\left[\bm\upxi^{(1)}(\bm{{\hat{\uptheta}}}_{k})^\top\bm\upxi^{(1)}(\bm{{\hat{\uptheta}}}_{k})\Big|\bm{{\hat{\uptheta}}}_{k}\right]\\
%=&-a_k^{(1)}\bm{f'}(\bm{{\hat{\uptheta}}}_{k})^\top\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\\
%&+\frac{c}{2}\cdot\left(a_{k}^{(1)}\right)^2\left(\|\bm{g}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\|^2+E[\|\bm{\upxi}^{(1)}(\bm{{\hat{\uptheta}}}_{k})\|^2\big|\bm{{\hat{\uptheta}}}_{k}]\right)
%\end{align*}
%for a constant $c>0$. By condition A4:
Using our previous notation for $W_{k}$ and $\upalpha_k$ while replacing $\bm{g}$ with $\bar{\bm{g}}$ we derive (in the same manner as in the proof of theorem 1) the inequality:
\begin{align*}
E[W_{k+1}-W_k|\bm\uptheta(k)]\leq -\upalpha_k\upvarphi_k
\end{align*}
 so that $W_k$ is eventually (for $k$ large enough) a nonnegative supermartingale. As before, this implies $f(\bm\uptheta(k))$ has a finite limit. The rest of the proof is identical to that of Theorem 1. \hfill $\Box$

%\section{Deterministic Patterns}
%\section{Randomized Coordinate Selection}
%\section{Randomized Patterns}


==> thesis arXiv 2/chapter4p.tex <==
%!TEX root = root.tex

\chapter{Efficiency of GCSA}
\label{chap:imefficient}
%\chaptermark{Efficiency Analysis}

%In the previous section we derived an asymptotic normality result for Algorithm \ref{kirkey} (deterministic pattern for coordinate detection).
 This chapter attempts to quantify the {{relative efficiency}} between a strictly cyclic version of GCSA and its non-cyclic counterpart, where efficiency is defined in terms of the mean squared error (MSE) after taking into consideration the cost of implementation (the term ``cost'' is used in a very general sense and the precise definition is highly problem-specific). Specifically, if  $\hat{\bm\uptheta}_k^{\text{cyc}}$ denotes the $k$th iterate of a strictly cyclic implementation of GCSA and $\hat{\bm\uptheta}_k^{\text{non}}$ denotes the $k$th iterate of its non-cyclic counterpart, the focus of this chapter is on the ratio:
 \begin{align}
\label{eq:ratio}
\frac{E\|\hat{\bm\uptheta}_{k_1}^{\text{cyc}}-\bm\uptheta^\ast\|^2}{E\|\hat{\bm\uptheta}_{k_2}^{\text{non}}-\bm\uptheta^\ast\|^2},
\end{align}
 where the cumulative cost of implementing the cyclic algorithm up to iteration $k_1$ is equal (or approximately equal) to that of its non-cyclic counterpart up to iteration $k_2$ ($k_2$ is then a function of $k_1$ and vice versa). An analogue to (\ref{eq:ratio}) would be to set the MSEs in the numerator and in the denominator to be equal and then study how $k_1$ and $k_2$ differ (e.g, Spall 1992\nocite{spall1992}). In general, the definition of per-iteration cost  is highly problem-specific and plays an important role in computing (\ref{eq:ratio}). Section \ref{sec:costoport} discusses the per-iteration cost issue in more detail. Section \ref{sec:aseficwiener} then obtains an asymptotic approximation to the ratio in (\ref{eq:ratio}). Section \ref{sec:apsecialcaserelefff} uses the approximation from Section \ref{sec:aseficwiener} to study the relative efficiency between a special case of Algorithm \ref{kirkey} and its non-cyclic counterpart. Lastly, Section \ref{eq:hodgmodgepodge} contains concluding remarks.
 
 
% By seeing if the ratio in (\ref{eq:ratio}) is equal to one, less than one, or greater than one we can compare the efficinency of Algorithm \ref{kirkey} to that of its non-cyclic counterpart.
 

\section{Cost of Implementation}
\label{sec:costoport}


In order to perform a fair comparison between any two algorithms  it is necessary to  take the cost of implementation into consideration. Here, the precise definition of ``cost'' varies depending on the specific algorithm at hand. For example, cost could be a measure of the number of iterations, the actual run-time of an algorithm, the number of times a certain simulation has to be run, the amount of storage required, or a combination of these. 
%
As another example, Knight et al. (2014)\nocite{knightetal2013} consider a simplified machine model with several processors and represents run-time as a linear function of the arithmetic (flop) cost and other variables (e.g., number of messages sent). Thus, if cost is defined as run-time, the cost of implementation will be a function of the flop count as well as of other variables. This section focuses on comparing the cost of implementing the cyclic seesaw SA algorithm (the ideas can easily be generalized to the case where $\bm\uptheta$ is partitioned into more than two subvectors) to the cost of implementing its non-cyclic counterpart when cost is a measure of the arithmetic computations needed to perform a single iteration. Specifically, this section pinpoints the type of arithmetic computations that can result in a significant difference between the per-iteration cost of implementing a cyclic algorithm and the per-iteration cost of implementing its non-cyclic formulation.
% when both algorithms are implemented in the {{ manner}} to be discussed next.


 Letting $\hat{\bm{\uptheta}}_k^{\text{cyc}}$ denote an iterate of the cyclic seesaw SA algorithm (Section \ref{sec:keatonmodasd}) and using the notation in (\ref{eq:analgoysDRAGON}) we assume throughout this section that:
 \begin{subequations}
\begin{align}
{{\hat{\bm\uptheta}}}_{k}^{(I)} &=\left[\begin{array}{c}(\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}})^{[\bm{1}]} \\ \relax (\hat{\bm{\uptheta}}_k^{\text{cyc}})^{[\bm{2}]}\end{array}\right]=\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{cyc}},k,\bm{V}_{k})\in \mathbb{R}^p,\label{eq:huh0}\\
\hat{\bm\uptheta}_{k+1}^{\text{cyc}}&=\left[\begin{array}{c}(\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}})^{[\bm{1}]} \\ \relax (\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}})^{[\bm{2}]}\end{array}\right]=\hat{\bm{\uptheta}}_k^{(I)}-\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_{k}^{(I)},k,\bm{V}_{k}^{(I)})\in \mathbb{R}^p,\label{eq:huh}
\end{align}
\end{subequations}
for a {{known}} vector-valued function satisfying $\bm\Phi(\bm\uptheta,k,\bm{V}){: \mathbb{R}^p\times \mathbb{Z}^+\times\Omega_{\bm{V}}\rightarrow \mathbb{R}^p}$ where $\bm\Phi^{(j)}(\cdot,\cdot,\cdot)$ is defined using the notation from (\ref{eq:electricpulsar}) and $\bm{V}_k$ and $\bm{V}_k^{(I)}$ are random variables with values in $\Omega_{\bm{V}}$.  We refer to the functions  $\bm\Phi^{(1)}(\cdot,\cdot,\cdot)$ and  $\bm\Phi^{(2)}(\cdot,\cdot,\cdot)$ as {\it{update functions}}. In the CSG algorithm (Section \ref{sec:ay}), for example, if $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})$ are obtained via the evaluation of an arithmetic function (e.g., the pure infinitesimal perturbation analysis (IPA) algorithm where the update direction is as in (\ref{eq:imanIPA})) then $\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{cyc}},k,\bm{V}_{k})=a_{k}^{(1)}[\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})]^{(1)}$ and $\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_{k}^{(I)},k,\bm{V}_{k}^{(I)})=a_{k}^{(2)}[\hat{\bm{g}}^{\text{SG}}(\bm{{\hat{\uptheta}}}_{k}^{(I)})]^{(2)}$.
%
Similarly, if $\hat{\bm{\uptheta}}_k^{\text{non}}$ denotes an iterate of the basic non-cyclic SA algorithm (see Section \ref{sec:dummieyouask}) we assume:
\begin{align}
\label{eq:herculedherculess}
\hat{\bm{\uptheta}}_{k+1}^{\text{non}}&=\left[\begin{array}{c}(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]} \\ \relax (\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\end{array}\right]\notag\\
&=\hat{\bm{\uptheta}}_k^{\text{non}}-\bm\Phi(\hat{\bm{\uptheta}}_k^{\text{non}},k,\bm{V}_k)\notag\\
&=\hat{\bm{\uptheta}}_k^{\text{non}}-\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,\bm{V}_k)-\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,\bm{V}_k)\in \mathbb{R}^p,
\end{align}
 where $\bm{V}_k$ is a random variable in $\Omega_{\bm{V}}$. 
% 
Both (\ref{eq:huh0},b) and (\ref{eq:herculedherculess}) 
%the non-cyclic- and the cyclic seesaw SA algorithms 
may be implemented in a distributed or non-distributed manner, in the sense that the vectors $\bm\Phi^{(1)}(\cdot,\cdot,\cdot)$ and $\bm\Phi^{(2)}(\cdot,\cdot,\cdot)$ are allowed (but not required) to be computed at different locations. Botts et al. (2016), for example, consider a multi-agent surveillance and tracking problem in which agent $j$ updates its state vector (corresponding to the vector $\bm\uptheta^{[\bm{j}]}$) using $\bm\Phi^{(j)}(\cdot,\cdot,\cdot)$.
%, a function which other agents generally do not need to compute. 
In this multi-agent problem, each of the vector-valued functions $\bm\Phi^{(j)}(\cdot,\cdot,\cdot)$ is computed at a different location by a different agent. This multi-agent algorithm is, therefore, a distributed algorithm. 
%Throughout this section we occasionally use this multi-agent analogy to facilitate our discussion regarding (\ref{eq:huh}) and (\ref{eq:herculedherculess}), although we note that the arguments in this section also hold when the algorithms are not implemented in a distributed manner. 
Next we define the cost of implementing (\ref{eq:huh0},b) and (\ref{eq:herculedherculess}).


 The definition of cost to be used in this section is based on the observation that any function, regardless of complexity, can be evaluated by performing a sequence of elementary operations involving one or two arguments at a time (e.g., addition, multiplication, division, the power operation, trigonometric functions, exponential functions, and logarithmic functions). 
 %
 Then, the cost of implementing an iteration of (\ref{eq:herculedherculess}), denoted by $c^{\text{non}}_k$, will be defined as the number of elementary  operations required to evaluate $\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,\bm{V}_k)$ and $\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,\bm{V}_k)$. Similarly, the cost of implementing an iteration of (\ref{eq:huh0},b), denoted by $c^{\text{cyc}}_k$,  will be defined as the number of elementary  operations required to evaluate both $\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{cyc}},k,\bm{V}_{k})$ and $\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_{k}^{(I)},k,\bm{V}_{k}^{(I)})$. Note that we are omitting the cost of performing the subtraction operations appearing in (\ref{eq:huh0},b) and the subtraction operation appearing in (\ref{eq:herculedherculess}). This was done due to the fact that performing these addition operations takes the same number of elementary operations, namely $p$, for both the cyclic and the non-cyclic algorithms. Therefore, the aforementioned subtraction operations are not significant given the focus of this section on pinpointing the sources of discrepancy between the cost of implementing a cyclic and the cost of implementing its non-cyclic counterpart.


\begin{figure}
\centering
        \begin{subfigure}[b]{0.49\textwidth}
                \centering
\begin{tikzpicture}

\node[draw,circle,minimum size=.8cm,inner sep=0pt, thick] (x) at (0,0) {$x$};
\node[draw,circle,minimum size=.8cm,inner sep=0pt, thick] (y) at (0,-1.5) {$y$};

\node[draw,rectangle, rounded corners, minimum height=2em, minimum width=28pt, thick] (xy) at (2,-0.75) {$xy$};

\node[draw,rectangle, rounded corners, minimum height=2em, minimum width=40pt, thick] (xys) at (4.4,-0.75) {$(xy)^2$};

\draw[->, thick] (x)--(xy) ;
\draw[->,thick] (y)--(xy);
\node at (1.1,-0.75) {$\ast$};
\draw[->,thick] (xy)--(xys) node[above,midway, above=3pt] {$(\cdot)^2$};

\end{tikzpicture}
                \caption{Requires two elementary operations.}
                \label{fig:gull}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.49\textwidth}
                \centering
\begin{tikzpicture}

\node[draw,circle,minimum size=.8cm,inner sep=0pt, thick] (x) at (0,0) {$x$};
\node[draw,circle,minimum size=.8cm,inner sep=0pt, thick] (y) at (0,-1.5) {$y$};

\node[draw,rectangle, rounded corners, minimum height=2em, minimum width=26pt, thick] (xs) at (2,0) {$x^2$};

\node[draw,rectangle, rounded corners, minimum height=2em, minimum width=26pt, thick] (ys) at (2,-1.5) {$y^2$};

\draw[->, thick] (x)--(xs) node[above,midway, above=3pt] {$(\cdot)^2$};
\draw[->,thick] (y)--(ys) node[above,midway, above=3pt] {$(\cdot)^2$};
\node at (3.2,-0.75) {$\ast$};

\node[draw,rectangle, rounded corners, minimum height=2em, minimum width=40pt, thick] (xys) at (4.3,-0.75) {$(xy)^2$};
\draw[->,thick] (xs)--(xys);
\draw[->,thick] (ys)--(xys);

\end{tikzpicture}
                \caption{Requires three elementary operations.}
                \label{fig:gull2}
        \end{subfigure}\hfill
%        \begin{subfigure}[b]{0.22\textwidth}
%                \centering
%                \includegraphics[width=\linewidth]{example-image-a}
%                \caption{A tiger}
%                \label{fig:tiger}
%        \end{subfigure}\hfill
%        \begin{subfigure}[b]{0.22\textwidth}
%                \centering
%                \includegraphics[width=\linewidth]{example-image-a}
%                \caption{A mouse}
%                \label{fig:mouse}
%        \end{subfigure}
        \caption[Two computational graphs (CGs) for computing $f(x,y)=(xy)^2$]{Two CGs for evaluating the function $\uprho(x,y)=(xy)^2$. 
%        In general, there is no unique CG associated with the evaluation of a function.
        }\label{fig:oneatmosphere}
\end{figure}
 
 The sequence of elementary operations performed when evaluating any real-valued function can be represented by a computational graph (CG) (e.g., Nocedal and Wright, p. 205) which is generally not unique (see Figure \ref{fig:oneatmosphere}). In this section we will assume that each entry of $\bm\Phi(\cdot,\cdot,\cdot)\in \mathbb{R}^p$ is associated with a predetermined CG whose shape is independent of the arguments of $\bm\Phi(\cdot,\cdot,\cdot)$. In general, the elementary computations performed when evaluating $\bm\Phi(\bm\uptheta,k,\bm{V})$ must fall into one of the following (mutually exclusive) categories:
%  (any dependence/independence assumptions mentioned in the following categories is a probabilistic dependence/independence conditional on $\bm\uptheta$ and $k$): 
 \label{catpage}
 \begin{DESCRIPTION}
 \item[Cat. 1:] Computations involving $\bm\uptheta^{[\bm{1}]}$ but not $\bm\uptheta^{[\bm{2}]}$.
 \item[Cat. 2:] Computations involving $\bm\uptheta^{[\bm{2}]}$ but not $\bm\uptheta^{[\bm{1}]}$.
 \item[Cat. 3:]  Computations involving both $\bm\uptheta^{[\bm{1}]}$ and $\bm\uptheta^{[\bm{2}]}$.
 \item[Cat. 4:] Computations not involving $\bm\uptheta$.
% depend neither on $\bm\uptheta^{[\bm{a}]}$ nor on $\bm\uptheta^{[\bm{b}]}$.  
 \end{DESCRIPTION}
% (The dependence/independence assumptions in the above four categories is a probabilistic dependence/independence conditional on $\bm\uptheta$ and $k$.)
%In the CG from Figure \ref{fig:gull}, for example, two elementary computations are performed: the product and the power function. Both of these operations depend on $x$ and $y$. In contrast, in the CG from Figure \ref{fig:gull2} three elementary computations are performed: two power function evaluations and a product. Here, only the product function depends on both $x$ and $y$ while each of the power functions depends on either $x$ or $y$ (but not both).
%
With this in mind, an elementary operation performed when computing any of the entries of $\bm\Phi^{(j)}(\bm\uptheta,k,\bm{V})$ will be denoted by $f_{\ell}^{(j)}(\bm\uptheta^{[\bm{1}]})$, $s_{\ell}^{(j)}(\bm\uptheta^{[\bm{1}]})$, $b_{\ell}^{(j)}(\bm\uptheta^{[\bm{1}]},\bm\uptheta^{[\bm{2}]})$, or $n_{\ell}^{(j)}(k)$ depending on whether it belongs to category 1, 2, 3, or 4 above, respectively. The letter ``$f$'' was chosen to emphasize the fact that an operation depends only on the {\it{first}} part of $\bm\uptheta$. Similarly, the letters ``$s$'', ``$b$'', and ``$n$'', were used to emphasize the fact that an operation depends on the {\it{second}} part of $\bm\uptheta$, on {\it{both}} parts of $\bm\uptheta$, or {\it{neither}} on the first- {\it{nor}} on the second part of $\bm\uptheta$.
% (although the letters $f$, $b$, $s$, and $n$ have been used to denote other variables in previous chapters, the level of detail in this section makes reusing notation inevitable from a practical perspective). 
 The collection of all elementary operations performed when computing the vectors $\bm\Phi^{(j)}(\bm\uptheta,k,\bm{V})$ can then be summarized by the following sets whose elements can be thought of as labels of the operations to be performed:
% 
% Note that the variable $\bm{V}$ is implicity. Specifically, because the distribution of $\bm{V}$ can depend on $\bm\uptheta^{[\bm{a}]}$, on $\bm\uptheta^{[\bm{b}]}$, on both $\bm\uptheta^{[\bm{a}]}$ and $\bm\uptheta^{[\bm{b}]}$, or be independent of $\bm\uptheta$ altogether, any elementary operations involving $\bm{V}$ must belong to one of the four aforementioned categories. 
% 
% 
% We now define the following sets:
\begin{subequations}
 \begin{align}
 &F^{(j)}(\bm\uptheta^{[\bm{1}]})\equiv \left\{ f_{\ell}^{(j)}(\bm\uptheta^{[\bm{1}]})\right\}_{\ell},\ \ \ S^{(j)}(\bm\uptheta^{[\bm{2}]})\equiv \left\{ s_{\ell}^{(j)}(\bm\uptheta^{[\bm{2}]})\right\}_{\ell}, \label{eq:fier0}\\
 &B^{(j)}(\bm\uptheta^{[\bm{1}]},\bm\uptheta^{[\bm{2}]})\equiv \left\{ b_{\ell}^{(j)}(\bm\uptheta^{[\bm{1}]},\bm\uptheta^{[\bm{2}]})\right\}_{\ell},\ \ \ N^{(j)}(k)\equiv \left\{ n_{\ell}^{(j)}(k)\right\}_{\ell}.
 \label{eq:fier}
\end{align}
\end{subequations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Next we provide insight into the reason why (\ref{eq:huh0},b) and (\ref{eq:herculedherculess}) may have different per-iteration costs (i.e., why $c^{\text{non}}_k$ may not equal $c^{\text{cyc}}_k$).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Consider a simple situation where $\bm\uptheta=[x,y]^\top\in \mathbb{R}^2$ (so that $\bm\uptheta^{[\bm{1}]}=x$ and $\bm\uptheta^{[\bm{2}]}=y$), $V$ is a real-valued random variable whose distribution does not depend on $\bm\uptheta$, and assume that:
\begin{align}
\label{eq:blindmeyyyy}
\bm\Phi(\bm\uptheta,k,{V})=k^{-1}\left[\begin{array}{c}y(xy)^{9}+V \\0\end{array}\right]+k^{-1}\left[\begin{array}{c}0 \\ x (xy)^{9}+V\end{array}\right]
\end{align}
%\begin{align}
%\label{eq:zeldabelddys}
%\bm\Phi(\bm\uptheta,k,{V})=\left[\begin{array}{c}x \\y\end{array}\right]-\frac{1}{k}\left[\begin{array}{c}y(xy)^{9}+V \\x (xy)^{9}+V\end{array}\right]+\left[\begin{array}{c}x \\y\end{array}\right]-\frac{1}{k}\left[\begin{array}{c}y(xy)^{9}+V \\x (xy)^{9}+V\end{array}\right]
%\end{align}
%
%Note that (\ref{eq:zeldabelddys}) can also be written as follows:
%\begin{align}
%\label{eq:blindmeyyyy}
%\bm\Phi(\bm\uptheta,k,{V})=\left[\begin{array}{c}x-[y(xy)^{9}+V]/k \\0\end{array}\right]+\left[\begin{array}{c}0 \\y-[x (xy)^{9}+V]/k\end{array}\right]
%\end{align}
so that the first vector, respectively second vector, on the right-hand side of (\ref{eq:blindmeyyyy}) represents $\bm\Phi^{(1)}(\bm\uptheta,k,V)$, respectively $\bm\Phi^{(2)}(\bm\uptheta,k,V)$ (in the context of Section \ref{sec:sgfosa}, $k\bm\Phi(\bm\uptheta,k,{V})$ corresponds to the gradient of the noisy function $Q(\bm\uptheta,V)=(xy)^{10}/10+(x+y)V$).
%
The non-cyclic algorithm in (\ref{eq:herculedherculess}) with $\bm\Phi(\bm\uptheta,k,{V})$ as in (\ref{eq:blindmeyyyy}) would 
% be to let $\hat{\bm{\uptheta}}_{k+1}^{\text{non}}=\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k,k,V_k)+\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_k,k,V_k)$ where $\hat{\bm{\uptheta}}_k=[x_k,y_k]^\top$. Equivalently, 
% 
%The non-cyclic algorithm would 
be implemented as follows:
\begin{align*}
\hat{\bm{\uptheta}}_{k+1}^{\text{non}}=\hat{\bm{\uptheta}}_k^{\text{non}}-k^{-1}\left[\begin{array}{c}y_k(x_ky_k)^{9}+V_k \\0\end{array}\right]-k^{-1}\left[\begin{array}{c}0 \\ x_k (x_ky_k)^{9}+V_k\end{array}\right],
%\label{eq:asdsad}
\end{align*}
where $\hat{\bm{\uptheta}}_k^{\text{non}}=[x_k,y_k]^\top$. Because the possibly non-zero entries of $\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,V_k)$ and $\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,V_k)$ are very similar, it may be advantageous to share certain computations in order to minimize the overall arithmetic cost. For example, the quantity $(x_ky_k)^9$ appears in both  $\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,V_k)$ and $\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_k^{\text{non}},k,V_k)$. In the multi-agent setting, if agents are allowed to communicate then the first agent could compute $(x_ky_k)^{9}$ and share it with the second agent. The ability to share the value of $(x_ky_k)^{9}$ is lost when considering a cyclic implementation (regardless of whether the implementation is distributed or not).\label{page:transferincossst} 
% of the algorithm as is discussed next.


The implementation of the cyclic seesaw algorithm in (\ref{eq:huh0},b) is as follows:
\begin{align*}
\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}=\hat{\bm{\uptheta}}_{k}^{\text{cyc}}-k^{-1}\left[\begin{array}{c}y_k(x_ky_k)^{9}+V_k \\0\end{array}\right]-k^{-1}\left[\begin{array}{c}0 \\ x_{k+1} (x_{k+1}y_k)^{9}+V_k^{(I)}\end{array}\right],
%\label{eq:trancotronic}
\end{align*}
where $\hat{\bm{\uptheta}}_k^{\text{cyc}}=[x_k,y_k]^\top$ (in this case, $\hat{\bm{\uptheta}}_k^{(I)}$ would be equal to $[x_{k+1},y_k]^\top$). Since $(x_ky_k)^{9}\neq (x_{k+1}y_k)^{9}$, in a cyclic implementation it would not be possible to reduce cost by sharing the value of $(xy)^9$. However, since $(xy)^9=x^9y^9$, a reduction in the arithmetic cost could be obtained by sharing the values of $x_{k+1}^9$ and $y_k^9$. 
%Alternatively, if the first agent (the agent in charge of updating $x_k$) were to share the value of $(x_ky_k)^9$ with the second agent (the agent in charge of updating $y_k$) 
In general, the types of arithmetic computations that can be shared (and the associated reduction in cost) depends on the CGs of the entries of $\bm\Phi(\bm\uptheta,k,\bm{V})$.
% (e.g., if the quantities $x^9$ and $y^9$ are never computed then these quantities cannot be shared). 


In the remainder of this section we derive expressions for $c^{\text{non}}_k$ and $c^{\text{cyc}}_k$ that take into consideration a possible reduction in cost through the sharing of arithmetic computations.
%
We make the following assumptions:
 \begin{DESCRIPTION}
 \item[D0] The CG corresponding to the $i$th entry of $\bm\Phi(\bm\uptheta,k,\bm{V})$ is the same for both the cyclic- and non-cyclic implementations and does not depend on $\bm\uptheta$, $k$, or $\bm{V}$.
% \item[D1] We will assume the CG associated with a given entry of $\bm\Phi^{(1)}(\hat{\bm{\uptheta}}_k,k,\bm{V}_{k})$ is set to be equal to that of the corresponding entry in $\bm\Phi^{(1)}(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$. 
% \item[D2] Similarly, we assume the CG associated with any entry of $\bm\Phi^{(2)}(\hat{\bm{\uptheta}}_{k[I]},k,\bm{V}_{k[I]})$ is set to be equal to that of the corresponding entry in $\bm\Phi^{(2)}(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$.
\item [D1] If the algorithm is implemented in a distributed manner, $\bm\uptheta$, $k$ and $\bm{V}$ are known to the agent computing $\bm\Phi^{(j)}(\bm\uptheta,k,\bm{V})$.
\item[D2] During iteration $k$, it is possible to share/reuse computations corresponding to nodes in the CGs which were computed during iterations $1,\dots,k$.
 \end{DESCRIPTION}
Under D0--D1 let $\text{Naive-Cost}^{(1)}$ be the total number of elementary operations required to evaluate the $p'$ CGs  associated with the evaluation of $\bm\Phi^{(1)}(\cdot,\cdot,\cdot)$. Similarly, let $\text{Naive-Cost}^{(2)}$ be the total number of elementary operations required to evaluate the $p'$ CGs  associated with the evaluation of $\bm\Phi^{(2)}(\cdot,\cdot,\cdot)$.
%
Then, under D0--D2 the following holds for both the cyclic- and non-cyclic algorithms:
\vspace{-.5in}
\begin{subequations}
\begin{align}
c_k^{\text{non}}&= \text{Naive-Cost}^{(1)}+\text{Naive-Cost}^{(2)}- c^{\text{non}}_{\text{share}}(k)- c^{\text{non}}_{\text{carry}}(k),\label{eq:opahhh0}\\
c_k^{\text{cyc}}&= \text{Naive-Cost}^{(1)}+\text{Naive-Cost}^{(2)}- c^{\text{cyc}}_{\text{share}}(k)- c^{\text{cyc}}_{\text{carry}}(k),\label{eq:opahhh}
\end{align}
\end{subequations}
where $c^{\text{non}}_{\text{share}}(k)$ and $c^{\text{cyc}}_{\text{share}}(k)$ denote the cost saved by sharing information on calculations performed during the $k$th iteration, and where $c^{\text{non}}_{\text{carry}}(k)$ and $c^{\text{cyc}}_{\text{carry}}(k)$ denote the cost saved by reusing and/or sharing computations carried from previous iterations.
%
Next we provide expressions for $c_{\text{share}}^{\text{non}}(k)$, $c_{\text{carry}}^{\text{non}}(k)$, $c_{\text{share}}^{\text{cyc}}(k)$, and $c_{\text{carry}}^{\text{cyc}}(k)$ based on the terminology from (\ref{eq:fier0},b).
% $c_k^{\text{non}}$ and $c_k^{\text{cyc}}$.

%
%when computing $\bm\Phi(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$ by sharing information regarding $\bm\Phi^{(1)}(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$ and $\bm\Phi^{(2)}(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$ during the $k$th iteration.
%
%$F^{(j)}(\tilde{\bm{\uptheta}}_k^{(1)})$, $S^{(j)}(\tilde{\bm{\uptheta}}_k^{(2)})$, $B^{(j)}(\tilde{\bm{\uptheta}}_k^{(1)},\tilde{\bm{\uptheta}}_k^{(2)})$, and $N^{(j)}(k)$ represent the operations required to compute $\bm\Phi(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$. 
%
%In order to compare $c_k^{\text{non}}$ and $c_k^{\text{cyc}}$ let us define
 Let $\mathcal{A}_k$ be the set of computations performed during the $k$th iteration that are shared during iteration $k$. 
% ($\mathcal{A}_k$ is then a subset of the set $F^{(j)}(\bm\uptheta^{[\bm{1}]})\cup S^{(j)}(\bm\uptheta^{[\bm{2}]})\cup B^{(j)}(\bm\uptheta^{[\bm{1}]},\bm\uptheta^{[\bm{2}]})\cup N^{(j)}(k)$).
%Sharing elements of $\mathcal{A}$ is assumed to be worth the cost of sharing this information (such as the increase in the amount of communication and added storage cost). 
Similarly, let $\mathcal{B}_k$ be the set of computations performed during iterations $1,\dots, k-1$ that are reused and/or shared during iteration $k$. Additionally, let $\upalpha_{F,\ell}$, $\upalpha_{S,\ell}$, $\upalpha_{B,\ell}$, and $\upalpha_{N,\ell}$ represent the cost saved during the $k$th iteration by sharing $f_{\ell}^{(1)}(\bm\uptheta^{[\bm{1}]})$, $s_{\ell}^{(1)}(\bm\uptheta^{[\bm{2}]})$, $b_{\ell}^{(1)}(\bm\uptheta^{[\bm{1}]},\bm\uptheta^{[\bm{2}]})$, and $n_{\ell}^{(1)}(k)$, respectively. 
%(note that we have not made any assumptions regarding which agent is responsible for computing a shared element). 
%
%of elements in (\ref{eq:fier}) that are to be stored from previous iterations for use during the $k$th iteration.
% (once again, it is assumed storing these elements is beneficial overall). 
%
 Then, assuming $\upalpha_{F,\ell}$, $\upalpha_{S,\ell}$, $\upalpha_{B,\ell}$, and $\upalpha_{N,\ell}$ do not depend on $\bm\uptheta$ or $k$:
% , $c_{\text{share}}^{\text{non}}(k)$ can be expressed as follows:
\begin{align}
c_{\text{share}}^{\text{non}}(k)=&\ \sum_{\ell}\upalpha_{F,\ell}\hspace{.03in} \chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\cap \mathcal{A}_k\Big\}\notag\\
&+\sum_{\ell}\upalpha_{S,\ell}\hspace{.03in}\chi\Big\{s_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\in S^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\cap\mathcal{A}_k\Big\}\notag\\
&+\sum_{\ell}\upalpha_{B,\ell}\hspace{.03in}\chi\Big\{b_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\in B^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\cap\mathcal{A}_k\Big\}\notag\\
&+\sum_{\ell}\upalpha_{N,\ell}\hspace{.03in}\chi\Big\{n_{\ell}^{(1)}(k)\in N^{(2)}(k)\cap\mathcal{A}_k\Big\}.\label{eq:nonshared}
\end{align}
%where ${\mathcal{X}}\{\mathcal{E}\}$ is the indicator function of the event $\mathcal{E}$ and 
%where  Here, we are making the following assumption:

%Note that while (\ref{eq:nonshared}) 
 
 To compute  $c_{\text{carry}}^{\text{non}}(k)$ let $\upbeta_{N,\ell}^{(j)}$ represent the arithmetic cost saved during the $k$th iteration by reusing the elements $n_{\ell}^{(j)}(i)$ for $i=0,\dots,k-1$. Then, assuming $\upbeta_{N,\ell}^{(j)}$ does not depend on $\bm\uptheta$ or $k$:
 %
% (this is because any computations involving $\bm\uptheta$ will change from iteration to iteration)
% it follows that:
%
%Let us now compute the cost saved by reusing information from previous iterations. Let $c^{\text{carried}}_{\text{non}}(\tilde{\bm{\uptheta}}_k,k)$ denote the cost saved during the $k$th iteration when computing $\bm\Phi(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$ by reusing elements computed in previous iterations. Then,
\begin{align}
c_{\text{carry}}^{\text{non}}(k)=&\ \sum_{\ell}\upbeta_{N,\ell}^{(1)}\hspace{.03in}\chi\left\{n_{\ell}^{(1)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\notag\\
&+\sum_{\ell}\upbeta_{N,\ell}^{(2)}\hspace{.03in}\chi\left\{n_{\ell}^{(2)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\notag\\
&-\sum_{\ell}\upbeta_{N,\ell}^{(1)}\hspace{.03in}\chi\left\{n_{\ell}^{(1)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\times\notag\\
&\chi\left\{n_{\ell}^{(2)}\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\},\label{eq:halfdome}
%\chi\left\{n_{\ell}^{(1)}(k)\in\mathcal{B}_k\right\}\chi\left\{n_{\ell}^{(2)}(k)\in\mathcal{B}_k\right\},
\end{align}
this follows after noting that the only terms from previous iterations that could be reused during iteration $k$ are terms that do not depend on $\bm\uptheta$.
%
For the cyclic seesaw algorithm, the cost of sharing computations is different than for the non-cyclic algorithm (as was discussed on p. \pageref{page:transferincossst}). Specifically, 
%for the cyclic seesaw algorithm we have:
\begin{align}
c_{\text{share}}^{\text{cyc}}(k)=&\ \sum_{\ell}\upalpha_{S,\ell}\hspace{.03in} \chi\Big\{s_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\in S^{(2)}\left((\hat{\bm\uptheta}_{k}^{\text{non}})^{[\bm{2}]}\right)\cap \mathcal{A}_k\Big\}\notag\\
&+\sum_{\ell}\upalpha_{N,\ell}\hspace{.03in} \chi\Big\{n_{\ell}^{(1)}(k)\in N^{(2)}(k)\cap \mathcal{A}_k\Big\}.\label{eq:cycshared}
\end{align}
%The reason (\ref{eq:cycshared}) is different from (\ref{eq:nonshared}) stems from the fact that during the $k$th iteration the vector $\hat{\bm{\uptheta}}_k^{(I)}=[(\hat{\bm{\uptheta}}_{k+1}^{[\bm{1}]})^\top,(\hat{\bm{\uptheta}}_{k}^{[\bm{2}]})^\top]^\top$ must be computed prior to computing $\hat{\bm{\uptheta}}_{k+1}=[(\hat{\bm{\uptheta}}_{k+1}^{[\bm{1}]})^\top,(\hat{\bm{\uptheta}}_{k+1}^{[\bm{2}]})^\top]^\top$.
%, then the only computations that can be shared between agents are operations which depend only on $\hat{\bm{\uptheta}}_k^{[\bm{2}]}$ or operations that do not depend on $
%
%computations may be shares is when $\hat{\bm{\uptheta}}_{k+1}$ is computed
Next, letting $\upbeta_{F,\ell}^{(1)}$ represent the arithmetic cost saved during the $k$th iteration by reusing the element $f_{\ell}^{(1)}(\hat{\bm{\uptheta}}_k^{(1)})$ computed during the previous iteration and assuming $\upbeta_{F,\ell}^{(1)}$ does not depend on $\bm\uptheta$ or $k$ it follows that:
%
%Now, let $c^{\text{carried}}_{\text{cyc}}(\hat{\bm{\uptheta}}_k,\hat{\bm{\uptheta}}_{k[I]},k)$ denote the cost saved during the $k$th iteration of the cyclic algorithm when computing $\bm\Phi^{(1)}(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$ and $\bm\Phi^{(2)}(\tilde{\bm{\uptheta}}_k,k,\bm{V}_k)$ by reusing elements computed in previous iterations. Analogous to (\ref{eq:halfdome}) we have
\begin{align}
&c_{\text{carry}}^{\text{cyc}}( k)=\sum_{\ell}\upbeta_{N,\ell}^{(1)}\hspace{.03in}\chi\left\{n_{\ell}^{(1)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\notag\\
&+\sum_{\ell}\upbeta_{N,\ell}^{(2)}\hspace{.03in}\chi\left\{n_{\ell}^{(2)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\notag\\
&-\sum_{\ell}\upbeta_{N,\ell}^{(1)}\hspace{.03in}\chi\left\{n_{\ell}^{(1)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\times\notag\\
&\chi\left\{n_{\ell}^{(2)}(k)\in\bigcup_{i=0}^{k-1}\big( N^{(1)}(i)\cup N^{(2)}(i)\big)\cap\mathcal{B}_k\right\}\notag\\
%\chi\left\{n_{\ell}^{(1)}(k)\in\mathcal{B}_k\right\}\chi\left\{n_{\ell}^{(2)}(k)\in\mathcal{B}_k\right\}
&+ \sum_{\ell}\upbeta_{F,\ell}^{(1)}\hspace{.03in}\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{cyc}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm\uptheta}_{k}^{\text{cyc}})^{[\bm{1}]}\right)\cap\mathcal{B}_k\Big\}.\label{eq:tenk}
\end{align}
%where . Similar to assumption D4 we assume the following:
%
%Now we can write
%\begin{align}
%c_{\text{cyc}}(k)=&\ \text{Naive-Cost}^{(1)}+\text{Naive-Cost}^{(2)}\notag\\
%    &-c^{\text{shared}}_{\text{cyc}}(\hat{\bm{\uptheta}}_k, \hat{\bm{\uptheta}}_{k[I]}, k)-c^{\text{carried}}_{\text{cyc}}(\hat{\bm{\uptheta}}_k, \hat{\bm{\uptheta}}_{k[I]}, k).\label{eq:cyccost}
%\end{align}
%where we are making the following assumption:
%(this assumption is similar to assumption D4).
Note that (\ref{eq:tenk}) is different from (\ref{eq:halfdome}) since it contains an extra term (the last line in (\ref{eq:tenk})),
%\begin{align*}
%\sum_{\ell}\upbeta_{F,\ell}^{(1)}\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{cyc}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm\uptheta}_{k}^{\text{cyc}})^{[\bm{1}]}\right)\cap\mathcal{B}_k\Big\},
%\end{align*}
 which originates from the fact that the first $p'$ entries of $\hat{\bm{\uptheta}}_{k-1}^{(I)}$ are the same as the first $p'$ entries of $\hat{\bm{\uptheta}}_k^{\text{cyc}}$. Therefore, calculations involving $(\hat{\bm{\uptheta}}_{k-1}^{(I)})^{[\bm{1}]}$ which were computed during iteration $k-1$ could be used to evaluate the computations involving $(\hat{\bm{\uptheta}}_{k}^{\text{cyc}})^{[\bm{1}]}$ during the $k$th iteration.
%
The following Proposition compares $c_k^{\text{non}}$ and $c_k^{\text{cyc}}$.

\begin{proposition}
Assume D0--D2 hold along with the following conditions:
\begin{DESCRIPTION}
\item[D3] $\upalpha_{F,\ell}$, $\upalpha_{S,\ell}$, $\upalpha_{B,\ell}$, and $\upalpha_{N,\ell}$ do not depend on $\bm\uptheta$ or $k$.
\item[D4] $\upbeta_{N,\ell}^{(j)}$ does not depend on $\bm\uptheta$ or $k$.
\item[D5] $\upbeta_{F,\ell}^{(j)}$ does not depend on $\bm\uptheta$ or $k$.
\end{DESCRIPTION}
Then,
\begin{align}
\label{eq:core}
c_k^{\text{non}}-c_k^{\text{cyc}}= T_2(k)-T_1(k),
\end{align}
where $T_1(k)\geq 0$ is defined as:
\begin{align*}
T_1(k)&\equiv \sum_{\ell}\upalpha_{F,\ell}\hspace{.03in}\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\cap \mathcal{A}_k\Big\}\notag\\
&\sum_{\ell}\upalpha_{B,\ell}\hspace{.03in}\chi\Big\{b_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\in B^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\cap\mathcal{A}_k\Big\}
%\label{eq:tutururutuli}
\end{align*}
and $T_2(k)\geq 0$ is defined as:
\begin{align*}
%\label{eq:hahhahhorse}
T_2(k)&\equiv \sum_{\ell}\upbeta_{F,\ell}^{(1)}\hspace{.03in}\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{cyc}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm\uptheta}_{k}^{\text{cyc}})^{[\bm{1}]}\right)\cap\mathcal{B}_k\Big\}.
\end{align*}
\end{proposition}
%
\begin{proof}
First, (\ref{eq:nonshared}) and (\ref{eq:cycshared}) imply $T_1(k)=c_{\text{share}}^{\text{non}}(k)-c_{\text{share}}^{\text{cyc}}(k)$ while (\ref{eq:halfdome}) and (\ref{eq:tenk}) imply $T_2(k)=c_{\text{carry}}^{\text{cyc}}(k)-c_{\text{carry}}^{\text{non}}(k)$. The result then follows from (\ref{eq:opahhh0},b).
\end{proof}

%The significance of (\ref{eq:core}) is that
%\begin{align*}
%c_k^{\text{non}}-c_k^{\text{cyc}} 
%\begin{cases} \geq 0 &\mbox{if } |T_1(k)|\leq T_2(k), \\ 
%\leq 0 & \mbox{if } |T_1(k)|\geq T_2(k). 
%\end{cases} 
%\end{align*}
%In other words, $c_k^{\text{non}}$ will be greater or equal to $c_k^{\text{cyc}}$ 
To facilitate the interpretation of (\ref{eq:core}) we assume the following:
\begin{DESCRIPTION}
\item[D6]  $\upalpha_{F,\ell}^{(1)}=\upbeta_{F,\ell}^{(1)}$. 
This assumption is satisfied whenever the cost saved by sharing a computation involving only $\bm\uptheta^{[\bm{1}]}$ is independent of whether the computation was performed during the $k$th iteration or during an earlier iteration.
\end{DESCRIPTION}
Then, (\ref{eq:core}) becomes
\begin{align*}
&c_k^{\text{non}}-c_k^{\text{cyc}}= \sum_{\ell}\upalpha_{F,\ell}^{(1)}\hspace{.03in}\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{cyc}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm\uptheta}_{k}^{\text{cyc}})^{[\bm{1}]}\right)\cap\mathcal{B}_k\Big\}\notag\\
& -\sum_{\ell}\upalpha_{F,\ell}\hspace{.03in}\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\cap \mathcal{A}_k\Big\}\notag\\
&-\sum_{\ell}\upalpha_{B,\ell}\hspace{.03in}\chi\Big\{b_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\in B^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\cap\mathcal{A}_k\Big\}.
%& \sum_{\ell}\upalpha_{F,\ell}^{(1)}\mathcal{X}\Big\{f_{\ell}^{(1)}(\tilde{\bm{\uptheta}}_k^{(1)})\in F^{(2)}(\tilde{\bm\uptheta}_k^{(1)})\cap \mathcal{A}\Big\}\notag\\
%&+\sum_{\ell}\upalpha_{B,\ell}^{(1)}\mathcal{X}\Big\{b_{\ell}^{(1)}(\tilde{\bm{\uptheta}}_k^{(1)},\tilde{\bm{\uptheta}}_k^{(2)})\in B^{(2)}(\tilde{\bm\uptheta}_k)\cap\mathcal{A}\Big\}\notag\\
%&-\sum_{\ell}\upalpha_{F,\ell}^{(1)}\mathcal{X}\Big\{f_{\ell}^{(1)}(\hat{\bm{\uptheta}}_k^{(1)})\in F^{(2)}(\hat{\bm\uptheta}_{(k-1)[I]}^{(1)})\cap\mathcal{B}\Big\}.
\end{align*}
Furthermore, provided it is possible to share $f_{\ell}^{(1)}\left(\bm\uptheta^{[\bm{1}]}\right)$ if and only if it is possible to carry $f_{\ell}^{(1)}\left(\bm\uptheta^{[\bm{1}]}\right)$ from the previous iteration, then
%\begin{align*}
%&\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]}\right)\cap \mathcal{A}_k\Big\}=\notag\\
%&\chi\Big\{f_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{cyc}})^{[\bm{1}]}\right)\in F^{(2)}\left((\hat{\bm\uptheta}_{k}^{\text{cyc}})^{[\bm{1}]}\right)\cap\mathcal{B}_k\Big\},
%\end{align*}
%% To see this note that $\hat{\bm\uptheta}_{(k-1)[I]}^{(1)}=\hat{\bm{\uptheta}}_k^{(1)}$ and that $f_{\ell}^{(1)}(\tilde{\bm{\uptheta}}_k^{(1)})\in F^{(2)}(\tilde{\bm\uptheta}_k^{(1)})$ if and only if $f_{\ell}^{(1)}(\hat{\bm{\uptheta}}_k^{(1)})\in F^{(2)}(\hat{\bm\uptheta}_k^{(1)})$. 
%in which case
 the difference between $c_k^{\text{cyc}}$ and $c_k^{\text{non}}$ under D0--D6 is given by:
% the main result on comparative cost between the cyclic and non-cyclic algorithm is that
\begin{align*}
%\label{eq:dijiliagypsy}
c_k^{\text{cyc}}-c_k^{\text{non}}=\sum_{\ell}\upalpha_{B,\ell}\hspace{.03in}\chi\Big\{b_{\ell}^{(1)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\in B^{(2)}\left((\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{1}]},(\hat{\bm{\uptheta}}_k^{\text{non}})^{[\bm{2}]}\right)\cap\mathcal{A}_k\Big\}.
\end{align*}
%
Here, we can see that under conditions D0--D6 the main difference between the arithmetic cost of a cyclic algorithm and that of its non-cyclic counterpart is due to sharing elements that combine information regarding both subvectors of $\bm\uptheta$. Intuitively, this is due to the fact that by implementing an algorithm in a cyclic manner we lose the ability to reuse any computations involving both $\bm\uptheta^{[\bm{1}]}$ and $\bm\uptheta^{[\bm{2}]}$. Therefore, if a significant cost reduction is achieved by sharing this type of element then an iteration of the non-cyclic algorithm will have a significantly lower cost. 
%If most of the cost reduction stems from sharing terms involving only $\bm\uptheta^{[\bm{1}]}$ or only $\bm{\bm\uptheta}^{[\bm{2}]}$ (no combined terms), then it is reasonable to assume the arithmetic cost is approximately equal for both algorithms.   

%The result from this section is fairly intuitive. However, we have made a few simplifying assumptions in order to facilitate the analysis. 
In practice, the per-iteration cost of implementation will depend strongly on the specific algorithm considered. For the cyclic seesaw SPSA algorithm, for example, a more appropriate definition of cost might be the number of noisy loss function evaluations used per-iteration. If cyclic seesaw SPSA is implemented according to (\ref{eq:moumousika}) along with (\ref{eq:howeardspos1}) and (\ref{eq:howeardspos2}) then the per-iteration cost of implementation would be equal to 4 loss function measurements per-iteration. In the case of the regular SPSA algorithm (see (\ref{eq:pocres})), however, the per-iteration cost of implementation would be only 2 loss function measurements per-iteration. The following section presents some general results on the relative asymptotic efficiency in (\ref{eq:ratio}).
% between cyclic algorithms and their non-cyclic counterparts.
% once cost has been defined.


\section{Approximating Relative Efficiency}
\label{sec:aseficwiener}



 In the previous chapter (see Section \ref{sec:upperpotomacshell}) it was shown that (under certain assumptions) $k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }}\mathcal{N}({\bm\upmu}^{\text{cyc}},{\bm\Sigma}^{\text{cyc}})$
%\begin{align*}
%k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }}\mathcal{N}({\bm\upmu}^{\text{cyc}},{\bm\Sigma}^{\text{cyc}})
%\end{align*}
for some mean vector $\bm\upmu^{\text{cyc}}$ and covariance matrix $\bm\Sigma^{\text{cyc}}$, where $\hat{\bm\uptheta}_k^{\text{cyc}}$ denotes the $k$th iterate of Algorithm \ref{kirkey} and the notation ``$\xrightarrow{\text{\ dist\ }}$'' means convergence in distribution. A similar result is readily obtained for its non-cyclic counterpart. In particular, let $\hat{\bm{\uptheta}}_k^{\text{non}}$ denote the $k$th iterate obtained using the non-cyclic counterpart of Algorithm \ref{kirkey}. Then, under certain assumptions (see Fabian 1968)\nocite{fabian1968} it can be shown that $k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }} \mathcal{N}({\bm\upmu}^{\text{non}},{\bm\Sigma}^{\text{non}})$
%\begin{align*}
%k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }} \mathcal{N}({\bm\upmu}^{\text{non}},{\bm\Sigma}^{\text{non}})
%\end{align*}
for some mean vector ${\bm\upmu}^{\text{non}}$ and covariance matrix ${\bm\Sigma}^{\text{non}}$. This section shows how results on asymptotic normality can be used to approximate the relative efficiency in (\ref{eq:ratio}). 
%An analysis of the approximate relative efficiency is also performed.



 Following the ideas in (Spall, 1992) we assume:
\begin{align}
\label{eq:thressandfive}
\lim_{k\rightarrow \infty}E[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)]=\bm\upmu^{\text{cyc}}, \ \ \ \lim_{k\rightarrow \infty}E[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)]={\bm\upmu}^{\text{non}},
\end{align}
and that:
\begin{align}
\lim_{k\rightarrow \infty}\Var{[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)]}=\bm\Sigma^{\text{cyc}},\ \ \ \lim_{k\rightarrow \infty}\Var{[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)]}=\bm\Sigma^{\text{non}}.
%&\lim_{k\rightarrow \infty}E\left[k^{\upbeta}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)^\top-E[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)]E[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)]^\top\right]=\bm\Sigma^{\text{cyc}},\notag\\
%&\lim_{k\rightarrow \infty}E\left[k^{\upbeta}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)^\top-E[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)]E[k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)]^\top\right]={\bm\Sigma}^{\text{non}}.
\label{eq:suchawalkschon}
\end{align}
Spall (1992) discusses how (\ref{eq:thressandfive}) and (\ref{eq:suchawalkschon}) hold if the terms $\|k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)\|^2$ and $\|k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)\|^2$ are uniformly integrable (see also Laha and Rohatgi, pp. 138--140). Equations (\ref{eq:thressandfive}) and (\ref{eq:suchawalkschon}) allow us to obtain the following approximation for large $k$:
\begin{align*}
E\|\hat{\bm\uptheta}_{k}^{\text{cyc}}-\bm\uptheta^\ast\|^2=&\ \trace{\left[E(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)^\top\right]}
%=k^{-\upbeta} E(k^{\upbeta}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^{\ast})(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^{\ast})^\top\notag\\
\approx k^{-\upbeta}\trace{\left[\bm\Sigma^{\text{cyc}}+\bm\upmu^{\text{cyc}}(\bm\upmu^{\text{cyc}})^\top\right]}.
\end{align*}
Similarly, for large $k$ we approximate:
\begin{align*}
E\|\hat{\bm\uptheta}_{k}^{\text{non}}-\bm\uptheta^\ast\|^2
%=\text{trace}\left[E(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)^\top\right]
\approx k^{-\upbeta}\trace{\left[\bm\Sigma^{\text{non}}+\bm\upmu^{\text{non}}(\bm\upmu^{\text{non}})^\top\right]}.
%E(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)^\top\approx k^{-\upbeta}\left({\bm\Sigma}^{\text{non}}+{\bm\upmu}^{\text{non}}[{\bm\upmu}^{\text{non}}]^\top\right).
\end{align*}
Then, for large $k_1$ and $k_2$ we may approximate (\ref{eq:ratio}) as follows:
\begin{align}
\frac{E\|\hat{\bm\uptheta}_{k_1}^{\text{cyc}}-\bm\uptheta^\ast\|^2}{E\|\hat{\bm\uptheta}_{k_2}^{\text{non}}-\bm\uptheta^\ast\|^2}\approx \left(\frac{k_2}{k_1}\right)^\upbeta\frac{\trace{\left[\bm\Sigma^{\text{cyc}}\right]}+[\bm\upmu^{\text{cyc}}]^\top\bm\upmu^{\text{cyc}}}{\trace{\left[\bm\Sigma^{\text{non}}\right]}+[{\bm\upmu}^{\text{non}}]^\top{\bm\upmu}^{\text{non}}}.
\label{eq:michbuuubl}
\end{align}
%In order to complete our approximation of (\ref{eq:ratio}) all that remains is to . 
Here, we remind the reader that in order to perform a fair comparison between the cyclic and non-cyclic algorithm, the cumulative cost of implementing the cyclic algorithm up to iteration $k_1$ is assumed to be equal (or approximately equal) to that of its non-cyclic counterpart up to iteration $k_2$; an analysis of the asymptotic properties of (\ref{eq:michbuuubl}) would therefore require increasing $k_1$ and $k_2$ at a rate that ensures the comparison is fair at all times. With this in mind, we introduce the following proposition.
\begin{proposition}
\label{prop:omygodsthunder}
Let  $0<c^{\text{cyc}}$ and $0<c^{\text{non}}$ be finite constants such that
% denote the per-iteration cost associated with the cyclic and non-cyclic algorithms, respectively. 
% Assume $c^{\text{cyc}}$ and $c^{\text{non}}$ do not depend on $k$ and that 
 $c^{\text{cyc}}/c^{\text{non}}$ is a rational number. Then, there exists an infinite sequence $\{(k_{1(i)},k_{2(i)})\}_{i=1}^\infty$ in $\mathbb{Z}^+\times\mathbb{Z}^+$ with $k_{1(i-1)}<k_{1(i)}$ and $k_{2(i-1)}<k_{2(i)}$ such that $c^{\text{cyc}}k_{1(i)}=c^{\text{non}}k_{2(i)}$.
\end{proposition}
\begin{proof}
Let $c^{\text{cyc}}/c^{\text{non}}=p/q$ where $p$ and $q$ are strictly positive integers. The desired sequence can be obtained by letting $k_{1(i)}=qi$ and $k_{2(i)}=pi$.
\end{proof}

The significance of Proposition \ref{prop:omygodsthunder} is that if the per-iteration costs $c_k^{\text{cyc}}$ and $c_k^{\text{non}}$ are nonzero, finite, independent of $k$ (so that $c_k^{\text{cyc}}=c^{\text{cyc}}$ and $c_k^{\text{non}}=c^{\text{non}}$), and if $c^{\text{cyc}}/c^{\text{non}}$ is a rational number, then the cost of computing $\hat{\bm{\uptheta}}_{k_{1(i)}}^{\text{cyc}}$ is exactly equal to the cost of computing $\hat{\bm{\uptheta}}_{k_{2(i)}}^{\text{non}}$ for any strictly-positive integer $i$ when $k_{1(i)}$ and $k_{2(i)}$ are as in Proposition \ref{prop:omygodsthunder}. We can then obtain the following result:
\begin{align}
\label{eq:wobble}
\lim_{i\rightarrow \infty}\frac{E\|\hat{\bm\uptheta}_{k_{1(i)}}^{\text{cyc}}-\bm\uptheta^\ast\|^2}{E\|\hat{\bm\uptheta}_{k_{2(i)}}^{\text{non}}-\bm\uptheta^\ast\|^2}= \left(\frac{c^{\text{cyc}}}{c^{\text{non}}}\right)^\upbeta\frac{\trace{\left[{\bm\Sigma}^{\text{cyc}}\right]}+[\bm\upmu^{\text{cyc}}]^\top\bm\upmu^{\text{cyc}}}{\trace{\left[{\bm\Sigma}^{\text{non}}\right]}+[{\bm\upmu}^{\text{non}}]^\top{\bm\upmu}^{\text{non}}}.
\end{align}
%for large values of $i$ (i.e., for large values of $k_{1(i)}$ and $k_{2(i)}$ such that the cumulative cost of the cyclic algorithm up to iteration $k_{1(i)}$ is the same as the cumulative cost of the non-cyclic algorithm up to iteration $k_{2(i)}$). 
The following section uses the limit in (\ref{eq:wobble}) to study the relative efficiency between a special case of Algorithm \ref{kirkey} and its non-cyclic counterpart.




\section{Relative Efficiency: A Special Case}
\label{sec:apsecialcaserelefff}



This section computes the asymptotic relative efficiency between a non-cyclic algorithm and a cyclic algorithm which is a special case of Algorithm \ref{kirkey} in which the sets $\mathcal{S}_j$ do not intersect (this is equivalent to saying that any single entry of $\hat{\bm{\uptheta}}_k$ can only be updated by one processor/agent although each processor/agent may update several entries) and updates are produced in a strictly cyclic manner; this cyclic algorithm is described in more detail in Algorithm \ref{kirkeyspecial}. Given our desire to analyze the effect of a cyclic implementation on asymptotic efficiency, an appropriate non-cyclic counterpart to Algorithm \ref{kirkeyspecial} is given in {\ref{alg:apeparingairshow}}. Here, in order to to isolate the effects of a cyclic implementation on asymptotic efficiency, a diagonal matrix of gains was used in an attempt to make the non-cyclic algorithm as similar to the cyclic algorithm as possible. In the remainder of this section we obtain expressions for the terms $\bm\Sigma^{\text{cyc}}$, $\bm\Sigma^{\text{non}}$, $\bm\upmu^{\text{cyc}}$, and $\bm\upmu^{\text{non}}$ (defined in the opening paragraph of Section \ref{sec:aseficwiener}) in order to estimate the relative efficiency between Algorithms \ref{kirkeyspecial} and \ref{alg:apeparingairshow} in the manner of (\ref{eq:wobble}).

 \begin{algorithm}[!t]                     
\caption{Strictly Cyclic Version of Algorithm \ref{kirkey}}      
\label{kirkeyspecial}                
\begin{algorithmic} [1]                  % enter the algorithmic environment
\setstretch{1.5} 
\REQUIRE    $\hat{\bm{\uptheta}}_0^{\text{cyc}}$, $\{a_k^{(j)}\}_{k\geq 0}$ for $j=1,\dots,d$, and let $\mathcal{S}_1,\dots, \mathcal{S}_d$ be such that (\ref{eq:scurry}) holds. Set $k=0$.
%\STATE{Set $k=0$}.
\WHILE{stopping criterion has not been reached}
\STATE{Set $\hat{\bm\uptheta}_k^{(I_{0})}=\hat{\bm{\uptheta}}_k^{\text{cyc}}$.}
         \FOR{$j=1,\dots,d$}
	\STATE{Define $\hat{\bm\uptheta}_k^{(I_{j})}\equiv \hat{\bm\uptheta}_k^{(I_{j-1})}- {a}_{k}^{(j)}\ \hat{\bm{g}}^{(j)}\left(\hat{\bm\uptheta}_k^{(I_{j-1})}\right)$.
	}
	 \ENDFOR
	 \STATE{Let $\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}\equiv\hat{\bm{\uptheta}}_k^{(I_{d})}$.
	 }
	\STATE{set $k=k+1$}
\ENDWHILE
\end{algorithmic}
\end{algorithm}

%.rather than using a scalar gain sequence we have considered a diagonal matrix of gains. 
%
%The gain sequence has a significant impact on the asymptotic behavior of SA algorithms. Therefore, because of our desire 

 

The following corollary to Theorem \ref{thm:fnogg} will be used to derive expressions for  $\bm\Sigma^{\text{cyc}}$ and $\bm\upmu^{\text{cyc}}$, the parameters of the asymptotic distribution of $k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)$.

\begin{corollary}
\label{eq:hjointcoffees}
Let $\hat{\bm{\uptheta}}_k^{\text{cyc}}$ be generated according to Algorithm \ref{kirkeyspecial}. Additionally, let $\mathcal{F}_k$ denote the sigma field generated by $\{\hat{\bm{\uptheta}}_\ell^{\text{cyc}}\}_{\ell=0}^k$ as well as by any random variables generated  by the algorithm in the production of $\hat{\bm{\uptheta}}_k^{\text{cyc}}$. 
%Let $\bm{W}_k$, $\bm\Gamma_k$, $\bm{T}_k$, $\bm\Phi_k$, and $\bm{V}_k$ be defined as in (\ref{eq:pantyponcho})--(\ref{eq:othingcoodsd}) and assume these variables have real-valued entries. 
Also, assume the following conditions hold (all scalars, matrices, and vectors are assumed to have real entries):
%
%Assume  the iterates for Algorithm \ref{kirkeyspecial} satisfy the following conditions:
%The notation in conditions C0--C8 for the asymptotic normality can be simplified in the case of Algorithm \ref{kirkeyspecial}.
% First, write $\hat{\bm{g}}^{(j)}(\bm\uptheta)=\bm{g}^{(j)}(\bm\uptheta)+\bm\upbeta^{(j)}(\bm\uptheta)+\bm\upxi^{(j)}(\bm\uptheta)$. Then, C0--C8 become:
\begin{description}
\item[C0$'$] $L(\bm\uptheta)$ is twice continuously differentiable, $\bm{H}(\bm\uptheta)$ has bounded entries, and $\hat{\bm\uptheta}_k^{(I_j)}\rightarrow \bm\uptheta^\ast$ w.p.1 for $j=1,\dots, d$.
\item[C1$'$] The same as C1.
%For each $j$,  $a_k^{(j)}>0$ and $k^\upalpha {a}_k^{(j)}\rightarrow r_j<\infty$.
\begin{algorithm}[!t]                     
\caption{Non-Cyclic Counterpart to Algorithm \ref{kirkeyspecial}}      
\label{alg:apeparingairshow}                
\begin{algorithmic} [1]                  % enter the algorithmic environment
\setstretch{1.5} 
\REQUIRE    $\hat{\bm{\uptheta}}_0^{\text{non}}$, $\{a_k^{(j)}\}_{k\geq 0}$ for $j=1,\dots,d$, let $\mathcal{S}_1,\dots, \mathcal{S}_d$ be such that (\ref{eq:scurry}) holds, and let $\bm{A}_k$ be a diagonal matrix with $i$th diagonal entry equal to $a_k^{(j)}$, where $j$ is such that $i\in \mathcal{S}_j$. Set $k=0$.
%\STATE{Set $k=0$}.
\WHILE{stopping criterion has not been reached}
	 \STATE{Let $\hat{\bm{\uptheta}}_{k+1}^{\text{non}}=\hat{\bm{\uptheta}}_k^{\text{non}}-\bm{A}_k\hat{\bm{g}}(\hat{\bm{\uptheta}}_k^{\text{non}})$.
	 }
	\STATE{set $k=k+1$}
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\item[C2$'$]  There exists  an diagonal matrix $\bm{\Lambda}\in \mathbb{R}^{p\times p}$ with strictly positive eigenvalues and a nonsingular matrix $\bm{S}\in \mathbb{R}^{p\times p}$ such that
%\begin{align}
%\label{eq:macnealhuh}
$\bm\Gamma\equiv \sum_{j=1}^{d} r_{j} \bm{J}^{(j)}(\bm\uptheta^\ast)=\bm{AH}(\bm\uptheta^\ast)=\bm{S\Lambda S}^{-1}$ where $\bm{A}$ is the diagonal matrix with $i$th diagonal entry equal to $r_i$, and where $\bm{J}^{(j)}(\bm\uptheta)$ denotes the Jacobian of $\bm{g}^{(j)}(\bm\uptheta)$.
%\end{align}
\item[C3$'$]
 $\upbeta$ and $\upalpha$ satisfy $0<\upbeta\leq \upalpha$. Additionally, for all $j$ there exist a finite vector $\bm{b}^{(j)}\in \mathbb{R}^p$ such that 
%  Let $0<\upbeta\leq \upalpha$. For all $j$ there exists a finite vector $\bm{b}^{(j)}\in \mathbb{R}^p$ such that 
  $k^{\upbeta/2}{\bm{\upbeta}}^{(j)}(\hat{\bm\uptheta}_k^{(I_{j})})\rightarrow \bm{b}^{(j)}$ w.p.1 for all $j$.
%\begin{description}
%\item[(a)] $k^{\upbeta/2}{\bm{\upbeta}}^{(j)}(\hat{\bm\uptheta}_k^{(I_{j})})\rightarrow \bm{b}^{(j)}$ w.p.1.
%\item[(b)] $k^{\upbeta/2}E[{\bm{\upbeta}}^{(j)}(\hat{\bm\uptheta}_k^{(I_{j})})]\rightarrow \bm{b}^{(j)}$.
%\end{description}
\item[C4$'$] For all $j$,
  $E[{\bm{\upxi}}^{(j)}(\hat{\bm\uptheta}_k^{(I_{j})})|\hat{\bm\uptheta}_k^{(I_{j})}]=\bm{0}$. 
%  Furthermore, the vectors $\{{\bm{\upxi}}^{(j)}(\hat{\bm\uptheta}_k^{(I_{j})})\}_{j=1}^d$ are conditionally independent given $\mathcal{F}_k$.
\item[C5$'$]  There exists a constant $C>0$ and a matrix $\bm\Sigma^{(j)}$ such that one of the following holds w.p.1:
\begin{enumerate}[label=(\roman*)]
\item $\upbeta=\upalpha$, $C>\|E[{\bm{\upxi}}^{(j)}\big(\hat{\bm\uptheta}_k^{(I_{j})}\big)[{\bm{\upxi}}^{(j)}\big(\hat{\bm\uptheta}_k^{(I_{j})}\big)]^\top|\mathcal{F}_k]-\bm\Sigma^{(j)}\|\rightarrow 0$.
\item $\upbeta<\upalpha$, $C>\|k^{\upbeta-\upalpha}E[{\bm{\upxi}}^{(j)}\big(\hat{\bm\uptheta}_k^{(I_{j})}\big)[{\bm{\upxi}}^{(j)}\big(\hat{\bm\uptheta}_k^{(I_{j})}\big)]^\top|\mathcal{F}_k]-\bm\Sigma^{(j)}\|\rightarrow 0$.
\end{enumerate}
Additionally, if $\bm{v}_1$ and $\bm{v}_2$ are two different elements of $\{{\bm{\upxi}}_k^{(j)}\big(\hat{\bm\uptheta}_k^{(I_j)}\big)\}_{j}$, then one of the following holds w.p.1:
\begin{enumerate}[label=(\roman*)]
\setcounter{enumi}{2}
\item C5$'$-(i) holds and $C>\|E[\bm{v}_1\bm{v}_2^\top|\mathcal{F}_k]\|\rightarrow 0$.
\item C5$'$-(ii) holds and $C>\|k^{\upbeta-\upalpha}E[\bm{v}_1\bm{v}_2^\top|\mathcal{F}_k]\|\rightarrow 0$.
\end{enumerate}
\item[C6$'$] Let $\bm{M}_B\equiv \sum_{j=1}^d\bm\Sigma^{(j)}$. The matrix $\bm{A}\bm{M}_B\bm{A}$ is positive definite.
\item[C7$'$] One of the following holds:
\begin{enumerate}[label=(\roman*)]
\item $\upbeta=\upalpha$ and B5-(i) holds with $\bm{V}_k$ replaced by ${\bm{\upxi}}^{(j)}\big(\hat{\bm\uptheta}_k^{(I_{j})}\big)$.
\item $\upbeta<\upalpha$ and B5-(i) holds with $\bm{V}_k$ replaced by $k^{(\upbeta-\upalpha)/2}{\bm{\upxi}}^{(j)}\big(\hat{\bm\uptheta}_k^{(I_{j})}\big)$.
\end{enumerate}
\item[C8$'$] The same as B6$'$ with $U_{ii}$ replaced by $\Lambda_{ii}$.
%Let $\uplambda\equiv \min_i{\{\Lambda^{[i,i]}\}}$ where $\Lambda^{[i,i]}$ is the $i$th diagonal entry of $\bm\Lambda$. Let $\upalpha$ and $\upbeta$ be constants such that $0<\upalpha\leq 1$ and $0\leq \upbeta$. Define $\upbeta_+=\upbeta$ if $\upalpha=1$ and $\upbeta_+=0$ otherwise. Let $\upbeta_+<2\uplambda$.
\end{description}
Then, $k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }}\mathcal{N}({\bm\upmu}^\text{cyc},{\bm\Sigma}^\text{cyc})$
%\begin{align*}
%k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{cyc}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }}\mathcal{N}({\bm\upmu}^\text{cyc},{\bm\Sigma}^\text{cyc}),
%\end{align*}
 with $\bm\upmu^{\text{cyc}}= -\bm{S}[\bm{\Lambda}-\upbeta_+/2\bm{I}]^{-1} \bm{S}^{-1}\bm{A}\bm{b}^\text{cyc}$ and $\bm\Sigma^{\text{cyc}}=\bm{SQ}^{\text{cyc}}\bm{S}^\top$, where
\begin{align}
\label{eq:jepanuj}
\bm{b}^\text{cyc}\equiv\sum_{j=1}^d \bm{b}^{(j)}, \ \ \ {Q}^\text{cyc}_{ij}&=\frac{\left[\bm{S}^{-1}\bm{A}\bm{M}_B\bm{A}(\bm{S}^{-1})^\top\right]_{ij}}{\Lambda_{ii}+\Lambda_{jj}-\upbeta_+}.
\end{align}
\end{corollary}
\begin{proof}
Since C0$'$--C8$'$ imply C0--C8, the result follows from Theorem \ref{thm:fnogg}.
\end{proof}



The following corollary to Theorem \ref{thm:fnogg} will be used to derive expressions for  $\bm\Sigma^{\text{non}}$ and $\bm\upmu^{\text{non}}$, the parameters of the asymptotic distribution of $k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)$.

\begin{corollary}
\label{eq:tarattatarantanand}
Let $\hat{\bm{\uptheta}}_k^{\text{non}}$ be generated according to Algorithm \ref{alg:apeparingairshow}. Additionally, let $\mathcal{F}_k$ denote the sigma field generated by $\{\hat{\bm{\uptheta}}_\ell^{\text{non}}\}_{\ell=0}^k$ as well as by any random variables generated  by the algorithm in the production of $\hat{\bm{\uptheta}}_k^{\text{non}}$. Also, assume the following conditions hold (all scalars, matrices, and vectors are assumed to have real entries):
%
% Let us now derive similar conditions for the asymptotic normality of the non-cyclic variant (Algorithm \ref{alg:apeparingairshow}).  Translating C0$'$--C8$'$ into conditions for the asymptotic normality of Algorithm \ref{alg:apeparingairshow} (i.e., setting the number of subvectors and the number of updates per-iteration equal to one) gives:
\begin{description}
\item[C0$''$] $L(\bm\uptheta)$ is twice continuously differentiable, $\bm{H}(\bm\uptheta)$ has bounded entries, and $\hat{\bm\uptheta}_k^{\text{non}}\rightarrow \bm\uptheta^\ast$ w.p.1.
%\item[C1$''$] The same as C1$'$.
%\item[C2$''$] The same as C2$'$.
% There exists  an diagonal matrix $\bm{\Lambda}\in \mathbb{R}^{p\times p}$ with strictly positive eigenvalues and a nonsingular matrix $\bm{S}\in \mathbb{R}^{p\times p}$ such that
%$\bm\Gamma\equiv \bm{AH}(\bm\uptheta^\ast)=\bm{S\Lambda S}^{-1}$.
\item[C3$''$]  $\upbeta$ and $\upalpha$ satisfy $0<\upbeta\leq \upalpha$. Additionally, there exist a finite vector $\bm{b}^{\text{non}}\in \mathbb{R}^p$ such that  $k^{\upbeta/2}{\bm{\upbeta}}\big(\hat{\bm\uptheta}_k\big)\rightarrow \bm{b}^{\text{non}}$ w.p.1.
% , where $\bm{b}^{\text{cyc}}$ is as in C3$'$.
\item[C4$''$]  $E[{\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)|\hat{\bm{\uptheta}}_k]=\bm{0}$.
\item[C5$''$]  There exists a constant $C>0$ and a matrix $\bm{M}$ such that one of the following holds w.p.1:
\begin{enumerate}[label=(\roman*)]
\item $\upbeta=\upalpha$, $C>\|E[{\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)[{\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)]^\top|\mathcal{F}_k]-\bm{M}\|\rightarrow 0$.
\item $\upbeta<\upalpha$, $C>\|k^{\upbeta-\upalpha}E[{\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)[{\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)]^\top|\mathcal{F}_k]-\bm{M}\|\rightarrow 0$.
\end{enumerate}
\item[C6$''$] $\bm\Sigma\equiv \bm{A}{\bm{M}}\bm{A}$ is a positive definite matrix.
\item[C7$''$] One of the following holds:
\begin{enumerate}[label=(\roman*)]
\item $\upbeta=\upalpha$ and B5-(i) holds with $\bm{V}_k$ replaced by ${\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)$.
\item $\upbeta<\upalpha$ and B5-(i) holds with $\bm{V}_k$ replaced by $k^{(\upbeta-\upalpha)/2}{\bm{\upxi}}\big(\hat{\bm\uptheta}_k\big)$.
\end{enumerate}
\item[C1$''$, C2$''$, \& C8$''$] The same as C1$'$, C2$'$, and C8$'$, respectively.
\end{description}
%If $\hat{\bm{\uptheta}}_k^{\text{non}}$ satisfies conditions C0$''$--C8$''$ Theorem \ref{thm:generalizefabian} implies
Then, $k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }}\mathcal{N}({\bm\upmu}^\text{non},{\bm\Sigma}^\text{non})$ with ${\bm\upmu}^\text{non}= -\bm{S}[\bm{\Lambda}-\upbeta_+/2\bm{I}]^{-1} \bm{S}^{-1}\bm{A}\bm{b}^\text{non}$ and $\bm\Sigma^{\text{non}}=\bm{SQ}^{\text{non}}\bm{S}^\top$, where
%
%\begin{align*}
%k^{\upbeta/2}(\hat{\bm\uptheta}_k^{\text{non}}-\bm\uptheta^\ast)\xrightarrow{\text{\ dist\ }}\mathcal{N}({\bm\upmu}^\text{cyc},{\bm\Sigma}^\text{non}),
%\end{align*}
%where  with
\begin{align}
\label{eq:diamonddrone}
{Q}^\text{non}_{ij}=\frac{\left[\bm{S}^{-1}\bm{A}\bm{M}\bm{A}(\bm{S}^{-1})^\top\right]_{ij}}{\Lambda_{ii}+\Lambda_{jj}-\upbeta_+}.
\end{align}
\end{corollary}
\begin{proof}
Since C0$''$--C8$''$ imply C0--C8, the result follows from Theorem \ref{thm:fnogg}
%The result follows from Theorem \ref{thm:generalizefabian}. The proof is very similar to the proof of Theorem \ref{thm:fnogg}.
\end{proof}


The validity of C0$'$--C8$'$ and C0$''$--C8$''$ is directly related to the validity of C0--C8 (see Section \ref{sec:bonestrailseason} for an in-depth discussion on this topic). Using the expressions for $\bm\Sigma^{\text{cyc}}$, $\bm\upmu^{\text{cyc}}$, $\bm\Sigma^{\text{non}}$, and $\bm\upmu^{\text{non}}$ from Corollaries \ref{eq:hjointcoffees} and \ref{eq:tarattatarantanand} along with the values of $c^\text{non}$ and $c^\text{cyc}$ we can compute the estimate in (\ref{eq:wobble}). In general, however, the study of this ratio is rather complicated. In order to obtain a simple expression for (\ref{eq:wobble}) we will consider a special case.
 
\begin{proposition}
\label{prop:exploringeoss}
Let $\hat{\bm{\uptheta}}_k^{\text{cyc}}$ be obtained according to Algorithm \ref{kirkeyspecial} and let $\hat{\bm{\uptheta}}_k^{\text{non}}$ be obtained according to Algorithm \ref{alg:apeparingairshow}. Assume the following:
\begin{DESCRIPTION}
\item[E0] Conditions C0$'$--C8$'$ and C0$''$--C8$''$ hold.
\item[E1]  $\upbeta>0$ and ${a}_k^{(j)}>0$ for $j=1,\dots,d$ are the same for both Algorithms \ref{kirkeyspecial} and \ref{alg:apeparingairshow}.
\item[E2] $\bm{b}^{\text{cyc}}=\bm{b}^{\text{non}}$ (e.g., as in the SG and CSG algorithms).
\item[E3] At least one of the following holds:
\begin{enumerate}[label=(\roman*)]
\item $\bm{S}=c\bm{I}$ for some constant $c$ (i.e., $\bm{H}(\bm\uptheta^\ast)$ is a diagonal matrix).
\item $\bm{M}_B=\bm{M}$ (e.g., when the entries of the $\bm\upxi_k$ are independent given $\mathcal{F}_k$).
\end{enumerate}
\end{DESCRIPTION}
%
Then, when $k_{1(i)}$ and $k_{2(i)}$ are as in Proposition \ref{prop:omygodsthunder} the limit in (\ref{eq:wobble}) becomes:
\begin{align}
\label{eq:horsesrrsesriding}
\lim_{i\rightarrow \infty}\frac{E\|\hat{\bm\uptheta}_{k_{1(i)}}^{\text{cyc}}-\bm\uptheta^\ast\|^2}{E\|\hat{\bm\uptheta}_{k_{2(i)}}^{\text{non}}-\bm\uptheta^\ast\|^2}= \left(\frac{c^{\text{cyc}}}{c^{\text{non}}}\right)^\upbeta.
\end{align}
%for large values of $i$.
\end{proposition}
\begin{proof}
First, note that E0 implies the results of Corollaries \ref{eq:hjointcoffees} and \ref{eq:tarattatarantanand} hold. Then, E1 and E2 imply $\bm\upmu^{\text{cyc}}=\bm\upmu^{\text{non}}$. Next, E2 along with (\ref{eq:jepanuj}) and (\ref{eq:diamonddrone}) implies that $\trace{[{\bm\Sigma}^{\text{cyc}}]}=\trace{[{\bm\Sigma}^{\text{non}}]}$. The relationship in (\ref{eq:horsesrrsesriding}) then follows from (\ref{eq:wobble}).
\end{proof}

An implication of Proposition \ref{prop:exploringeoss} is that the asymptotic relative efficiency is entirely determined by $c^{\text{cyc}}$ and $c^{\text{non}}$. If ${c^{\text{cyc}}}/{c^{\text{non}}}>1$ then the non-cyclic algorithm is more efficient, if ${c^{\text{cyc}}}/{c^{\text{non}}}<1$ then the cyclic algorithm is more efficient, and if ${c^{\text{cyc}}}/{c^{\text{non}}}=1$ then both algorithms are equally efficient. 
%The approximation in (\ref{eq:horsesrrsesriding}) also holds if the condition that $\bm{S}=c\bm{I}$ is replaced by the assumption 
%
In general, however, it is not easy to see whether ratio in (\ref{eq:wobble}) is greater than one, less than one, or equal to one. Next we show that when E3 does not hold
% simply relaxing the assumption that $\bm{H}(\bm\uptheta^\ast)$ is a diagonal matrix can result in 
 then having ${c^{\text{cyc}}}/{c^{\text{non}}}<1$ does not imply the cyclic algorithm is asymptotically more efficient. Similarly, having ${c^{\text{cyc}}}/{c^{\text{non}}}>1$ does not imply the non-cyclic algorithm is asymptotically more efficient and having ${c^{\text{cyc}}}/{c^{\text{non}}}=1$ does not imply both algorithms are asymptotically equally efficient.
% when $\bm{M}_B\neq \bm{M}$.
 
 
 % One assumption we make is that the constant $\upbeta$ and the sequence ${a}_k^{(j)}$ for $j=1,\dots,d$ are the same for both Algorithm \ref{kirkeyspecial} and Algorithm \ref{alg:apeparingairshow} (this assumption is imposed in order to isolate the effects of a cyclic implementation on efficiency).

Let us assume that condition E3 does not hold. Specifically, the matrix $\bm{S}$ is not a multiple of the identity matrix and that $\bm{M}_B\neq \bm{M}$. In this case, the limit of the ratio in (\ref{eq:wobble}) may be greater than one even when ${c^{\text{cyc}}}/{c^{\text{non}}}<1$, less than one even when ${c^{\text{cyc}}}/{c^{\text{non}}}>1$, and different from one even when ${c^{\text{cyc}}}/{c^{\text{non}}}=1$. To illustrate this fact we consider the special case where $\bm{b}^{\text{cyc}}$ and $\bm{b}^{\text{non}}$, the asymptotic values of normalized bias vectors (see (\ref{eq:jepanuj}) and conditions C3$'$ and C3$''$ for the formal definitions of these vectors), are identically $\bm{0}$. This is a valid assumption when the update directions are SG-based. Here,
\begin{align}
\label{eq:provewrongnewsjoey}
\lim_{i\rightarrow \infty}\frac{E\|\hat{\bm\uptheta}_{k_{1(i)}}^{\text{cyc}}-\bm\uptheta^\ast\|^2}{E\|\hat{\bm\uptheta}_{k_{2(i)}}^{\text{non}}-\bm\uptheta^\ast\|^2}= \left(\frac{c^{\text{cyc}}}{c^{\text{non}}}\right)^\upbeta\frac{\trace{\left[{\bm\Sigma}^{\text{cyc}}\right]}}{\trace{\left[{\bm\Sigma}^{\text{non}}\right]}}.
\end{align}
%We then show that the ratio $\trace{\left[\bm\Sigma^{\text{cyc}}\right]}/\trace{\left[\bm\Sigma^{\text{non}}\right]}$ can be greater- or less than $(c^{\text{cyc}}/c^{\text{non}})^{-\upbeta}$. 
%
%(as in the SG and CSG algorithms) and $\bm{A}=\bm{I}$. Then, we give an example of a loss function
%
Furthermore, we assume $\bm{A}=\bm{I}$, $\upalpha<1$ (so that $\upbeta_+=0$ in condition B6$'$) and that the block-diagonal matrix $\bm{M}_B$ (appearing in condition C5$'$) coincides with $\bm{M}$ (appearing in condition  C5$''$) on the block-diagonal part of $\bm{M}_B$. Specifically, there exist block matrices $\bm{B}_1,\dots,\bm{B}_p$ such that:
\begin{align}
\label{eq:timewillshowr}
\setstretch{1.8} 
\bm{M}_B=\left[\begin{array}{ccc}\bm{B}_1 & \bm{0} & \bm{0} \\\bm{0} & \ddots & \bm{0} \\\bm{0} & \bm{0} & \bm{B}_d\end{array}\right], \ \ \ \bm{M}=\left[\begin{array}{ccc}\bm{B}_1 & \bm{\ast} & \bm{\ast} \\\bm{\ast} & \ddots & \bm{\ast} \\\bm{\ast} & \bm{\ast} & \bm{B}_d\end{array}\right],
\end{align}
where $\bm\ast$ denote possibly non-zero entries and $\bm{0}$ denotes a matrix of zeros of the appropriate dimension. Let us discuss a situation where the assumption in (\ref{eq:timewillshowr}) is satisfied. First, under conditions C4$'$ and C4$''$ it follows from (\ref{eq:avatarparticulatsfs}) that $\bm{M}_B$ corresponds to the limiting (conditional) covariance of $k^{(\upbeta-\upalpha)/2}[\bm\upxi_k^{(1)}(\hat{\bm{\uptheta}}_k^{(I_1)})+\cdots+\bm\upxi_k^{(d)}(\hat{\bm{\uptheta}}_k^{(I_d)})]$ while $\bm{M}$ represents the limiting (conditional) covariance of $k^{(\upbeta-\upalpha)/2}\bm\upxi_k(\hat{\bm{\uptheta}}_k^{\text{non}})$. Under condition C5$'$-(iii) and C5$'$-(iv), however,
% C5$'$-(i), C5$'$-(ii), and C5$''$-(i),
%% Assume that hold. Then, $\bm{M}_B$ represents the limiting (conditional) covariance of $\bm\upxi_k^{(1)}(\hat{\bm{\uptheta}}_k^{(I_1)})+\cdots+\bm\upxi_k^{(d)}(\hat{\bm{\uptheta}}_k^{(I_d)})$ while $\bm{M}$ represents the limiting (conditional) covariance of $\bm\upxi_k(\hat{\bm{\uptheta}}_k^{\text{non}})$.
%  If the noise terms (the $\bm\upxi_k$'s) do not depend on $\bm\uptheta$ then, due to the (conditional) independence of the $\bm\upxi_k^{(j)}$ terms in the cyclic algorithm, 
 it follows that $\bm{M}_B$ must be a block diagonal matrix (i.e., $\bm{M}_B$ must have the form in (\ref{eq:timewillshowr})), this contrasts with the matrix $\bm{M}$ which may have extra nonzero entries due to the possible asymptotic correlation between the entries of $\bm\upxi_k$.

  
  Consider now the following example. Let :
\begin{align}
\label{eq:firstcontactwars}
\setstretch{1.25} 
\bm{H}(\bm\uptheta^\ast)=\left[\begin{array}{cc}2 & -1 \\-1 & 2\end{array}\right],\ \ \ \bm{M}_B=\left[\begin{array}{cc}2 & 0 \\0 & 2\end{array}\right],\ \ \  \bm{M}=\left[\begin{array}{cc}2 & 1 \\1 & 2\end{array}\right].
\end{align}
The positive definite matrix $\bm{H}(\bm\uptheta^\ast)$ (with eigenvalues 1 and 3) might correspond, for example, to the loss function $L(\bm\uptheta)=\bm\uptheta^\top \bm{H}(\bm\uptheta^\ast)\bm\uptheta$. Then $\bm\Gamma=\bm{AH}(\bm\uptheta^\ast)=\bm{H}(\bm\uptheta^\ast)$ is positive definite and satisfies:
\begin{align*}
\setstretch{1.25} 
\bm\Gamma=\bm{S}\left[\begin{array}{cc}1 & 0 \\0 & 3\end{array}\right]\bm{S}^{-1},\text{ with }\bm{S}=\frac{1}{\sqrt{2}}\left[\begin{array}{cc}-1 & -1 \\-1 & 1\end{array}\right].
\end{align*}
Under the above conditions and using the definitions of $\bm\Sigma^{\text{cyc}}$ and $\bm\Sigma^{\text{non}}$ given in Corollaries \ref{eq:hjointcoffees} and \ref{eq:tarattatarantanand}: $\trace{\left[\bm\Sigma^{\text{cyc}}\right]}/\trace{\left[\bm\Sigma^{\text{non}}\right]}=4/5$. Here, (\ref{eq:provewrongnewsjoey}) implies that the {\it{cyclic algorithm is asymptotically more efficient if and only if}} $c^{\text{cyc}}/c^{\text{non}}<(5/4)^{-\upbeta}$. 
%
 Now, say we modify $\bm{M}_B$ and $\bm{M}$ as follows (while keeping $\bm{H}(\bm\uptheta^\ast)$ as in (\ref{eq:firstcontactwars})):
\begin{align*}
%\label{eq:packincase2}
\setstretch{1.25} 
\bm{M}_B=\left[\begin{array}{cc}2 & 0 \\0 & 2\end{array}\right], \ \ \ \bm{M}=\left[\begin{array}{cc}2 & -1 \\-1 & 2\end{array}\right]
\end{align*}
%(notice the off diagonal entries of $\bm{M}$ are now negative). 
Then, $\trace{\left[\bm\Sigma^{\text{cyc}}\right]}/\trace{\left[\bm\Sigma^{\text{non}}\right]}=4/3$. In this case, (\ref{eq:provewrongnewsjoey}) implies that the {\it{cyclic}} {\it{algorithm is asymptotically more efficient if and only if}} $c^{\text{cyc}}/c^{\text{non}}<(3/4)^{-\upbeta}$. 
%
%
%$\text{trace} \left(\bm\Sigma^{\text{non}}-\bm\Sigma^{\text{cyc}}\right)=-1/3<0$ so that the non cyclic implementation is more efficient. 
This example illustrates the fact that there is a delicate balance between $\bm{S}$, $\bm\Lambda$, $\bm{A}$, $\bm{M}$, $\upbeta$, and ${c^{\text{cyc}}}/{c^{\text{non}}}$ that determines which algorithm is more efficient. 
%The following section contains a numerical study on efficiency.
%Table \ref{} summarizes the results of this section.


%
%\section{On Confidence Regions}
%\label{sec:effinconfreg}




\section{Concluding Remarks}
\label{eq:hodgmodgepodge}

In order to perform a fair comparison between any two algorithms it is necessary to define the cost of implementing each algorithm. Generally, the definition of ``cost'' is highly problem-specific. This chapter begins by considering the case where cost is a measure of the number of arithmetic operations needed to perform a single iteration. Under certain assumptions, Section \ref{sec:costoport} pinpointed the type of arithmetic operations that result in a difference between the cost of implementing the cyclic seesaw algorithm and the cost of implementing its non-cyclic counterpart. This chapter also provided an approximation to the limiting value of the relative efficiency in (\ref{eq:ratio}), which takes into consideration the per-iteration costs of implementing the cyclic- and non-cyclic algorithms, for comparing Algorithm \ref{kirkeyspecial} to Algorithm \ref{alg:apeparingairshow}. The approximation to the asymptotic relative efficiency was based on the asymptotic normality results from Section \ref{sec:upperpotomacshell}. This chapter also showed that the approximate asymptotic relative efficiency is, under certain conditions, entirely determined by the per-iteration costs of implementing the two algorithms. In general, however, there is a delicate balance between the gain sequences, the covariance matrix of the noise terms, the Hessian matrix of $L(\bm\uptheta)$, and the per-iteration implementation costs that determines which method is more efficient. 










==> thesis arXiv 2/chapter5.tex <==
%!TEX root = root.tex

\chapter[A Zero-Communication Multi-Agent Problem]{A Zero-Communication Multi-Agent Problem}
\label{chap:multiagent}
\chaptermark{A Zero-Communication Multi-Agent Problem}

This chapter investigates the numerical performance of cyclic SA applied to a multi-agent optimization problem for tracking and surveillance with no communication between agents. Here, a group of agents equipped with finite-range sensors and no communication abilities can adjust their positions in order to collectively accomplish the following objectives:
\begin{DESCRIPTION}
\label{eq:sandywpusstod}
%\item[Objective 1:] Detect the presence of moving targets within a certain area.
\item[Objective 1:] Track any detected targets within a certain area.
\item[Objective 2:] Maximize the probability of detecting other targets in the area, that is maximize the collective coverage of the area of interest.
\end{DESCRIPTION}
To address the two points above, it is assumed that each agent can obtain noisy information regarding the current position of nearby agents and targets and, using this noisy information, each agent decides what its next action should be. The outline of this chapter is as follows. Section \ref{sec:probdescription} describes the details behind the multi-agent optimization problem. Section \ref{sec:proposedapproach} then proposes a cyclic SA approach for solving the optimization problem from Section \ref{sec:probdescription}. Lastly, Section \ref{sec:numericsamultiagent} contains numerical results and Section \ref{sec:finalcommentsagent} contains concluding remarks.

\section{Problem Description}
\label{sec:probdescription}

Throughout this chapter we let $\bm{x}_j(t)=[x_j^N(t),x_j^E(t), \dot{x}_j^N(t), \dot{x}_j^E(t)]^\top\in \mathbb{R}^4$ denote the vector of positions (in $\mathbb{R}^2$) and velocity (in $\mathbb{R}^2$) of agent $j$ at time $t$. The four-dimensional $\bm{x}_j(t)$ is said to be the state vector of agent $j$ at time $t$. Here, the superscripts ``E'' and ``N'' are used to denote agent $j$'s position in the east and north directions, respectively, relative to some artificial center (corresponding to the point $(0,0)$ on the Cartesian plane) that is universal to all agents and targets (this notation is used as a proxy for the standard $(x,y)$ coordinate notation due to the fact that the letter ``$\bm{y}$'' will be used to denote the state vector of a target). 
%The vector $\bm\uptheta(t)\in \mathbb{R}^{4n}$ will then denote the vector composed of the vectors $\bm{x}_1(t),\dots, \bm{x}_n(t)$. Thus, $\bm\uptheta(t)$ is the vector of positions and velocities of $n$ agents. 
The position and velocity of the $i$th target at time $t$ will be represented by the state vector $\bm{y}_i(t)=[y_i^N(t),y_i^E(t), \dot{y}_i^N(t), \dot{y}_i^E(t)]^\top\in \mathbb{R}^4$ 
%$\bm{y}_i(t)$ is said to be the state vector of target $i$ at time $t$ 
(the range of $i$ is unspecified since the number of targets is unknown and may change with time). Each agent is assumed to be equipped with a sensor capable of estimating the positions of nearby agents and targets. The sensor model is described next.

\subsection{The Sensor Model}


When the target location is unknown, each agent is allowed to take a readings from its surroundings and collect estimated positions of any detected agents and targets. To model a sensor's probability of detection we use a variant of the sensor model from Kim et al. (2005)\nocite{kimsensormodel2005}. Here, it is assumed that there exists a constant $r>0$, referred to as the range of the sensor, such that an agent cannot detect any target/agent located at a distance greater than $r$ from the sensor. It is also assumed that there exists a constant $r'>0$ with $r'<r$ such that any target/agent located within a distance of $r'$ from the sensor's location will be detected (w.p.1). A target/agent located within the range of the sensor but at a distance larger than $r'$ will be detected with a probability that decreases linearly as the distance to the target approaches $r$. Specifically, if $d$ is the distance from a target/agent to a sensor, then the probability of detecting said target/agent is given by: 
\begin{align}
{\text{Probability of Detection}} = \begin{cases} 1 &\mbox{if } d \leq  r', \\
1-\frac{d-r'}{r-r'} &\mbox{if } r'<d \leq  r,\\
 0 & \mbox{if } d>r. \end{cases}
 \label{eq:sensorequationmodel}
\end{align}
\afterpage{%
\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{242, 242, 242}
   \definecolor{mynewcoloring2}{RGB}{217, 217, 217}
%\node[inner sep=0pt] (probe) at (0,0.1) {\includegraphics[scale=0.2]{Graphics/submarine_white-eps-converted-to.pdf}}; 
\draw[thick, draw=white, fill=mynewcoloring2] (0,0) circle (2.5cm);
%\draw[thick, dashed] (0,0) circle (2.2cm);
\draw[thick, draw=white, fill=white] (0,0) circle (1.5cm);

\draw[->, dotted, thick] (0,0)--(0,1.5);
\draw[->, dotted, thick] (0,0)--(-1.76,-1.76);
\node at (-1.6, -1.1) {$r$};
\node at (-0.35,0.75) {$r'$};

\node[inner sep=0pt] (probe) at (0,0.1) {\includegraphics[scale=0.2]{Graphics/submarine-eps-converted-to.pdf}}; 


\end{tikzpicture}
\caption[The sensor model]{The probability of detection is 1 for agents/targets located within a radius of $r'$. The probability of detection in the gray annulus decreases as the distance to the agent's sensor increases.  An agent cannot detect any agent/target located at a radius greater than $r$, the sensor's range.}
\label{fig:sensormodel}
\end{figure} 
}
Figure \ref{fig:sensormodel} illustrates (\ref{eq:sensorequationmodel}).{\footnote{The submarine graphic in Figure \ref{fig:sensormodel} was created by Freepik (www.freepik.com) and is licensed under the Attribution 3.0 Unported (CC BY 3.0) license.}} The difference between the sensor model in sensor model in (\ref{eq:sensorequationmodel}) and the sensor model in Kim et al. (2005)\nocite{kimsensormodel2005} is that (\ref{eq:sensorequationmodel}) assumes the probability of detection decreases linearly within the gay annulus in Figure \ref{fig:sensormodel}, whereas Kim et al. (2005)\nocite{kimsensormodel2005} allow this decrease to be nonlinear.




When an agent's sensor detects a target or another agent, we assume the sensor can also collect noisy information regarding the position of said target/agent. In the case where target $i$ is detected by agent $j$ at time $t$, then agent $j$ 
%
%an agent with state vector $\bm{x}(t)\in \mathbb{R}^4$ (we are omitting the index $j$ for simplicity) detects a target with state vector $\bm{y}(t)\in \mathbb{R}^4$ (we are omitting the index $i$ for simplicity) at time $t$, then the agent 
%
can also obtain noisy measurements of
\begin{align}
\upvarphi(\bm{x}_j(t),\bm{y}_i(t))\equiv&\ \text{tan}^{-1}{\left[\frac{y_i^{N}(t)-x_j^{N}(t)}{y_i^{E}(t)-x_j^{E}(t)}\right]}\notag\\
&+\chi\{y_i^{E}(t)-x_j^{E}(t)<0\} \uppi,
\label{eq:badabada1}
\end{align}
 the angle to the target (here $\chi\{\mathcal{E}\}$ is the indicator function of the event $\mathcal{E}$), and
 \begin{align}
 \label{eq:badabada2}
 \uprho(\bm{x}_j(t),\bm{y}_i(t))\equiv\sqrt{(y_i^{N}(t)-x_j^{N}(t))^2+(y_i^{E}(t)-x_j^{E}(t))^2},
 \end{align}
  the Euclidean distance to the target. The noisy measurements regarding the position of target $i$ that are available to agent $j$ are assumed to be of the form:
%   captured by the vector $\bm{z}_{j:i}(t)\in \mathbb{R}^2$ defined as:
\begin{align}
\label{eq:elevatormusic}
\bm{z}_{j:i}(t)\equiv \left[\begin{array}{c}\upvarphi(\bm{x}_j(t),\bm{y}_i(t)) \\\uprho(\bm{x}_j(t),\bm{y}_i(t))\end{array}\right]+\bm{v}\in \mathbb{R}^2,
\end{align}
where $\bm{v}\sim \mathcal{N}(\bm{0},\bm{R})$ for a diagonal covariance matrix $\bm{R}$. A similar model to  (\ref{eq:elevatormusic}) is assumed for an agent detecting another agent. 
%More specifically, if agent $j$ detects agent $i$, it is assumed that agent $j$ can obtain noisy measurements of the angle and distance to agent $i$.
In the sensor model above, agents do now know the true position or velocity of the target(s) or of any other agent; only noisy observations of the distance and angle to any detected agent/target are available. However, it is assumed that an agent can correctly classify any detected individual as either an agent or a target. It is also assumed that an agent can temporarily assign names or ``tags'' to detected agents/targets  order to match an agent/target's previous observed position to its current observed position. If an agent ever loses track (i.e., fails to detect) a previously detected agent/target, it is assumed that the tag for that agent/target resets, that is the agent can no longer match the previously detected agent/target to any agent/target detected in the future.

\subsection{The Loss Function to Minimize}
\label{sec:idealloss}

In order to motivate the choice of loss function to minimize, let us begin by considering a simplified setting where there is only one agent and one target. Here, if the agent detects the target at time $t$, a natural strategy for the agent to implement is to attempt to have $[x_1^E(t+\updelta t),x_1^N(t+\updelta t)]$, the agent's position at time $t+\updelta t$ with $\updelta t>0$, resemble $[y_1^E(t+\updelta t),y_1^N(t+\updelta t)]$, the target's position at time $t+\updelta t$. If $\bm{y}_1(t+\updelta t)$ were known, the agent could attempt to minimize the function $\|[x_1^E(t+\updelta t),x_1^N(t+\updelta t)]-[y_1^E(t+\updelta t),y_1^N(t+\updelta t)]\|^2/2$ with respect to $[x_1^E(t+\updelta t),x_1^N(t+\updelta t)]$. 
%Although $\bm{y}_1(t+\updelta t)$ is unknown in practice, let us temporarily continue under this simplified setting where $\bm{y}_1(t+\updelta t)$ is known.
 Consider now the case where there are $n$ agents and one target and assume agent $j$ detects the target at time $t$. Furthermore, let us temporarily assume that agent $j$ knows the values of $[y_1^E(t+\updelta t),y_1^N(t+\updelta t)]$ and  $[x_i^E(t+\updelta t),x_i^N(t+\updelta t)]$ for $i\neq j$, that is agent $j$ knows the future positions of all agents and targets (this assumption will be weakened later on). If agent $j$ determines that several agents will be close to the target at time $t+\updelta t$ then, in light of Objective 2 on p. \pageref{eq:sandywpusstod}, it may no longer be desirable for agent $j$ to move towards the target's position. Instead, a more appropriate strategy for agent $j$ might be to move away from the target's position in an attempt to maximize the overall probability of detecting other targets that may be in the area of interest (AOI). Even in this simplified setting where we are assuming that the future positions of the target and of all other agents are known to agent $j$, it is unclear {\it{where specifically}} agent $j$ should move if it decides to move away from the target's position. Motivated by the paper by Lee et al. (2015)\nocite{leeetal2015robotics}, we propose to let agent $j$ move to the center of mass of its estimated Voronoi cell. This approach is based on the idea of attempting to have agents ``spread out'' when not actively tracking a target. Details are given next.


\afterpage{%
\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/multiagent/voronoi-eps-converted-to.pdf}};  
\end{tikzpicture}
\caption[A Voronoi tesselation based on the positions of the agents]{Voronoi tessellation where circles mark the positions of the agents. The Voronoi tessellation is unique. Cells depend on the positions of the agents.}
\label{fig:voronoi}
\end{figure} 
}

When agent $j$ is not actively tracking a target, that is when the agent is not addressing Objective 1, the agent should be attempting to address Objective 2. In this light, agent $j$ should take action to increase the overall coverage of the AOI (loosely speaking, we want the agents to ``spread out'' when not actively tracking a target). For this we define the following coverage function:
\begin{align}
\label{eq:coveragefunc}
H(P_1,\dots,P_n,[x_1^E,x_1^N]^\top,\dots, [x_n^E,x_n^N]^\top)\equiv \sum_{j=1}^n\int_{P_j}\|\bm{q}-[x_j^E,x_j^N]^\top\|^2\  d\bm{q},
\end{align}
where $P_1,\dots, P_n$ are subsets of $\mathbb{R}^2$ that form a partition of the AOI (a partition of the AOI is a collection of disjoint cells whose union is equal to the entire AOI). Minimizing (\ref{eq:coveragefunc}) is equivalent to maximizing the coverage of the AOI. Moreover, it is known (see, for example, Lee et al. 2015)\nocite{leeetal2015robotics} that minimizing (\ref{eq:coveragefunc}) is equivalent to minimizing the following function:
\begin{align}
\label{eq:minimizemeImhard}
F([x_1^E,x_1^N]^\top,\dots, [x_n^E,x_n^N]^\top)\equiv  \sum_{j=1}^n\int_{V_j}\|\bm{q}-[x_j^E,x_j^N]^\top\|^2\  d\bm{q},
\end{align}
where $V_j\subset \mathbb{R}^2$ is the $j$th Voronoi cell defined as the set of points that are at least as close (in Euclidean distance) to agent $j$ than to any other agent (Figure \ref{fig:voronoi} gives an example of a Voronoi tessellation, a partition where the cells are Voronoi cells). While minimizing (\ref{eq:minimizemeImhard}) is difficult, a critical point of (\ref{eq:minimizemeImhard}) is obtained when $[x_j^E,x_j^N]^\top=\bm{c}_j$, where
\begin{align*}
\bm{c}_j=[c_j^E,c_j^N]^\top\equiv \frac{\int_{\bm{q}\in V_j}\bm{q}\ d\bm{q}}{\text{Area of $V_j$}}
\end{align*}
is the center of mass of $V_j$. This suggests that 
%he fact that $[x_j^E,x_j^N]^\top=\bm{c}_j$ is a critical point of (\ref{eq:minimizemeImhard}) suggests that 
a possible strategy for agent $j$ to implement is to move towards $\bm{c}_j$ when not actively tracking a target.
%) so that $\bm{x}_j(t+\updelta t)=[\bm{c}_j^\top, 0,0]^\top$.

So far, the discussion in this section suggests that if $[y_1^E(t+\updelta t),y_1^N(t+\updelta t)]$ and  $\{[x_i^E(t+\updelta t),x_i^N(t+\updelta t)]\}_{i\neq j}$ are known to agent $j$ at time $t$ (a generally unreasonable assumption), then agent $j$ should adjust its vector of velocities to attempt to minimize the function:
\begin{align}
& L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))\equiv\notag\\
& \chi\{\upgamma_1(t+\updelta t)< \uptau\}\left[\frac{\left\|[{x}_j^E(t+\updelta t),{x}_j^N(t+\updelta t)]-[{y}_1^E(t+\updelta t),{y}_1^E(t+\updelta t)]\right\|^2}{2}\right]\notag\\
&+\chi\{\upgamma_1(t+\updelta t)\geq \uptau\}\left[\frac{\left\|[{x}_j^E(t+\updelta t),{x}_j^N(t+\updelta t)]-\bm{c}_j(t)^\top\right\|^2}{2}\right],
\label{eq:losssunknown}
\end{align}
where $\upgamma_1(t+\updelta t)$ is the number of agents (not counting agent $j$) that will be close  to target 1 at time $t+\updelta t$ (the definition of ``close'' is flexible), $\uptau$ is a predetermined nonnegative integer, $\bm{c}_j(t)$ is the center of mass of the Voronoi cell, $V_j$, computed based on $\{[{x}_i^E(t+\updelta t),{x}_i^N(t+\updelta t)]\}_{i\neq j}$ and $[{x}_j^E(t),{x}_j^N(t)]$, and
\begin{align}
\label{eq:azucarmoreno}
\left[\begin{array}{c}{x}_j^E(t+\updelta t) \\{x}_j^N(t+\updelta t)\end{array}\right]=\left[\begin{array}{c}{x}_j^E(t) \\{x}_j^N(t)\end{array}\right]+\updelta t \left[\begin{array}{c}\dot{x}_j^E(t) \\\dot{x}_j^N(t)\end{array}\right].
\end{align} 
%where $\updelta t\equiv t+\updelta t-t$. 
The function:
\begin{align}
&L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))\equiv \Bigg[\sum_{i=1}^{\text{\# Targets}} \chi\{i=i^\ast\}\chi\{\upgamma_i(t+\updelta t)< \uptau\}\times\notag\\
&\frac{\left\|[{x}_j^E(t+\updelta t),{x}_j^N(t+\updelta t)]-[{y}_i^E(t+\updelta t),{y}_i^N(t+\updelta t)]\right\|^2}{2}\Bigg]\notag\\
&+\Bigg[ \chi\{\upgamma_i(t+\updelta t)\geq \uptau \text{ for all } i{\text{ or }} \text{\# Targets} = 0\}\times \notag\\
&\frac{\left\|[{x}_j^E(t+\updelta t),{x}_j^N(t+\updelta t)]-\bm{c}_j(t)^\top\right\|^2}{2}\Bigg]
\label{eq:proactivefeet}
\end{align}
provides a natural generalization to (\ref{eq:losssunknown}) for the case where there may be zero or multiple targets; in (\ref{eq:proactivefeet}), $\upgamma_i(t+\updelta t)$ is the number of agents (other than agent $j$) that will be close  to target $i$ at time $t+\updelta t$, and $i^\ast\in S\equiv \{i{\text{ such that }} \upgamma_i(t+\updelta t)< \uptau\}$ is such that out of all $i\in S$, $i^\ast$ is the label/name of the target whose future position (at time $t+\updelta t$) is closest to agent $j$'s current position (at time $t$).\label{page:defineS} If multiple targets in the set $S$ are to be equally close to agent $j$ at time $t+\updelta t$, select one of these targets at random and let the selected target be target $i^\ast$. The indicator functions in (\ref{eq:proactivefeet}) indicate whether agent $j$ believes target $i$ is already sufficiently tracked/covered by other agents. 
%Note that the loss function is depends on the unknown (possible random) position of the target.

 
   
%If two targets, say $i_1$ and $i_2$, are located at the exact same distance from agent $j$ and if $\upgamma_i(t+\updelta t)< \uptau$ for both $i=i_1$ and $i=i_2$, $i^\ast$ will be taken to be the smallest of $i_1$ and $i_2$.\label{eq:ID} 
%The indicator $\mathcal{X}\{i=i^\ast\}$ being equal to 1 tells agent $j$ to move towards target $i$.


 Let us comment on the loss function from (\ref{eq:proactivefeet}). First, note that this loss function is time-varying and possibly random since it depends on the time-varying position of the target and of all other agents. Second, $L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))$ is agent-specific in that each agent is minimizing a different function (this can be seen by noting the presence of $\bm{c}_j(t)$ in the loss function, a term that is agent-dependent).  Another thing to note is that although we have used the number of agents near the target as a measure of how well the target's location is covered, other measurements of target coverage could be used such as the probability that the target will be detected at time $t+\updelta t$. The last observation we make pertains to the fact that the values of $[y_1^E(t+\updelta t),y_1^N(t+\updelta t)]$ and  $\{[x_i^E(t+\updelta t),x_i^N(t+\updelta t)]\}_{i\neq j}$ are unknown to agent $j$ at time $t$, as are the velocities of all other agents and targets. Therefore, the value of the function (\ref{eq:proactivefeet}) is unknown to agent $j$ (recall that the variable $\upgamma_i(t+\updelta t)$ appearing in (\ref{eq:proactivefeet}) depends on the state vectors of the other agents). The following section uses Kalman Filter-based estimates of agent- and target positions to approximate (\ref{eq:proactivefeet}). 
 
 Using estimated values of the other agents' positions introduces an important issue. Suppose that agent $j$ were to predict that $\upgamma_i(t+\updelta t)$ other agents would be located near target $i$ at time $t+\updelta t$ where $\upgamma_i(t+\updelta t)\geq \uptau$. Then,the decision of agent $j$ will be to move towards the center of mass of its Voronoi cell which could result in the agent moving away from the target. Note, however, that if the other $n-1$ agents were to also predict that at least $\uptau$ agents would be located near the target at time $t+\updelta t$, then all $n$ agents would move towards the centers of their Voronoi cells and away from the target, which  could result in a problematic situation where the target is left ``unguarded''. To avoid this problem, we consider a setting in which agents update their velocity vectors in a strictly cyclic manner.
% , that is agents take turns deciding whether to track- or move away from a target. 
 As a result, when the time comes for agent $j$ to update its velocity, the other agents will have already begun moving towards- or away from the target, giving agent $j$ information about their intentions.
 %
%  if at time $t$ agent $j$ makes a decision regarding its next action, the remaining agents will have already begun to move towards- or away from the target, thus reducing the probability of all agents simultaneously moving away from the target. 
 %
% To accommodate the cyclic nature of the implementation, the loss function in (\ref{eq:proactivefeet}) can be rewritten as:
% \begin{align}
%&L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))\equiv\notag\\
%& \sum_{i=1}^{\text{\# Targets}} \mathcal{X}\{\upgamma_i(t+\updelta t)< \uptau\}\mathcal{X}\{i=i^\ast\} \left[\frac{\left\|[{x}_j^E(t_{k+n}),{x}_j^N(t_{k+n})]-[{y}_i^E(t_{k+n}),{y}_i^N(t_{k+n})]\right\|^2}{2}\right]\notag\\
%&+ \mathcal{X}\{\upgamma_i(t+\updelta t)\geq \uptau \text{ for all } i{\text{ or }} \text{\# Targets} = 0\} \left[\frac{\left\|[{x}_j^E(t_{k+n}),{x}_j^N(t_{k+n})]-\bm{c}_j(t)^\top\right\|^2}{2}\right],
%\label{eq:proactivefeet2}
%\end{align}
 % 
 

%agents take turns trying to optimize their corresponding loss function given in (\ref{eq:losssunknown}). Therefore, an agent will not change its state vector (i.e., its position and velocity)


\section{Proposed Cyclic SA-Based Approach}
\label{sec:proposedapproach}
This section describes the precise way in which an agent estimates the future positions of detected agents and targets and how the agent uses this information to adjust its state vector based on the loss function in (\ref{eq:proactivefeet}). Specifically, this section answers the following questions:
\begin{enumerate}
\item How does agent $j$ estimate $\{\bm{x}_i(t+\updelta t)\}_{i\neq j}$ and $\bm{y}_i(t+\updelta t)$ (i.e., the future state vectors of other agents and the state vectors of targets)?
\item How does agent $j$ use the estimates of $\{\bm{x}_i(t+\updelta t)\}_{i\neq j}$ and $\bm{y}_i(t+\updelta t)$ to update its own state vector (position and velocity)?
\end{enumerate}
 Section \ref{sec:estimatingstate} addresses the first question and Section \ref{sec:algooutline} addresses the second question.


\subsection{Extended Kalman Filter for Estimating State Vectors}
\label{sec:estimatingstate}

At time $t$, agent $j$ uses the extended Kalman filter (EKF) to obtain an estimate for $\bm{y}_i(t+\updelta t)$, the true state vector of target $i$ at time $t+\updelta t$. The EKF is used due to the fact that (\ref{eq:elevatormusic}) is nonlinear in the state vector. To use the EKF, agent $j$ first models the dynamics of target $i$ as follows:
\begin{align}
\label{eq:qbert}
\bm{y}_i(t+\updelta t)=\bm\Phi\bm{y}_i(t)+\bm{w}(t)
\end{align}
for $t$ in a discrete set of points $\updelta t$ time units apart, where 
\begin{align}
\label{eq:qbert2mass}
\setstretch{1.25} 
\bm{\Phi}\equiv \left[\begin{array}{cccc}1 & 0 & \updelta t & 0 \\0 & 1 & 0 & \updelta t \\0 & 0 & 1 & 0 \\0 & 0 & 0 & 1\end{array}\right]
\end{align}
and where $\bm{w}$ is a vector of zero-mean Gaussian white noise with covariance matrix $\bm{Q}$. 
%
 The EKF algorithm used by agent $j$ for estimating the target's state vector is illustrated in Algorithm \ref{alg:EKF}. Loosely speaking, at time $t-\updelta t$ agent $j$ predicts the position of target $i$ at time $t$ (Line \ref{line:predictline} of Algorithm \ref{alg:EKF}). The predicted state estimate is denoted by $\hat{\bm{y}}_i(t|t-\updelta t)$. Then, at time $t$, agent $j$ uses the latest noisy information on the position of target $i$ to correct its previous estimate (Line \ref{line:correctline} of Algorithm \ref{alg:EKF}) . The corrected state estimate is denoted by $\hat{\bm{y}}_i(t|t)$ (although $\bm{H}$, $\bm{K}$, and $\bm{\upeta}$ are functions of time, this dependance has been omitted for simplicity).  We assume that agent $j$ also estimates the state vector of another detected agent, say agent $i$, using Algorithm \ref{alg:EKF} after a natural modification to replace $\hat{\bm{y}}_i(t|t)$ and $\hat{\bm{y}}_i(t|t-\updelta t)$ with $\hat{\bm{x}}_i(t|t)$ and $\hat{\bm{x}}_i(t|t-\updelta t)$, respectively.
% , the corrected- and predicted state vectors corresponding to agent $i$. 
 
   \begin{algorithm}[!t]                     
\caption{The Extended Kalman Filter (EKF) for Estimating $\bm{y}_i(t)$}      
\label{alg:EKF}                
\begin{algorithmic} [1]                  % enter the algorithmic environment
\setstretch{1.5} 
\REQUIRE    $\hat{\bm{y}}_i(t-\updelta t|t-\updelta t)\in \mathbb{R}^4$ and $\bm{P}_{t-\updelta t|t-\updelta t}\in \mathbb{R}^{4\times 4}$.
\STATEx{\bf{Predict}} (execute at time $t-\updelta t$):
\STATE{$\hat{\bm{y}}_i(t|t-\updelta t)= \bm\Phi\hat{\bm{y}}_i(t-\updelta t|t-\updelta t)$, where $\bm\Phi$ is defined in (\ref{eq:qbert2mass}).}\label{line:predictline}
\STATE{$\bm{P}_{t|t-\updelta t}=\bm\Phi \bm{P}_{t-\updelta t|t-\updelta t}\bm\Phi^\top+\bm{Q}$, where $\bm{Q}$ is defined below (\ref{eq:qbert2mass}).}
\STATEx{\bf{Correct}} (execute at time $t$):
\STATE{$\bm\upeta = \bm{z}_{j:i}(t)-[{\upvarphi}(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t)), {\uprho}(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t))]^\top$, where ${\upvarphi}(\cdot,\cdot)$ and ${\uprho}(\cdot,\cdot)$ are defined in (\ref{eq:badabada1}) and (\ref{eq:badabada2}).}
\STATE{$\bm{S}=\bm{H}\bm{P}_{t|t-\updelta t}\bm{H}^\top+\bm{R}$, where $\bm{R}$ is defined below (\ref{eq:elevatormusic}) and:\label{eq:linedefineH}
\begin{align*}
\setstretch{3} 
\bm{H}\equiv \left[\begin{array}{cccc}\displaystyle{\frac{x^N-y^N}{\uprho^2(\bm{x},\bm{y})}}  & \displaystyle{\frac{-(x^E-y^E)}{\uprho^2(\bm{x},\bm{y})}}  & 0 & 0 \\ \displaystyle{\frac{-(x^E-y^E)}{\uprho(\bm{x},\bm{y})}}  & \displaystyle{\frac{-(x^N-y^N)}{\uprho(\bm{x},\bm{y})}}  & 0 & 0\end{array}\right] {\text{ with $\bm{x}=\bm{x}_j(t)$ and $\bm{y}=\hat{\bm{y}}_i(t|t-\updelta t)$.}}
\end{align*}
}
\STATE{$\bm{K}=\bm{P}_{t|t-\updelta t}\bm{H}^\top\bm{S}^{-1}$.}
\STATE{$\hat{\bm{y}}_i(t|t)=\hat{\bm{y}}_i(t|t-\updelta t)+\bm{K}\bm\upeta$.}\label{line:correctline}
\STATE{$\bm{P}_{t|t}=(\bm{I}-\bm{K}\bm{H})\bm{P}_{t|t-\updelta t}$.}
\end{algorithmic}
\end{algorithm}

 
  One important thing to note is that the EKF algorithm defines $\bm{H}$ (appearing in Line \ref{eq:linedefineH} of Algorithm \ref{alg:EKF}) as the Jacobian matrix of the vector:
  \begin{align}
\left[\begin{array}{c}\upvarphi(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t)) \\\uprho(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t))\end{array}\right]
%=  [\upvarphi(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t)),  \uprho(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t))]^\top
\label{eq:imighthaveto}
  \end{align}
   with respect to $\bm{x}_j(t)$. However, the vector in (\ref{eq:imighthaveto}) is not differentiable if and only if at least one of the following holds:
   \begin{enumerate}
\item $x_j^E(t)=\hat{y}_j^E(t|t-\updelta t)$ and $x_j^N(t)>\hat{y}_j^N(t|t-\updelta t)$, where the vector $[\hat{y}_j^E(t|t-\updelta t),\hat{y}_j^N(t|t-\updelta t)]^\top$ corresponds to the first two entries of the vector $\hat{\bm{y}}_i(t|t-\updelta t)$.
% and is the estimated position of the target.
% \begin{align}
% {\text{$x_j^E(t)=\hat{y}_j^E(t|t-\updelta t)$ and $x_j^N(t)>\hat{y}_j^N(t|t-\updelta t)$}},
% \label{eq:uberlights}
% \end{align}
 \item $\uprho(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t))=0$.
 \end{enumerate}
 In other words, a successful implementation of the EKF algorithm requires avoiding scenarios 1 and 2 above, possibly by perturbing $\hat{\bm{y}}_i(t|t-\updelta t)$.
% 




\subsection{Algorithm Description}
\label{sec:algooutline}

We consider a setting in which the $n$  agents update their directional velocities in a strictly cyclic manner. 
%The proposed algorithm is summarized as follows. 
At time $t_0$, agent 1 uses its sensor to detect any nearby agents and targets. Agent 1 then estimates the future state vectors (at time $t_0+\updelta t$) of all detected agents and targets using the EKF algorithm (Algorithm \ref{alg:EKF} ). Next, using the  estimated future states of detected agents and targets, agent 1 updates its velocity vector (more details about this step will be given in the sequel). In the same manner, agent 2 updates its velocity vector at time $t_0+\updelta t/n$. In general, agent $j$ updates its directional velocity at the times $\{t_0+(j-1)\updelta t/n+k \updelta t \}_{k\geq0}$ using the predicted positions of agents and targets $\updelta t$ time units into the future. 
%Note that agents do not need to communicate since each agent has a predetermined set of times where it can update its velocity vector. 
Before implementing the algorithm, it is necessary to specify exactly how agent $j$ updates its state vector. This is done next.

The objective of Agent $j$ is to minimize the loss function in (\ref{eq:proactivefeet}). As discussed in Section \ref{sec:idealloss}, however, agent $j$ does not have access to a closed form expression for the loss function because the function depends on the unknown future state vectors of targets and of other agents. In our proposed approach, agent $j$ uses the predicted agent- and target state vectors to estimate the gradient of the loss function (the differentiability of the loss function is addressed in Section \ref{sec:connectiontocyclicSA}). Agent $j$ then updates its state vector using the noisy gradient estimate in a steepest-descent manner. Specifically, agent $j$ updates its state vector at times $t\in \{t_0 + (j-1)\updelta t/n+k\updelta t\}_{k\geq0}$ by following the steps below.
\begin{DESCRIPTION}
\item[Step 1:] Use sensor to detect nearby agents and targets.
\item[Step 2:] Estimate the future (at time $t+\updelta t$) state vectors of all detected agents and targets using the EKF (Algorithm \ref{alg:EKF}).
\item[Step 3:] Let $\uplambda\geq 0$ be a number such that an agent is considered to be close to the target if the distance between the agent and the target is less than $\uplambda$ (n general $\uplambda\neq r$). For each detected target, estimate $\upgamma_i(t+\updelta t)$ (defined below (\ref{eq:proactivefeet})), based on $\uplambda$ and
%the number of agents (other than agent $j$) that will be near target $i$ at time $t+\updelta t$. 
denote the estimate by $\hat{\upgamma}_i(t+\updelta t)$.
\item[Step 4:] Find the set of targets for which $\hat{\upgamma}_i(t+\updelta t)<\uptau$ (with $\uptau>0$). 
%is strictly less than some predetermined threshold, $\uptau>0$. 
Denote this set by $\hat{S}$ ($\hat{S}$ is therefore an estimate of the set $S$ defined on p. \pageref{page:defineS}).
\item[Step 5:] If $\hat{S}=\emptyset$ (here $\emptyset$ denotes the empty set), use the estimated future positions (at time $t+\updelta t$) of the other agents along with the  current position (at time $t$) of agent $j$ to estimate $\bm{c}_j(t)$. Denote the estimate by $\hat{\bm{c}}_j(t)$. If $S\neq \emptyset$, pick the target in $\hat{S}$ whose predicted position is closest to agent $j$ (in the event of a tie, choose a target at random). Denote that target ``target $\hat{i}^\ast$''  ($\hat{i}^\ast$ is an estimate for the integer $i^\ast$ defined on p. \pageref{page:defineS}).
%In the event of a tie when attempting to obtain $i^\ast$, let $i^\ast$ be the target with smallest ID (see the example on p. \pageref{eq:ID}).
\item[Step 6:] Select $a>0$ and update agent $j$'s velocity vector as follows:
\begin{align}
%&{\text{\bf{Update Velocity:}}}\notag\\
&[\dot{x}_j^E(t), \dot{x}_j^N(t)]^\top=(1-a)[\dot{x}_j^E(t-\updelta t),\dot{x}_j^N(t-\updelta t)]^\top\notag\\
 &+a\Bigg[ \chi\{\hat{\upgamma}_i(t+\updelta t)\geq \uptau \text{ for all } i {\text{ or \# Detected Targets}}=0\} \times\notag\\
&\frac{\hat{\bm{c}}_j(t)-[x_j^E(t),x_j^N(t)]^\top}{\updelta t}\Bigg]+ \sum_{i=1}^{\text{\# Detected Targets}} a \Bigg[\chi\{\hat{\upgamma}_i(t+\updelta t)< \uptau\}\chi\{i=\hat{i}^\ast\}\times \notag\\
& \frac{[\hat{y}_i^E(t+\updelta t|t),\hat{y}_i^N(t+\updelta t|t)]^\top-[x_j^E(t),x_j^N(t)]^\top}{\updelta t} \Bigg].
\label{eq:step6}
\end{align}
\item[Step 7:] Update agent $j$'s position using (\ref{eq:azucarmoreno}) and (\ref{eq:step6}).
\end{DESCRIPTION}
%The following section discusses the motivation behind (\ref{eq:step6}) in more detail. 
%
%Loosely speaking, Step 6 requires agent $j$ to adjust its velocity vector in the direction of an estimate of the negative gradient of (\ref{eq:proactivefeet}) after conditioning on the values of $\hat{\upgamma}_i(t+\updelta t)$, $\hat{i}^\ast$, $\hat{\bm{c}}_j(t)$, $\hat{\bm{y}}_i(t+\updelta t|t)$, and $[x_j^E(t),x_j^N(t)]$. 

\subsection{Connection to Cyclic SA}
\label{sec:connectiontocyclicSA}

First, note that the loss function in (\ref{eq:proactivefeet}) is differentiable
%% with respect to $[\dot{x}_j^E(t),\dot{x}_j^N(t)]$. 
% To see this, note that the vector $\bm{c}_j(t)$ as well as the indicator functions in (\ref{eq:proactivefeet}) are independent of  $[\dot{x}_j^E(t),\dot{x}_j^N(t)]$. Therefore,
%% these variables may be treated as constants when differentiating with respect to $[\dot{x}_j^E(t),\dot{x}_j^N(t)]$.
%% Once the values of the indicator functions have been computed, the resulting function is differentiable with respect to $[\dot{x}_j^E(t),\dot{x}_j^N(t)]$.
%% (recall that $\bm{c}_j(t)$ does not depend on $[\dot{x}_j^E(t),\dot{x}_j^N(t)]$ and can therefore be treated as a constant). 
% the gradient of $L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))$ is 
% 
 with gradient:
\begin{align}
\frac{\partial L_j(\dot{x}_j^E,\dot{x}_j^N)}{\partial [\dot{x}_j^E,\dot{x}_j^N])^\top}=&\ \Bigg[\chi\{\upgamma_i(t+\updelta t)\geq \uptau \text{ for all } i {\text{ or \# Targets}}=0\}\updelta t\times\notag\\
& \left([x_j^E,x_j^N]^\top+\updelta t[\dot{x}_j^E,\dot{x}_j^N]^\top-\bm{c}_j(t)^\top\right) \Bigg]\notag\\
&+ \sum_{i=1}^{\text{\# Targets}} \Bigg[\chi\{\upgamma_i(t+\updelta t)< \uptau\}\chi\{i=i^\ast\}\updelta t\times \notag\\
& \left([x_j^E,x_j^N]^\top+\updelta t[\dot{x}_j^E,\dot{x}_j^N]^\top-[{y}_i^E(t+\updelta t),{y}_i^N(t+\updelta t)]^\top\right) \Bigg],
\label{eq:truegradientIam}
\end{align}
(assuming the future positions of the target do not depend on the positions of the agents, a simplifying consequence of (\ref{eq:qbert})). %where the dependance of $\bm{x}_j$ on $t$ has been omitted for simplicity. 
%
The update in (\ref{eq:step6}) is based on the idea that the gradient in (\ref{eq:truegradientIam}) can be estimated using the values of $\hat{\bm{x}}_i(t+\updelta t|t)$, and $\hat{\bm{y}}_i(t+\updelta t|t)$. Specifically, define the stochastic gradient:
\begin{align}
&\hat{\bm{g}}_j(\dot{x}_j^E(t-\updelta t),\dot{x}_j^N(t-\updelta t))\equiv\notag\\
 &\Bigg[ \chi\{\hat{\upgamma}_i(t+\updelta t)\geq \uptau \text{ for all } i {\text{ or \# Detected Targets}}=0\}\updelta t \times\notag\\
&\left([x_j^E(t),x_j^N(t)]+\updelta t[\dot{x}_j^E(t-\updelta t),\dot{x}_j^N(t-\updelta t)]-\hat{\bm{c}}_j(t)^\top\right)\Bigg]^\top\notag\\
&+ \sum_{i=1}^{\text{\# Detected Targets}} \Bigg[\chi\{\hat{\upgamma}_i(t+\updelta t)< \uptau\}\chi\{i=\hat{i}^\ast\}\updelta t\times \notag\\
& \left([x_j^E(t),x_j^N(t)]+\updelta t[\dot{x}_j^E(t-\updelta t),\dot{x}_j^N(t-\updelta t)]-[\hat{y}_i^E(t+\updelta t|t),\hat{y}_i^N(t+\updelta t|t)]\right) \Bigg]^\top.
\label{eq:kettoout}
\end{align}
%However, one would be remiss to discuss gradient-based updates without discussing the differentiability of the corresponding loss function. As it turns out, the loss function in (\ref{eq:proactivefeet}) {\it{is}} differentiable. 
%%note that the term $\bm{c}_{j}(t)$ can be treated as constant since it does not depend on $[\dot{x}_j^E(t),\dot{x}_j^N(t)]$.
%%, the variable with respect to which the loss function is to be minimized. 
The vector in (\ref{eq:kettoout}) can be seen as a stochastic estimate of the gradient in (\ref{eq:truegradientIam}). Moreover, the update in (\ref{eq:step6}) can be rewritten as:
\begin{align*}
[\dot{x}_j^E(t), \dot{x}_j^N(t)]^\top=[\dot{x}_j^E(t-\updelta t), \dot{x}_j^N(t-\updelta t)]^\top-a(\updelta t)^{-2}\hat{\bm{g}}_j(\dot{x}_j^E(t-\updelta t),\dot{x}_j^N(t-\updelta t)).
\end{align*}
%
Thus, the update in (\ref{eq:step6}) has the general form of the SA update in (\ref{eq:youknownothing}) with $a_k= a(\updelta t)^{-2}$. A constant gain sequence was used due to the time-varying nature of the loss function. One important thing to note is that the noisy gradient estimate in (\ref{eq:kettoout}) is not an unbiased estimate of  the true gradient in (\ref{eq:truegradientIam}). The bias is due to the fact that the EKF does not generally produce unbiased predictions of the future positions of any detected agents and targets. The magnitude of the bias will increase or decrease as the bias in the EKF estimates increases or decreases, respectively.

Because agents take turns performing the update in (\ref{eq:step6}), the resulting algorithm resembles a distributed implementation of Algorithm \ref{kirkey}, a cyclic algorithm which is a special case of the GCSA algorithm (Algorithm \ref{findme}). However, the multi-agent algorithm from this chapter does not fit perfectly into the framework of Algorithm \ref{findme} due to the fact that each agent is optimizing a different loss function and each of these loss functions is time-varying. As a result, the theory from Chapters \ref{sec:cyclicseesaw}--\ref{chap:imefficient} is not directly applicable. The following section investigates the {\it{numerical}} performance of the 
%multi-agent optimization 
algorithm 
%that was introduced 
in Section \ref{sec:algooutline}.



\section{Numerical Analysis}
\label{sec:numericsamultiagent}


This section investigates the numerical performance of the algorithm from Section \ref{sec:algooutline}. 
%While some of the parameters in the algorithm (e.g., the range of the sensors) change throughout the numerical experiments, a few settings are uniform throughout this section. Specifically, 
The numerical results assume that the AOI is always a $\text{6} \times \text{6}$ square centered at the origin and that the value of $a$ in (\ref{eq:step6}) is such that $0<a<1$. The reason for forcing $a$ to be strictly less than 1 stems from the fact that setting $a=1$ implies that the distance measure $\uprho(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t))=0$, which implies that the matrix $\bm{H}$ (see Line \ref{eq:linedefineH} of Algorithm \ref{alg:EKF}) as well as the angle to the target's predicted position are not well-defined. Having $a<1$ guarantees that $\uprho(\bm{x}_j(t),\hat{\bm{y}}_i(t|t-\updelta t))\neq0$, avoiding the aforementioned complications. 
%Note that using a value of $a$ that is strictly less than 1 is equivalent to the agent moving to a location that ``undershoots'' the target's predicted position. 
%Specifically, Steps 6 and 7 of Section \ref{sec:algooutline} imply that the agent moves to a location that is $(a\times 100)\%$ of the way between the agent's current position and the target's predicted position.
%Another case where $\bm{H}$ is well-defined is when $a>1$, a setting which is equivalent to the agent moving to a location that ``overshoots'' the target's predicted position. Technically, there is no theoretical reason for choosing $a<1$ versus $a>1$.

\subsection{Software}

The numerical results in this Section are all performed in MATLAB. The MATLAB Multi-Parametric Toolbox 3.0 (Herceg et all. 2013) \nocite{MPT3} was used to compute the vertices defining the Voronoi cells, based on the current positions of the $n$ agents, while simultaneously constraining the cells to be contained within the AOI. Then, the centers of mass of the resulting Voronoi cells (i.e., the $\hat{\bm{c}}_j(t)$s) were computed using the function {\verb|polygeom|} by Sommer (2016)\nocite{polygeom}. 

%o compute $\hat{\bm{c}}_j(t)$ in Step 5 of the Algorithm,

\subsection{Effect of the Sensor Range}
\label{subsec:effsensorrange}

\begin{figure}
\centering
\begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}


\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/multiagent/gotovoronoiFOURagents-eps-converted-to.pdf}};

\end{tikzpicture}
 \caption{$r=4$, $r'=3.8$.}
 \label{fig:sensorrange1}
\end{subfigure}\hfill
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}

\node[inner sep=0pt] (probe) at (0,0)
{\includegraphics[scale=0.35]{Plots/multiagent/gotocenterFOURagents-eps-converted-to.pdf}};
\end{tikzpicture}
\caption{$r=0.5$, $r'=0.4$.}
\label{fig:sensorrange2}
\end{subfigure}\hfill
\caption[The effect of the sensor range on area coverage]{The effect of the sensor range on area coverage for the case where there are 4 agents and 0 targets. Each empty square denotes the starting position of an agent. Similarly, each filled square denotes the final position of an agent. Note that in Figure \ref{fig:sensorrange2} agents fail to spread out.}
\label{fig:effectofrange}
\end{figure}


Because the algorithm in Section \ref{sec:algooutline} involves zero communication between agents, the quality of the agents' sensors directly affects the performance of the algorithm. Figure \ref{fig:effectofrange} presents two cases illustrating the effect of sensor range on area coverage for a setting where there are four agents and zero targets (both Figures \ref{fig:sensorrange1} and \ref{fig:sensorrange2} are the result of the agents updated their velocity 50 times). The first case, presented in Figure \ref{fig:sensorrange1}, shows the evolution of four agents' positions when the radii $r=2$ and $r'=1.5$ (see (\ref{eq:sensorequationmodel}) for the definitions of $r$ and $r'$). Here, the four agents are frequently able to detect each other and can therefore spread out to maximize area coverage (i.e., minimize (\ref{eq:minimizemeImhard})). In contrast, Figure \ref{fig:sensorrange2} shows the evolution of four agents' positions when $r=0.5$ and $r'=0.4$. Here, the agents start relatively far apart and fail to detect each other due to the limited range of the sensors. Consequently, the agents tend to gravitate towards the center of the AOI, an action that is not optimal when attempting to maximizing area coverage. In summary, Figure \ref{fig:effectofrange} illustrates the fact that a larger sensor range provides agents with more of the information they need to distribute their positions optimally relative to the objective function in (\ref{eq:minimizemeImhard}). Figure \ref{fig:effectofrange} was produced using $\bm{R}=0.05\bm{I}$, $\updelta t=0.4$, and $a=0.5$.

\begin{figure}
\centering
\begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}


\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/multiagent/gettargetlargesensor-eps-converted-to.pdf}};

\end{tikzpicture}
 \caption{$r=2$, $r'=1.5$.}
 \label{fig:rangetrack1}
\end{subfigure}\hfill
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}

\node[inner sep=0pt] (probe) at (0,0)
{\includegraphics[scale=0.35]{Plots/multiagent/ignoretargetsmallsensor-eps-converted-to.pdf}};
\end{tikzpicture}
\caption{$r=0.5$, $r'=0.4$.}
\label{fig:rangetrack2}
\end{subfigure}\hfill
\caption[The effect of the sensor range on target tracking]{The effect of sensor range on target tracking for the case where there is 1 agent and 1 target. An empty square (respectively empty triangle) denotes the starting position of the agent (respectively target). The filled square (respectively filled triangle) denotes the final position of the agent (respectively target). Note that in Figure \ref{fig:rangetrack2} the agent fails to track the target.}
\label{fig:rangetrack}
\end{figure}


Aside from improving area coverage, a larger sensor range has the (not surprising) benefit of also improving target tracking. In Figure \ref{fig:rangetrack1}, for example, a single agent whose sensor has a large range is able to track a single target fairly well. When the sensor's range is significantly decreased, however, Figure \ref{fig:rangetrack2} shows that the agent is no longer able to continuously detect and keep track of the target. The simulations in Figure \ref{fig:rangetrack} were produced using $\bm{R}=0.05\bm{I}$, $\updelta t =0.1$, and $a=0.5$; and the target was assumed to move according to the linear model in (\ref{eq:qbert}) with $\bm{Q}=0.01\bm{I}$ and velocity equal to 1 (i.e., the last two entries of $\bm{y}_i(t)$ are equal to 1). Note that Figure \ref{fig:effectofrange}  uses $\updelta t=0.4$ while Figure \ref{fig:rangetrack} uses $\updelta t=0.1$. This was done with the objective of simulating a setting which the agents begin updating their parameter vectors at times that are 0.1 time units apart, which implies $\updelta t=0.n$ when there are $n$ agents.



\begin{figure}
\centering
\begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}


\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/multiagent/largegain-eps-converted-to.pdf}};

\end{tikzpicture}
 \caption{$a=1.3$.}
 \label{fig:gaintoolarge}
\end{subfigure}\hfill
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}

\node[inner sep=0pt] (probe) at (0,0)
{\includegraphics[scale=0.35]{Plots/multiagent/smallgain-eps-converted-to.pdf}};
\end{tikzpicture}
\caption{$a=0.01$.}
\label{fig:gaintoosmall}
\end{subfigure}\hfill
\caption[The effect of the gain sequence on target tracking]{The effect of the gain sequence on target tracking for the case where there is 1 agent and 1 target. An empty square (respectively empty triangle) denotes the starting position of the agent (respectively target). The filled square (respectively filled triangle) denotes the final position of the agent (respectively target). }
\label{fig:magnitudepfthegain}
\end{figure}

\subsection{Effect of the Gain Sequence}
\label{subsec:effofgan}

Like the sensor range, the value of $a$ (the gain appearing in Step 6 of the multi-agent algorithm) plays a crucial role in the performance of the algorithm. Figure \ref{fig:gaintoolarge}, for example, shows an agent attempting to track a target when the gain sequence is too large. Here, the agent's velocity vector is highly sensitive to small changes in the target's predicted position, this eventually results in the agent moving too far from the target to the point where the agent is no longer able to detect it. Similarly, Figure \ref{fig:gaintoosmall} shows how using a gain sequence that is too small also results in the agent not being able to remain close enough the target. Consequently, the agent eventually loses track of the target. The simulations in Figure \ref{fig:magnitudepfthegain} were produced using $\bm{R}=0.05\bm{I}$,  $\updelta t =0.1$, $a=0.5$, $r=2$, and $r'=1.5$; and the target was assumed to move according to the linear model in (\ref{eq:qbert}) with $\bm{Q}=0.01\bm{I}$ and velocity equal to 1 (i.e., the last two entries of $\bm{y}_i(t)$ are equal to 1). The agent and target updated their velocities 50 times.

Unfortunately, there is no general way to determine the best value of $a$ in practice. One observation regarding the update in (\ref{eq:step6}) that can be helpful in selecting the value of $a$ is the following: setting $a=1$ implies that $[{x}_j^{E}(t+\updelta t),{x}_j^{N}(t+\updelta t)]^\top$, the position of agent $j$ at time $t+\updelta t$, will be exactly equal to one of $[\hat{y}_i^E(t+\updelta t|t),\hat{y}_i^N(t+\updelta t|t)]^\top$ and $\hat{\bm{c}}_j(t)$, depending on whether the agent decides to move towards the target or towards the center of mass of its Voronoi cell. Therefore, when an agent is actively tracking a target, setting $a=1$ implies that $\uprho(\bm{x}_j(t+\updelta t),\hat{\bm{y}}_i(t+\updelta t|t))=0$. This observation implies that setting $a=1$ is not an ideal strategy for two reasons: 
\begin{enumerate}
\item The EKF algorithm is not well-defined when $\uprho(\bm{x}_j(t+\updelta t),\hat{\bm{y}}_i(t+\updelta t|t))=0$ (see the discussion following (\ref{eq:imighthaveto})).
\item In reality, two bodies cannot occupy the same space so that having $\uprho(\bm{x}_j(t+\updelta t),\hat{\bm{y}}_i(t+\updelta t|t))=0$ is not physically possible when $\hat{\bm{y}}_i(t+\updelta t|t)$ is close to the target's true position at time $t+\updelta t$.
\end{enumerate}
In light of the discussion above, a general guideline for choosing $a$ is to pick a value that is only slightly less than 1 if the target's predicted state is expected to be somewhat accurate. For our numerical experiments we select values of $a$ that are strictly less than one in an attempt to ensure that the algorithm is not too sensitive to changes in the EKF's predictions.


\subsection{Maximum Spread and Minimum Distance to Target}
\label{sec:spreadanddistance}

Sections \ref{subsec:effsensorrange} and \ref{subsec:effofgan} explained the significance of $r$, $r'$, and $a$ when a single agent is attempting to track a target. It was observed that if the sensor range is too small or if the value of $a$ is either too small or too large, the terminal distance between the agent and the target tends to be large. When there are multiple agents in the AOI, two other variables that govern the algorithm's performance are $\uplambda$,  the distance at which a target is assumed to be close to an agent (see Step 3 of the algorithm), and $\uptau$,  the number of agents that need to be near a target for that target to be considered to be well-guarded (see Step 4 of the algorithm). A large value of $\uptau$ combined with a small value of $\uplambda$ implies that an agent will only move away from a detected target if it predicts that several agents will be extremely close to the target. In contrast, a small value of $\uptau$ combined with a large value of $\uplambda$ implies that agents very easily move away from a detected target. Thus, a poor choice of $\uptau$ and $\uplambda$ could result in either all agents moving away from the target or all agents gathering near the target; neither of these scenarios is ideal given objectives 1 and 2 on p. \pageref{eq:sandywpusstod}. With this in mind,
%Tables \ref{eq:jonnsm1}, \ref{eq:jonnsm2}, \ref{eq:jonnsm3}, and \ref{eq:jonnsm4} investigate the effects of $r$, $r'$, $\uptau$, and $\uplambda$, on the distance between a target and the nearest agent as well as on the maximum distance between agents. 
%Specifically, 
Tables \ref{eq:jonnsm1}--\ref{eq:jonnsm4} compute: 1) the mean terminal distance between the target and the nearest agent divided by the initial value of this distance (see the column  ``Dist. to Nearest Agent''), and 2) the mean terminal maximum distance between agents divided by the initial value of this distance (see the column ``Max. Dist. Between Agents''), for different combinations of $r$, $r'$, $\uptau$, and $\uplambda$ when there are 4 agents. Small values in the first column indicate agents are tracking the target while large values of the second column indicate agents are spreading out. The means in Tables \ref{eq:jonnsm1}--\ref{eq:jonnsm4} are computed from 20 i.i.d. replications, each consisting of 50 velocity updates per-agent. Each replication was produced by initializing the positions of agents and targets uniformly at random within the AOI; using $\bm{R}=0.05\bm{I}$, $\updelta t =0.1$, and $a=0.5$; and the target was assumed to move according to the linear model in (\ref{eq:qbert}) with $\bm{Q}=0.01\bm{I}$, velocity equal to 1 (i.e., the last two entries of $\bm{y}_i(t)$ are equal to 1). 


\begin{table}[p]
\centering
\begin{tabular}{c c c c c c} \toprule
   {$\uptau$} & {$\uplambda$}  & {Dist. to Nearest Agent} & {Max. Dist. Between Agents}  \\ \midrule
     $1$  & $0.1$ & $0.1569\ (\hat{\upsigma}^2=0.0124)$  & $0.9537\ (\hat{\upsigma}^2=0.1967)$      \\
     $1$ & $0.5$ &  $0.3348\ (\hat{\upsigma}^2=0.1029)$ & $1.1006\ (\hat{\upsigma}^2=0.3250)$   \\
     $1$  & $2$ & $0.3048\ (\hat{\upsigma}^2=0.0546)$  & $1.4699\ (\hat{\upsigma}^2=0.1375)$     \\
   $1$  & $3$ & $0.4875\ (\hat{\upsigma}^2=0.1947)$  & $1.4973\ (\hat{\upsigma}^2=0.5830)$       \\ \midrule
   $2$  & $0.1$ & $ 0.2964\ (\hat{\upsigma}^2=0.0592)$  & $0.7556\ (\hat{\upsigma}^2=0.1740)$      \\
    $2$ & $0.5$ & $0.1976 \ (\hat{\upsigma}^2=0.0265)$ & $1.1087\ (\hat{\upsigma}^2=0.4836)$    \\
    $2$  & $2$ & $0.3080\ (\hat{\upsigma}^2=0.0471)$  & $ 1.2940\ (\hat{\upsigma}^2=0.3126)$     \\
    $2$  & $3$ & $0.2400\ (\hat{\upsigma}^2=0.0308)$  & $1.5787\ (\hat{\upsigma}^2=0.6409)$      \\ \midrule
    $3$  & $0.1$ & $0.1949\ (\hat{\upsigma}^2=0.0191)$  & $0.7750\ (\hat{\upsigma}^2=0.2952)$    \\
    $3$  & $0.5$ & $0.2330\ (\hat{\upsigma}^2=0.0648)$  & $1.1551\ (\hat{\upsigma}^2=1.0617)$     \\
    $3$  & $2$ & $0.2703\ (\hat{\upsigma}^2=0.0347)$  & $1.1701\ (\hat{\upsigma}^2=0.3006)$   \\
    $3$  & $3$ & $0.3261\ (\hat{\upsigma}^2=0.1056)$  & $1.0590\ (\hat{\upsigma}^2=0.1192)$          \\ \bottomrule
\end{tabular}
\caption[Normalized mean terminal distance from the target to the nearest agent and normalized mean terminal maximum distance between agents when there are four agents, one target, $r=3$, and $r'=2.5$]{Mean terminal distance from the target to the nearest agent and mean terminal maximum distance between agents when there are four agents, one target, $r=3$, and $r'=2.5$ (distances are divided by their values at the beginning of the replication prior to averaging). $\hat{\upsigma}^2$ is the sample variance. The variables $\uptau$ and $\uplambda$ have a significant effect over the behavior of the agents.}
\label{eq:jonnsm1}
\end{table}

\begin{table}[p]
\centering
\begin{tabular}{c c c c c c} \toprule
   {$\uptau$} & {$\uplambda$}  & {Dist. to Nearest Agent} & {Max. Dist. Between Agents}  \\ \midrule
     $1$  & $0.1$ & $0.3557\ (\hat{\upsigma}^2=0.0860)$  & $0.9675\ (\hat{\upsigma}^2=0.2911)$      \\
     $1$ & $0.5$ &  $0.3261\ (\hat{\upsigma}^2= 0.0597)$ & $1.2445\ (\hat{\upsigma}^2=0.2934)$   \\
     $1$  & $2$ & $0.6423\ (\hat{\upsigma}^2=0.3227)$  & $1.0706\ (\hat{\upsigma}^2=0.1149)$     \\
   $1$  & $3$ & $0.7195\ (\hat{\upsigma}^2=0.3410)$  & $0.9462\ (\hat{\upsigma}^2=0.0800)$       \\ \midrule
   $2$  & $0.1$ & $ 0.3513\ (\hat{\upsigma}^2=0.1028)$  & $1.1958\ (\hat{\upsigma}^2=0.3893)$      \\
    $2$ & $0.5$ & $0.2993 \ (\hat{\upsigma}^2=0.0726)$ & $1.2100\ (\hat{\upsigma}^2=0.1166)$    \\
    $2$  & $2$ & $0.3120\ (\hat{\upsigma}^2=0.0771)$  & $ 1.3101\ (\hat{\upsigma}^2=0.2050)$     \\
    $2$  & $3$ & $0.5354\ (\hat{\upsigma}^2=0.3261)$  & $1.3315\ (\hat{\upsigma}^2=0.4669)$      \\ \midrule
    $3$  & $0.1$ & $0.3448\ (\hat{\upsigma}^2=0.3936)$  & $1.3020\ (\hat{\upsigma}^2=0.3143)$    \\
    $3$  & $0.5$ & $0.2593\ (\hat{\upsigma}^2=0.0673)$  & $0.8850\ (\hat{\upsigma}^2=0.1520)$     \\
    $3$  & $2$ & $0.2373\ (\hat{\upsigma}^2=0.0310)$  & $1.2419\ (\hat{\upsigma}^2=0.1599)$   \\
    $3$  & $3$ & $0.3159\ (\hat{\upsigma}^2=0.1042)$  & $1.2420\ (\hat{\upsigma}^2=0.1427)$          \\ \bottomrule
\end{tabular}
\caption[Normalized mean terminal distance from the target to the nearest agent and normalized mean terminal maximum distance between agents when there are four agents, one target, $r=2$, and $r'=1.5$]{Mean terminal distance from the target to the nearest agent and mean terminal maximum distance between agents when there are four agents, one target, $r=2$, and $r'=1.5$ (distances are divided by their values at the beginning of the replication prior to averaging). $\hat{\upsigma}^2$ is the sample variance. The variables $\uptau$ and $\uplambda$ have a significant effect over the behavior of the agents.}
\label{eq:jonnsm2}
\end{table}

\begin{table}[p]
\centering
\begin{tabular}{c c c c c c} \toprule
   {$\uptau$} & {$\uplambda$}  & {Dist. to Nearest Agent} & {Max. Dist. Between Agents}  \\ \midrule
     $1$  & $0.1$ & $1.0161\ (\hat{\upsigma}^2=0.6779)$  & $0.7132\ (\hat{\upsigma}^2=0.1144)$      \\
     $1$ & $0.5$ &  $1.2612\ (\hat{\upsigma}^2=0.7190)$ & $0.6005\ (\hat{\upsigma}^2=0.1207)$   \\
     $1$  & $2$ & $1.1480\ (\hat{\upsigma}^2=0.8477)$  & $0.6960\ (\hat{\upsigma}^2=0.1133)$     \\
   $1$  & $3$ & $1.0841\ (\hat{\upsigma}^2=0.3906)$  & $0.6978\ (\hat{\upsigma}^2=0.2923)$       \\ \midrule
   $2$  & $0.1$ & $ 0.8769\ (\hat{\upsigma}^2=0.4911)$  & $0.7907\ (\hat{\upsigma}^2=0.1680)$      \\
    $2$ & $0.5$ & $1.3092 \ (\hat{\upsigma}^2=0.8296)$ & $0.6923\ (\hat{\upsigma}^2=0.1428)$    \\
    $2$  & $2$ & $1.2736\ (\hat{\upsigma}^2=0.3907)$  & $ 0.6780\ (\hat{\upsigma}^2=0.1095)$     \\
    $2$  & $3$ & $1.2974\ (\hat{\upsigma}^2=1.2430)$  & $0.6500\ (\hat{\upsigma}^2=0.0818)$      \\ \midrule
    $3$  & $0.1$ & $0.9303\ (\hat{\upsigma}^2=0.6797)$  & $0.5529\ (\hat{\upsigma}^2= 0.0540)$    \\
    $3$  & $0.5$ & $0.9133\ (\hat{\upsigma}^2=0.4332)$  & $0.6480\ (\hat{\upsigma}^2=0.1503)$     \\
    $3$  & $2$ & $1.0092\ (\hat{\upsigma}^2=0.4750)$  & $0.6979\ (\hat{\upsigma}^2=0.0554)$   \\
    $3$  & $3$ & $1.0755\ (\hat{\upsigma}^2=0.5873)$  & $0.6411\ (\hat{\upsigma}^2=0.0706)$          \\ \bottomrule
\end{tabular}
\caption[Normalized mean terminal distance from the target to the nearest agent and normalized mean terminal maximum distance between agents when there are four agents, one target, $r=1$, and $r'=0.5$]{Mean terminal distance from the target to the nearest agent and mean terminal maximum distance between agents when there are four agents, one target, $r=1$, and $r'=0.5$ (distances are divided by their values at the beginning of the replication prior to averaging). $\hat{\upsigma}^2$ is the sample variance. The variables $\uptau$ and $\uplambda$ have a significant effect over the behavior of the agents.}
\label{eq:jonnsm3}
\end{table}

\begin{table}[p]
\centering
\begin{tabular}{c c c c c c} \toprule
   {$\uptau$} & {$\uplambda$}  & {Dist. to Nearest Agent} & {Max. Dist. Between Agents}  \\ \midrule
     $1$  & $0.1$ & $1.4262\ (\hat{\upsigma}^2=0.5683)$  & $0.4505\ (\hat{\upsigma}^2=0.0398)$      \\
     $1$ & $0.5$ &  $1.0955\ (\hat{\upsigma}^2=0.3439)$ & $0.4335\ (\hat{\upsigma}^2=0.0288)$   \\
     $1$  & $2$ & $1.4668\ (\hat{\upsigma}^2=0.1747)$  & $0.4351\ (\hat{\upsigma}^2=0.0359)$     \\
   $1$  & $3$ & $1.3079\ (\hat{\upsigma}^2=0.5449)$  & $0.4665\ (\hat{\upsigma}^2=0.0306)$       \\ \midrule
   $2$  & $0.1$ & $ 1.3213\ (\hat{\upsigma}^2=0.5002)$  & $0.4293\ (\hat{\upsigma}^2=0.0227)$      \\
    $2$ & $0.5$ & $1.4793 \ (\hat{\upsigma}^2=0.9726)$ & $0.3979\ (\hat{\upsigma}^2=0.0312)$    \\
    $2$  & $2$ & $1.4770\ (\hat{\upsigma}^2=0.3656)$  & $ 0.3648\ (\hat{\upsigma}^2=0.0234)$     \\
    $2$  & $3$ & $1.2614\ (\hat{\upsigma}^2=0.6410)$  & $0.4079\ (\hat{\upsigma}^2=0.0158)$      \\ \midrule
    $3$  & $0.1$ & $ 1.2997\ (\hat{\upsigma}^2=0.3756)$  & $0.4262\ (\hat{\upsigma}^2=0.0330)$    \\
    $3$  & $0.5$ & $1.4249\ (\hat{\upsigma}^2=0.8190)$  & $0.4505\ (\hat{\upsigma}^2=0.0338)$     \\
    $3$  & $2$ & $1.0037\ (\hat{\upsigma}^2=0.1506)$  & $0.4659\ (\hat{\upsigma}^2=0.0946)$   \\
    $3$  & $3$ & $ 1.4076\ (\hat{\upsigma}^2=0.7358)$  & $0.4224\ (\hat{\upsigma}^2=0.0145)$          \\ \bottomrule
\end{tabular}
\caption[Normalized mean terminal distance from the target to the nearest agent and normalized mean terminal maximum distance between agents when there are four agents, one target, $r=0.5$, and $r'=0.4$]{Mean terminal distance from the target to the nearest agent and mean terminal maximum distance between agents when there are four agents, one target, $r=0.5$, and $r'=0.4$ (distances are divided by their values at the beginning of the replication prior to averaging). $\hat{\upsigma}^2$ is the sample variance. The variables $\uptau$ and $\uplambda$ have a significant effect over the behavior of the agents.}
\label{eq:jonnsm4}
\end{table}

An overall trend that can be observed in Tables \ref{eq:jonnsm1}--\ref{eq:jonnsm4} is that larger values of $r$ are correlated with a decrease in the mean terminal distance between the target and the nearest agent. 
%(i.e., agents attempt to address objective 1 on p. \pageref{eq:sandywpusstod} by ensuring the target is always near an agent). 
Additionally, larger values of $r$ are associated with larger values of the mean maximum distance between agents. 
%(i.e., agents attempt to address objective 2 on p. \pageref{eq:sandywpusstod} by spreading out). 
In contrast, small values of $r$ are correlated with a large mean terminal distance between the target and the nearest agent and a small mean terminal maximum distance between agents. 
Larger values of $r$ allow agents to minimize the distance between the target and the nearest agent while simultaneously maximizing the maximum distance between agents. 



For the case where $r=2$ and $r'=1.5$, $\uptau=1$, and $\uplambda=0.5$, Figure \ref{fig:toysstory1} shows the evolution of the mean distance between the target and the nearest agent relative to the initial value of this distance using the settings from Tables \ref{eq:jonnsm1}--\ref{eq:jonnsm4}.  The result in Figure \ref{fig:toysstory1} is consistent with the results in Table \ref{eq:jonnsm2}. Figure \ref{fig:toysstory2} repeats the experiment of Figure \ref{fig:toysstory1} for the case where there is one agent and one target. The mean terminal distance in Figure \ref{fig:toysstory2} seems to be approximately the same as the mean terminal distance in Figure \ref{fig:toysstory1}, although it is important to note the high variance of the individual realizations 



\begin{figure}[!p]
\centering
\begin{subfigure}[b]{1\textwidth}
 \centering
\begin{tikzpicture}


\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.6]{Plots/multiagent/RelativeDistance/4a1t-eps-converted-to.pdf}};

\end{tikzpicture}
 \caption{Four agents, one target.}
 \label{fig:toysstory1}
\end{subfigure}\hfill


\begin{subfigure}[b]{1\textwidth}
\centering
\begin{tikzpicture}

\node[inner sep=0pt] (probe) at (0,0)
{\includegraphics[scale=0.6]{Plots/multiagent/RelativeDistance/1a1t-eps-converted-to.pdf}};
\end{tikzpicture}
\caption{One agent, one target.}
\label{fig:toysstory2}
\end{subfigure}\hfill
\caption[Mean distance from the target to the nearest agent divided by the initial value of this distance]{Mean distance from the target to the nearest agent divided by the initial value of this distance. The thick line represents the mean relative distance obtained by averaging 20 i.i.d. realizations while each of the thinner lines represents one of the first 5 realizations. }
\label{fig:toysstory}
\end{figure}





\section{Concluding Remarks}
\label{sec:finalcommentsagent}


This chapter investigates the numerical performance of cyclic SA applied to a multi-agent optimization problem for tracking and surveillance. An attractive feature of the resulting multi-agent optimization algorithm is that it can be implemented when agents are not allowed to communicate with each other, although it is entirely possible to extend the algorithm to include communication between agents. One assumption made throughout this section is that each agent knows their own position and velocity at any point in time. Through a natural modification, the algorithm in this chapter could also be implemented in the same manner when these variables are estimated. The numerical results indicate that, when the sensor radius is sufficiently large, the proposed algorithm allows agents to track the target while simultaneously increasing the distance between agents. 
%However, the performance of the algorithm is strongly dependent on the values of $\uptau$ and $\uplambda$ appearing in Steps 3 and 4 of the algorithm (see Section \ref{sec:algooutline}).
%

A few directions for future research regarding this chapter's multi-agent algorithm include investigating other methods for predicting target/agent state positions (aside from the EKF), considering adaptive gain sequences (instead of the using the constant gain $a$), and considering other objective functions. With regards to this last topic, we remind the reader that  in this chapter each agent is minimizing a different loss function, which is a different setting than the setting from Chapters \ref{chap:descriptionofGCSA}--\ref{chap:numericschap} where there is a universal (i.e., common to all agents) loss function to minimize. A universal loss function can be constructed for the multi-agent problem in this chapter by simply adding the individual loss functions. Specifically, the universal loss function could be defined as $L(\bm\uptheta)\equiv \sum_{j=1}^n L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))$, where $\bm\uptheta$ is a vector containing the velocity vectors of all $n$ agents. Note that the value of $[\dot{x}_j^E(t),\dot{x}_j^N(t)]^\top$ affects the value of $L_i(\dot{x}_i^E(t),\dot{x}_i^N(t))$ even when $i\neq j$ (through the terms $\bm{c}_i(t)$ and $\upgamma_\ell(t+\updelta t)$ for $\ell=1,\dots,{\text{\# Agents}}$).
%, minimizing $L(\bm\uptheta)$ is not the same as minimizing each $L_j(\dot{x}_j^E(t),\dot{x}_j^N(t))$ separately. 
Furthermore, if agent $j$ is located at a distance of exactly $\uplambda$ from any target (under the usual Gaussian state model this occurs with probability zero) then $L(\bm\uptheta)$ is not differentiable with respect to $[\dot{x}_j^E(t),\dot{x}_j^N(t)]^\top$. Future work could focus on studying this more complex scenario.




==> thesis arXiv 2/chapter6.tex <==
%!TEX root = root.tex

\chapter[Overall Concluding Remarks and Future Work]{Overall Concluding Remarks\\ and Future Work}


This dissertation investigated the asymptotic properties of the generalized cyclic stochastic approximation (GCSA) algorithm (Algorithm \ref{findme}) including the convergence (w.p.1) of the iterates, the asymptotic normality of the normalized iterates, and the asymptotic efficiency of GCSA relative to its non-cyclic counterpart. Next we review some of the contributions of this dissertation. 

The main theorem on convergence, Theorem \ref{thm:hoeshoo}, provided sufficient conditions for the convergence w.p.1 of the GCSA iterates to a zero of the gradient of the function to minimize. Although some of the convergence conditions closely resemble well-known conditions for the convergence of the standard (i.e., non-cyclic) SA algorithms, a few conditions are inherent only to the GCSA algorithm (see Section \ref{sec:discussconvergence} for a discussion on the validity of the convergence conditions in Theorem \ref{thm:hoeshoo}). Section \ref{sec:convergencenumericos} contains numerical examples illustrating the convergence of GCSA using both SG- and SPSA-based gradient estimates. 

 
With the goal of computing the rate of convergence of the GCSA algorithm, a generalization to Theorem 2.2 in Fabian (1968)\nocite{fabian1968} (regarding the asymptotic normality of SA procedures) was provided in Chapter \ref{sec:ROC}  (see Theorem \ref{thm:generalizefabian}). Theorem \ref{thm:fnogg} then used the generalization from Theorem \ref{thm:generalizefabian} to derive conditions for the asymptotic normality of the normalized iterates of a special case of GCSA (which helps define the rate of convergence of the algorithm) as well as to obtain expressions for the parameters of its asymptotic distribution (see Section \ref{sec:bonestrailseason} for a discussion on the conditions of Theorem \ref{thm:fnogg} for asymptotic normality).  A few other applications of our generalization to Theorem 2.2 in Fabian (1968)\nocite{fabian1968} are discussed in Appendix \ref{sec:fabiansecgeneralize}, including an application to an adaptive SA algorithm.  Numerical examples supporting the theory on asymptotic normality are given in Section \ref{sec:normalitycenumericos}.  

Using the result on asymptotic normality from Theorem \ref{thm:fnogg}, Chapter \ref{chap:imefficient} provided an analytical estimate for the asymptotic efficiency (in the MSE sense) of a special case of GCSA relative to the efficiency of its non-cyclic counterpart after taking into consideration the cost of implementing each algorithm. It was shown that, in general, either algorithm may be (asymptotically) more efficient than the other (it is important to keep in mind, however, that the relative efficiency in Chapter \ref{chap:imefficient} is only one possible way to compare the cyclic and non-cyclic algorithms). Section \ref{sec:Numericssimples} contains numerical experiments estimating the aforementioned relative efficiency under different definitions of cost when the update directions are either SG- or SPSA-based. 
 
 
 While the numerical examples in Chapter \ref{chap:numericschap} focused on cases where the conditions for convergence and/or asymptotic normality were met, Chapter \ref{chap:multiagent} investigated the numerical performance of a cyclic SA algorithm applied to a zero-communication multi-agent optimization problem where the loss function is time-varying. As a result, the theory of Chapters \ref{sec:cyclicseesaw}--\ref{chap:imefficient} (which assumes that the loss function is not time-varying) does not apply. It was observed that the performance of the cyclic SA approach had a strong correlation with the quality of the agents' sensors: the better the sensors' quality, the better the cyclic algorithm performed (this behavior is not surprising and, more importantly, is not specific to the cyclic algorithm).
 
 We end this chapter by giving a few topics for future research.
%
%{\underline{\it{Future Research on Convergence}}}. 
One natural direction for future research pertains to the convergence of a constrained variant of GCSA. A possible approach to constructing a constrained version of GCSA could involve projecting $\hat{\bm{\uptheta}}_k$ at every step (we refer the reader to the comment on p. \pageref{page:onconditionA4444} regarding condition A4)\nocite{ISSO}. Another approach could consist on constructing a variant of GCSA for which the constraints are satisfied asymptotically (e.g., Wang and Spall 2011, where the iterates of the algorithm asymptotically satisfy the requirement of lying in a discrete set)\nocite{dspsa}. The work of Wang and Spall (2008)\nocite{otherwang} presents an SA algorithm based on the penalty functions method  for solving stochastic optimization problems with general inequality constraints, the ideas of this paper may also be of interest when considering constrained versions of the GCSA algorithm.


 A second avenue for future research involves the generalization of the GCSA algorithm to an asynchronous setting (i.e., parallelizing GCSA), this could possibly be done using ideas similar to those in Tsitsiklis (1994)\nocite{tsitsiklis1994}. Additionally, it would also be interesting to study the behavior of cyclic procedures for time-varying loss functions (many multi-agent optimization problems, such as the problem in Chapter \ref{chap:multiagent}, have a time-varying loss function). 

A few other topics for future research are the following: 
\begin{enumerate}
\item Can the boundedness assumption of condition A1 (see p. \pageref{cond:conditiona1}) be weakened? (Answering this question may prove useful in when obtaining practical conditions for the convergence of an asynchronous variant of GCSA.)
\item   Borkar and Meyn (2000) show that:
\begin{quote}
. . . the ODE method can be extended to establish both the stability and convergence of the stochastic approximation method, as opposed to only the latter. (Borkar and Meyn 2000)
\end{quote}
Might the ideas of the paper by Borkar and Meyn (2000)\nocite{borkarmeyn2000} be used to extend the theory of convergence of the GCSA iterates in an analogous manner?
%\item In Algorithm \ref{}, the probability of updating subvector $j$ was equal to $q_j$ independently of the iteration number. What can be said about convergence when 
\item Could iterate averaging be combined with Algorithm \ref{beastwasdone} (see p. \pageref{beastwasdone}) so that the iterates of the resulting algorithm are asymptotically normally distributed (after an appropriate centering and scaling)?
\item What finite-time performance guarantees can be obtained for the GCSA algorithm (e.g., in terms of bounds on the MSE as a function of the iteration number)?
\item As discussed in Sections \ref{sec:costoport} and \ref{sec:aseficwiener}, the cost of implementation is an important aspect to consider when comparing a cyclic algorithm to its non-cyclic counterpart. Future work might consist of a more detailed investigation into how the cost of implementing a cyclic algorithm compares to the cost of implementing a non-cyclic algorithm.
\end{enumerate}
In summary, this dissertation addressed several important (and previously unanswered) questions regarding cyclic implementations of SA procedures. Still, several interesting questions remain unanswered (as indicated in the discussion above). It is expected that some of the directions for future work mentioned above will make heavy use of the results and ideas in this dissertation.






==> thesis arXiv 2/chapterNUMERICS.tex <==

%!TEX root = root.tex

\chapter{Numerical Analysis}
\label{chap:numericschap}
%\chaptermark{The Cyclic Seesaw Algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Chapter \ref{sec:cyclicseesaw} of this dissertation derived conditions for the convergence of the GCSA algorithm, Chapter \ref{sec:ROC} derived conditions for the asymptotic normality of a special case of GCSA, and Chapter \ref{chap:imefficient} discussed the asymptotic relative efficiency between a special case of GCSA and its non-cyclic counterpart. This chapter contains numerical results that illustrate the theory of Chapters \ref{sec:cyclicseesaw}--\ref{chap:imefficient}. Specifically, Section \ref{sec:convergencenumericos} contains numerical results on the convergence of the GCSA algorithm, Section \ref{sec:normalitycenumericos} contains results on asymptotic normality, and Section \ref{sec:Numericssimples} contains results on relative efficiency.


\section{Numerical Examples on Convergence}
\label{sec:convergencenumericos}

This section provides a few numerical examples on the convergence of Algorithms \ref{beastwasdone} (where the subvector to update is selected at random) and \ref{kirkey} (where the subvector to update is selected following a deterministic pattern). Each of these two algorithms is implemented using SPSA-based noisy update directions (Section \ref{sec:clubsodeashrimp}) and SG-based noisy update directions (Section \ref{sec:omgimanothersectionsssd}). Algorithms \ref{beastwasdone} and \ref{kirkey} are also compared to two non-cyclic variants.
%More numerical experiments are performed in Section \ref{sec:normalitycenumericos}, Section \ref{sec:Numericssimples}, and Chapter \ref{chap:multiagent}. 

\subsection{Algorithms \ref{beastwasdone} \& \ref{kirkey} with SPSA-Based Gradient Estimates}
\label{sec:clubsodeashrimp}

This section considers the problem of stochastic optimization using Algorithms \ref{beastwasdone} and \ref{kirkey} (special cases of GCSA) with SPSA-based gradient estimates of the form in (\ref{eq:howeardspos1}) and (\ref{eq:howeardspos2}). Here only the subvector to update is perturbed at each subiteration. The loss function to minimize is the {\it{skewed quartic}} function (Spall 2003, Chapter 6):
\begin{align}
\label{func:skewedquartic}
L(\bm\uptheta)=(\bm{B}\bm\uptheta)^\top\bm{B}\bm\uptheta +0.1\sum_{i=1}^p(\bm{B}\bm\uptheta)_i^3+0.01\sum_{i=1}^p(\bm{B}\bm\uptheta)_i^4,
\end{align}
where $p=10$ is the dimension of $\bm\uptheta$, $p\bm{B}\in \mathbb{R}^{p\times p}$ is an upper-triangular matrix of ones, and $\bm{v}_i$ denotes the $i$th entry of the vector $\bm{v}$. $L(\bm\uptheta)$ achieves its minimum at $\bm\uptheta^\ast=\bm{0}$ with $L(\bm\uptheta^\ast)=\bm{0}$. Figure \ref{eq:whatyouwillnotbring} illustrates the function in (\ref{func:skewedquartic}) for the special case where $p=2$. We assume that the loss function is corrupted by i.i.d. Gaussian noise, that is $Q(\bm\uptheta,\bm{V})=L(\bm\uptheta)+\upvarepsilon$
%\begin{align*}
%Q(\bm\uptheta,\bm{V})=L(\bm\uptheta)+\upvarepsilon,
%\end{align*}
where $\upvarepsilon\sim\mathcal{N}(0,0.1^2)$. 

\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.5]{Plots/squartic-eps-converted-to.pdf}};  
     \node[left= -0.6cm of probe]{$L(\bm\uptheta)$};
      \node at (0.8,-3.7) {$\uptau_1$};
      \node at (-3.6,-3.4) {$\uptau_2$};
\end{tikzpicture}
%
%\centering
%  \begin{tikzpicture}
%\input{Plots/squartic.tex}
%\end{tikzpicture}
\caption[The skewed quartic function in two dimensions]{The skewed quartic function in two dimensions. In this example, $\bm\uptheta=[\uptau_1,\uptau_2]^\top\in\mathbb{R}^2$ and $L(\bm\uptheta)$ is defined as in (\ref{func:skewedquartic}).}
\label{eq:whatyouwillnotbring}
\end{figure}


In order to implement Algorithms \ref{beastwasdone} and \ref{kirkey} the vector $\bm\uptheta=[\uptau_1,\dots,\uptau_{10}]^\top$ is divided into $d=5$ subvectors of length $2$ where the $j$th subvector is equal to $[\uptau_{2j-1},\uptau_{2j}]^\top$. The values for $a_k^{(j)}$ and $c_k^{(j)}$ are given by $a_k^{(j)}=a/(1+k)^{\upalpha}$ and $c_k^{(j)}=c/(1+k)^{\upgamma}$ for all $j$ with $a=1$, $\upalpha=0.602$, $c=1$, and $\upgamma=0.101$. These values of $\upalpha$ and $\upgamma$ are standard values for the SPSA algorithm while the values of $a$, $A$, and $c$ were {\it{lightly}} tuned. The non-zero entries of the perturbation vectors (the non-zero entries of $\bm\Delta$) are independent  and take the value $\pm1$ with equal probability. For Algorithm \ref{beastwasdone}, all subvectors were equally likely to be selected for updating (i.e., $q(j)=1/5$ for all $j$). We let $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{beastwasdone}}}$ and $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}$ denote the iterates of Algorithms \ref{beastwasdone} and \ref{kirkey}, respectively, after having performed $u$ subvector updates (in general, the number of subvector updates is not necessarily equal to the number of iterations). Figure \ref{eq:iamapigeon2} presents the values of $\overline{\|\hat{\bm{\uptheta}}_u^{\text{Alg \ref{beastwasdone}}}-\bm\uptheta^\ast\|}/\|\hat{\bm{\uptheta}}_0^{\text{Alg \ref{beastwasdone}}}-\bm\uptheta^\ast\|$ and  $\overline{\|\hat{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}-\bm\uptheta^\ast\|}/\|\hat{\bm{\uptheta}}_0^{\text{Alg \ref{kirkey}}}-\bm\uptheta^\ast\|$ with $\hat{\bm{\uptheta}}_0\equiv\hat{\bm{\uptheta}}_0^{\text{Alg \ref{beastwasdone}}}=\hat{\bm{\uptheta}}_0^{\text{Alg \ref{kirkey}}}=[1,\dots,1]^\top$, where $\bar{\bm\uptheta}_u^{\text{Alg \ref{beastwasdone}}}$ and $\bar{\bm\uptheta}_u^{\text{Alg \ref{kirkey}}}$ denote the mean values of the algorithm iterates over 100 replications. It is seen that the mean distance between $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{beastwasdone}}}$ and $\bm\uptheta^\ast$ (relative to $\|\hat{\bm{\uptheta}}_0^{\text{Alg \ref{beastwasdone}}}-\bm\uptheta^\ast\|$) and the mean distance between $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}$ and $\bm\uptheta^\ast$ (relative to $\|\hat{\bm{\uptheta}}_0^{\text{Alg \ref{kirkey}}}-\bm\uptheta^\ast\|$) are both decreasing in magnitude (i.e., the iterates approach $\bm\uptheta^\ast$). 
%While Figure \ref{eq:iamapigeon2} is technically showing convergence of the scaled norm of the expected values of $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{beastwasdone}}}$ and $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}$, similar (but noisier) behavior was observed for single replications of the algorithms (i.e., a decrease in loss).

\begin{figure}[t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
   

% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/mycyclicSPSA2outside-eps-converted-to.pdf}};  
     \node[left= -0.8cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm{\uptheta}}_u-\bm\uptheta^\ast\|}}{\|\hat{\bm{\uptheta}}_0-\bm\uptheta^\ast\|}}$};
\end{tikzpicture}
%
%
\caption[Performance of SPSA-based GCSA with skewed quartic loss]{An illustration of Algorithms \ref{beastwasdone} (randomized selection) and \ref{kirkey} (deterministic patterns) on the noisy skewed quartic loss function when the gradient estimates are SPSA-based. Here, $\hat{\bm{\uptheta}}_u$ represents either $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{beastwasdone}}}$ or $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}$.}
\label{eq:iamapigeon2}
\end{figure}

We now consider the same setting as in Figure \ref{eq:iamapigeon2} with two modifications. First, the sequences $a_k^{(1)}$ and $a_k^{(2)}$ are not required to be equal but both are assumed to have the form:
\begin{align*}
a_k^{(j)}=\frac{a^{(j)}}{(1+k+A^{(j)})^{0.602}}
\end{align*}
for $a^{(j)}>0$ and $A^{(j)}\geq 0$. Second, $\bm\uptheta$ is divided into only two subvectors corresponding to the first- and second halves of $\bm\uptheta$ (i.e., $d=2$). 
%Third, we allow $c\neq 1$ in $c_k^{(j)}$ (this sequence is the same for all $j$).
 We compare the following algorithms:
\begin{DESCRIPTION}
\item[Case 1:] The SPSA algorithm with $a_k=a/(1+k+A)^{0.602}$.
\item[Case 2:] The SPSA algorithm with $a_k$ replaced by a diagonal matrix, $\bm{A}_k$, such that the $i$th diagonal entry of $\bm{A}_k$ is equal to $a_k^{(j)}$ where $i\in \mathcal{S}_j$.\label{pageref:toccasesSPSA}
\item[Case 3:] Algorithm \ref{beastwasdone} (the subvector to update is selected according to a random variable) with SPSA-based gradient estimates. Each of the two subvectors is updated with equal probability.
\item[Case 4:] Algorithm \ref{kirkey} (the subvector to update is selected following a strictly alternating pattern) with SPSA-based gradient estimates.
\end{DESCRIPTION}
%To minimize the number of parameters to tune we set $\upalpha=0.602$.
 For each case, the algorithms were run for a total of $T=5000$ subvector updates and each realization was initialized at a vector following a uniform distribution on $[-5,5]^{10}$. Thus, there were 2,500 iterations in Cases 1 and 2 (since each iteration requires updating both subvectors) and 5,000 iterations in Cases 3 and 4 (since each iteration requires updating only one subvector). We also set $c_k=c_k^{(j)}=0.1/(1+k)^{0.101}$ and use the same distribution for the perturbation vectors as before. Table \ref{table:omgmyfirsttable} presents the results of part of the tuning process for Cases 1--4. 
% Here, $\overline{L(\hat{\bm{\uptheta}}_T)}$ represents an estimate of the loss function at the terminal value. For each algorithm, $\overline{L(\hat{\bm{\uptheta}}_T)}$ was obtained by averaging the terminal loss values of 100 replications. 
 Figure \ref{fig:gainyourownsga} shows the evolution of the loss function (for three replications) as the number of updates increases for Cases 1--4 using the best choice of parameters from Table \ref{table:omgmyfirsttable} (for all cases the same gain sequence yielded the smallest mean terminal loss function value). Table \ref{table:omgmyfirsttable} and Figure \ref{fig:gainyourownsga} indicate that all algorithms had comparable performance. Moreover, the results support the theory on convergence of the GCSA algorithm. 


\begin{table}[p]
\centering
\begin{tabular}{SSSSSS} \toprule
    {Algorithm} & {$a^{(1)}$} & {$a^{(2)}$}  & {$A^{(1)}$} & {$A^{(2)}$} & {$\overline{L(\hat{\bm{\uptheta}}_T)}$} \\ \midrule
    {Case 1}  & 1  & {--} & 0  & {--}  & {$5.1781\times 10^{88}$}    \\
    {SPSA}  & 1 & {--} & 100 & {--} & 0.1733\ $\ast$   \\
    {(regular)}  & 0.1  & {--} & 0  & {--} & 0.5291    \\
    {}  & 0.1  & {--} & 100  & {--} &  0.5613       \\ \midrule
    {Case 2}  & 1  & 1 & 0  & 0  & {$6.7502\times 10^{119}$}    \\
    {SPSA}  & 1 & 1 & 100 & 100 & 0.1650\ $\ast$   \\
    {(diagonal gain)}  & 1  & 0.1 & 0  & 0 & 0.4335    \\
    {}  & 1  & 0.1 & 100  & 100 & 0.4236    \\
    {}  & 0.1  & 1 & 0  & 0 & 0.3941    \\
    {}  & 0.1  & 1 & 100  & 100 & 0.3691    \\
   {}  & 0.1  & 0.1 & 0  & 0 & 0.5060    \\
    {}  & 0.1  & 0.1 & 100  & 100 & 0.5727          \\ \midrule
    {Case 3}  & 1  & 1 & 0  & 0  &  0.2282    \\
    {SPSA}  & 1 & 1 & 100 & 100 & 0.1982\ $\ast$   \\
    {(random selection)}  & 1  & 0.1 & 0  & 0 & 0.2191    \\
    {}  & 1  & 0.1 & 100  & 100 & 0.2025    \\
    {}  & 0.1  & 1 & 0  & 0 & 0.6915    \\
    {}  & 0.1  & 1 & 100  & 100 &  0.5772    \\
   {}  & 0.1  & 0.1 & 0  & 0 & 0.6109   \\
    {}  & 0.1  & 0.1 & 100  & 100 & 0.6477          \\ \midrule
    {Case 4}  & 1  & 1 & 0  & 0  & 0.1992    \\
    {SPSA}  & 1 & 1 & 100 & 100 & 0.1732\ $\ast$   \\
    {(deterministic patterns)}  & 1  & 0.1 & 0  & 0 & 0.3406    \\
    {}  & 1  & 0.1 & 100  & 100 & 0.3796    \\
    {}  & 0.1  & 1 & 0  & 0 & 0.3841    \\
    {}  & 0.1  & 1 & 100  & 100 & 0.3750    \\
   {}  & 0.1  & 0.1 & 0  & 0 & 0.4812
    \\
    {}  & 0.1  & 0.1 & 100  & 100 & 0.5286         \\ \bottomrule
\end{tabular}
\caption[Tuning the gain sequence parameters for Cases 1--4 from p. \pageref{pageref:toccasesSPSA} where the noisy gradient updates are SPSA-based]{Tuning the gain sequence parameters. Note that for Case 1 there is only one gain sequence, $a_k$, which we have set equal to $a^{(1)}/(1+k+A^{(1)})^{0.602}$. See p. \pageref{pageref:toccasesSPSA} for a description of each of the four cases above. Here, $\overline{L(\hat{\bm{\uptheta}}_T)}$ represents an estimate of the loss function at the terminal value obtained by averaging the terminal loss values of 100 replications. For comparison, $L(\bm\uptheta^\ast)=0$. An asterisk marks the smallest mean terminal loss function value for each case.}
\label{table:omgmyfirsttable}
\end{table}

% -------------------------------------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------------------------------------------
% A DIFFERENT PLOT BELOW
% -------------------------------------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------------------------------------------

\begin{figure}[p]
\centering
  \begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/cases/SPSAcases1-eps-converted-to.pdf}};
 \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};
%\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/cases/SPSAcases2-eps-converted-to.pdf}};
     \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

\end{tikzpicture}
 \end{subfigure}
 \caption*{Above: the 1st replication. }

% -------------------------------------------------------------------------------------------------------------------------

 \vspace{.03in}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
    \begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/cases/SPSAcases3-eps-converted-to.pdf}};
 \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

\end{tikzpicture}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/cases/SPSAcases4-eps-converted-to.pdf}};
     \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

\end{tikzpicture}
 \end{subfigure}%
 \caption*{Above: the 2nd replication.}
 
 
 % -------------------------------------------------------------------------------------------------------------------------
 
  \vspace{.03in}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
    \begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/cases/SPSAcases5-eps-converted-to.pdf}};
 \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};
%\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/cases/SPSAcases6-eps-converted-to.pdf}};
     \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

\end{tikzpicture}
 \end{subfigure}
  \caption*{Above: the 3rd replication.}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
 \vspace{.03in}
         
% -------------------------------------------------------------------------------------------------------------------------
        
\caption[Performance of Cases 1--4 from p. \pageref{pageref:toccasesSPSA} where the noisy gradient estimates are SPSA-based]{Performance of Cases 1 (deterministic patterns), 2 (random selection), 3 (regular SPSA), and 4 (SPSA with diagonal gains) for three i.i.d. replications (i.e., three i.i.d. realizations of each of the four cases) using the tuned parameters from Table \ref{table:omgmyfirsttable}. The term $\hat{\bm{\uptheta}}_u$ is a generic vector representing the vector obtained after having performed $u$ subvector updates.}
\label{fig:gainyourownsga}
\end{figure}





\subsection{Algorithms \ref{beastwasdone} \& \ref{kirkey} with SG-Based Gradient Estimates}
\label{sec:omgimanothersectionsssd}
This section is concerned with an implementation of Algorithms \ref{beastwasdone} and \ref{kirkey} where the noisy gradient estimates are SG-based. Here, we consider the problem of linear regression with scalar output. We assume that the output, $z_k$, of some random process is given by $z_k=\bm{h}_k^\top \bm\uptheta^\ast+\upvarepsilon_k$
%\begin{align*}
%z_k=h(\hat{\bm{\uptheta}}_k,\bm{x}_k)+\upvarepsilon_k
%\end{align*}
for a sequence $\bm{h}_k\in\mathbb{R}^p$ of inputs and an i.i.d. sequence of mean-zero random variables $\upvarepsilon_k$. The objective is to recover the true value of $\bm\uptheta$, denoted by $\bm\uptheta^\ast$, using a set of input-output pairs $\{(\bm{h}_k,z_k)\}_{k\geq 1}$. An online approach to solving this problem is the following:
\begin{align}
\label{eq:colorlocalcouncil}
\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\left[(\bm{h}_{k+1}^\top \bm\uptheta-z_{k+1})\bm{h}_{k+1}\right]_{\bm\uptheta=\hat{\bm{\uptheta}}_k}.
\end{align}
The algorithm in (\ref{eq:colorlocalcouncil}) is known as the least-mean-squares (LMS) algorithm.
%. Specifically, the SG produces updates according to $\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k$


Before proceeding with the numerical experiments let us briefly motivate (\ref{eq:colorlocalcouncil}). First, note that if $\{\upvarepsilon_k\}_{k\geq 0}$ and $\{\bm{h}_{k}\}_{k\geq 0}$ are each i.i.d. sequences (with $\bm{h}_k$ being independent of $\upvarepsilon_k$) then, under certain conditions (e.g., Spall 2003, p. 136), the loss function $L(\bm\uptheta)\equiv (1/2)E[(z_k-\bm{h}_{k}^\top\bm\uptheta)^2]$ is independent of $k$, $L(\bm\uptheta)$ has a unique minimum at $\bm\uptheta^\ast$, and the vector in square brackets in (\ref{eq:colorlocalcouncil}) is an unbiased measurement of the gradient of $L(\bm\uptheta)$. Therefore, under certain conditions the LMS algorithm in (\ref{eq:colorlocalcouncil}) is a special case of the SG algorithm (which requires an unbiased estimate of the gradient of the loss function). Figure \ref{fig:substitutionoperation} illustrates $L(\bm\uptheta)$ for the special case where $\bm\uptheta\in \mathbb{R}^2$, the entries of $\bm{h}_k$ are independent and uniformly distributed in $[-3,3]$, $\upvarepsilon_k\sim\mathcal{N}(0,1)$, and $\bm\uptheta^\ast=[1,1]^\top$.





\begin{figure}[!t]
% Generated with matlab2tikz('width', '.6\textwidth') in MATLAB 
% Changed location in .tex file with at={(0.04\textwidth,0\textwidth)}
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.5]{Plots/lmsfunc-eps-converted-to.pdf}};  
     \node[left= -0.6cm of probe]{$L(\bm\uptheta)$};
      \node at (4.6,-2.5) {$\uptau_2$};
      \node at (-2.1,-3.4) {$\uptau_1$};
\end{tikzpicture}
%  \begin{tikzpicture}
%\input{Plots/lmsfunc.tex}
%\end{tikzpicture}
\caption[The loss function associated with the LMS algorithm in (\ref{eq:colorlocalcouncil}).]{The loss function, $L(\bm\uptheta)= (1/2)E{[}(z_k-\bm{h}_{k}^\top\bm\uptheta)^2{]}$, associated with the least-mean-squares (LMS) algorithm in (\ref{eq:colorlocalcouncil}) for the special case where $\bm\uptheta\in \mathbb{R}^2$,  $\bm\uptheta^\ast=[1,1]^\top$, the entries of $\bm{h}_k$ are uniformly distributed in $[-3,3]$, and $\upvarepsilon_k\sim\mathcal{N}(0,1)$ is independent of $\bm{h}_k$. Here, $L(\bm\uptheta)=(1/2)[1+3(\bm\uptheta-\bm\uptheta^\ast)^\top(\bm\uptheta-\bm\uptheta^\ast)]$.}
\label{fig:substitutionoperation}
\end{figure}

A cyclic implementation of (\ref{eq:colorlocalcouncil}) in the manner of Algorithms \ref{beastwasdone} and \ref{kirkey} would involve defining the subvectors, defining the gains sequences $a_k^{(j)}$, determining how the subvector to update in Algorithm \ref{beastwasdone} is selected, and determining how the data $\{(\bm{h}_k,z_k)\}_{k\geq 1}$ are to be generated and processed. In regards to the subvector definition, we assume $p=10$ and use the same partition as in Section \ref{sec:clubsodeashrimp} (here there are 5 subvectors of length 2 each). In regards to the gain sequences, we set $a_k^{(j)}=a/(1+k+A)^{\upalpha}$ for all $j$ where $a=1$, $A=100$, and $\upalpha=1$. The value of $\upalpha$ is a standard choice for the SG algorithms and the values of $a$ and $A$ were {\it{lightly}} tuned. Next, for Algorithm \ref{beastwasdone} each of the 5 subvectors has equal probability of being selected ($q(j)=q$ for $j=1,\dots,5$). The input-output pair $(\bm{x}_k,z_k)$ was generated letting $\bm\uptheta^\ast=[1,\dots,1]^\top$, $\upvarepsilon_k\sim \mathcal{N}(0,1)$, and letting the entries of $\bm{h}_k$ be independent and uniformly distributed in $[-3,3]$. Finally, each input-output pair was used to perform 5 subvector updates. Once 5 updates have been performed using the same input-output pair, a new pair is generated. Using the notation of Section \ref{sec:clubsodeashrimp}, Figure \ref{fig:feedhimabunchofapples} presents the value of $\|\hat{\bm{\uptheta}}_u-\bm\uptheta^\ast\|/\|\hat{\bm{\uptheta}}_0-\bm\uptheta^\ast\|$ for 5 replications of Algorithms \ref{beastwasdone} and \ref{kirkey} initialized at $-\bm\uptheta^\ast$. It can be seen that the iterates of both algorithms appear to converge to $\bm\uptheta^\ast$.

%\subsection{Cyclic Seesaw SPSA on the Rosenbrock Function}


%and  $\|\bar{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}\|/\|\hat{\bm{\uptheta}}_0^{\text{Alg \ref{kirkey}}}\|$ with $\hat{\bm{\uptheta}}_0^{\text{Alg \ref{beastwasdone}}}=\hat{\bm{\uptheta}}_0^{\text{Alg \ref{kirkey}}}=-[1,\dots,1]^\top$, where $\bar{\bm\uptheta}_k^{\text{Alg \ref{beastwasdone}}}$ and $\bar{\bm\uptheta}_k^{\text{Alg \ref{kirkey}}}$ denote the mean values of the algorithm iterates over 1000 replications. 


\begin{figure}[!t]
% Generated with matlab2tikz('width', '.6\textwidth') in MATLAB 
% Changed location in .tex file with at={(0.04\textwidth,0\textwidth)}
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/mycyclicSG-eps-converted-to.pdf}};  
        \node[left= -0.8cm of probe]{$\displaystyle{\frac{\|\hat{\bm{\uptheta}}_u-\bm\uptheta^\ast\|}{\|\hat{\bm{\uptheta}}_0-\bm\uptheta^\ast\|}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
%      \node at (-2.1,-3.4) {$\uptheta_1$};
\end{tikzpicture}
%  \begin{tikzpicture}
%\input{Plots/mycyclicSG.tex}
%\end{tikzpicture}
\caption[Performance of SG-based GCSA implementations of LMS]{Cyclic implementations, in the manner of Algorithms \ref{beastwasdone} (random selection) and \ref{kirkey} (deterministic patterns), of the LMS algorithm in (\ref{eq:colorlocalcouncil}). Pictured are 5 realizations of each algorithm. Here, $\hat{\bm{\uptheta}}_u$ represents either $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{beastwasdone}}}$ (dashed lines) or $\hat{\bm{\uptheta}}_u^{\text{Alg \ref{kirkey}}}$ (solid lines).}
\label{fig:feedhimabunchofapples}
\end{figure}

We now consider the same setting as in Figure \ref{fig:feedhimabunchofapples} with three modifications. First, the gain sequences take the form:
\begin{align*}
a_k^{(j)}=\frac{a^{(j)}}{(1+k+A^{(j)})^{0.501}},
\end{align*}
for $a^{(j)}>0$ and $A^{(j)}\geq 0$. Second, the vector $\bm\uptheta$ is divided into only two subvectors corresponding to the first- and second halves of $\bm\uptheta$ (i.e., $d=2$). Third,  we assume $\upvarepsilon_k\sim\mathcal{N}(0,0.1^2)$. 
%Third, we allow $c\neq 1$ in $c_k^{(j)}$ (this sequence is the same for all $j$).
 We compare the following algorithms:
\begin{DESCRIPTION}
\item[Case 1:] The SG algorithm from (\ref{eq:colorlocalcouncil}) with $a_k=a/(1+k+A)^{0.501}$.
\item[Case 2:] The SG algorithm from (\ref{eq:colorlocalcouncil}) with $a_k$ replaced by a diagonal matrix, $\bm{A}_k$, such that the $i$th diagonal entry of $\bm{A}_k$ is equal to $a_k^{(j)}$ where $i\in \mathcal{S}_j$.\label{pageref:toccasesSG}
\item[Case 3:] Algorithm \ref{beastwasdone} (the subvector to update is selected according to a random variable) with SG-based gradient estimates. Each of the two subvectors is updated with equal probability.

\item[Case 4:] Algorithm \ref{kirkey} (the subvector to update is selected following a strictly alternating pattern) with SG-based gradient estimates.
\end{DESCRIPTION}
%To minimize the number of parameters to tune we set $\upalpha=0.602$.
 Each algorithm was run for a total of $T=5000$ subvector updates and each realization was initialized at a vector uniformly distributed on $[-4,6]^{10}$.  Thus, there were 2,500 iterations in Cases 1 and 2 (since each iteration requires updating both subvectors) and 5,000 iterations in Cases 3 and 4 (since each iteration requires updating only one subvector). The entries of  $\bm{h}_k$ were independent and uniformly distributed in $[-3,3]$. 
% For Case 3, each of the two subvectors was updated with equal probability. 
 Table \ref{table:omgmySECONDtable} presents the results of part of the tuning process for Cases 1--4 and Figure \ref{fig:betterplaybetstts} shows the evolution of the loss function as the number of updates increases. 
%
Table \ref{table:omgmySECONDtable} and Figure \ref{fig:betterplaybetstts} indicate that all algorithms had a comparable performance (for all cases the same gain sequence yielded the smallest mean terminal loss function value). Moreover, the results support the theory on convergence of the GCSA algorithm. 
%Furthermore, the same gain sequence was optimal for all algorithms.
%Table \ref{table:omgmySECONDtable} shows that the terminal loss function value was, on average, equal for all algorithms.


\begin{table}[p]
\centering
\begin{tabular}{SSSSSS} \toprule
    {Algorithm} & {$a^{(1)}$} & {$a^{(2)}$}  & {$A^{(1)}$} & {$A^{(2)}$} & {$\overline{L(\hat{\bm{\uptheta}}_T)}$} \\ \midrule
    {Case 1}  & 1  & {--} & 0  & {--}  & 0.0073    \\
    {SG}  & 1 & {--} & 100 & {--} & 0.0072   \\
    {(regular)}  & 0.1  & {--} & 0  & {--} & 0.0052  \\
    {}  & 0.1  & {--} & 100  & {--} & 0.0052\ $\ast$       \\ \midrule
    {Case 2}  & 1  & 1 & 0  & 0  & 0.0072    \\
    {SG}  & 1 & 1 & 100 & 100 & 0.0071   \\
    {(diagonal gain)}  & 1  & 0.1 & 0  & 0 & 2.6669    \\
    {}  & 1  & 0.1 & 100  & 100 & 0.0060    \\
    {}  & 0.1  & 1 & 0  & 0 & 0.7573    \\
    {}  & 0.1  & 1 & 100  & 100 & 0.0060    \\
   {}  & 0.1  & 0.1 & 0  & 0 & 0.0052    \\
    {}  & 0.1  & 0.1 & 100  & 100 & 0.0052\ $\ast$          \\ \midrule
    {Case 3}  & 1  & 1 & 0  & 0  & 0.0064    \\
    {SG}  & 1 & 1 & 100 & 100 & 0.0063   \\
    {(random selection)}  & 1  & 0.1 & 0  & 0 & 0.0258    \\
    {}  & 1  & 0.1 & 100  & 100 & 0.0056    \\
    {}  & 0.1  & 1 & 0  & 0 & 0.0081    \\
    {}  & 0.1  & 1 & 100  & 100 & 0.0056    \\
   {}  & 0.1  & 0.1 & 0  & 0 & 0.0051   \\
    {}  & 0.1  & 0.1 & 100  & 100 & 0.0051\ $\ast$          \\ \midrule
    {Case 4}  & 1  & 1 & 0  & 0  & {$1.3221\times 10^{8}$}    \\
    {SG}  & 1 & 1 & 100 & 100 & 0.0067   \\
    {(deterministic patterns)}  & 1  & 0.1 & 0  & 0 & {$1.5906\times 10^{17}$}    \\
    {}  & 1  & 0.1 & 100  & 100 & 0.0060    \\
    {}  & 0.1  & 1 & 0  & 0 & 0.0060    \\
    {}  & 0.1  & 1 & 100  & 100 & 0.0060 \\
   {}  & 0.1  & 0.1 & 0  & 0 & 0.0051    \\
    {}  & 0.1  & 0.1 & 100  & 100 & 0.0051\ $\ast$         \\ \bottomrule
\end{tabular}
\caption[Tuning the gain sequence parameters for Cases 1--4 from p. \pageref{pageref:toccasesSG} where the noisy gradient updates are SG-based]{Tuning the gain sequence parameters. Note that for Case 1 there is only one gain sequence, $a_k$, which we have set equal to $a^{(1)}/(1+k+A^{(1)})^{0.501}$. See p. \pageref{pageref:toccasesSG} for a description of each of the four cases above. Here, $\overline{L(\hat{\bm{\uptheta}}_T)}$ represents an estimate of the loss function at the terminal value obtained by averaging the terminal loss values of 100 replications. For comparison, $L(\bm\uptheta^\ast)=0$. An asterisk marks the smallest mean terminal loss function value for each case.}
\label{table:omgmySECONDtable}
\end{table}

% -------------------------------------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------------------------------------------
% A DIFFERENT PLOT BELOW
% -------------------------------------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------------------------------------------

\begin{figure}[p]
\centering
  \begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/cases/SGcases1-eps-converted-to.pdf}};
\node[rotate=90] at (-3.75,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

%\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/cases/SGcases2-eps-converted-to.pdf}};
    \node[rotate=90] at (-3.75,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

\end{tikzpicture}
 \end{subfigure}
 \caption*{Above: the 1st replication.}

% -------------------------------------------------------------------------------------------------------------------------

 \vspace{.03in}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
    \begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/cases/SGcases3-eps-converted-to.pdf}};
\node[rotate=90] at (-3.8,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};

%\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/cases/SGcases4-eps-converted-to.pdf}};
    \node[rotate=90] at (-3.35,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};


\end{tikzpicture}
 \end{subfigure}%
 \caption*{Above: the 2nd replication.}
 
 
 % -------------------------------------------------------------------------------------------------------------------------
 
  \vspace{.03in}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
    \begin{subfigure}[b]{0.5\textwidth}
 \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/cases/SGcases5-eps-converted-to.pdf}};
\node[rotate=90] at (-3.8,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};
%\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/cases/SGcases6-eps-converted-to.pdf}};
    \node[rotate=90] at (-3.5,0) {\small{$L(\hat{\bm{\uptheta}}_u)$}};


\end{tikzpicture}
 \end{subfigure}
  \caption*{Above: the 3rd replication.}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
 \vspace{.03in}
         
% -------------------------------------------------------------------------------------------------------------------------
        
\caption[Performance of Cases 1--4 from p. \pageref{pageref:toccasesSG} where the noisy gradient updates are SG-based]{Performance of Cases 1 (deterministic patterns), 2 (random selection), 3 (regular SG), and 4 (SG with diagonal gains) for three i.i.d. replications (i.e., three i.i.d. realizations of each of the four cases) using the tuned parameters from Table \ref{table:omgmySECONDtable}. The term $\hat{\bm{\uptheta}}_u$ is a generic vector representing the vector obtained after having performed $u$ subvector updates.}
\label{fig:betterplaybetstts}
\end{figure}



\section{Numerical Examples on Normality}
\label{sec:normalitycenumericos}


This section provides a few simple numerical examples regarding the asymptotic normality of the iterates from Algorithm \ref{kirkey} (where the subvector to updates is selected following a deterministic pattern). This algorithm is implemented using SG-based noisy update directions (Section \ref{subsec:normalitySG}) and SPSA-based noisy update directions (Section \ref{sec:hannahashley}).
%More numerical experiments are performed in Section \ref{sec:Numericssimples} and Chapter \ref{chap:multiagent}. 


\subsection{Algorithm \ref{kirkey} with SG-Based Gradient Estimates}
\label{subsec:normalitySG}

Consider the minimization of $L(\bm\uptheta)=E[Q(\bm\uptheta,\bm{V})|\bm\uptheta]$ where $Q(\bm\uptheta,\bm{V})=\uprho(\bm\uptheta)+\bm\uptheta^\top\bm{V}$ for some real-valued function $\uprho(\bm\uptheta)$ and a vector-valued random variable $\bm{V}$ that is independent of $\bm\uptheta$. Then, $L(\bm\uptheta)=\uprho(\bm\uptheta)+\bm\uptheta^\top E[\bm{V}]$. If the mean of $\bm{V}$ is unknown and $\uprho(\bm\uptheta)$ is continuously differentiable, an SG-based approach to solving this problem is obtained by letting $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)= [\partial \uprho(\bm\uptheta)/\partial \bm\uptheta]_{\bm\uptheta=\hat{\bm{\uptheta}}_k} + \bm{V}$. Here, $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$ is an unbiased estimate of the gradient of $L(\bm\uptheta)$ at $\hat{\bm{\uptheta}}_k$. If it is possible to sample from $\bm{V}$ then it is possible to obtain $\hat{\bm{g}}_k(\hat{\bm{\uptheta}}_k)$ and update $\hat{\bm{\uptheta}}_k$ using SG:
\begin{align}
\label{eq:firfoes}
\hat{\bm{\uptheta}}_{k+1}=\hat{\bm{\uptheta}}_k-a_k\left(\left[\frac{\partial \uprho(\bm\uptheta)}{\partial \bm\uptheta}\right]_{\bm\uptheta=\hat{\bm{\uptheta}}_k}+\bm{V}_k\right),
\end{align}
where $\bm{V}_k$ denotes a measurement of $\bm{V}$. A strictly cyclic implementation of (\ref{eq:firfoes}) (i.e, an implementation resembling the cyclic seesaw SG algorithm except with $d$ subvectors) with non-overlapping subvectors is as follows: 
 \begin{align}
 \label{eq:tinkertonpinks}
\hat{\bm{\uptheta}}_{k}^{(I_j)}=\hat{\bm{\uptheta}}_k^{(I_{j-1})}-a_k^{(j)}\left(\left[\frac{\partial \uprho(\bm\uptheta)}{\partial \bm\uptheta}\right]_{\bm\uptheta=\hat{\bm{\uptheta}}_k^{(I_{j-1})}}+\bm{V}_k^{(I_{j-1})}\right)^{(j)}
\end{align}
for $1\leq j\leq d$, where $\hat{\bm{\uptheta}}_k^{(I_0)}\equiv \hat{\bm{\uptheta}}_k^{\text{cyc}}$, $\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}\equiv\hat{\bm{\uptheta}}_k^{(I_d)}$, and $\bm{V}_k^{(I_j)}$ is a vector-valued random variable representing a measurement of $\bm{V}$. Here, Theorem \ref{thm:fnogg} could be used to derive conditions for the asymptotic normality of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\uptheta^\ast)$ where $\upbeta>0$ is some constant and $\bm\uptheta^\ast$ is a minimizer of $L(\bm\uptheta)$. We do this next.

Let us discuss conditions under which C0--C8, the conditions of Theorem \ref{thm:fnogg}, are satisfied. First note that if $\uprho(\bm\uptheta)$ is twice continuously differentiable with a bounded Jacobian matrix $\bm{J}(\bm\uptheta)$ and if $\hat{\bm{\uptheta}}_k^{(I_j)}\rightarrow \bm\uptheta^\ast$ w.p.1 for all $j$ then condition C0 is satisfied. Next, if $a_k^{(j)}=a_k=a/(1+k+A)^\upalpha$ for some $a, A >0, \upalpha>0$ then C1 is also satisfied with $r_j=a$. Moreover, since we are assuming the $d$ subvectors do not overlap when the matrix $\bm\Gamma$ in (\ref{eq:macnealhuh}) is equal to $a \bm{J}(\bm\uptheta^\ast)$. Therefore, if $\bm{J}(\bm\uptheta^\ast)$ is positive definite then condition C2 would also be satisfied with $a\bm{J}(\bm\uptheta^\ast)=\bm{P\Lambda P}^\top$ where $\bm{P}\in\mathbb{R}$ is an orthogonal matrix and $\bm\Lambda$ is a positive definite diagonal matrix. Next, letting $\mathcal{F}_k$ be the $\upsigma$-field generated by $\{\hat{\bm{\uptheta}}_i^{\text{cyc}}\}_{i=1}^{k}$, the bias term in condition C3 is identically zero (i.e., equal to the zero vector). Therefore, C3 is automatically satisfied. Finally, if the variables $\bm{V}_k^{(I_j)}$ for $j=1,\dots,d$ and $k\geq 0$ are i.i.d. and have (finite) positive definite covariance matrix, then conditions C4, C5-(i), C5-(iii), C6, and C7-(i) hold with $\bm\Sigma=a^2\sum_{j=1}^d \Var{([\bm{V}_k^{(I_j)}]^{(j)})}$, a positive definite block-diagonal matrix. Finally, if $0<\upalpha\leq 1$ (note that $\upbeta=\upalpha$ by C5-(i)), then a {\it{sufficient}} condition for B6 to be satisfied is if  the smallest diagonal entry of $\bm\Lambda$ is strictly greater than $1/2$ (if $\upalpha<1$ then this condition may be relaxed to having the smallest diagonal entry of $\bm\Lambda$ be strictly positive).

The discussion above gave conditions for the asymptotic normality of the vector $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\uptheta^\ast)$ with $\upbeta=\upalpha$. One important condition was the convergence w.p.1 of $\hat{\bm{\uptheta}}_k^{(I_j)}$ to $\bm\uptheta^\ast$. Corollary \ref{thm:hoeshooHarry} could be used to show convergence of $\hat{\bm{\uptheta}}_k^{\text{cyc}}$ to $\bm\uptheta^\ast$. Then, Corollary \ref{eq:idamagedittarantatan} would imply the desired result. Conditions A0$''$, A3$''$, A5$''$,  and A6$''$, are automatically satisfied given the assumptions of the previous paragraph. It remains to discuss the validity of A4$''$, A7$''$, and A8$''$. Condition A4$''$ requires the algorithm's iterates to be bounded w.p.1. Verifying this in practice is impossible (see Section \ref{sec:discussconvergence}). 
%and in our numerical experiments we will not impose any bounds on the iterates. 
Next, A7$''$ requires $\bm{\uptheta^{\ast}}$ to be a locally asymptotically stable (in the sense of Lyapunov) solution of:
% $\dot{\bm{Z}}(t)=- a\bm{g}(\bm{Z}(t))$, where $\bm{g}(\bm\uptheta)$ denotes the gradient of $L(\bm\uptheta)$.
\begin{align}
\label{eq:chirrinpinpin4}
\dot{\bm{Z}}(t)=- a \left(\left[\frac{\partial \uprho(\bm\uptheta)}{\partial \bm\uptheta}\right]_{\bm\uptheta=\bm{Z}(t)}+E[\bm{V}]\right).
\end{align}
One example of a situation in which $\bm\uptheta^\ast$ is a locally asymptotically stable solution to (\ref{eq:chirrinpinpin4}) is when $\uprho(\bm\uptheta)=[\bm\uptheta^\top\bm{H}\bm\uptheta]/2$ for some positive definite matrix $\bm{H}$. Throughout the remainder of this section we will assume $\uprho(\bm\uptheta)$ has this form. In this case, $\dot{\bm{Z}}(t)=- a\bm{H}(\bm\uptheta+\bm{H}^{-1}E[\bm{V}])$. Because $\bm\uptheta^\ast=-\bm{H}^{-1}E[\bm{V}]$, $\bm\uptheta^\ast$ is an equilibrium point of $\dot{\bm{Z}}(t)$.
%=- a\bm{H}(\bm\uptheta+\bm{H}^{-1}E[\bm{V}])$. 
The desired Lyapunov stability follows from Lyapunov's second method for stability (e.g., Cronin 2007\nocite{cronin2007}), and therefore A7$''$ holds. Condition A8$''$ is also impossible to verify in practice. It requires the iterates to be contained within the domain of attraction of (\ref{eq:chirrinpinpin4}) infinitely often w.p.1. Next we conduct a small numerical experiment to illustrate convergence and asymptotic normality under the assumptions made thus far. Aside from A4$''$ and A8$''$, all the conditions for convergence w.p.1 and asymptotic normality are satisfied. 



For our numerical experiments we implement (\ref{eq:tinkertonpinks}) assuming $p=2$ (i.e., $\bm\uptheta\in\mathbb{R}^2$) and that the vectors $\bm{V}_k^{(I_j)}$ are i.i.d. with $\bm{V}_k^{(I_j)}\sim\mathcal{N}(\bm\upmu,\bm{I})$, where $\bm{\upmu}=[5, 5]^\top$. In this setting there are two subvectors to update corresponding to the first- and second entries of $\bm\uptheta$. The matrix $\bm{H}$ was set to be equal to the identity matrix. For the gain sequences the values used were $\upalpha=0.501$, $a=1$, and $A=100$.  Under these assumptions, $\bm\uptheta^\ast=-[5,5]^\top$ and $k^{0.501/2}(\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\uptheta^\ast)$ should converge in distribution to a random variable with distribution $\mathcal{N}(\bm{0},0.5\bm{I})$. Figure \ref{fig:figgyanotherorbs} gives the results for $\hat{\bm{\uptheta}}_0^{\text{cyc}}=[1,1]^\top$. The results in Figure \ref{fig:lilly1} appear to support the fact that the values of $T^{0.501/2}(\hat{\bm{\uptheta}}_T^{\text{cyc}}-\bm\uptheta^\ast)$ are expected to have a multivariate normal distribution with a diagonal covariance matrix (this can be seen since the cluster of points in Figure \ref{fig:lilly1} is roughly symmetric) for $T=1000$. Additionally, because the sum of the entries of a random variable with distribution $\mathcal{N}(\bm{0},0.5\bm{I})$ should have a normal distribution with mean zero and variance 1, a Q-Q plot could be used to compare the quantiles of a standard normal random variable to the quantiles of the sum of the entries of $T^{0.501/2}(\hat{\bm{\uptheta}}_T^{\text{cyc}}-\bm\uptheta^\ast)$. Figure \ref{fig:lilly2} shows the resulting Q-Q plot. It appears that the sum of the entries of the normalized iterates closely approximates a standard normal random variable as desired. 




\begin{figure}
\centering
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/scatterSG-eps-converted-to.pdf}};
\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
                \caption{Scatter plot of $T^{\upbeta/2}(\hat{\bm{\uptheta}}_{T}^{\text{cyc}}-\bm\uptheta^\ast)$.}
                \label{fig:lilly1}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/normalitySG-eps-converted-to.pdf}};

\end{tikzpicture}
                \caption{Q-Q plot of $[T^{\upbeta/2}(\hat{\bm{\uptheta}}_{T}^{\text{cyc}}-\bm\uptheta^\ast)]^\top\bm{1}$.}
                \label{fig:lilly2}
        \end{subfigure}\hfill
        \caption[Scatter- and Q-Q plots supporting the asymptotic normality of the normalized cyclic seesaw SG iterates]{In the plots above the term ``$\bm{1}$'' denotes the vector of ones, $\upbeta=0.501$, and $T=1000$. The plots are the result of 2,000 i.i.d. replications.}
        \label{fig:figgyanotherorbs}
\end{figure}



\subsection{Algorithm \ref{kirkey} with SPSA-Based Gradient Estimates}
\label{sec:hannahashley}

This section considers the same problem from Section \ref{subsec:normalitySG}, that is the minimization of $L(\bm\uptheta)=\bm\uptheta^\top\bm{H}\bm\uptheta/2+\bm\uptheta^\top E[\bm{V}]$. However, rather than using noisy gradient measurements of the form  used in (\ref{eq:tinkertonpinks}), this section relies only on noisy measurements, $Q(\bm\uptheta,\bm{V})=\bm\uptheta^\top\bm{H}\bm\uptheta/2+\bm\uptheta^\top\bm{V}$, in the optimization process. This is done using the cyclic seesaw SPSA algorithm from Section \ref{sect:cspsa}. Specifically, an iteration of the algorithm is given by:
\begin{subequations}
\begin{align}
\label{eq;tratarakatnatantan0}
\hat{\bm{\uptheta}}_{k}^{(I)}&=\hat{\bm{\uptheta}}_k^\text{cyc}-a_k^{(1)}\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^\text{cyc}),\\
 \hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}&=\hat{\bm{\uptheta}}_k^{(I)}-a_k^{(2)}\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)}),\label{eq;tratarakatnatantan}
\end{align}
\end{subequations}
where $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^\text{cyc})$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})$ are as  in (\ref{eq:howeardspos1}) and (\ref{eq:howeardspos2}), respectively. In order to implement the cyclic seesaw SPSA algorithm in (\ref{eq;tratarakatnatantan0},b) it is necessary to specify the values of $a_k^{(j)}$, $c_k^{(j)}$, $\bm\Delta_k$, and $\bm\Delta_k^{(I)}$ (see p. \pageref{eq:howeardspos2} for the definition of the last three terms). In this section's numerical experiment the non-zero entries of $\bm\Delta_k$ and $\bm\Delta_k^{(I)}$ were set to be i.i.d. random variables taking the values $\pm 1$ with equal probability. We also set $a_k^{(j)}=1/(1+k+A)^\upalpha$ and $c_k^{(j)}=1/(1+k)^\upgamma$ for all $j$, where $\upalpha=0.602$, $\upgamma=0.101$, and $A=500$. All measurements of the random variable $\bm{V}$ are assumed to be i.i.d. with distribution $\mathcal{N}(\bm\upmu,0.1\bm{I})$ where $\bm\upmu$ is the vector of fives. Next, we show convergence w.p.1 of $\hat{\bm{\uptheta}}_k^{\text{cyc}}$ to $\bm\uptheta^\ast$ (the minimizer of $L(\bm\uptheta)$) and we derive the asymptotic distribution of $k^{\upbeta/2}(\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\uptheta^\ast)$ for $\upbeta=\upalpha-2\upgamma$.

To prove convergence of $\hat{\bm{\uptheta}}_k^{\text{cyc}}$ to $\bm\uptheta^\ast$, we verify that the conditions of Corollary \ref{thm:hoeshooHarry} hold. The convergence of $\hat{\bm{\uptheta}}_k^{(I)}$ to $\bm\uptheta^\ast$ follows from Corollary \ref{eq:idamagedittarantatan}. First, it is easy to see that condition A0$''$ holds with $r_j=1$ for all $j$. Similarly, it is easy to see that condition A3$''$ is satisfied. Condition A4$''$ is impossible to guarantee in practice and, in our numerical experiment, we do not impose any bounds forcing A4$''$ to hold. In order to verify A5$''$ and A6$''$ we must express the noisy gradient vectors $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^\text{cyc})$ and $\hat{\bm{g}}^{\text{SP}}_k(\hat{\bm{\uptheta}}_k^{(I)})$ in terms of their bias- and noise terms given in (\ref{eq:savemebias0},b) and (\ref{eq:savemenoise0},b), respectively. 
%Because $L(\bm\uptheta)$ has such a simple form, computing the bias- and noise terms is fairly simple. 
In our example ${\bm{\upbeta}}^{(1)}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})={\bm{\upbeta}}^{(1)}_k(\hat{\bm{\uptheta}}_k^{(I)})=\bm{0}$ (due to the fact that the loss function is quadratic in $\bm\uptheta$) and 
%noise terms must be equal to the distance between the estimated gradient and the true gradient. Specifically, 
the $m$th entry of the noise term ${\bm{\upxi}}^{(1)}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})$ is equal to:
%. We do this next. Let $\mathcal{F}_k$ be the $\upsigma$-field generated by $\{\hat{\bm{\uptheta}}_0^{\text{cyc}}\}$
\begin{align*}
\left[{\bm{\upxi}}^{(1)}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})\right]^{[m]}&=\frac{\bm\Delta_k^\top(\bm{V}_k^++\bm{V}_k^-)}{2\Delta_k^{[m]}}+\frac{\bm\Delta_k^\top\bm{H}\hat{\bm{\uptheta}}_k^{\text{cyc}}}{\Delta_k^{[m]}}+\frac{(\hat{\bm{\uptheta}}_k^{\text{cyc}})^\top(\bm{V}_k^+-\bm{V}_k^-)}{2c_k\Delta_k^{[m]}}-\left[\bm{g}(\hat{\bm{\uptheta}}_k^{\text{cyc}})\right]^{[m]}
%\frac{\left(\bm{H}\hat{\bm{\uptheta}}_k+E[\bm{V}]\right)^\top\bm\Delta_k}{\Delta_k^{[m]}}-(\bm{H}\hat{\bm{\uptheta}}_k+E[\bm{V}])^{[m]}+\frac{\bm{V}_k^+-\bm{V}_k^-}{2c_k\Delta_k^{[m]}}
\end{align*}
for $m\in \mathcal{S}_1$ (see p. \pageref{eq:notexclusive} for the definition of $\mathcal{S}_j$) and $[{\bm{\upxi}}^{(1)}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})]^{[m]}=0$ otherwise. Similarly, the $m$th entry of the noise term ${\bm{\upxi}}^{(2)}_k(\hat{\bm{\uptheta}}_k^{\text{cyc}})$ is equal to:
\begin{align*}
&\left[{\bm{\upxi}}^{(2)}_k(\hat{\bm{\uptheta}}_k^{(I)})\right]^{[m]}=\notag\\
&\frac{(\bm\Delta_k^{(I)})^\top(\bm{V}_k^{(I)+}+\bm{V}_k^{(I)-})}{2(\bm\Delta_k^{(I)})^{[m]}}+\frac{(\bm\Delta_k^{(I)})^\top\bm{H}\hat{\bm{\uptheta}}_k^{(I)}}{(\bm\Delta_k^{(I)})^{[m]}}+\frac{(\hat{\bm{\uptheta}}_k^{(I)})^\top(\bm{V}_k^{(I)+}-\bm{V}_k^{(I)-})}{2c_k(\bm\Delta_k^{(I)})^{[m]}}-\left[\bm{g}(\hat{\bm{\uptheta}}_k^{(I)})\right]^{[m]}
%\frac{\left(\bm{H}\hat{\bm{\uptheta}}_k^{(I)}+E[\bm{V}]\right)^\top\bm\Delta_k^{(I)}}{(\bm\Delta_k^{(I)})^{[m]}}-(\bm{H}\hat{\bm{\uptheta}}_k^{(I)}+E[\bm{V}])^{[m]}+\frac{\bm{V}_k^{(I)+}-\bm{V}_k^{(I)-}}{2c_k(\bm\Delta_k^{(I)})^{[m]}}
\end{align*}
for $m\in \mathcal{S}_2$ and $[{\bm{\upxi}}^{(2)}_k(\hat{\bm{\uptheta}}_k^{(I)})]^{[m]}=0$ otherwise.
Given that the bias terms are identically zero, condition A5$''$ is satisfied. Using the independence of the $\bm\Delta$ and $\bm{V}$ and the fact that both these variables have finite variance, condition A6$''$ follows from the discussion on p. \pageref{eq:ranch} (using the fact that $\sum_{k=1}^\infty a_k^2/c_k^2<\infty$). The validity of condition A7$''$ has already been shown in Section \ref{subsec:normalitySG}. Finally, condition A8$''$, like  condition A4$''$, is impossible to verify. Aside from conditions A4$''$ and A8$''$, all the conditions for convergence w.p.1 hold. Next, we verify the conditions for the asymptotic normality of $k^{(\upalpha-2\upgamma)/2}(\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\uptheta^\ast)$ and compute the parameters of the asymptotic distribution.

To prove the desired result on asymptotic normality we show that the conditions of Theorem \ref{thm:fnogg} are satisfied. For simplicity, we will assume $\bm\uptheta\in \mathbb{R}^2$. The validity of C0--C3 has already been shown (see Section \ref{subsec:normalitySG} and the previous paragraph). Condition C4 follows immediately by construction. Let us now show that condition C5-(iv) holds.
%does not hold for this problem. However, we will show that the conditional covariance of the noise terms multiplied by $k^{\upbeta-\upalpha}$ converges to zero w.p.1. From the discussion on p. \pageref{pageref:melclts} this weaker condition can be used instead of C4. 
First, because both noise terms have mean zero (conditionally on $\mathcal{F}_k$, where $\mathcal{F}_k$ was defined in Section \ref{subsec:normalitySG}), the conditional covariance matrix of ${\bm{\upxi}}^{(1)}_k(\hat{\bm{\uptheta}}_k)$ and ${\bm{\upxi}}^{(2)}_k(\hat{\bm{\uptheta}}_k^{(I)})$ is $E[\bm\upxi_k^{(1)}(\hat{\bm{\uptheta}}_k)\bm\upxi_k^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})^\top|\mathcal{F}_k]$. Using the convergence (w.p.1) of the iterates to $\hat{\bm{\uptheta}}_k^\ast$ along with the continuity of the gradient of $L(\bm\uptheta)$  it is easy to show that $E[\bm\upxi_k^{(1)}(\hat{\bm{\uptheta}}_k)\bm\upxi_k^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})^\top|\mathcal{F}_k]=O(1/c_k)$ w.p.1. However, $c_k=O(1/k^{\upgamma})$ which implies $\lim_{k\rightarrow \infty}k^{\upbeta-\upalpha}/c_k= 0$. Therefore, $k^{\upbeta-\upalpha}E[\bm\upxi_k^{(1)}(\hat{\bm{\uptheta}}_k)\bm\upxi_k^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})^\top|\mathcal{F}_k]\rightarrow \bm{0}$ w.p.1. Next we verify the remaining conditins for asymptotic normality.


\begin{figure}
\centering
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0) 
{\includegraphics[scale=0.35]{Plots/scatterSPSA-eps-converted-to.pdf}};
\node at (0,-2.6) {\textcolor{white}{$\uptheta_1$}};

\end{tikzpicture}
                \caption{Scatter plot of $T^{\upbeta/2}(\hat{\bm{\uptheta}}_{T}^{\text{cyc}}-\bm\uptheta^\ast)$.}
                \label{fig:lorberton1}
        \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
\begin{tikzpicture}

  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.35]{Plots/normalitySPSA-eps-converted-to.pdf}};

\end{tikzpicture}
                \caption{Q-Q plot of $(8/10)^{1/2}[T^{\upbeta/2}(\hat{\bm{\uptheta}}_{T}^{\text{cyc}}-\bm\uptheta^\ast)]^\top\bm{1}$.}
                \label{fig:lorberton2}
        \end{subfigure}\hfill
        \caption[Scatter- and Q-Q plots supporting the asymptotic normality of the normalized cyclic seesaw SPSA iterates]{In the plots above the term ``$\bm{1}$'' denotes the vector of ones, $\upbeta=\upalpha-2\upgamma=0.4$, and $T=3000$. The plots are the result of 3,000 i.i.d. replications.}
        \label{fig:flyingorber}
\end{figure}


%follows from the independence of the measurements of $\bm{V}$ and the definition of $\bm\Delta_k$ and $\bm\Delta_k^{(I)}$. 

After a direct calculation of the conditional covariance matrices of the two noise terms it follows that C5-(ii) and C6 hold with $\bm\Sigma=(0.1/4)(\bm\uptheta^\ast)^\top\bm\uptheta^\ast\bm{I}$. Condition C7--(ii) follows form the uniform integrability of the weighted (by $k^{\upbeta-\upalpha}$) noise terms.
  Condition C8 follows from the fact that $\bm{H}$ is positive definite. If we assume $\bm{H}=\bm{I}$ for simplicity, the asymptotic distribution of $k^{(\upalpha-2\upgamma)/2}(\hat{\bm{\uptheta}}_k^{\text{cyc}}-\bm\uptheta^\ast)$ according to Theorem \ref{thm:fnogg} is then $\mathcal{N}(\bm{0},(5/8)\bm{I})$. Furthermore, $(8/10)^{1/2}[T^{\upbeta/2}(\hat{\bm{\uptheta}}_{T}^{\text{cyc}}-\bm\uptheta^\ast)]^\top\bm{1}\sim \mathcal{N}(0,1)$. Figure \ref{fig:flyingorber} gives the results for $\hat{\bm{\uptheta}}_0^{\text{cyc}}=[1,1]^\top$. The results in Figure \ref{fig:lorberton1} appears to support the fact that the values of $T^{(\upalpha-2\upgamma)/2}(\hat{\bm{\uptheta}}_T^{\text{cyc}}-\bm\uptheta^\ast)$ are expected to have a multivariate normal distribution with a diagonal covariance matrix (this can be seen since the cluster of points in Figure \ref{fig:lorberton1} is roughly symmetric) for $T=3000$. Moreover, Figure \ref{fig:lorberton2} shows that $(8/10)^{1/2}[T^{\upbeta/2}(\hat{\bm{\uptheta}}_{T}^{\text{cyc}}-\bm\uptheta^\ast)]^\top\bm{1}$ appears to have a standard normal distribution as desired.




  
  
  \section{Numerical Analysis on Efficiency}
\label{sec:Numericssimples}

This section contains simulation-based estimates of  the relative efficiency ratio (\ref{eq:wobble}) for comparing the SG- and cyclic seesaw SG algorithms when $c^{\text{cyc}}$ and $c^{\text{non}}$ are defined as in Section \ref{sec:costoport} (this is done in Section \ref{eq:Indyiedie1}) and for comparing the SPSA- and cyclic seesaw SPSA algorithms under a few different definitions of $c^{\text{cyc}}$ and $c^{\text{non}}$ (this is done in Section \ref{eq:Indyiedie12}).
%\begin{enumerate}
%\item Comparing 
%\item  Comparing the SPSA- to the cyclic seesaw SPSA algorithm (see Section \ref{eq:Indyiedie12}).
%\end{enumerate}
%%Note that the relative efficiency depends on the definition of $c^{\text{cyc}}$ and $c^{\text{non}}$ (the per-iteration costs of the cyclic- and non-cyclic algorithms).
% This second considers a few different definitions of $c^{\text{cyc}}$ and $c^{\text{non}}$.

\subsection{Efficiency: SG versus Cyclic Seesaw SG}
\label{eq:Indyiedie1}

This section compares the SG algorithm to the cyclic seesaw SG algorithm by estimating the relative efficiency given by the ratio in (\ref{eq:wobble}). The SG algorithm treated is a distributed version of the LMS algorithm in (\ref{eq:colorlocalcouncil}) where measurements of the pair $(\bm{h}_k,z_k)$ with $z_k=\bm{h}_k^\top \bm\uptheta^\ast+\upvarepsilon_k$ are used to estimate $\bm\uptheta^\ast$. The non-cyclic implementation of LMS considered is the following:
\begin{subequations}
\begin{align}
[\hat{\bm{\uptheta}}_{k+1}^{\text{non}}]^{(1)}=[\hat{\bm{\uptheta}}_k^{\text{non}}]^{(1)}-a_k^{(1)}\left[(\bm{h}_{k+1}^\top \hat{\bm{\uptheta}}_k^{\text{non}}-z_{k+1})\bm{h}_{k+1}\right]^{(1)},\label{eq:fafafafafafufahfah0}\\
[\hat{\bm{\uptheta}}_{k+1}^{\text{non}}]^{(2)}=[\hat{\bm{\uptheta}}_k^{\text{non}}]^{(2)}-a_k^{(2)}\left[(\bm{h}_{k+1}^\top \hat{\bm{\uptheta}}_k^{\text{non}}-z_{k+1})\bm{h}_{k+1}\right]^{(2)}, \label{eq:fafafafafafufahfah}
\end{align}
\end{subequations}
where $\bm\uptheta\in \mathbb{R}^p$ for $p=12$ even and $p'=p/2=6$ is the subvector length. In the distributed implementation considered here, (\ref{eq:fafafafafafufahfah0}) and (\ref{eq:fafafafafafufahfah}) are computed at physically different locations. To highlight the distributed nature of the implementation, throughout the remainder of this section we use the multi-agent analogy from Section \ref{sec:costoport} (see p. \pageref{eq:herculedherculess}). In other words, we assume that each of the two lines in (\ref{eq:fafafafafafufahfah0},b) is computed by a different agent.


The cyclic seesaw counterpart to (\ref{eq:fafafafafafufahfah0},b), which is also assumed to be implemented in a distributed manner, is defined as follows:
\begin{subequations}
\begin{align}
\hat{\bm{\uptheta}}_k^{(I)}&=\hat{\bm{\uptheta}}_k^{\text{cyc}}-a_k^{(1)}\left[(\bm{h}_{k+1}^\top \hat{\bm{\uptheta}}_k^{\text{cyc}}-z_{k+1})\bm{h}_{k+1}\right]^{(1)},\label{eq:addalabeltomee0}\\
\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}&=\hat{\bm{\uptheta}}_k^{(I)}-a_k^{(2)}\left[(\bm{h}_{k+1}^\top \hat{\bm{\uptheta}}_k^{(I)}-z_{k+1})\bm{h}_{k+1}\right]^{(2)}.
\label{eq:addalabeltomee}
\end{align}
\end{subequations}
Once again, we use the multi-agent analogy from Section \ref{sec:costoport} (see p. \pageref{eq:herculedherculess}) to highlight the fact that the cyclic seesaw algorithms is assumed to be implemented in a distributed manner. Note that 
%the input-output pair 
$(\bm{h}_{k+1},z_{k+1})$ is used to perform two subvector updates 
%
in  (\ref{eq:addalabeltomee0},b): once to obtain $\hat{\bm{\uptheta}}_k^{(I)}$ and once to obtain $\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}$. The pair $(\bm{h}_{k+1},z_{k+1})$ is also used to perform two subvector updates in 
% one update to obtain $\hat{\bm{\uptheta}}_k^{(I)}$ and one update to obtain $\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}$. The pair $(\bm{h}_{k+1},z_{k+1})$ is also used to perform two subvector updates in 
 (\ref{eq:fafafafafafufahfah0},b). 
%Of course there are many more ways in which the input-otput data could be used.


\subsubsection{Cost as a Measure of Arithmetic Computations}
\label{sec:SGarithmetic}

The first definition of cost we consider for comparing (\ref{eq:fafafafafafufahfah0},b) to  (\ref{eq:addalabeltomee0},b) via  (\ref{eq:ratio}) is the arithmetic cost of Section \ref{sec:costoport}. Here, the per-iteration costs $c^{\text{non}}$ and $c^{\text{cyc}}$ denote the number of basic arithmetic operations required to obtain $\hat{\bm{\uptheta}}_{k+1}^\text{non}$ from $\hat{\bm{\uptheta}}_{k}^\text{non}$ and to obtain $\hat{\bm{\uptheta}}_{k+1}^\text{cyc}$ from $\hat{\bm{\uptheta}}_{k}^\text{cyc}$, respectively. In order to compute these quantities it is necessary to specify the computational graphs (CGs) associated with the algorithms, these are given in Figures \ref{fig:figgystuff1} and \ref{fig:figgystuff2}. From Figure \ref{fig:figgystuff1} we see that the per-iteration cost associated with the SG algorithm is $c^{\text{non}}=4p+3$ operations ($3p+1$ operations from the first graph and $p+2$ from the second). In contrast, Figure \ref{fig:figgystuff2} implies $c^{\text{cyc}}=5p+3$ operations ($3p+1$ operations from the first graph and $2p+2$ from the second).

In our numerical examples we use $p=12$ so that $c^\text{non}=51$, $c^\text{cyc}=63$, and $c^\text{cyc}/c^\text{non}=21/17\approx 5/4$. The significance of this ratio, as was explained in the discussion following Proposition \ref{prop:omygodsthunder}, is that the cost of computing $\hat{\bm{\uptheta}}_{4i}^{\text{cyc}}$ is approximately equal to the cost of computing $\hat{\bm{\uptheta}}_{5i}^{\text{non}}$ for any strictly-positive integer $i$. Therefore, for every four iterations of the cyclic seesaw SG algorithm in (\ref{eq:addalabeltomee0},b) we may run five iterations of the SG algorithm in (\ref{eq:fafafafafafufahfah0},b) at the same computational cost. Consequently, $k_1=4i$ and $k_2=5i$ are valid values for $k_1$ and $k_2$ in (\ref{eq:ratio}) for any strictly-positive integer $i$. Figure \ref{eq:GOTITPEEPOPAH} estimates the relative efficiency ratio in (\ref{eq:ratio}) with $k_1=4i$ and $k_2=5i$. The estimates were obtained by using $\bm\uptheta^\ast=[1,\dots,1]^\top$, letting the entries of $\bm{h}_k$ be independent and uniformly distributed in $[-3,3]$, $\upepsilon_k\sim \mathcal{N}(0,0.5^2)$, and setting $a_k=a_k^{(j)}=0.1/(1+k+100)$.  The expectations in (\ref{eq:ratio}) were estimated using the average of 100 i.i.d. replications. For each replication, both algorithms were initialized at $-\bm\uptheta^\ast$.
%Using the same gain sequence for both the cyclic- and non-cyclic implementations helps isolate the effects of a cyclic implementation on relative efficiency.
%Both 
%%the cyclic and non-cyclic 
%algorithms were initialized at $-\bm\uptheta^\ast$.  

Figure \ref{eq:GOTITPEEPOPAH} shows that the cyclic implementation was asymptotically less efficient (by approximately 15\%).
% when cost is defined as the number of basic operations required 
% (assuming computations are performed using the CG's in Figures \ref{fig:figgystuff1} and \ref{fig:figgystuff2}). 
 While the cyclic algorithm was more efficient for small values of $i$ (small values of $i$ correspond to earlier iterations of the algorithms), the relative efficiency for small $i$ was found to be highly sensitive to the initialization of the algorithms while the asymptotic relative efficiency
% , on the other hand, 
 appeared to be more robust to
%  the 
  initialization; 
%  of the algorithms. 
this pattern was observed based on 10 other initializations of the algorithms.

 
\begin{figure}[p]
\centering
  \begin{subfigure}[b]{1\textwidth}
 \centering
\begin{tikzpicture}

\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (x) at (0,0) {$\hat{\bm{\uptheta}}_k^\text{non}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (y) at (0,-1.5) {$\bm{h}_{k+1}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (z) at (6.55,1.05) {$z_k$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (a) at (11.4,1.05) {$a_k^{(1)}$};
\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=90pt, ultra thick] (newinput) at (2.6,1.05) {$(\hat{\bm{\uptheta}}_k^\text{non})^\top\bm{h}_{k+1}$};
\node [above of=newinput] {Share this Value};


\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=74pt, thick] (xy) at (2.6,-0.75) {$(\hat{\bm{\uptheta}}_k^\text{non})^\top\bm{h}_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=110pt, thick] (xyz) at (6.55,-0.75) {$(\hat{\bm{\uptheta}}_k^\text{non})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=128pt, thick] (xyza) at (11.4,-0.75) {$a_k^{(1)}(\hat{\bm{\uptheta}}_k^\text{non})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.8em, minimum width=168pt, thick] (xyzah) at (11.4,-2.55) {$a_k^{(1)}\left[(\hat{\bm{\uptheta}}_k^\text{non})^\top\bm{h}_{k+1}-z_{k+1}\right]\bm{h}_{k+1}^{(1)}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=55pt, ultra thick] (final) at (11.4,-4.35) {$[\hat{\bm{\uptheta}}_{k+1}^\text{non}]^{(1)}$};

\draw[->, thick] (x)--(xy) ;
\draw[->, thick] (xy)--(newinput) ;
\draw[->,thick] (y)--(xy);
\draw[->,thick] (z)--(xyz);
\draw[->,thick] (xy)--(xyz);
\draw[->,thick] (a)--(xyza);
\draw[->,thick] (xyz)--(xyza);
\draw[->,thick] (xyza)--(xyzah);
\draw[->,thick] (y)--(0,-2.55)--(xyzah);
\draw[->,thick] (xyzah)--(final);
\draw[->,thick] (x)--(-.8,0)--(-.8,-4.35)--(final);

\end{tikzpicture}
 \end{subfigure}
 \caption*{The CG for computing (\ref{eq:fafafafafafufahfah0}).}


% -------------------------------------------------------------------------------------------------------------------------

 \vspace{.5in}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
    \begin{subfigure}[b]{1\textwidth}
 \centering
\begin{tikzpicture}

\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (x) at (0,0) {$\hat{\bm{\uptheta}}_k^{\text{non}}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (y) at (0,-1.5) {$\bm{h}_{k+1}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (z) at (6.55,1.05) {$z_k$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (a) at (11.4,1.05) {$a_k^{(2)}$};
\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=90pt, thick] (newinput) at (2.6,1.05) {$(\hat{\bm{\uptheta}}_k^\text{non})^\top\bm{h}_{k+1}$};
\node [above of=newinput] {Borrow this Value};


\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=74pt, thick] (xy) at (2.6,-0.75) {$(\hat{\bm{\uptheta}}_k^{\text{non}})^\top\bm{h}_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=110pt, thick] (xyz) at (6.55,-0.75) {$(\hat{\bm{\uptheta}}_k^{\text{non}})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=128pt, thick] (xyza) at (11.4,-0.75) {$a_k^{(2)}(\hat{\bm{\uptheta}}_k^{\text{non}})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.8em, minimum width=168pt, thick] (xyzah) at (11.4,-2.55) {$a_k^{(2)}\left[(\hat{\bm{\uptheta}}_k^{\text{non}})^\top\bm{h}_{k+1}-z_{k+1}\right]\bm{h}_{k+1}^{(2)}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=55pt, ultra thick] (final) at (11.4,-4.35) {$[\hat{\bm{\uptheta}}_{k+1}^\text{non}]^{(2)}$};

\draw[->, thick] (x)--(xy) ;
\draw[->, thick] (newinput)--(xy) ;
\draw[->,thick] (y)--(xy);
\draw[->,thick] (z)--(xyz);
\draw[->,thick] (xy)--(xyz);
\draw[->,thick] (a)--(xyza);
\draw[->,thick] (xyz)--(xyza);
\draw[->,thick] (xyza)--(xyzah);
\draw[->,thick] (y)--(0,-2.55)--(xyzah);
\draw[->,thick] (xyzah)--(final);
\draw[->,thick] (x)--(-.8,0)--(-.8,-4.35)--(final);

\end{tikzpicture}
 \end{subfigure}%
 \caption*{The CG for computing (\ref{eq:fafafafafafufahfah}).}
 
 
 % -------------------------------------------------------------------------------------------------------------------------
 
  \vspace{.03in}
 
 % -------------------------------------------------------------------------------------------------------------------------
    
\caption[CGs for computing the distributed SG update in (\ref{eq:fafafafafafufahfah0},b)]{CGs for computing the distributed SG update in (\ref{eq:fafafafafafufahfah0},b).  In the distributed setting considered (i.e., in the multi-agent setting) the first graph, respectively the second graph, corresponds to computations performed by Agent 1, respectively Agent 2. Note that we are assuming both agents have access to $\hat{\bm{\uptheta}}_k^\text{non}$, $\bm{h}_{k+1}$, and $z_k$. In general these CGs are not unique.}
\label{fig:figgystuff1}
\end{figure}





 % -------------------------------------------------------------------------------------------------------------------------
 % -------------------------------------------------------------------------------------------------------------------------
% NEW FIGURE BEGINS BELOW
 % -------------------------------------------------------------------------------------------------------------------------
  % -------------------------------------------------------------------------------------------------------------------------

\begin{figure}[p]
\centering
  \begin{subfigure}[b]{1\textwidth}
 \centering
\begin{tikzpicture}

\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (x) at (0,0) {$\hat{\bm{\uptheta}}_k^\text{cyc}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (y) at (0,-1.5) {$\bm{h}_{k+1}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (z) at (6.55,1.05) {$z_k$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (a) at (11.4,1.05) {$a_k^{(1)}$};
\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=90pt, ultra thick] (newinput) at (2.6,1.05) {$[\bm{h}_{k+1}^{(2)}]^\top[\hat{\bm{\uptheta}}_k^\text{cyc}]^{(2)}$};
\node [above of=newinput] {Share this Value};


\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=74pt, thick] (xy) at (2.6,-0.75) {$(\hat{\bm{\uptheta}}_k^\text{cyc})^\top\bm{h}_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=110pt, thick] (xyz) at (6.55,-0.75) {$(\hat{\bm{\uptheta}}_k^\text{cyc})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=128pt, thick] (xyza) at (11.4,-0.75) {$a_k^{(1)}(\hat{\bm{\uptheta}}_k^\text{cyc})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.8em, minimum width=168pt, thick] (xyzah) at (11.4,-2.55) {$a_k^{(1)}\left[(\hat{\bm{\uptheta}}_k^\text{cyc})^\top\bm{h}_{k+1}-z_{k+1}\right]\bm{h}_{k+1}^{(1)}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=35pt, ultra thick] (final) at (11.4,-4.35) {$\hat{\bm{\uptheta}}_{k}^{(I)}$};

\draw[->, thick] (x)--(xy) ;
\draw[->, thick] (xy)--(newinput) ;
\draw[->,thick] (y)--(xy);
\draw[->,thick] (z)--(xyz);
\draw[->,thick] (xy)--(xyz);
\draw[->,thick] (a)--(xyza);
\draw[->,thick] (xyz)--(xyza);
\draw[->,thick] (xyza)--(xyzah);
\draw[->,thick] (y)--(0,-2.55)--(xyzah);
\draw[->,thick] (xyzah)--(final);
\draw[->,thick] (x)--(-.8,0)--(-.8,-4.35)--(final);

\end{tikzpicture}
 \end{subfigure}
 \caption*{The CG for computing (\ref{eq:addalabeltomee0}).}


% -------------------------------------------------------------------------------------------------------------------------

 \vspace{.5in}
 
 % -------------------------------------------------------------------------------------------------------------------------
 
    \begin{subfigure}[b]{1\textwidth}
 \centering
\begin{tikzpicture}

\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (x) at (0,0) {$\hat{\bm{\uptheta}}_k^{(I)}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (y) at (0,-1.5) {$\bm{h}_{k+1}$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (z) at (6.55,1.05) {$z_k$};
\node[draw,circle,minimum size=1.2cm,inner sep=0pt, thick] (a) at (11.4,1.05) {$a_k^{(2)}$};
\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=90pt, thick] (newinput) at (2.6,1.05) {$[\bm{h}_{k+1}^{(2)}]^\top[\hat{\bm{\uptheta}}_k^\text{cyc}]^{(2)}$};
\node [above of=newinput] {Borrow this Value};


\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=74pt, thick] (xy) at (2.6,-0.75) {$(\hat{\bm{\uptheta}}_k^{(I)})^\top\bm{h}_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=110pt, thick] (xyz) at (6.55,-0.75) {$(\hat{\bm{\uptheta}}_k^{(I)})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=128pt, thick] (xyza) at (11.4,-0.75) {$a_k^{(2)}(\hat{\bm{\uptheta}}_k^{(I)})^\top\bm{h}_{k+1}-z_{k+1}$};

\node[draw,rectangle, rounded corners, minimum height=2.8em, minimum width=168pt, thick] (xyzah) at (11.4,-2.55) {$a_k^{(2)}\left[(\hat{\bm{\uptheta}}_k^{(I)})^\top\bm{h}_{k+1}-z_{k+1}\right]\bm{h}_{k+1}^{(2)}$};

\node[draw,rectangle, rounded corners, minimum height=2.3em, minimum width=35pt, ultra thick] (final) at (11.4,-4.35) {$\hat{\bm{\uptheta}}_{k+1}^{\text{cyc}}$};

\draw[->, thick] (x)--(xy) ;
\draw[->, thick] (newinput)--(xy) ;
\draw[->,thick] (y)--(xy);
\draw[->,thick] (z)--(xyz);
\draw[->,thick] (xy)--(xyz);
\draw[->,thick] (a)--(xyza);
\draw[->,thick] (xyz)--(xyza);
\draw[->,thick] (xyza)--(xyzah);
\draw[->,thick] (y)--(0,-2.55)--(xyzah);
\draw[->,thick] (xyzah)--(final);
\draw[->,thick] (x)--(-.8,0)--(-.8,-4.35)--(final);

\end{tikzpicture}
 \end{subfigure}%
 \caption*{The CG for computing (\ref{eq:addalabeltomee}).}
 
 
 % -------------------------------------------------------------------------------------------------------------------------
 
  \vspace{.03in}
 
 % -------------------------------------------------------------------------------------------------------------------------
    
\caption[CGs for computing the distributed cyclic SG update in (\ref{eq:addalabeltomee0},b)]{CGs for computing the distributed cyclic seesaw SG update in (\ref{eq:addalabeltomee0},b). In the multi-agent setting the first graph, respectively the second graph, corresponds to computations performed by Agent 1, respectively Agent 2. Note that we are assuming both agents have access to $\bm{h}_{k+1}$ and $z_k$. We are also assuming Agent 1 has access to $\hat{\bm{\uptheta}}_k^\text{cyc}$ and that Agent 2 has access to $\hat{\bm{\uptheta}}_k^{(I)}$. In general these CGs are not unique. }
\label{fig:figgystuff2}
\end{figure}



\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/efficiency/effSGalg-eps-converted-to.pdf}};  
        \node[left= -0.6cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm\uptheta}_{4i}^{\text{cyc}}-\bm\uptheta^\ast\|^2}}{\overline{\|\hat{\bm\uptheta}_{5i}^{\text{non}}-\bm\uptheta^\ast\|^2}}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
      \node at (0.3,-4.3) {$i$ (a strictly-positive integer)};
\end{tikzpicture}
\caption[Relative efficiency between SG and cyclic seesaw SG when cost is a measure of the number of arithmetic computations]{An estimate of the relative efficiency in (\ref{eq:ratio}) for comparing the cyclic seesaw SG algorithm to the regular (i.e., non-cyclic) SG algorithm when cost is a measure of the number of arithmetic computations.  }
\label{eq:GOTITPEEPOPAH}
\end{figure}



\subsubsection{Cost as the Number of Subvector Updates}

The second type of cost we consider is the number of subvector updates performed. Under this definition of cost the SG algorithm and its cyclic counterpart have exactly the same cost since two subvector updates are performed every iteration. In other words, when cost is defined as the per-iteration number of subvector updates, it follows that $c^\text{non}=c^\text{cyc}$. Therefore, $k_1=i=k_2$ are valid values for $k_1$ and $k_2$ in (\ref{eq:ratio}) for any strictly-positive integer $i$. Figure \ref{fig:2013eura100k} estimates (\ref{eq:ratio}) for multiple values of $i$ using the same settings from Section \ref{sec:SGarithmetic}. The expectations in (\ref{eq:ratio}) were estimated using the average of 100 i.i.d. replications. For each replication, both the cyclic and non-cyclic algorithms were initialized at $-\bm\uptheta^\ast$.
% the cyclic and non-cyclic 
% algorithms were initialized at $-\bm\uptheta^\ast$. 
 Asymptotically, 
% It can be seen that 
%the asymptotic relative efficiency is close to 1.005 indicating that 
the cyclic algorithm was 5\% less efficient. Based on 10 other initializations of the algorithms, it was observed that the relative efficiency was more sensitive to initialization for early iterations than for later iterations.
% (asymptotically).
 \begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/efficiency/effSGupdt-eps-converted-to.pdf}};  
        \node[left= -0.3cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm\uptheta}_{i}^{\text{cyc}}-\bm\uptheta^\ast\|^2}}{\overline{\|\hat{\bm\uptheta}_{i}^{\text{non}}-\bm\uptheta^\ast\|^2}}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
      \node at (0.3,-4.3) {$i$ (a strictly-positive integer)};
\end{tikzpicture}
\caption[Relative efficiency between SG and cyclic seesaw SG when cost is a measure of the number of subvector updates]{An estimate of the relative efficiency in (\ref{eq:ratio}) for comparing the cyclic seesaw SG algorithm to the regular (i.e., non-cyclic) SG algorithm when cost is a measure of the number of subvector updates. 
%The expectations in (\ref{eq:ratio}) were estimated using the average of 100 i.i.d. replications. For each replication, both the cyclic and non-cyclic algorithms were initialized at $-\bm\uptheta^\ast$. 
}
\label{fig:2013eura100k}
\end{figure}

\subsubsection[Cost as Time allowing for Agent Unavailability]{Cost as Time allowing for Agent Unavailability} 
\label{secsec:originalunavailability}

The efficiency analysis in this section once again relies on drawing parallels between the distributed implementations of (\ref{eq:fafafafafafufahfah0},b) and (\ref{eq:addalabeltomee0},b) and the multi-agent setting. In the multi-agent setting, the first and second subvectors of $\bm\uptheta$ correspond, respectively, to parameters that Agent No. 1 and Agent No. 2 can update. Implementing the SG algorithm in (\ref{eq:fafafafafafufahfah0},b) in a distributed manner would require both agents to be available at the same time. However, in practice it is not uncommon for agents to be tasked with secondary objectives that may make them temporarily unavailable to update their parameter vector.
% Agents may also be unable to update their parameters due to some type of malfunction (e.g., ).
%When a subvector correspond to an agent's physical position, an agent may also be unavailable to update its parameter vector (i.e., its position) due to malfunction. 
A slight modification to the cyclic seesaw SG algorithm in (\ref{eq:addalabeltomee0},b) would be to allow a single agent, while available, to continuously update its parameters until the moment when the other agent becomes available. The resulting algorithm would be a special case of Algorithm \ref{findme}. This section constructs a simple model of agent availability in order to estimate  (\ref{eq:ratio}) when cost is a measure of time.

% such that $c^\text{non}=1$ and $c^\text{cyc}=2$ (this definition of cost is used to reflect the fact that  an iteration of the cyclic seesaw algorithm requires two time steps whereas an iteration of the SG algorithm requires one time step).


%Beginning at time $T=0$ both algorithms (\ref{eq:fafafafafafufahfah}) and (\ref{eq:addalabeltomee}) are implemented until the time at which an agent becomes unavailable. 
To model agent availability we begin by defining a unit of time as the time it takes to perform a subvector update, this time is assumed to be equal for all subvectors independently of whether we are implementing the SG algorithm or its modified cyclic version and independently of the magnitude of the update (note that for the regular SG algorithm the time needed to perform a single iteration is one time unit since the two subvector updates are performed simultaneously).   We will assume that any agent can become unavailable with probability $q$ after completing its latest subvector update (for simplicity we assume an agent cannot become unavailable while in the middle of performing an update). Furthermore, at the next time unit an agent that was previously unavailable will remain unavailable with probability $q$. Because implementing the SG algorithm in (\ref{eq:fafafafafafufahfah0},b) requires both agents to be available simultaneously, no updates can be performed using the non-cyclic algorithm if at least one of the agents is unavailable. In contrast, the proposed modification to the cyclic algorithm (where an available agent continuously updates its parameters) could still be implemented provided at least one of the agents is available. 

Given our definition of a time unit and our model of agent unavailability, the relative efficiency ratio in (\ref{eq:ratio}) is estimated as the ratio:
\begin{align}
\label{eq:datamissinon}
\frac{E\|\hat{\bm\uptheta}^{\text{cyc}}(t)-\bm\uptheta^\ast\|^2}{E\|\hat{\bm\uptheta}^{\text{non}}(t)-\bm\uptheta^\ast\|^2},
\end{align}
where $t$ denotes time and where $\hat{\bm{\uptheta}}^{\text{cyc}}(t)$ and $\hat{\bm{\uptheta}}^{\text{non}}(t)$ denote algorithm iterate values at time $t$ (we deliberately avoid writing $t$ as a subscript of $\hat{\bm{\uptheta}}$ due to the fact that subscripts in (\ref{eq:fafafafafafufahfah0},b) and (\ref{eq:addalabeltomee0},b) are reserved for the iteration number, which is not the same as $t$). In order to select a value of $q$ for our numerical examples we note the following. At any given time the probability of updating the parameter vector using the SG algorithm is $P_1\equiv (1-q)^2$ whereas the probability of updating the parameter vector using the modified cyclic seesaw algorithm is $P_2\equiv 2(1-q)-(1-q)^2$. For $q\in [0,1]$, $P_2\geq P_1$ and the maximum difference between $P_1$ and $P_2$ occurs at $q=1/2$.  Figure \ref{fig:failureagentsgraphy} estimates (\ref{eq:datamissinon}) using $q=1/2$ 
%(this value of $q$ was chosen in an attempt to maximize the effect of agent unavailability on relative efficiency)
 with $a_k=a_k^{(j)}=0.1/(1+100+k)^{0.501}$. The expectations in (\ref{eq:datamissinon}) were estimated using the average of 100 i.i.d. replications. For each replication, both algorithms were initialized at $-\bm\uptheta^\ast$. We use the same distributions for  $\bm{h}_k$ and $\upvarepsilon_k$ from Section \ref{sec:SGarithmetic}. It was assumed that a new input-output pair $(\bm{h}_k,z_k)$ became available with the passing of every time unit. Agents were assumed to use the latest input-output pair to perform their updates.  The results of Figure \ref{fig:failureagentsgraphy} indicate that the cyclic variant was approximately 10\% more efficient (asymptotically), likely due to the fact that using a cyclic implementation implies the parameter vector is updated more frequently than when using a non-cyclic implementation.
%  slightly more efficient than the non-cyclic implementation. 
% Asymptotically, both algorithms become equally efficient. 
% (similar results were obtained for other initializations of the algorithms). 
% Although Figure \ref{fig:failureagentsgraphy} indicates that the cyclic algorithm is much more efficient initially, 
%
Based on 10 other initializations of the algorithms, it was observed that the relative efficiency was more sensitive to initialization for small values of $t$ than for larger values.
%iterations.
%  The relative efficiency for small values of $t$ was highly sensitive to the initialization of the algorithms. 
%For example, Figure \ref{fig:failureagentsgraphy2} repeats the experiment in Figure \ref{fig:failureagentsgraphy} when the algorithm realizations are initialized at the vector $-[4,\dots,4]^\top$.
\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/efficiency/effSGtime3-eps-converted-to.pdf}};  
        \node[left= -0.6cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm\uptheta}^{\text{cyc}}(t)-\bm\uptheta^\ast\|^2}}{\overline{\|\hat{\bm\uptheta}^{\text{non}}(t)-\bm\uptheta^\ast\|^2}}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
      \node at (0.3,-4.3) {$t$};
\end{tikzpicture}
\caption[An estimate of the relative efficiency in (\ref{eq:datamissinon}) for comparing the SG algorithm to a generalized cyclic seesaw SG algorithm where agents may be unavailable to perform updates]{An estimate of the relative efficiency in (\ref{eq:datamissinon}) for comparing the SG to a generalized cyclic seesaw SG algorithm where agents may be unavailable to perform updates with probability $q=1/2$. }
\label{fig:failureagentsgraphy}
\end{figure} 



\subsection{Efficiency: SPSA versus Cyclic Seesaw SPSA}
\label{eq:Indyiedie12}

This section compares the SPSA algorithm to the cyclic seesaw SPSA algorithm by estimating the relative efficiency in (\ref{eq:ratio}). The SPSA algorithm treated is the SPSA algorithm from Section \ref{sec:clubsodeashrimp} where the objective is to minimize the skewed quartic loss function with $p=10$.
% (recall that $p$ is the dimension of $\bm\uptheta$).
%  As in Section \ref{sec:clubsodeashrimp} 
  We assume $Q(\bm\uptheta,\bm{V})=L(\bm\uptheta)+\upvarepsilon$ where $\upvarepsilon\sim\mathcal{N}(0,0.1^2)$. For the cyclic seesaw implementation we let $p'=5$ 
%  (recall $p'$ is the length of the subvectors) 
  and use noisy gradient estimates of the form in (\ref{eq:howeardspos1}) and (\ref{eq:howeardspos2}), SPSA-based noisy gradient estimates where only the subvector to update is perturbed.


\subsubsection{Cost as the Number of Noisy Loss Measurements}
\label{secsec:whennoticreep}




The first definition of cost we consider is the number of noisy loss function measurements required per-iteration. Under this definition $c^\text{non}=2$ for the the regular SPSA algorithm whereas $c^\text{cyc}=4$ for the cyclic seesaw SPSA algorithm. Therefore, in order to conduct a fair comparison between  SPSA and cyclic SPSA we would need to run twice as many iterations for the regular SPSA algorithm.  Therefore, $k_1=i$ and $k_2=2i$ are valid values for $k_1$ and $k_2$ in (\ref{eq:ratio}) for any strictly-positive integer $i$. As such, Figure \ref{fig:sassyconcREG} estimates the relative efficiency in (\ref{eq:ratio}) with $k_1=i$ and $k_2=2i$ for different values of $i$. The expectations in (\ref{eq:ratio}) were estimated using the average of 500 i.i.d. replications. For each replication, both algorithms were initialized at $-[1,\dots,1]^\top$. As suggested by Table \ref{table:omgmyfirsttable}, we use the gain sequences $a_k=a_k^{(j)}=1/(1+k+100)^{0.602}$ and set $c_k=c_k^{(j)}=0.1/(1+k)^{0.101}$. We let the non-zero entries of the $\bm\Delta$ be independent and take the value $\pm1$ with equal probability. We can see that the relative efficiency favors the cyclic algorithm for early iterations (although this behavior was, once again, sensitive to the initialization of the algorithms) while the non-cyclic algorithm becomes more efficient (by about 8\%) in the long run. Based on 10 different initializations of the other, it was observed that the relative efficiency was more sensitive to initialization for small values of $t$ than for larger values. 
%Similar asymptotic results were observed for 10 different initializations of the algorithms.




\subsubsection{Cost as the Number of Subvector Updates}


\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/efficiency/effSPSAlossNEW-eps-converted-to.pdf}};  
        \node[left= -0.6cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm\uptheta}^{\text{cyc}}_i-\bm\uptheta^\ast\|^2}}{\overline{\|\hat{\bm\uptheta}^{\text{non}}_{2i}-\bm\uptheta^\ast\|^2}}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
      \node at (0.3,-4.3) {$i$ (a strictly-positive integer)};
\end{tikzpicture}
\caption[Relative efficiency between SPSA and cyclic seesaw SPSA when cost is a measure of the number of noisy loss measurements]{An estimate of the relative efficiency in (\ref{eq:ratio}) for comparing the cyclic seesaw SPSA algorithm to the regular (i.e., non-cyclic) SPSA algorithm when cost is a measure of the number of noisy loss function evaluations.  }
\label{fig:sassyconcREG}
\end{figure} 

\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/efficiency/effSPSAupdates-eps-converted-to.pdf}};  
        \node[left= -0.6cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm\uptheta}^{\text{cyc}}_i-\bm\uptheta^\ast\|^2}}{\overline{\|\hat{\bm\uptheta}^{\text{non}}_{i}-\bm\uptheta^\ast\|^2}}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
      \node at (0.3,-4.3) {$i$ (a strictly-positive integer)};
\end{tikzpicture}
\caption[Relative efficiency between SPSA and cyclic seesaw SPSA when cost is a measure of the number of subvector updates]{An estimate of the relative efficiency in (\ref{eq:ratio}) for comparing the cyclic seesaw SPSA algorithm to the regular (i.e., non-cyclic) SPSA algorithm when cost is a measure of the number of subvector updates. }
\label{fig:sassyconc}
\end{figure} 

This section estimates the ratio in (\ref{eq:ratio}) by viewing cost as the number of subvector updates per-iteration, which implies $c^\text{non}=c^\text{cyc}=2$. Therefore, $k_1=i=k_2$ are valid values for $k_1$ and $k_2$ in (\ref{eq:ratio}) for any strictly-positive integer $i$. Figure \ref{fig:sassyconc} presents the results with $k_1=i=k_2$ using the settings from Section \ref{secsec:whennoticreep}. The expectations in (\ref{eq:ratio}) were estimated using the average of 500 i.i.d. replications. For each replication, both the cyclic and non-cyclic algorithms were initialized at $-[1,\dots,1]^\top$.  It can be seen that cyclic algorithm slightly outperforms its non-cyclic counterpart (by about 6\%) when the number of iterations is large. Based on 10 other initializations of the algorithms, the relative efficiency for small values of $i$ appeared to be more sensitive to initialization  than for large values of $i$.
%both algorithms appear to be (asymptotically) equally efficient. 
%The asymptotic results, however, appeared to be more robust to the initialization of the algorithms.



\subsubsection[Cost as Time allowing for Agent Unavailability]{Cost as Time allowing for Agent Unavailability} 



Similarly to Section \ref{secsec:originalunavailability}, this section estimates relative efficiency in a multi-agent setting where agents can be unavailable with probability $q=1/2$. The difference between the experiment in this section and the experiment from Section \ref{secsec:originalunavailability} is that SPSA-based gradient estimates, instead of SG-based estimates, are used to perform the subvector updates. For this reason we refer the reader to Section \ref{secsec:originalunavailability} for a more detailed description of the model for agent unavailability. Figure \ref{fig:eleveatedday} presents the estimate of (\ref{eq:datamissinon}) as a function of $t$, denoting time, using the settings from Section \ref{secsec:whennoticreep}. The expectations in (\ref{eq:datamissinon}) were estimated using the average of 500 i.i.d. replications. For each replication, both algorithms were initialized at the vector $-[1,\dots,1]^\top$. 
\begin{figure}[!t]
\centering
\begin{tikzpicture}
  \definecolor{mynewcoloring}{RGB}{102, 128, 153}
% 1 block
\node[inner sep=0pt] (probe) at (0,0)
    {\includegraphics[scale=0.6]{Plots/efficiency/effSPSAtimeNEW-eps-converted-to.pdf}};  
        \node[left= -0.6cm of probe]{$\displaystyle{\frac{\overline{\|\hat{\bm\uptheta}^{\text{cyc}}(t)-\bm\uptheta^\ast\|^2}}{\overline{\|\hat{\bm\uptheta}^{\text{non}}(t)-\bm\uptheta^\ast\|^2}}}$};
%      \node at (4.6,-2.5) {$\uptheta_2$};
      \node at (0.3,-4.3) {$t$};
\end{tikzpicture}
\caption[An estimate of the relative efficiency in (\ref{eq:datamissinon}) for comparing the SPSA algorithm to a generalized cyclic seesaw SPSA algorithm where agents may be unavailable to perform updates]{An estimate of the relative efficiency in (\ref{eq:datamissinon}) for comparing the SPSA to a generalized cyclic seesaw SPSA algorithm where agents may be unavailable to perform updates with probability $q=1/2$. }
\label{fig:eleveatedday}
\end{figure} 
We see that asymptotically
% the cyclic variant is more efficient than its non-cyclic counterpart for small values of $t$. However, the relative efficiency for small values of $t$ was highly sensitive to the initializations of the algorithms. Asymptotically, however, 
 the cyclic algorithm appeared to be only slightly more efficient than its non-cyclic counterpart (based on 10 other initializations, this appeared to be independent of the initialization of the cyclic and non-cyclic algorithms).




\section{Concluding Remarks}

This chapter contains numerical results illustrating the theory on convergence from Chapter \ref{sec:cyclicseesaw} and the theory on asymptotic normality from Chapter \ref{sec:ROC}. Additionally, numerical experiments were conducted to investigate the relative efficiency (as defined in (\ref{eq:ratio})) between cyclic algorithms and their non-cyclic counterparts. For the numerical experiments that were conducted, the cyclic and non-cyclic algorithms had comparable asymptotic efficiency. However, it is important to keep in mind that there are many factors that affect asymptotic relative efficiency (e.g., the shape of the loss function to minimize, the number of subvectors, the definition of cost) and the results of this Chapter do not imply that the cyclic and non-cyclic algorithms are equally efficient in general. For a theoretical analysis of asymptotic relative efficiency we refer the reader to Sections \ref{sec:aseficwiener} and \ref{sec:apsecialcaserelefff}.




==> thesis arXiv 2/notation.tex <==
%!TEX root = root.tex
\fancyhead{} % clear all header and footer fields
\fancyhead[L]{FREQUENTLY USED NOTATION} % except the center
\chapter*{Frequently Used Notation} 
\setcounter{chapter}{2}% Equivalent to "letter B"
\renewcommand{\thechapter}{\Alph{chapter}}%
\addcontentsline{toc}{chapter}{Frequently Used Notation} 
\label{chap:fun}

\noindent A list of the most commonly used notation arranged by category. The notation in this list is consistent throughout the entire dissertation (with the exception of Section \ref{sec:literaturesurveyrev} where some of the notation was borrowed from the references being surveyed).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{.2in}
\noindent{\bf{\large{General Notation}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent $\equiv$ is the symbol for ``defined as''.

\noindent $A \cup B$ denotes the union of the sets $A$ and $B$.

\noindent $A \cap B$ denotes the intersection of the sets $A$ and $B$.

\noindent $S^c$ denotes the complement of the set $S$.

\noindent $\emptyset$ denotes the empty set.

\noindent $\Box$ denotes the end of a proof.

\noindent $a\choose{b}$ represents the quantity ${a!}/[{(a-b)!b!}]$.

\noindent $\mathbb{Z}^+$ denotes the set of strictly positive integers.

\noindent $\mathbb{R}^p$ denotes the Euclidean space of dimension $p$.

\noindent w.l.o.g. means ``without loss of generality''.

\noindent $\ceil{a}$ is the ceiling function applied to a real number $a$.

\noindent $\floor{a}$ is the floor function applied to a real number $a$.

\noindent $I_T$ denotes the interval $[-T,T]$ for $T> 0$.

%\noindent $\bar{I}$ denotes a closed and bounded interval in the real line.

%\noindent $C^{\infty}$ is the set of functions that are infinitely differentiable.

\noindent $O(\cdot)$ denotes the standard big-{\it{O}} notation.

\noindent $o(\cdot)$ denotes the standard little-{\it{o}} notation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{.2in}
\noindent{\bf{\large{Matrices and Vectors}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent Bolded variables represent either vectors or matrices.

\noindent $\bm{A}^\top$ denotes the transpose of the matrix $\bm{A}$.

%\noindent $\bm{A}\succ 0$ means that the matrix $\bm{A}$ is positive definite.
%
%\noindent $\bm{A}\succeq 0$ means that the matrix $\bm{A}$ is positive semidefinite.
%
%\noindent $\text{det}{(\bm{A})}$ is the determinant of the matrix $\bm{A}$.

\noindent $\trace{(\bm{A})}$ is the trace of the matrix $\bm{A}$.

%\noindent $\text{diag}\left(\bm{A}\right)$ is the vector of diagonal elements of the square matrix $\bm{A}$.
%
%\noindent $\text{diag}\left(\bm{v}\right)$ is the diagonal matrix with diagonal entries specified by the vector $\bm{v}$.

%\noindent $\text{rank}{(\bm{A})}$ is the rank of the matrix $\bm{A}$.

\noindent $\|\cdot\|$ represents the Frobenius norm.

%\noindent $\vertiii{\cdot}$ represents the induced matrix norm (e.g., Horn and Johnson 2010, p. 292)\nocite{hornnjohnson2010}.

\noindent $\bm{I}$ denotes the identity matrix of unspecified dimensions.

%\noindent $\bm{I}_n$ denotes the $n\times n$ identity matrix.

\noindent ${M}_{ij}$ (also $(\bm{M})_{ij}$ or $[\bm{M}]_{ij}$) denotes the $(i,j)$th entry of the matrix $\bm{M}$.

\noindent ${M}_{k(ij)}$ denotes the $(i,j)$th entry of the matrix $\bm{M}_k$.

\noindent ${v}_j$ (also $(\bm{v})_j$ or $[\bm{v}]_j$) denotes the $j$th entry of the vector $\bm{v}$.

\noindent ${v}_{k(j)}$ denotes the $j$th entry of the vector $\bm{v}_k$.

\noindent $p$ is reserved for the dimension of $\bm\uptheta$ so that $\bm\uptheta=[\uptau_1,\dots,\uptau_p]^\top\in \mathbb{R}^p$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{.2in}
\noindent{\bf{\large{Probability}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent $\chi\{\mathcal{E}\}$ denotes the indicator function of the event $\mathcal{E}$.

\noindent $P(\mathcal{E})$ denotes the probability of the event $\mathcal{E}$.

\noindent $E[\mathcal{X}]$ represents the expectation of the random variable $\mathcal{X}$.

\noindent $\Var{(\mathcal{X})}$ is the variance or covariance matrix of $\mathcal{X}$.

\noindent $\mathcal{N}(\bm\upmu,\bm\Sigma)$ is a normal random variable with mean $\bm\upmu$ and variance/covariance $\bm\Sigma$.

\noindent $\text{Bernoulli}(p)$ denotes a Bernoulli random variable with parameter $p$.

\noindent i.i.d. means ``independent and identically distributed''.

\noindent w.p.1 means ``with probability one''.

\noindent $\xrightarrow{\text{\ dist\ }}$ means convergence in distribution.

\noindent $\mathcal{X} \sim$ is used to indicate that the random variable $\mathcal{X}$ has certain distribution.

\noindent $(\Omega, \mathcal{F}, P)$ is a probability space with sample space $\Omega$, $\upsigma$-field $\mathcal{F}$, and measure $P$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{.2in}
\noindent{\bf{\large{Sequences and Sums}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent $g_n=o(h_n)$ if $h_n^{-1}g_n\rightarrow 0$ as $n\rightarrow \infty$.

\noindent $G_n=O(h_n)$ if $\|h_n^{-1}G_n\|\leq c$ for some $c\in \mathbb{R}$ and all $n$.

%\noindent $q_n=o_u(h_n)$ if $h_n^{-1}q_n\rightarrow 0$ uniformly on a set of probability one.

\noindent $\sum_{i=a}^b(\cdot)_i = 0$ whenever $b<a$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{.2in}
\noindent{\bf{\large{Stochastic Optimization}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent $L(\bm\uptheta)$ denotes a loss function to minimize.

\noindent $\bm\uptheta$ denotes the vector of parameters being estimated.

\noindent $\bm{g}(\bm\uptheta)$ denotes the gradient vector of $L(\bm\uptheta)$.

\noindent $\bm{H}(\bm\uptheta)$ denotes the Hessian matrix of $L(\bm\uptheta)$.

\noindent $\bm\uptheta^\ast$ denotes a minimizer of $L(\bm\uptheta)$ or a solution to $\bm{g}(\bm\uptheta)=\bm{0}$.

\noindent $\hat{\bm{\uptheta}}_k$ is the iterate produced in the $k$th iteration of an algorithm searching for $\bm\uptheta^\ast$.

\noindent $\hat{\bm{g}}_k(\bm\uptheta)$ denotes a noisy gradient measurement obtained during iteration $k+1$.

\noindent $Q(\bm\uptheta,\bm{V})$ denotes a noisy measurement of $L(\bm\uptheta)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{.2in}
\noindent{\bf{\large{GCSA-Specific Notation}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\noindent $d$ is the total number of subvectors which may be updated.

\noindent $\mathcal{S}_j$ for $j=1,\dots, d$ is a set of coordinates defining a subvector of $\bm\uptheta$ (see p. \pageref{eq:notexclusive}).

\noindent $j_k(m)$ is a random variable in $\{1,\dots,d\}$. 

\noindent $\bm{v}^{(j)}$ for $\bm{v}\in\mathbb{R}^p$ forces certain entries of $\bm{v}$ to be zero according to (\ref{eq:alonesong}).

\noindent $\bm{\hat{\bm{\uptheta}}_k}^{(I_{m,i})}$ denotes an intermediate step within an iteration (see p. \pageref{def:intermediate}).

\noindent $\bm{J}^{(j)}(\bm\uptheta)$ denotes the Jacobian of $\bm{g}^{(j)}(\bm\uptheta)$.

\noindent $a_k^{(j)}$ for $j=1,\dots,d$ denotes a gain sequence.\label{faq:GCSAspecific}

%\noindent $r_j$ for $j=1,\dots,d$ denotes the limit of $k^\upalpha a_k^{(j)}$.

\noindent $s_k$ is the random number of blocks in the $(k+1)$st iteration.

\noindent $n_k(m)$ is the number of updates in the $m$th block of the $(k+1)$st iteration.

%\noindent $d$ the total number of (possibly overlapping) subvectors (see also p. \pageref{eq:notexclusive}).

\noindent $\tilde{A}_{k}(m)=\sum_{j=1}^d{\mathcal{X}}\{j_k(m)=j\}\tilde{a}_k^{(j)}$ (see p. \pageref{eq:attaritapo}).

\noindent $\tilde{a}_{k+1}^{(j)}=a_0^{(j)}+\sum_{i=0}^k {\mathcal{X}}\{\upvarphi_k^{(j)}\geq i\}(a_{i+1}^{(j)}-a_{i}^{(j)})$ (see p. \pageref{eq:saropian}).

\noindent $\upvarphi_k^{(j)}=\sum_{i=0}^k {\mathcal{X}}\left\{\left(\sum_{m=1}^{s_i}{\mathcal{X}}\{j_i(m)=j\}\right)>0\right\}-1$ (see p. \pageref{eq:wheretheasaredefinedd}).

\noindent $x_k(j)= ({\tilde{a}_{k}^{(j)} }/{a_{k}})\sum_{m=1}^{s_k}{\mathcal{X}}\{j_k(m)=j\}n_k(m)$ (see p. \pageref{eq:tinkelpan}).

\noindent $\upmu_k(j) =E[x_k(j)]$ (see p. \pageref{eq:tinkelpan}).

\noindent $\upmu(j)=\lim_{k\rightarrow \infty} \upmu_k(j)$ (see p. \pageref{eq:tinkelpan}).

\noindent $X_k= \sum_{j=1}^dx_k(j)$ (see p. \pageref{eq:apoint}).

\noindent $\bm{h}_k(\bm\uptheta)= \sum_{j=1}^d \upmu_k(j)\bm{g}^{(j)}(\bm\uptheta)$ (see p. \pageref{eq:unrealantartica}).

\noindent $\bm{h}(\bm\uptheta)= \sum_{j=1}^d \upmu(j)\bm{g}^{(j)}(\bm\uptheta)$ (see p. \pageref{eq:unrealantartica}).\label{def:lastpage}







